Finite-Graph-Cover-Based Analysis of Factor Graphs in Classical and Quantum Information Processing Systems

In this thesis, we leverage finite graph covers to analyze the SPA and the Bethe partition function for both S-FGs and DE-FGs. There are two main contributions in this thesis. The first main contribution concerns a special class of S-FGs where the partition function of each S-FG equals the permanent of a nonnegative square matrix. The Bethe partition function for such an S-FG is called the Bethe permanent. A combinatorial characterization of the Bethe permanent is given by the degree-$M$ Bethe permanent, which is defined based on the degree-$M$ graph covers of the underlying S-FG. In this thesis, we prove a degree-$M$-Bethe-permanent-based lower bound on the permanent of a non-negative square matrix, resolving a conjecture proposed by Vontobel in [IEEE Trans. Inf. Theory, Mar. 2013]. We also prove a degree-$M$-Bethe-permanent-based upper bound on the permanent of a non-negative matrix. In the limit $M \to \infty$, these lower and upper bounds yield known Bethe-permanent-based lower and upper bounds on the permanent of a non-negative square matrix. The second main contribution is giving a combinatorial characterization of the Bethe partition function for DE-FGs in terms of finite graph covers. In general, approximating the partition function of a DE-FG is more challenging than for an S-FG because the partition function of the DE-FG is a sum of complex values and not just a sum of non-negative real values. Moreover, one cannot apply the method of types for proving the combinatorial characterization as in the case of S-FGs. We overcome this challenge by applying a suitable loop-calculus transform (LCT) for both S-FGs and DE-FGs. Currently, we provide a combinatorial characterization of the Bethe partition function in terms of finite graph covers for a class of DE-FGs satisfying an (easily checkable) condition.

==> appendices/SST.tex <==
%***************************************************************************
In this appendix, we will use the Gamma function, \textit{i.e.},
$\Gamma(z) \defeq \int_{0}^{\infty} s^{z-1} \e^{-s} \dd{s}$ for $z \in \sC$
with $\Re(z) > 0$. Note that $\Gamma(z) = (z -  1)!$ if $z$ is a
positive-valued integer. However, we will use the Gamma function $ \Gamma $ also with
non-integral real arguments. Moreover, let $S_n$ be the
$(n \! - \! 1)$-dimensional area of the unit sphere in $\sR^n$. It holds that
$S_n = 2 \cdot \pi^{n/2} / \Gamma(n/2)$ (see, \textit{e.g.}, \cite{Folland2001}).

%***************************************************************************

The following lemma contains a useful technical result.

%***************************************************************************

\begin{lemma}
  \label{lemma:special:binomial:sum:1}

  Let $k \in \sZp$. It holds that
  \begin{align*}
    \sum_{\ell=0}^{k}
      \binom{k}{\ell}
        \cdot
        \Gamma(\ell \! + \! 1/2) 
        \cdot 
        \Gamma(k \! - \! \ell \! + \! 1/2)
      &= \frac{S_2}{2}
         \cdot
         k! \ .
  \end{align*}
\end{lemma}

%***************************************************************************

\begin{proof}
  Let $\cvw \defeq (\cw_0, \cw_1)^\tran \in \sR^2$ be the vector with norm one, \textit{i.e.}, $ \cw_0^{2} + \cw_1^{2} = 1 $, as defined in Definition~\ref{sec:SST:def:3}. Using a Fubini-Study measure
  of dimension one, we obtain
  \begin{align*}
    1
      &= \int
           1
         \dd{\muFSsimple(\cvw)} \\
      &\overset{(a)}{=} \int
           \bigl( \cw_0^2 + \cw_1^2 \bigr)^{\! k}
         \dd{\muFSsimple(\cvw)} \\
      &= \int
           \sum_{\ell=0}^{k}
             \binom{k}{\ell}
             \cdot
             \cw_0^{2\ell}
             \cdot
             \cw_1^{2(k-\ell)}
           \dd{\muFSsimple(\cvw)} \\
      &= \sum_{\ell=0}^{k}
           \binom{k}{\ell}
             \cdot
             \int
               \cw_0^{2\ell}
               \cdot
               \cw_1^{2(k-\ell)}
             \dd{\muFSsimple(\cvw)} \\
       &\overset{(b)}{=}  \sum_{\ell=0}^{k}
           \binom{k}{\ell}
           \cdot
           \frac{2 \cdot \Gamma(\ell+1/2) \cdot \Gamma(k-\ell+1/2)}
                {\Gamma(k+1)}
           \cdot
           \frac{1}{S_2},
  \end{align*}
  where step $(a)$ follows from the fact that $\cw_0^2 + \cw_1^2 = 1$
  for all $\cvw = (\cw_0,\cw_1)^\tran$ where the measure $\muFSsimple(\cvw)$
  is nonzero, and where step $(b)$ follows from the main theorem
  in~\cite{Folland2001}.
\end{proof}

%***************************************************************************

We come now to the actual proof of the lemma. By Lemma~\ref{sec:SST:lem:4}, it is equivalent to prove that
\begin{align*}
  \int
    \funcFS_{e,\cpsi_e}\bigl( \vx_{\efi,[M]}, \vx_{\efj,[M]} \bigr)
    \dd{\muFSsimple\bigl( \cvpsi_e \bigr)} 
    &= \begin{cases}
         \frac{1}{|\set{T}_{e,\vt_e}|}
           & \vt_e = \vt_e\bigl(\vx_{\efi,[M]}\bigr) 
            = \vt_e\bigl( \vx_{\efj,[M]} \bigr) 
          \\
         0
           & \text{otherwise}
    \end{cases}
\end{align*}
for all $ \vx_{\efi,[M]}, \vx_{\efj,[M]} \in \set{X}_e^M $.
In the following, we will
use the following notation:
\begin{itemize}

\item We define $d \defeq |\set{
X}_e|$.

\item We assume, without loss of generality, that $\set{X}_e = \{ 0, 1, \ldots, d \! - \! 1 \}$.

\item We write $x$ instead of the more precise $x_e$.

\item We use the short hand $\prod_x$ and $ \sum_{x} $ for $\prod_{x \in \set{X}_e}$ and $ \sum_{x \in \set{X}_e} $, respectively.

\item We let
  $\vk_e = ( k_{e,x} )_{x \in \set{X}_e} = M \cdot \vt_e(\vx_{\efi,[M]})$ and
  $\vk'_e = ( k'_{e,x} )_{x \in \set{X}_e} = M \cdot \vt_e(\vx_{\efj,[M]})$.

\end{itemize}

%***************************************************************************

First, we consider the case where $\vk_e = \vk'_e = \frac{1}{M} \cdot \vt_{e}$. In this case, by the definition of $ \funcFS_{e,\cpsi_{e}} $ in Definition~\ref{sec:SST:def:3}, we have
%-----------------------------------------------------------------------
\begin{align*}
    \int
        \funcFS_{e,\cpsi_e}(x_{\efi}, x_{\efj})
    \dd{\muFSsimple(\cvpsi_{e})}
    &=  
    |\set{B}_{\set{X}_e^M}| \cdot
    \int
        \prod_{x}
           |\cpsi_e(x)|^{2k_{e,x}}
    \dd{\muFSsimple(\cvpsi_{e})}.
\end{align*}
%-----------------------------------------------------------------------
Using a Fubini-Study
measure of dimension $|\set{X}_e|$, we get
\begin{align*}
    \hspace{0.5 cm}&\hspace{-0.5 cm}\int
        \prod_{x}
        |\cpsi_e(x)|^{2k_{e,x}}
       \dd{\muFSsimple(\cvpsi_{e})} 
     \nonumber\\
    &= \int
         \prod_x
           \bigl( \cw_{x,0}^2 + \cw_{x,1}^2 \bigr)^{\! k_{e,x}}
       \dd{\muFSsimple(\cvw)} \nonumber \\
    &= \int
         \prod_x
           \sum_{\ell_{e,x}=0}^{k_{e,x}}
             \binom{k_{e,x}}{\ell_{e,x}}
             \cdot \cw_{x,0}^{2\ell_{e,x}}
             \cdot
             \cw_{x,1}^{2(k_{e,x}-\ell_{e,x})}
       \dd{\muFSsimple(\cvw)} \nonumber \\
    &= \sum_{\ell_{e,0}=0}^{t_{e,0}}
       \cdots
       \sum_{\ell_{e,d-1}=0}^{t_{e,d-1}}
         \left(
           \prod_x
             \binom{k_{e,x}}{\ell_{e,x}}
         \right)
         \cdot
         \int
           \prod_x
             \cw_{x,0}^{2\ell_{e,x}}
             \cdot
             \cw_{x,1}^{2(k_{e,x}-\ell_{e,x})}
           \dd{\muFSsimple(\cvw)} \nonumber  \\
    &\overset{(a)}{=} \sum_{\ell_{e,0}=0}^{t_{e,0}}
       \cdots
       \sum_{\ell_{e,d-1}=0}^{t_{e,d-1}}
         \left(
           \prod_x
             \binom{k_{e,x}}{\ell_{e,x}}
         \right)
         \cdot
           \frac{2 
                   \cdot
                   \Bigl(
                     \prod_x
                       \Gamma(\ell_{e,x}+1/2) 
                       \cdot 
                       \Gamma(k_{e,x}-\ell_{e,x}+1/2)
                   \Bigr)
                 }
                 {\Gamma(M + d) \cdot S_{2d}}
       \nonumber \\
    &= \frac{2}{S_{2d}}
       \cdot
       \frac{1}{(M+d-1)!}
       \cdot
       \prod_x
         \sum_{\ell_{e,x}=0}^{k_{e,x}}
           \binom{k_{e,x}}{\ell_{e,x}}
           \cdot
           \Gamma(\ell_{e,x}+1/2) 
           \cdot 
           \Gamma(k_{e,x}-\ell_{e,x}+1/2) \nonumber \\
    &\overset{(b)}{=} \frac{S_2^d}{2^{d-1} \cdot S_{2d}}
       \cdot
       \frac{\prod_x (k_{e,x}!)}{(M+d-1)!} \nonumber \\
    &\overset{(c)}{=} (d \! - \! 1)!
       \cdot
       \frac{\prod_x (k_{e,x}!)}{(M+d-1)!} \nonumber \\
    &= \frac{1}{\binom{d+M-1}{M}}
       \cdot
       \frac{1}{ \binom{M}{k_0, \ldots, k_{d-1}} } \nonumber \\
    &\overset{(d)}{=} \frac{1}{|\set{B}_{\set{X}_e^M}|}
       \cdot
       \frac{1}{|\set{T}_{e,\vt_e}|}, 
\end{align*}
where step $(a)$ follows from the main theorem in~\cite{Folland2001} and
$\sum_x k_{e,x} = M$, where step $(b)$ follows from
Lemma~\ref{lemma:special:binomial:sum:1}, where step $(c)$ follows
from $S_2 = 2 \pi$ and $S_{2d} = 2 (\pi^d) / \Gamma(d) = 2 (\pi^d) / (d-1)!$, and where step $(d)$ follows from Lemma~\ref{sec:SST:lem:2}.

%***************************************************************************

Let us now consider the case $\vk_e \neq \vk'_e$, \ie, $ \vt_e\bigl(\vx_{\efi,[M]}\bigr) \neq \vt_e\bigl( \vx_{\efj,[M]} \bigr) $. In this case there is at
least one $x \in \set{X}_e$ such that $k_{e,x} \neq k'_{e,x}$. (In fact, there
must be at least two $x \in \set{X}_e$ such that $k_{e,x} \neq k'_{e,x}$ because
$\sum_x k_{e,x} = \sum_x k'_{e,x} = M$.) Let $\alpha_x \in \sR$,
$x \in \set{X}_e$, be some parameters. Using a Fubini-Study measure of dimension
$|\set{X}_e|$, we consider the expressions
\begin{align}
  \int
    \left(
      \prod_x
        \cpsi_e(x)^{k_{e,x}}
    \right)
    \cdot
    \left(
      \prod_x
        \Bigl( \overline{\cpsi_e(x)} \Bigr)^{\! k'_{e,x}}
    \right)
  \dd{\muFSsimple(\cvpsi)},
    \label{sec:SST:eqn:6} \\
  \int
    \left(
      \prod_x
        \left(
          \e^{\imagunit \alpha_k} \cdot \cpsi_e(x)
        \right)^{k_{e,x}}
    \right)
    \cdot
    \left(
      \prod_x
        \left(
          \overline{\e^{\imagunit \alpha_k} \cdot \cpsi_e(x)}
        \right)^{\! k'_{e,x}}
    \right)
  \dd{\muFSsimple(\cvpsi)}.
      \label{sec:SST:eqn:4}
\end{align}
Because of symmetries of the measure
$\muFSsimple$, the expressions in~\eqref{sec:SST:eqn:6}
and~\eqref{sec:SST:eqn:4} must give the same numerical
value. However, the expression in~\eqref{sec:SST:eqn:4} is
equal to
\begin{align}
  \e^{\imagunit \sum_x \alpha_x \cdot (k_{e,x} - k'_{e,x})}
  \cdot
  \int
    \left(
      \prod_x
        \bigl( \cpsi_e(x) \bigr)^{k_{e,x}}
    \right)
    \cdot
    \left(
      \prod_x
        \Bigl( \overline{\cpsi_e(x)} \Bigr)^{\!\! k'_{e,x}}
    \right)
  \dd{\muFSsimple(\cvpsi)}.
      \label{sec:SST:eqn:5}
\end{align}
Because of the assumptions on $\vk_e$ and $\vk'_e$, it is easy to find
$\alpha_x \in \sR$, $x \in \set{X}_e$, such that
$\e^{\imagunit \sum_x \alpha_x \cdot (k_{e,x} - k'_{e,x})} \neq 1$. Given this, the
only possibility for all expressions
in~\eqref{sec:SST:eqn:6}--\eqref{sec:SST:eqn:5}
to be the same is that they are all equal to zero. From this observation one
can conclude that
\begin{align*}
    \int
    \funcFS_{e,\cpsi_e}(\vx_{e,f}, \vx_{e,f'})
    \dd{\muFSsimple(\cvpsi)}
    &= |\set{B}_{\set{X}_e^M}| \cdot
    \int
         \left(
           \prod_x
             \bigl( \cpsi_e(x) \bigr)^{\! k_{e,x}}
         \right)
         \cdot
         \left(
           \prod_x
             \Bigl( \overline{\cpsi_e(x)} \Bigr)^{\!\! k'_{e,x}}
         \right)
       \dd{\muFSsimple(\cvpsi)}
       \nonumber\\
    & = 0.
\end{align*}


%***************************************************************************
%***************************************************************************

\ifx\sectionheaderonnewpage\x
\clearpage
\fi

==> appendices/check_cond_lower.tex <==
\begin{figure}
    \centering
    \captionsetup{font=scriptsize}
    \begin{adjustbox}{minipage=\linewidth,scale=0.98}
    \subfloat[\label{sec:CheckCon:fig:8:subfig:1}]{
    \begin{minipage}[t]{0.45\linewidth}
      \centering
      \begin{tikzpicture}[on grid, auto, scale=0.98]
        \input{figures/lct_examples/scale_small.tex}
        \input{figures/head_files_figs.tex}
        \input{figures/lct_examples/penfg/background_nodes_original.tex}
        \node[state_long] (f1) at (-\ldis,0) [label=above: $\LCT{f}_{i}$] {};
        \node[state_long] (f2) at (\ldis,0) [label=above: $\LCT{f}_{j}$] {};
        % draw the lines
        \input{figures/lct_examples/penfg/background_lines_orignal.tex}
        %----------------------------------------------------------------------
        \begin{pgfonlayer}{main} 
            \node (x1) at (0,-0.2*\sdis) 
            [label=above: $\vx_{\pone}$] {}; 
            \node (x3) at (-1.5*\ldis,1.5*\sdis) 
            [label=above: $\LCTv{x}_{\ptwo}$] {}; 
            \node (x4) at (-1.5*\ldis,-1.5*\sdis) 
            [label=below: $\LCTv{x}_{\pthre}$] {};

            \node (x3) at (1.5*\ldis,1.5*\sdis) 
            [label=above: $\LCTv{x}_{\pfor}$] {}; 
            \node (x4) at (1.5*\ldis,-1.5*\sdis) 
            [label=below: $\LCTv{x}_{\pfif}$] {}; 
        \end{pgfonlayer}
        %----------------------------------------------------------------------
      \end{tikzpicture}
    \end{minipage}
  }
  \subfloat[\label{sec:CheckCon:fig:8:subfig:2}]{
    \begin{minipage}[t]{0.45\linewidth}
      \centering
      \begin{tikzpicture}[on grid, auto, scale=0.98]
        \input{figures/lct_examples/scale_small.tex}
        \input{figures/head_files_figs.tex}

        \input{figures/proof_lower_bound/background_nodes_after_lct_proof_s.tex}
        \input{figures/proof_lower_bound/background_variables_evd_s.tex}
        
        \input{figures/lct_examples/penfg/variables_after_lct_clb.tex}

        \input{figures/lct_examples/penfg/background_lines.tex}
        \input{figures/lct_examples/penfg/otb_dashed_boxes_evd_after_lct.tex}
        
      \end{tikzpicture}
    \end{minipage}
  }

  \subfloat[\label{sec:CheckCon:fig:8:subfig:3}]{
    \begin{minipage}[t]{0.45\linewidth}
      \centering
      \begin{tikzpicture}[on grid, auto, scale=0.98]
        \input{figures/proof_lower_bound/scale_large_pesnfg_lower_bound.tex}
        \input{figures/head_files_figs.tex}
        \tikzstyle{state_dash5}=[shape=rectangle, draw, dashed, minimum width= 1.7*\sdis cm, minimum height = 4.1*\ldis cm,outer sep=-0.3pt, fill=black!10]

        \input{figures/proof_lower_bound/background_nodes_after_lct_proof.tex}
        \input{figures/proof_lower_bound/function_otb_lct.tex}
        \input{figures/proof_lower_bound/background_variables_EVD_l}

        \input{figures/lct_examples/penfg/variables_after_lct_clb.tex}
        \input{figures/lct_examples/penfg/background_lines.tex}
        \input{figures/lct_examples/penfg/otb_dashed_boxes_evd_after_lct.tex}
  
      \end{tikzpicture}
    \end{minipage}
  }
  \subfloat[\label{sec:CheckCon:fig:8:subfig:4}]{
    \begin{minipage}[t]{0.45\linewidth}
      \centering
      \begin{tikzpicture}[on grid, auto, scale=0.98]
        \input{figures/proof_lower_bound/scale_large_pesnfg_lower_bound.tex}
        \input{figures/head_files_figs.tex}
        \begin{pgfonlayer}{behind} 
            \node[state_dash7] (db1) at (-0.8*\ldis,-0.6*\sdis) 
            [label=above: $ \MLUfn{i} $] {};
            \node[state_dash7] (db2) at (0.8*\ldis,-0.6*\sdis)  [label=above: 
            $ \MLUfn{j} $] {};

            \node[state_dash7] (db1) at (-0.8*\ldis,-5.18*\sdis) 
            [label=below: $ \overline{\MLUfn{i}} $] {};
            \node[state_dash7] (db2) at (0.8*\ldis,-5.18*\sdis)  
            [label=below: $ \overline{\MLUfn{j}} $] {};
        \end{pgfonlayer}

        \input{figures/proof_lower_bound/background_nodes_after_lct_proof.tex}
        \input{figures/proof_lower_bound/background_variables_EVD_l0.tex}
        \input{figures/proof_lower_bound/function_otb_lct.tex}
        
        \input{figures/lct_examples/penfg/variables_after_lct_clb.tex}
        \input{figures/lct_examples/penfg/background_lines.tex}
      \end{tikzpicture}
    \end{minipage}
  }
  \end{adjustbox}
  \caption{Illustrating the main idea of the proof in Appendix~\ref{apx:check_cond_lower} by an example PE-NFG.}
\end{figure}

To outline the main idea of the proof,  we introduce the following definitions for each $f \in \setF$.
%----------------------------------------------------------------------------
\begin{definition}
    We consider the Cholesky decomposition of the Choi-matrix representation $ \matr{C}_{\LCT{f}} $ provided in Item~\ref{prop:DENFG:LCT:1:item:5} in Proposition~\ref{prop:DENFG:LCT:1}, which yields the function $ \LCT{L}_{f} $ and the set $ \LCTset{L}_{f} $. Without loss of generality, we suppose that $ \setpf = (1,\ldots,|\setpf|) $.
    %----------------------------------------------------------------------------
    \begin{enumerate}
      \item We define 
        \begin{align*}
            \LCTv{U}_{L,f} \defeq 
            \Bigl( 
                \LCT{U}_{L,f} \bigl( \LCTellf', \LCTellf \bigr)
            \Bigr)_{ \LCTellf', \LCTellf \in \LCTset{L}_{f} } 
        \end{align*} 
        to be a unitary matrix with row indices $ \LCTellf' $ and column indices $ \LCTellf $ such that
        \begin{align*}
            \sum_{\LCTellf \in \LCTset{L}_{f}} 
            \LCT{U}_{L,f} \bigl( \LCTellf', \LCTellf \bigr)
            \cdot  
            \overline{ \LCT{U}_{L,f} \bigl( \LCTellf'', \LCTellf \bigr) }
            &= \Bigl[ \LCTellf' \! = \! \LCTellf'' \Bigr], \qquad 
            \LCTellf', \LCTellf'' \in \LCTset{L}_{f}, \nonumber\\
            \LCTv{U}_{L,f}(\LCTellf,0) &= 
            \frac{1}{ \sqrt{\LCT{f}(\bm{0})}  }
            \cdot
            \overline{ \LCT{L}_{f}(\bm{0},\LCTellf) }, \qquad 
            \LCTellf \in \LCTset{L}_{f}.
      \end{align*}
      %------------------------------------------------------------------------
      % which implies
      % %-----------------------------------------------------------------------
      % \begin{align*}
      %   \bigl( \LCTv{U}_{L,f}( :, 0 ) \bigr)^{\Herm}
      %   \cdot \LCTv{U}_{L,f}( :, 0 )
      %   = 1.
      % \end{align*}
      % %-----------------------------------------------------------------------

        \item We define $ \LCTv{L}_{f} $ as follows:
        \begin{align}
            \LCTv{L}_{f} \defeq 
            \biggl( 
              \LCT{L}_{f}\Bigl( \LCTv{x}_{\setpf},\LCTell{f} \Bigr) 
            \biggr)_{ \LCTv{x}_{\setpf} \in \LCTset{X}_{\setpf}, 
            \LCTell{f} \in \LCTset{L}_{f} }.
            \label{eqn: def of matrix Lf}
        \end{align}
        This matrix has row indices $ \LCTv{x}_{\setpf} = ( \LCT{x}_{1},\ldots,\LCT{x}_{|\setpf|} ) $, which take values from $ (0,\ldots,0) $, $ (1,\ldots,0) $ to $ ( \bigl| \LCTsetx_{1} \bigr|-1,\ldots, \bigl| \LCTsetx_{|\setpf|} \bigr|-1) $, and column indices $ \LCTell{f_{i}} $, which take values from $ 0 $, $ 1 $ to $ |\LCTset{L}_{f}|-1 $.
        Note that 
        $ \bigl| \LCTset{L}_{f} \bigr| = \bigl| \LCTsetx_{\setpf} \bigr| $.
        % and $ \bm{0} $ is the all-zero vector of size $|\setpf|$.

        \item We define $ \mMLUf $ to be a matrix having the same row and column indexing as $\LCTv{L}_{f}$:
        %------------------------------------------------------------------------
        \begin{align*}
            \mMLUf \defeq
            \Bigl( \MLUf\bigl( \LCTv{x}_{\setpf}, \LCTellf \bigr) 
            \Bigr)_{ \LCTv{x}_{\setpf} \in \LCTset{X}_{\setpf}, \LCTellf \in \LCTset{L}_{f} },
        \end{align*}
        %------------------------------------------------------------------------
        where the entries are defined to be
        \begin{align*}
            \MLUf\bigl( \LCTv{x}_{\setpf}, \LCTellf \bigr) 
            \defeq 
            \sum_{\LCTellf' \in \LCTset{L}_{f}}
            \LCT{L}_{f}\Bigl( \LCTv{x}_{\setpf},\LCTellf' \Bigr)
            \cdot \LCT{U}_{L,f} \bigl( \LCTellf', \LCTellf \bigr).
        \end{align*}  
        By the Cholesky decomposition in~\eqref{sec:LCT:eqn:17}, the matrix $ \mMLUf $ satisfies the following property:
        %------------------------------------------------------------------------
        \begin{align}
            \mMLUf(:,0) = \LCTv{L}_{f} \cdot \LCTv{U}_{L,f}(:,0)
            = \frac{1}{ \sqrt{\LCT{f}(\bm{0})} } 
            \cdot 
            \LCTv{L}_{f} 
            \cdot \LCTv{L}_{f}( \bm{0},: )^{\Herm}
            &= \frac{1}{ \sqrt{\LCT{f}(\bm{0})} } 
            \cdot \matr{C}_{\LCT{f}}( :, \bm{0} ), \label{sec:CheckCon:eqn:39}
        \end{align}
        %------------------------------------------------------------------------
        % where $ \matr{C}_{\LCT{f}} $ is . 
        % Following the similar idea in the proof of Lemma~\ref{lem: nonnegative of ZBSPA for PE-NFG}, we know that $ \LCT{f}(\bm{0}) = Z_{\LCT{f}}( \LCTv{\mu} ) \in \sR_{\geq 0} $ for the SPA fixed-point message vector $ \LCTv{\mu} $ for $ \LCT{\sfN} $.

        \item For $ M \in \sZpp $, we define the collection of variables $ \LCTv{\ell}^{(M)} $ to be
        %-----------------------------------------------------------------------
        \begin{align*}
            \LCTv{\ell}^{(M)} \defeq 
            \bigl( \LCT{\ell}_{f,m} \bigr)_{f \in \setF, m \in [M]}
            \in \prod_{f} \LCTset{L}_{f}^{M}.
            % \qquad 
            % \ell'^{(M)} \defeq ( \ellfm' )_{f \in \setF, m \in [M]}
            % \in \prod_{f} \set{L}_{f}^{M}, \qquad 
            % \ell''^{(M)} \defeq ( \ellfm'' )_{f \in \setF, m \in [M]}
            % \in \prod_{f} \set{L}_{f}^{M},
        \end{align*}
        %-----------------------------------------------------------------------
        To simplify notation, if there is no ambiguity, 
        we use $ \sum_{ \LCT{\ell}_{f} } $ for each $ f \in \setF $ and $ \sum_{\LCTv{\ell}^{(M)}} $ 
        instead of 
        $ \sum_{ \LCT{\ell}_{f} \in \LCTset{L}_{f} } $ 
        for each $ f \in \setF $ and
        $ \sum_{ \LCTv{\ell}^{(M)} \in \prod_{f} \LCTset{L}_{f}^{M} } $, respectively.

        \item We define the vectors $ \cvpsi_{\setpf,f} $ and $ \cvpsi_{\upsetpf,f} $ to be
        \begin{align*}
            \cvpsi_{\setpf,f}
            \defeq
            \bigotimes_{e \in \setpf} 
            \cvpsi_{e,f} \in 
            \sC^{\prod_{e \in \setpf}|\LCTset{X}_{e}|},
            \qquad
            \cvpsi_{\upsetpf,f}
            \defeq
            \bigotimes_{\upe \in \upsetpf} 
            \cvpsi_{\upe,f} \in 
            \sC^{\prod_{\upe \in \upsetpf}|\LCTset{X}_{\upe}|}
        \end{align*}
    \end{enumerate}
    \edefinition
\end{definition}

The proof started by considering a
specific PE-NFG $\LCT{\graphN}$ and assume that a part of it looks as shown in Fig.~\ref{sec:CheckCon:fig:8:subfig:1}. The proof then proceeds through the following steps.
%----------------------------------------------------------------------------
\begin{enumerate}
    \item The Choi-matrix representations of $ \LCT{f}_{i} $ and $ \LCT{f}_{j} $, denoted as $ \matr{C}_{\LCT{f}_{i}} $ and $ \matr{C}_{\LCT{f}_{j}} $, respectively, are PSD matrices. The PE-NFG in Fig.~\ref{sec:CheckCon:fig:8:subfig:2} is obtained from the PE-NFG
    in Fig.~\ref{sec:CheckCon:fig:8:subfig:1} by applying the Cholesky decomposition in~\eqref{sec:LCT:eqn:17} to $ \matr{C}_{\LCT{f}_{i}} $ and $ \matr{C}_{\LCT{f}_{j}} $.

    \item The PE-NFG in Fig.~\ref{sec:CheckCon:fig:8:subfig:3} is obtained from the PE-NFG
    in Fig.~\ref{sec:CheckCon:fig:8:subfig:2} by introducing suitable opening-the-box operations. Since $ \LCTv{U}_{L,f} $ is a unitary matrix for all $ f \in \setF $,
    the partition function of the PE-NFG in Fig.~\ref{sec:CheckCon:fig:8:subfig:3} is equal to that of the PE-NFG
    in Fig.~\ref{sec:CheckCon:fig:8:subfig:2}.

    \item The PE-NFG in Fig.~\ref{sec:CheckCon:fig:8:subfig:4} is obtained from the PE-NFG
    in Fig.~\ref{sec:CheckCon:fig:8:subfig:3} by applying suitable closing-the-box operations and setting $ \LCTell{f_{i}} = \LCTell{f_{j}} = 0  $. 
    For example, the exterior function of the upper left dashed box in Fig.~\ref{sec:CheckCon:fig:8:subfig:4} is given by
    %------------------------------------------------------------------------
    \begin{align*}
        \MLUfn{i}(\LCTv{x}_{\setpfi},0) &= 
        \sum_{\LCTell{f_{i}}'}
        \LCT{L}_{f_{i}}\Bigl( \LCTv{x}_{\setpfi},\LCTell{f_{i}}' \Bigr)
        \cdot \LCT{U}_{L,f_{i}} \bigl( \LCTell{f_{i}}', 0 \bigr)
        = \frac{1}{\sqrt{\LCT{f}_{i}(\bm{0})}}
        \cdot C_{\LCT{f}_{i}}( \LCTv{x}_{\setpfi}, \bm{0} ), \qquad 
        \LCTv{x}_{\setpfi} \in \LCTset{X}_{\setpfi}.
    \end{align*}
    %------------------------------------------------------------------------

    \item Finally, it is shown that the partition function of the PE-NFG in Fig.~\ref{sec:CheckCon:fig:8:subfig:4} is smaller than or equal to that of the PE-NFG in Fig.~\ref{sec:CheckCon:fig:8:subfig:3}. The details of this step are provided in the remaining part of this appendix.
\end{enumerate}
%----------------------------------------------------------------------------
These steps outline the main idea of the proof and describe how the PE-NFG evolves through various transformations to establish the desired result.

%----------------------------------------------------------------------------
\begin{lemma} \label{sec:CheckCon:lem:integral w.r.t. psi dot e equals psi e}
    It holds that
    %------------------------------------------------------------------------
    \begin{align*}
        &\int
            \prod_{m}
            \prod_f 
            \cvpsi_{\upsetpf,f}
            \cdot \overline{ \mMLUf\bigl( :, \LCTell{f,m} \bigr) }
        \prod_{\upe \in \upsetEfull}
        \dd{\muFSsimple(\cvpsi_{\upe})}
        = \overline{ \int
            \prod_{m}
            \prod_f 
            \cvpsi_{\setpf,f}
            \cdot \mMLUf\bigl( :, \LCTell{f,m} \bigr)
        \prod_{e \in \setEfull}
        \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)} 
        }, \qquad 
        \LCTv{\ell}^{(M)} 
        \in \prod_{f} \LCTset{L}_{f}^{M}.
    \end{align*}
    %------------------------------------------------------------------------
\end{lemma}
%----------------------------------------------------------------------------
%----------------------------------------------------------------------------
\begin{proof}
    The proof is similar to the derivations of the equalities in~\eqref{sec:SST:eqn:34} in Appendix~\ref{apx:property of ZBM for PENFG}, and thus the details are omitted here. 
    % we have
    % %------------------------------------------------------------------------
    % \begin{align*}
    %     \hspace{0.25cm}&\hspace{-0.25cm}\int
    %     \prod_{m}
    %     \prod_f 
    %     % \left(
    %         \bigotimes_{\upe \in \upsetpf} 
    %         \cvpsi_{\upe,f}^{\tran}
    %         \cdot \overline{ \mMLUf\bigl( :, \LCTell{f,m} \bigr) }
    %     % \right)
    %     \prod_{\upe \in \upsetEfull}
    %     \dd{\muFSsimple(\cvpsi_{\upe})}
    %     \nonumber\\
    %     &\overset{(a)}{=} \int
    %         \prod_{m}
    %         \prod_f 
    %         % \left(
    %             \bigotimes_{e \in \setpf} 
    %             \cvpsi_{e,f}^{\tran}
    %             \cdot \overline{ \mMLUf\bigl( :, \LCTell{f,m} \bigr) }
    %         % \right)
    %     \prod_{e \in \setEfull}
    %     \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
    %     \nonumber\\
    %     &\overset{(b)}{=} 
    %     \int
    %         \prod_{m}
    %         \prod_f 
    %         % \left(
    %             \bigotimes_{e \in \setpf} 
    %             \cvpsi_{e,f}^{\Herm}
    %             \cdot \overline{ \mMLUf\bigl( :, \LCTell{f,m} \bigr) }
    %         % \right)
    %     \prod_{e \in \setEfull}
    %     \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
    %     \nonumber\\
    %     &=
    %     \overline{ \int
    %         \prod_{m}
    %         \prod_f 
    %         \bigotimes_{e \in \setpf} 
    %         \cvpsi_{e,f}^{\tran}
    %         \cdot \mMLUf\bigl( :, \LCTell{f,m} \bigr)
    %     \prod_{e \in \setEfull}
    %     \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)} 
    %     },
    % \end{align*}
    % %------------------------------------------------------------------------
    % where step $(a)$ follows from $ \LCTset{X}_{e} = \LCTset{X}_{\upe} $ for all $ \pe \in \psetEfull $ as defined in Definition~\ref{def:DENFG:LCT:1},
    % where step $(b)$ follows from the fact that $ \muFSsimple\bigl( \cvpsi_{e} \bigr) $ is a Fubini-Study measure, \ie, a Haar measure, over the set
    % $ \{ \vpsi_{e} \in \sC^{|\LCTsetxe|} \ | \ \| \vpsi_{e} \|_{2} = 1 \} $, which implies that replacing $ \cvpsi_{e,f} $ with $ \overline{\cvpsi_{e,f}}$ for all $ e \in \setEfull $ in the integral keeps the value of the integral unchanged.
\end{proof}
%----------------------------------------------------------------------------
We obtain
%----------------------------------------------------------------------------
\begin{align}
    \hspace{0.25cm}&\hspace{-0.25cm}\Biggl(
            \prod_{e \in \setEfull}
            |\set{B}_{\LCTsetx_{e}^M}|^{2}
    \Biggr)^{\!\! -1}\cdot
    \bigl( \ZBM(\graphN) \bigr)^{\! M}
    \nonumber\\
    % &\overset{(a)}{=}
    % \Biggl(
    %         \prod_{e \in \setEfull}
    %         |\set{B}_{\LCTsetx_{e}^M}|^{2}
    % \Biggr)^{-1}\cdot
    % \int \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt) 
    % \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
    % \nonumber\\
    &\overset{(a)}{=}
    % \Biggl(
    %     \prod_{e \in \setEfull}
    %     |\set{B}_{\LCTsetx_{e}^M}|^{2}
    % \Biggr)
    % \cdot
    \int
        \prod_f 
          \Bigl( 
            \ZSSTLCTf\bigl( \cvpsi_{\psetpf} \bigr) 
          \Bigr)^{\!\! M}
    \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
    \nonumber
    \\
    &\overset{(b)}{=}
    % \Biggl(
    %     \prod_{e \in \setEfull}
    %     |\set{B}_{\LCTsetx_{e}^M}|^{2}
    % \Biggr)
    % \cdot
    \int
        \prod_f \left(
          \sum_{\LCTellf}
          \left( 
            \sum_{\LCTv{x}_{\setpf}}
            \LCT{L}_{f}\bigl( \LCTv{x}_{\setpf},\LCTellf \bigr) 
            \cdot
            \prod_{e \in \setpf} 
            \cpsi_{e,f}(\LCT{x}_{e}) 
          \right)
        \cdot
        \left( 
            \sum_{\LCTv{x}_{\upsetpf}}
            \overline{ \LCT{L}_{f}\bigl( \LCTv{x}_{\upsetpf},\LCTellf \bigr) }
            \cdot
            \prod_{\upe \in \upsetpf} 
            \cpsi_{\upe,f}(\LCT{x}_{\upe}) 
      \right)
    \right)^{\!\!\!\! M}
    \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
    \nonumber \\
    &\overset{(c)}{=}
    \int
        \prod_f \biggr(
            \cvpsi_{\setpf,f}^{\tran}
            \cdot 
            \LCTv{L}_{f}
            % \right)
            \cdot 
            % \Bigl( 
            \LCTv{L}_{f}^{\Herm}
            \cdot 
            \cvpsi_{\upsetpf,f}
            % \Bigr)^{\!\! \Herm}
        \biggl)^{\!\! M}
    \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
    \nonumber \\
    &\overset{(d)}{=}
    \int
        \prod_f \biggr(
                \cvpsi_{\setpf,f}^{\tran}
                \cdot 
                \mMLUf
            % \right)
                \cdot 
                \mMLUf^{\Herm}
                \cdot
                \cvpsi_{\upsetpf,f}
        \biggl)^{\!\! M}
    \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
    \nonumber \\
    &=
    \sum_{\LCTv{\ell}^{(M)}}
    \int
        \prod_{m}
        \prod_f 
        % \left(
            % \left(
                \cvpsi_{\setpf,f}^{\tran}
                \cdot 
                \mMLUf\bigl( :, \LCTell{f,m} \bigr)
            % \right)
            \cdot 
            % \left( 
                \cvpsi_{\upsetpf,f}^{\tran}
                \cdot \overline{ \mMLUf\bigl( :, \LCTell{f,m} \bigr) }
            % \right)
        % \right)
    \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
    \nonumber \\
    &\overset{(e)}{=}
    \sum_{\LCTv{\ell}^{(M)}}
    \int
        \prod_{m}
        \prod_f 
        % \Biggl(
            \cvpsi_{\setpf,f}^{\tran}
            \cdot 
            \mMLUf\bigl( :, \LCTell{f,m} \bigr)
        % \Biggr)
    \prod_{e \in \setEfull}
    \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
    \cdot 
        \int
            \prod_{m}
            \prod_f 
            % \left(
                \cvpsi_{\upsetpf,f}^{\tran}
                \cdot \overline{ \mMLUf\bigl( :, \LCTell{f,m} \bigr) }
            % \right)
        \prod_{\upe \in \upsetEfull}
        \dd{\muFSsimple(\cvpsi_{\upe})}
    \nonumber \\
    &\overset{(f)}{=}
    \sum_{\LCTv{\ell}^{(M)}}
    \Biggl| \int
        \prod_{m}
        \prod_f 
        % \Biggl(
            \cvpsi_{\setpf,f}^{\tran}
            \cdot 
            \mMLUf\bigl( :, \LCTell{f,m} \bigr)
        % \Biggr)
    \prod_{e \in \setEfull}
    \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)} \Biggr|^{2}
    \nonumber \\
    &\geq 
    \sum_{\LCTv{\ell}^{(M)}}
    \Bigl[ \LCTell{f,m} = 0,\, \forall f \in \setF,\, m \in [M] \Bigr]
    \cdot \Biggl| \int
        \prod_{m}
        \prod_f 
        % \Biggl(
            \cvpsi_{\setpf,f}^{\tran}
            \cdot 
            \mMLUf\bigl( :, \LCTell{f,m} \bigr)
        % \Biggr)
    \prod_{e \in \setEfull}
    \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)} \Biggr|^{2}
    \nonumber\\
    &=
    \Biggl| \int
        \prod_f 
        \Bigl(
           \cvpsi_{\setpf,f}^{\tran}
            \cdot 
            \mMLUf( :, 0 )
        \Bigr)^{\!\! M}
    \prod_{e \in \setEfull}
    \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)} \Biggr|^{2}
    \nonumber \\
    &\overset{(g)}{=}
    \bigl( \ZBSPA(\graphN) \bigr)^{\!-M}
    \cdot \Biggl| \int 
    \prod_f
    \Bigl( 
        \cvpsi_{\setpf,f}^{\tran}
        \cdot 
        \matr{C}_{\LCT{f}}(:,\bm{0})
    \Bigr)^{\!\! M}
    \prod_{e \in \setEfull}
    \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
    \Biggr|^{2},
    \nonumber\\
    &\overset{(h)}{=}
    \bigl( \ZBSPA(\graphN) \bigr)^{\! -M}
    \cdot \Biggl| \int 
    \prod_f
    \Biggl( 
        \sum_{\LCTv{x}_{\setpf}}
        \LCT{f}( \LCTv{x}_{\setpf}, \bm{0} )
        \prod_{e \in \setpf} 
        \cpsi_{e,f}(\LCT{x}_{e}) 
    \Biggr)^{\!\!\! M}
    \prod_{e \in \setEfull}
    \dd{\muFSsimple(\cvpsi_{e})}
    \Biggr|^{2},
    % \nonumber \\
    % &=
    % \frac{1}{ \bigl( \ZBSPA(\graphN) \bigr)^{M} } 
    % \cdot \Biggl| \int 
    % \prod_f
    % \Bigl( 
    %     \bigotimes_{e \in \setpf} 
    %     \cvpsi_{e,f}^{\tran}
    %     \cdot 
    %     \matr{C}_{\LCT{f}}(:,\bm{0})
    % \Bigr)^{M}
    % \prod_{e \in \setEfull}
    % \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
    % \Biggr|^{2}, \label{sec:CheckCon:eqn:Zsst M-th power ineq}
\end{align}
%----------------------------------------------------------------------------
%----------------------------------------------------------------------------
\begin{itemize}
    \item where step $(a)$ follows from the expression of $ \ZBM $ in~\eqref{sec:CheckCon:eqn:42},

    \item where step $(b)$ follows from the definition of $ \ZSSTLCTf $ in~\eqref{sec:algsin:eqn:158} and the decomposition of $ \LCT{f} $ 
    in~\eqref{sec:LCT:eqn:17},

    \item where step $(c)$ follows from definition of $ \LCTv{L}_{f} $ in~\eqref{eqn: def of matrix Lf},

    \item where step $(d)$ follows from the fact that $ \LCTv{U}_{L,f} $ is a unitary matrix, \ie,
    %----------------------------------------------------------------------------
    \begin{align*}
        \mMLUf \cdot \mMLUf^{\Herm}
        = \LCTv{L}_{f} \cdot \LCTv{U}_{L,f}
        \cdot \LCTv{U}_{L,f}^{\Herm} \cdot \LCTv{L}_{f}^{\Herm}
        = \LCTv{L}_{f} \cdot \LCTv{L}_{f}^{\Herm},
    \end{align*}
    %----------------------------------------------------------------------------

    \item where step $(e)$ follows from
    \begin{align*}
        \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)} =
        \Biggl( \prod_{e \in \setEfull} 
            \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)} 
        \Biggr)
        \cdot
        \Biggl( \prod_{\upe \in \upsetEfull} 
            \dd{\muFSsimple\bigl( \cvpsi_{\upe} \bigr)} 
        \Biggr), \qquad 
        \int \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}  
        = \int \dd{\muFSsimple\bigl( \cvpsi_{\upe} \bigr)} = 1, \qquad
        \pe \in \psetEfull,
    \end{align*}

    \item where step $(f)$ follows from 
    Lemma~\ref{sec:CheckCon:lem:integral w.r.t. psi dot e equals psi e},

    \item where step $(g)$ follows from the property of $ \mMLUf $ in~\eqref{sec:CheckCon:eqn:39} and the expression of $ \ZBSPA(\graphN) $ in~\eqref{sec:CheckCon:eqn:31},

    \item where step $(h)$ follows from the definition of $ \matr{C}_{\LCT{f}} $ in~\eqref{sec:LCT:eqn:6}.
\end{itemize}
%----------------------------------------------------------------------------






  
% XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX

% By the expression in~\eqref{sec:CheckCon:eqn:42}, proving Lemma~\ref{sec:CheckCon:lem:1} is equivalent to proving that
% %-----------------------------------------------------------------------
% \begin{align*}
%   &\Biggl(
%     \prod_{e \in \setEfull}
%     |\set{B}_{\LCTsetx_{e}^M}|^{2}
%   \Biggr)^{-1}\cdot\int 
%   \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
%   \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)} 
%   \nonumber\\
%   &\geq
%   \frac{  1
%   }{ \bigl( \ZBSPA(\graphN) \bigr)^{M} } 
%   \cdot \Biggl| \int 
%   \prod_{m \in [M]} 
%   \prod_f
%   \Biggl( 
%       \sum_{\LCTv{x}_{\setpff,m}}
%       \LCT{f}( \LCTv{x}_{\setpff,m}, \bm{0} )
%       \prod_{e \in \setpf} 
%       \cpsi_{e,f}(\LCT{x}_{e,f,m}) 
%   \Biggr)
%   \prod_{e \in \setEfull}
%   \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
%   \Biggr|^{2}.
% \end{align*}
% %-----------------------------------------------------------------------
% The proof consists of two parts.
% %---------------------------------------------------------------------------
% \begin{enumerate}
%   \item 
%   % we define $ \LCT{U}_{L,f} : \LCTset{L}_{f} \times \LCTset{L}_{f} $ to be the function satisfying
%   % %-----------------------------------------------------------------------
%   % \begin{align}
%   %   \LCT{U}_{L,f}( \LCTellf, 0 ) &= 
%   %   \frac{\overline{ \LCT{L}_{f}(\bm{0},\LCTellf) }
%   %   }{ \sqrt{\LCT{f}(\bm{0})}  }, \qquad \LCTellf, \in \LCTset{L}_{f}
%   %   \label{sec:CheckCon:eqn:36}\\
%   %   \sum_{\LCTellf}
%   %   \LCT{U}_{L,f}( \LCTellf', \LCTellf )
%   %   \cdot \overline{ \LCT{U}_{L,f}( \LCTellf'', \LCTellf ) }
%   %   &= [ \LCTellf' = \LCTellf'' ], \qquad 
%   %   \LCTellf', \LCTellf'' \in \LCTset{L}_{f}.
%   %   \label{sec:CheckCon:eqn:37}, \\
%   %   \sum_{\LCTellf}
%   %   \LCT{U}_{L,f}( \LCTellf, \LCTellf' )
%   %   \cdot \overline{ \LCT{U}_{L,f}( \LCTellf, \LCTellf'' ) }
%   %   &= [ \LCTellf' = \LCTellf'' ], \qquad 
%   %   \LCTellf', \LCTellf'' \in \LCTset{L}_{f}. \nonumber
%   % \end{align}
%   % %-----------------------------------------------------------------------
%   % % The associated matrix $ \mU_{L,f} $ is
%   % %-----------------------------------------------------------------------
%   % \begin{align*}
%   %   \mU_{L,f} \defeq \begin{pmatrix}
%   %     \LCT{U}_{L,f}( 0, 0 ) & \LCT{U}_{L,f}( 0, 1 ) & \cdots & 
%   %     \LCT{U}_{L,f}( 0, |\LCTset{L}_{f}| ) \\
%   %     \LCT{U}_{L,f}( 1, 0 ) & \LCT{U}_{L,f}( 1, 1 ) & \cdots & 
%   %     \LCT{U}_{L,f}( 1, |\LCTset{L}_{f}| ) \\
%   %     \vdots & \vdots & \ddots & \vdots \\
%   %     \LCT{U}_{L,f}( |\LCTset{L}_{f}|, 0 ) 
%   %     & \LCT{U}_{L,f}( |\LCTset{L}_{f}|, 1 ) & \cdots & 
%   %     \LCT{U}_{L,f}( |\LCTset{L}_{f}|, |\LCTset{L}_{f}| )
%   %   \end{pmatrix}.
%   % \end{align*}
%   % %-----------------------------------------------------------------------
%   % For each $ f \in \setF $, we require the matrix $ \mU_{L,f} $ satisfying
%   % %-----------------------------------------------------------------------
%   % \begin{align}
%   %   \mU_{L,f} \cdot \mU_{L,f}^{\Herm} &= \matr{I}.
%   %   \nonumber
%   % \end{align}
%   % %-----------------------------------------------------------------------
%   % For simplicity, we define
%   % %------------------------------------------------------------------------
%   % \begin{align*}
%   %   \mMLUf
%   %   \defeq 
%   %   \LCTv{L}_{f}
%   %   \cdot \LCTv{U}_{L,f}.
%   % \end{align*}
%   % %------------------------------------------------------------------------
%   % The matrix $ \mU_{L,f} $ has a property:
%   % %-----------------------------------------------------------------------
%   % \begin{align} 
    
%   %   % \\
%   %   % \sum_{\LCTellf}
%   %   % \LCT{L}_{f}(\LCTv{x}_{\setpff},\LCTellf) 
%   %   % \cdot \LCT{U}_{L,f}( \LCTellf, 0 )
%   %   % &\overset{(a)}{=} \frac{1}{ \sqrt{\LCT{f}(\bm{0})} }
%   %   % \sum_{\LCTellf}
%   %   % \LCT{L}_{f}(\LCTv{x}_{\setpff},\LCTellf) 
%   %   % \cdot 
%   %   % \overline{ \LCT{L}_{f}(\bm{0},\LCTellf) }
%   %   % \overset{(b)}{=} \frac{1}{ \sqrt{\LCT{f}(\bm{0})} } 
%   %   % \LCT{f}( \LCTv{x}_{\setpff}, \bm{0} )
%   %   % = \MLUf(\LCTv{x}_{\setpff},0), 
%   % \end{align}
%   % %-----------------------------------------------------------------------
%   % where step $(a)$ follows from the definition of $ \LCT{U}_{L,f} $ in~\eqref{sec:CheckCon:eqn:36}, and where step $(b)$ follows from the decomposition of $ \LCT{f} $ in~\eqref{sec:LCT:eqn:1}. 
  
%   \item By the expression of $ \ZSSTM $ in~\eqref{sec:CheckCon:eqn:8}, we have
%   %-----------------------------------------------------------------------
%   \begin{align}
%       &\Biggl(
%             \prod_{e \in \setEfull}
%             |\set{B}_{\LCTsetx_{e}^M}|^{2}
%       \Biggr)^{-1}\cdot\ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt) 
%       \nonumber \\
%       &=
%       \prod_f \left(
%         \sum_{\LCTellf}
%         \Biggl( 
%           \sum_{\LCTv{x}_{\setpff}}
%           \MLUf(\LCTv{x}_{\setpff},\LCTellf)
%           \cdot
%           \prod_{e \in \setpf} 
%           \cpsi_{e,f}(\LCT{x}_{e,f}) 
%         \Biggr)
%         \right.
%         \cdot
%         \left.
%         \Biggl( 
%           \sum_{\LCTv{x}_{\upsetpff}}
%           \overline{
%             \MLUf(\LCTv{x}_{\upsetpff},\LCTellf)
%           }
%           \cdot
%           \prod_{\upe \in \upsetpf} 
%           \cpsi_{\upe,f}(\LCT{x}_{\upe,f}) 
%         \Biggr)
%       \right)^{M}. \label{sec:CheckCon:eqn:38}
%   \end{align}
%   %-----------------------------------------------------------------------
%   Then it holds that
%   %-------------------------------------------------------------------
%   \begin{align}
%       &\Biggl(
%             \prod_{e \in \setEfull}
%             |\set{B}_{\LCTsetx_{e}^M}|^{2}
%       \Biggr)^{-1}\cdot\int 
%       \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
%       \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
%       \nonumber\\
%       &\overset{(a)}{=} 
%       \sum_{\LCTv{\ell}^{(M)}}
%       \int 
%       \prod_{m \in [M]} 
%       \prod_f
%       \Biggl( 
%           \sum_{\LCTv{x}_{\setpff,m}}
%           \MLUf(\LCTv{x}_{\setpff,m},\LCTell{f,m})
%           \cdot \prod_{e \in \setpf} 
%           \cpsi_{e,f}(\LCT{x}_{e,f,m}) 
%       \Biggr)
%       \nonumber\\
%       &\quad \cdot 
%       \Biggl( 
%           \sum_{\LCTv{x}_{\upsetpff,m}}
%           \overline{
%             \MLUf(\LCTv{x}_{\upsetpff,m},\LCTell{f,m})
%           }
%           \cdot \prod_{\upe \in \upsetpf} 
%           \cpsi_{\upe,f}(\LCT{x}_{\upe,f,m}) 
%        \Biggr)
%       \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
%       \nonumber\\
%       &\overset{(b)}{=} 
%       \sum_{\LCTv{\ell}^{(M)}}
%       \int 
%       \prod_{m \in [M]} 
%       \prod_f
%       \Biggl( 
%           \sum_{\LCTv{x}_{\setpff,m}}
%           \MLUf(\LCTv{x}_{\setpff,m},\LCTell{f,m})
%           \cdot \prod_{e \in \setpf} 
%           \cpsi_{e,f}(\LCT{x}_{e,f,m}) 
%       \Biggr)
%       \prod_{e \in \setEfull}
%       \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
%       \nonumber\\
%       &\quad  \cdot 
%       \int 
%       \prod_{m \in [M]} 
%       \prod_f
%       \Biggl( 
%           \sum_{\LCTv{x}_{\upsetpff,m}}
%           \overline{
%             \MLUf(\LCTv{x}_{\upsetpff,m},\LCTell{f,m})
%           }
%           \cdot \prod_{\upe \in \upsetpf} 
%           \cpsi_{\upe,f}(\LCT{x}_{\upe,f,m}) 
%        \Biggr)
%       \prod_{\upe \in \upsetEfull}
%       \dd{\muFSsimple(\cvpsi_{\upe})}
%       \nonumber\\
%       &\overset{(c)}{=}
%       \sum_{\LCTv{\ell}^{(M)}}
%       \Biggl| \int 
%       \prod_{m \in [M]} 
%       \prod_f
%       \Biggl( 
%           \sum_{\LCTv{x}_{\setpff,m}}
%           \MLUf(\LCTv{x}_{\setpff,m},\LCTell{f,m})
%           \cdot \prod_{e \in \setpf} 
%           \cpsi_{e,f}(\LCT{x}_{e,f,m}) 
%       \Biggr)
%       \prod_{e \in \setEfull}
%       \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
%       \Biggr|^{2}, \label{sec:CheckCon:eqn:57}
%   \end{align}
%   %-------------------------------------------------------------------
%   where step $(a)$ follows from the expression of $ \ZSSTM  $ in~\eqref{sec:CheckCon:eqn:38},
%   where step $(b)$ follows from fact that the measure for  $ \{ \cvpsi_{e} \}_{e \in \setEfull}$ is independent of the measure for $ \{ \cvpsi_{\upe} \}_{\upe \in \upsetEfull} $, as defined in items~\ref{sec:SST:def:7:item:1} and~\ref{sec:SST:def:7:item:2} in Definition~\ref{sec:SST:def:7},
%   and step $(b)$ also follows from the properties of $ \muFSsimple\bigl( \cvpsiavgalt \bigr) $ in~\eqref{sec:SST:eqn:30}, 
%   and where step $(c)$ follows from similar derivations of the expression in~\eqref{sec:SST:eqn:34} in the proof of Proposition~\ref{sec:SST:prop:3}:
%   %------------------------------------------------------------------------
%   \begin{align*}
%     &\int 
%       \Biggl( 
%           \sum_{\LCTv{x}_{\upsetpff,m}}
%           \overline{
%             \MLUf(\LCTv{x}_{\upsetpff,m},\LCTell{f,m})
%           }
%           \prod_{\upe \in \upsetpf} 
%           \cpsi_{\upe,f}(\LCT{x}_{\upe,f,m}) 
%       \Biggr)
%     \prod_{\upe \in \upsetEfull}
%     \dd{\muFSsimple(\cvpsi_{\upe})} \nonumber\\
%     &\overset{(d)}{=} \int 
%       \Biggl( 
%           \sum_{\LCTv{x}_{\setpff,m}}
%           \overline{
%             \MLUf(\LCTv{x}_{\setpff,m},\LCTell{f,m})
%           }
%           \prod_{e \in \setpf} 
%           \cpsi_{e,f}(\LCT{x}_{e,f,m}) 
%       \Biggr)
%     \prod_{e \in \setEfull}
%     \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
%     \nonumber\\
%     &= \overline{
%       \int 
%         \Biggl( 
%             \sum_{\LCTv{x}_{\setpff,m}}
%               \MLUf(\LCTv{x}_{\setpff,m},\LCTell{f,m})
%             \prod_{e \in \setpf} 
%             \overline{ \cpsi_{e,f}(\LCT{x}_{e,f,m}) }
%         \Biggr)
%       \prod_{e \in \setEfull}
%       \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
%     }
%     \nonumber\\
%     &\overset{(e)}{=} \overline{
%       \int 
%         \Biggl( 
%             \sum_{\LCTv{x}_{\setpff,m}}
%               \MLUf(\LCTv{x}_{\setpff,m},\LCTell{f,m})
%             \prod_{e \in \setpf} 
%             \cpsi_{e,f}(\LCT{x}_{e,f,m})
%         \Biggr)
%       \prod_{e \in \setEfull}
%       \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
%     }
%   \end{align*}
%   %------------------------------------------------------------------------
%   where step $(d)$ follows from the following facts:
%   %---------------------------------------------------------------------------
%   \begin{enumerate}

%       \item the properties of the SST in Section~\ref{sec:SST:sunbsec:2} still hold if we consider applying the LCT and then the SST on the PE-NFG $ \graphN $. In order to use the properties of the SST for the resulting PE-NFG $ \LCT{\graphN} $, we need to do the following changes:
%       %---------------------------------------------------------------------------
%       \begin{itemize}
%           \item for each $ \pe = (e,\upe) \in \psetEfull $, we replace $ \setxpe $, $ \setxe $, and $ \set{X}_{\upe} $ with $ \LCTset{X}_{\pe} $, $ \LCTsetxe $, and $ \LCTset{X}_{\upe} $, respectively;

%           \item for each $ \pe = (e,\upe) \in \psetEfull $, we replace $ \xpe $, $ \xe $, and $ \xupe $ with $ \LCTv{x}_{\pe} $, $ \LCT{x}_{e} $, and $ \LCT{x}_{\upe} $, respectively; 

%           \item for each $ f \in \setF $, we replace $ f $, $ u_{f} $, and $ \lambda_{f} $ with $ \LCT{f} $, $ \LCT{u}_{f} $, and $ \LCT{\lambda}_{f} $ which are given in~\eqref{sec:LCT:eqn:1} and~\eqref{sec:LCT:eqn:2}--\eqref{sec:LCT:eqn:3}, respectively;

%           \item for each $ f \in \setF $, we replace $ \vx_{\psetpff} $, $ \vx_{\setpf,f} $, and $ \vx_{\upsetpf,f} $ with $ \LCTv{x}_{\psetpff} $, $ \LCTv{x}_{\setpf,f} $, and $ \LCTv{x}_{\upsetpf,f} $, respectively;

%           \item in terms of other variables, \textit{e.g.}, $ \vx_{\pe,m} $, $ x_{e,m} $, $  $, and $ x_{\upe,m} $ for each $ \pe = (e,\upe) \in \psetEfull $ and $ \vx_{\psetpff,m} $, $ \vx_{\setpf,f,m} $, and $ \vx_{\upsetpf,f,m} $ for $ f \in \setF $ with $ m \in \sZpp $, we apply similar change as above,

%       \end{itemize}
%       %---------------------------------------------------------------------------

%       \item for each $ f \in \setF $ and $ m \in [M] $, the variables $ \LCTv{x}_{\setpff,m} $ and $ \LCTv{x}_{\upsetpff,m} $ defined as 
%       %------------------------------------------------------------------------
%       \begin{align}
%         \LCTv{x}_{\setpff,m} \defeq
%         ( \LCT{x}_{e,f,m} )_{e \in \setpf},
%         \qquad 
%         \LCTv{x}_{\upsetpff,m} \defeq
%         ( \LCT{x}_{\upe,f,m} )_{\upe \in \upsetpf},
%         \label{sec:CheckCon:eqn:27}
%       \end{align}
%       %------------------------------------------------------------------------
%       have the same alphabet $\LCTsetxf = \prod_{e \in \setpf} \LCTsetxe =  \prod_{\upe \in \upsetpf} \LCTset{X}_{\upe} = \LCTset{X}_{\upsetpf} $ with $ \LCTsetxe = \LCTset{X}_{\upe} $ for all $ \pe = (e,\upe) \in \psetEfull $ as stated in item~\ref{def:DENFG:LCT:1:item:1} in Definition~\ref{def:DENFG:LCT:1};  

%       \item for each $ f \in \setF $ and $ m \in [M] $, the variables $ \LCTell{f,m} $, $ \LCTell{f,m}' $ and $ \LCTell{f,m}'' $ also have the same alphabet $ \LCTset{L}_{f}$.

%       \item for each $ \pe = (e,\upe) \in \psetEfull $, both $ \cvpsi_{e} $ and $ \cvpsi_{\upe} $ are vectors in $ \sC^{|\LCTsetxe|} $ with $ \|\cvpsi_{e}\| = \|\cvpsi_{\upe}\| =1 $;

%       \item for each $ \pe= (e,\upe) \in \psetEfull $, both the measure $ \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)} $ and the measure $ \dd{\muFSsimple(\cvpsi_{\upe})} $ are independent Fubini-Study measures, \textit{i.e.}, Haar measures over $ \sC^{|\LCTsetxe|} $, which are defined following the similar idea in~\eqref{sec:SST:eqn:30};

%       \item based on that, it is equivalent to replacing $ \dd{\muFSsimple(\cvpsi_{\upe})} $ and $ \psi_{\upe} $ with $ \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)} $ and $ \psi_{e} $, respectively, for all $ \pe = (e,\upe) \in \psetEfull $ in the integral,

%   \end{enumerate}
%   %---------------------------------------------------------------------------
%   and where step $(e)$ again follows from the fact that for each $ e \in \setEfull $, the measure $ \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)} $ is a Fubini-Study measure, \textit{i.e.}, a Haar measure over $ \sC^{|\LCTsetxe|} $. 
%   % and where step $(f)$ follows from Assumption~\ref{sec:DENFG:asum:2}, Property 8 in Proposition~\ref{prop:DENFG:LCT:1} and the fact that $ \LCT{\lambda}_{f}(\ellf) \in \sR_{\geq 0} $ for all $ \ellf \in \set{L}_{f} $ and $ f \in \setF $ as defined in~\eqref{sec:LCT:eqn:2}--\eqref{sec:LCT:eqn:3}. }
%   Then we have
%   %-------------------------------------------------------------------
%   \begin{align}
%       &\Biggl(
%             \prod_{e \in \setEfull}
%             |\set{B}_{\LCTsetx_{e}^M}|^{2}
%       \Biggr)^{-1}\cdot\int 
%       \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
%       \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)} 
%       \nonumber\\
%       &\overset{(a)}{\geq}
%       \Biggl| \int 
%       \prod_{m \in [M]} 
%       \prod_f
%       \Biggl( 
%           \sum_{\LCTv{x}_{\setpff,m}}
%           \MLUf(\LCTv{x}_{\setpff,m},0)
%           \prod_{e \in \setpf} 
%           \cpsi_{e,f}(\LCT{x}_{e,f,m}) 
%       \Biggr)
%       \prod_{e \in \setEfull}
%       \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
%       \Biggr|^{2}
%       \nonumber\\    
%       &\overset{(b)}{=}
%       \frac{1}{ \bigl( \ZBSPA(\graphN) \bigr)^{M} } 
%       \cdot \Biggl| \int 
%       \prod_{m \in [M]} 
%       \prod_f
%       \Biggl( 
%           \sum_{\LCTv{x}_{\setpff,m}}
%           \LCT{f}( \LCTv{x}_{\setpff,m}, \bm{0} )
%           \prod_{e \in \setpf} 
%           \cpsi_{e,f}(\LCT{x}_{e,f,m}) 
%       \Biggr)
%       \prod_{e \in \setEfull}
%       \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
%       \Biggr|^{2}, \label{sec:CheckCon:eqn:41}
%   \end{align}
%   %-------------------------------------------------------------------
%   where step $(a)$ follows from the inequality in~\eqref{sec:CheckCon:eqn:57},
%   and where step $(b)$ follows from the property of $ \MLUf $ in~\eqref{sec:CheckCon:eqn:39} and the expression of $ \ZBSPA(\graphN) $ in~\eqref{sec:CheckCon:eqn:31}.
% \end{enumerate}

==> appendices/check_cond_upper.tex <==

Consider the case where there exist $ e_{1} \in \setpf$ and $e_{2} \in \setpf $ such that
%------------------------------------------------------------------------
\begin{align}
    e_{1} \neq e_{2}, \qquad
    \LCTv{x}_{e_{1},e_{2}}' \defeq (\LCT{x}_{e_{1}}',\LCT{x}_{e_{2}}')
    \in \argmax_{ \LCTv{x}_{\psetpf \setminus \psetEf} }
    \bigl| 
        \vpsi_{ \psetpf \setminus \setEf }( \LCTv{x}_{\psetpf \setminus \setEf} ) 
    \bigr|.
    \label{sec:algsin:eqn:148}
      % \Biggl\{
      %   \Biggl(\prod_{e \in \setpf \setminus \setEf(\LCTv{x}_{\psetpf})} 
      %   |\cpsi_{e}(\LCT{x}_{e})| \Biggr) 
      %   \cdot \Biggl( \prod_{\upe \in \upsetpf \setminus \upsetEf(\LCTv{x}_{\psetpf}')}
      %   |\cpsi_{\upe}(\LCT{x}_{\upe}')| \Biggr)
      % \Biggr\}. 
\end{align}
%------------------------------------------------------------------------
The proof for other cases where there does not exists $ e_{1}, e_{2} \in \setpf $ satisfying~\eqref{sec:algsin:eqn:148} is similar and thus is omitted here. It holds that
%-----------------------------------------------------------------------
\begin{align}
  | \ZSSTLCTf(\cvpsi_{\psetpf}) | 
  % %--------------------------------------------------------------------
  &\overset{(a)}{=}  \left|\LCT{f}(\bm{0}) \cdot 
  \cvpsi_{\psetpf}(\bm{0})
  + \sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2} \LCT{f}(\LCTv{x}_{\psetpf}) 
  \cdot 
  \cvpsi_{\psetpf}(\LCTv{x}_{\psetpf})
  \right|
  \nonumber\\
  %--------------------------------------------------------------------
  &\leq \LCT{f}(\bm{0}) \cdot 
  |\cvpsi_{\psetpf}(\bm{0})|
  + \sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2} |\LCT{f}(\LCTv{x}_{\psetpf})| 
  \cdot |\cvpsi_{\psetpf}(\LCTv{x}_{\psetpf})|
  \nonumber \\
  %--------------------------------------------------------------------
  &\overset{(b)}{\leq} \LCT{f}(\bm{0}) \cdot 
  |\cvpsi_{\psetpf}(\bm{0})|
  + |\cvpsi_{\{e_{1},e_{2}\}}(\LCTv{x}_{e_{1},e_{2}}')|
  \cdot \sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2}
  |\LCT{f}(\LCTv{x}_{\psetpf})| \cdot |\cvpsi_{ \psetEf }( \LCTv{x}_{\psetEf} )|
  \nonumber\\
  %--------------------------------------------------------------------
  &\overset{(c)}{\leq} \LCT{f}(\bm{0}) \cdot 
  |\cvpsi_{\psetpf}(\bm{0})|
  + |\cvpsi_{\{e_{1},e_{2}\}}(\LCTv{x}_{e_{1},e_{2}}')|
  \cdot \sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2}
  |\LCT{f}(\LCTv{x}_{\psetpf})| \cdot |\cvpsi_{ \psetEf }( \LCTv{x}_{\psetEf} ) |^{1/(\df -2)}
  \nonumber\\
  %--------------------------------------------------------------------
  &\overset{(d)}{\leq} \LCT{f}(\bm{0}) \cdot 
  |\cvpsi_{\psetpf}(\bm{0})|
  + |\cvpsi_{\{e_{1},e_{2}\}}(\LCTv{x}_{e_{1},e_{2}}')|
  \cdot \sigupper( |\LCT{f}| )
  \nonumber\\
  %--------------------------------------------------------------------
  &\overset{(e)}{\leq} \LCT{f}(\bm{0}) \cdot 
  \bigl(
    |\cvpsi_{ \{e_{1},e_{2}\}}(\bm{0})| 
    + |\cvpsi_{ \{e_{1},e_{2}\} }(\LCTv{x}_{e_{1},e_{2}}')|
  \bigr) \nonumber\\
  %--------------------------------------------------------------------
  &\overset{(f)}{\leq} \LCT{f}(\bm{0}),
\end{align}
%-----------------------------------------------------------------------
where step $(a)$ follows from the expression of $ \ZSSTLCTf $ in~\eqref{sec:algsin:eqn:158} and the property that if $ \wh(\LCTv{x}_{\psetpf}) =1 $, we have $ \LCT{f}(\LCTv{x}_{\psetpf}) = 0 $ as stated in Proposition~\ref{prop:DENFG:LCT:1},
where step $(b)$ follows from~\eqref{sec:algsin:eqn:148}, \ie,
%----------------------------------------------------------------------------
\begin{align*}
  \sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2} |\LCT{f}(\LCTv{x}_{\psetpf})| 
  \cdot |\vpsi_{\psetpf}(\LCTv{x}_{\psetpf})|
  &\leq 
  \left\{
    \max_{ \LCTv{x}_{\psetpf \setminus \psetEf} }
    \bigl| 
        \vpsi_{ \psetpf \setminus \setEf }( \LCTv{x}_{\psetpf \setminus \setEf} ) 
    \bigr|
  \right\}
  \cdot
  \sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2} |\LCT{f}(\LCTv{x}_{\psetpf})| 
  \cdot |\vpsi_{\psetEf}(\LCTv{x}_{\psetEf})|
  \nonumber\\
  &= 
  |\cvpsi_{\{e_{1},e_{2}\}}(\LCTv{x}_{e_{1},e_{2}}')|
  \cdot
  \sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2} |\LCT{f}(\LCTv{x}_{\psetpf})| 
  \cdot |\vpsi_{\psetEf}(\LCTv{x}_{\psetEf})|,
\end{align*}
%----------------------------------------------------------------------------
where step $(c)$ follows from the fact that $ \df \geq 4 $ 
and 
$  0 \leq |\cpsi_{e}(\LCT{x}_{e})|, |\cpsi_{\upe}(\LCT{x}_{\upe})| \leq 1 $ for all $ \LCTv{x}_{\pe} \in \LCTset{X}_{\pe} $ and $ \pe \in \psetpf $,
where step $(d)$ follows from the definition of $ \sigupper $ in Definition~\ref{sec:algsin:def:1},
where step $(e)$ follows from the assumption in~\eqref{sec:3:eqn:13}, 
and where step $(f)$ follows from the Cauchy-Schwarz inequality, \ie,
%----------------------------------------------------------------------------
\begin{align*}
  |\cvpsi_{\{e_{1},e_{2}\}}(\bm{0})| 
  + |\cvpsi_{\{e_{1},e_{2}\}}(\LCTv{x}_{e_{1},e_{2}}')|
  \leq
  \Bigl( 
  \bigl| \cpsi_{e_{1}}(0) \bigr|^{2}
  +
  \bigl| \cpsi_{e_{1}}(\LCT{x}_{e_{1}}') \bigr|^{2} 
  \Bigr)^{1/2}
  \cdot 
  \Bigl( 
  \bigl| \cpsi_{e_{2}}(0) \bigr|^{2}
  +
  \bigl| \cpsi_{e_{2}}(\LCT{x}_{e_{2}}') \bigr|^{2} 
  \Bigr)^{1/2}
  \leq 1, \qquad 
  \| \cvpsi_{e_{1}} \|_{2} = \| \cvpsi_{e_{2}} \|_{2} =1.
\end{align*}
%----------------------------------------------------------------------------

% In particular, the second term on the right-hand side of the inequality in~\eqref{sec:algsin:eqn:57} satisfies
% %-----------------------------------------------------------------------
% \begin{align}
%   &\sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2} |\LCT{f}(\LCTv{x}_{\psetpf})| 
%   \cdot \Biggl( \prod_{e \in  \setpf} \bigl| \cpsi_{e}(\LCT{x}_{e}) \bigr| \Biggr) 
%   \cdot \Biggl( \prod_{\upe \in  \upsetpf} \bigl| \cpsi_{\upe}(\LCT{x}_{\upe}) \bigr| \Biggr)
%   \nonumber\\
%   &\overset{(a)}{\leq} 
%   \Biggl( 
%       \sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2} 
%       |\LCT{f}(\LCTv{x}_{\psetpf})|
%       \cdot 
%       \Biggl(\prod_{e \in  \setEf(\LCTv{x}_{\psetpf})} |\cpsi_{e}(\LCT{x}_{e})| \Biggr) 
%       \cdot \Biggl( \prod_{\upe \in  \upsetEf(\LCTv{x}_{\psetpf})}|\cpsi_{\upe}(\LCT{x}_{\upe})| \Biggr)
%   \Biggr)
%   \nonumber\\
%   &\quad\cdot 
%   \max_{ \LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2 }
%   \Biggl\{
%     \Biggl(\prod_{e \in \setpf \setminus \setEf(\LCTv{x}_{\psetpf})} |\cpsi_{e}(\LCT{x}_{e})| \Biggr) 
%     \cdot \Biggl( \prod_{\upe \in \upsetpf \setminus \upsetEf(\LCTv{x}_{\psetpf})}|\cpsi_{\upe}(\LCT{x}_{\upe})| \Biggr)
%   \Biggr\},\label{sec:algsin:eqn:61}
% \end{align}
% %-----------------------------------------------------------------------
% where step $(a)$ follows from the definitions of $ \setEf(\LCTv{x}_{\psetpf}) $ and $ \upsetEf(\LCTv{x}_{\psetpf}) $ in Definition~\ref{sec:algsin:def:1}, which are defined based on $ \LCTv{x}_{\psetpf} $. By the definitions of $ \setEf(\LCTv{x}_{\psetpf}) $ and $ \upsetEf(\LCTv{x}_{\psetpf}) $ in Definition~\ref{sec:algsin:def:1}, we know that 
% %----------------------------------------------------------------------------
% \begin{itemize}
%     \item  $ | \setpf \setminus \setEf(\LCTv{x}_{\psetpf}) | + | \upsetpf \setminus \upsetEf(\LCTv{x}_{\psetpf}) |=2 $;
%     \item  $ \LCT{x}_{e} \neq 0 $ for $  e \in  \setpf \setminus \setEf(\LCTv{x}_{\psetpf}) $;
%     \item  $ \LCT{x}_{\upe} \neq 0$ for $ \upe \in \upsetpf \setminus \upsetEf(\LCTv{x}_{\psetpf}) $.
% \end{itemize}
% %----------------------------------------------------------------------------
% In this proof, we consider that there exist $ \LCTv{x}_{\psetpf}' \in \setx_{\psetpf} $ and edges $ e_{1} $ and $e_{2}$ such that  
% %------------------------------------------------------------------------
% \begin{align}
%     &e_{1}, e_{2} \in \setpf \setminus \setEf(\LCTv{x}_{\psetpf}),\, 
%     e_{1} \neq e_{2},\,
%     \LCT{x}_{e_{1}}' \in \set\LCT{x}_{e_{1}} \setminus \{0\}, \,
%     \LCT{x}_{e_{2}}' \in \set\LCT{x}_{e_{2}} \setminus \{0\}, \,
%     \nonumber\\ 
%     &\bigl| \cpsi_{e_{1}}(\LCT{x}_{e_{1}}')\cdot
%     \cpsi_{e_{2}}(\LCT{x}_{e_{2}}') \bigr|
%     = \max_{ \LCTv{x}_{\psetpf}':\ \wh(\LCTv{x}_{\psetpf}') \geq 2 }
%       \Biggl\{
%         \Biggl(\prod_{e \in \setpf \setminus \setEf(\LCTv{x}_{\psetpf}')} 
%         |\cpsi_{e}(\LCT{x}_{e}')| \Biggr) 
%         \cdot \Biggl( \prod_{\upe \in \upsetpf \setminus \upsetEf(\LCTv{x}_{\psetpf}')}
%         |\cpsi_{\upe}(\LCT{x}_{\upe}')| \Biggr)
%       \Biggr\}. \label{sec:algsin:eqn:148}
% \end{align}
% %------------------------------------------------------------------------
% The proof of other cases is similar and thus it is omitted here. Then we have
% %----------------------------------------------------------------------------
% \begin{align}
%   &\sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2} |\LCT{f}(\LCTv{x}_{\psetpf})| 
%   \cdot \Biggl( \prod_{e \in  \setpf} \cpsi_{e}(\LCT{x}_{e}) \Biggr) 
%   \cdot \Biggl( \prod_{\upe \in  \upsetpf} \cpsi_{\upe}(\LCT{x}_{\upe}) \Biggr)
%   \nonumber\\
%   &\overset{(a)}{\leq}
%   \bigl| \cpsi_{e_{1}}(\LCT{x}_{e_{1}}')\cdot
%   \cpsi_{e_{2}}(\LCT{x}_{e_{2}}') \bigr|
%   \cdot
%    \Biggl( 
%       \sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2} 
%       |\LCT{f}(\LCTv{x}_{\psetpf})|
%       \cdot 
%       \Biggl(\prod_{e \in  \setEf(\LCTv{x}_{\psetpf})} |\cpsi_{e}(\LCT{x}_{e})| \Biggr) 
%       \cdot \Biggl( \prod_{\upe \in  \upsetEf(\LCTv{x}_{\psetpf})}|\cpsi_{\upe}(\LCT{x}_{\upe})| \Biggr)
%   \Biggr)
%   \nonumber\\
%   &\overset{(b)}{\leq}
%   \bigl| \cpsi_{e_{1}}(\LCT{x}_{e_{1}}')\cdot
%   \cpsi_{e_{2}}(\LCT{x}_{e_{2}}') \bigr|
%   \cdot \sigupper( |\LCT{f}| )
%   \nonumber\\
%   &\overset{(e)}{\leq}\bigl| \cpsi_{e_{1}}(\LCT{x}_{e_{1}}')\cdot
%   \cpsi_{e_{2}}(\LCT{x}_{e_{2}}') \bigr|
%   \cdot \LCT{f}(\bm{0}),\label{sec:algsin:eqn:149}
% \end{align}
% %----------------------------------------------------------------------------
% where step $(a)$ follows from the inequality in~\eqref{sec:algsin:eqn:61} and the property of $ e_{1} $ and $ e_{2} $ in~\eqref{sec:algsin:eqn:148}, 
% where step $(b)$ follows from the following derivations
% %----------------------------------------------------------------------------
% \begin{align*}
%     &\sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2} 
%     |\LCT{f}(\LCTv{x}_{\psetpf})|
%     \cdot 
%     \Biggl(\prod_{e \in  \setEf(\LCTv{x}_{\psetpf})} |\cpsi_{e}(\LCT{x}_{e})| \Biggr) 
%     \cdot \Biggl( \prod_{\upe \in  \upsetEf(\LCTv{x}_{\psetpf})}|\cpsi_{\upe}(\LCT{x}_{\upe})| \Biggr)
%     \nonumber\\
%     &\overset{(c)}{\leq}
%     \sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2} 
%     |\LCT{f}(\LCTv{x}_{\psetpf})|
%     \cdot 
%     \Biggl(\prod_{e \in  \setpf:\ \LCT{x}_{e} = 0} |\gamma_{e}'(\LCT{x}_{e})| \Biggr)^{1/(\df-2)} 
%     \cdot \Biggl( \prod_{e \in \setpf:\LCT{x}_{\upe} = 0}|\gamma_{e}'(\LCT{x}_{\upe})| \Biggr)^{1/(\df-2)} 
%     \nonumber\\
%     & \overset{(d)}{\leq}
%     \sigupper( |\LCT{f}| )
% \end{align*}
% %----------------------------------------------------------------------------
% where step $(c)$ follows from the substitutions
% %------------------------------------------------------------------------
% \begin{align*}
%   \gamma_{e}'(\LCT{x}_{e}) = \bigl( \cpsi_{e}(\LCT{x}_{e}) \bigr)^{2} \in \sR_{\geq 0}, \qquad 
%   \LCT{x}_{e} \in \setxe, \, e \in \setpf, \qquad
%   \gamma_{\upe}'(\LCT{x}_{\upe}) = \bigl( \cpsi_{\upe}(\LCT{x}_{\upe}) \bigr)^{2}
%   \in \sR_{\geq 0}, \qquad 
%   \LCT{x}_{\upe} \in \setx_{\upe}, \, \upe \in \upsetpf,
% \end{align*}
% %------------------------------------------------------------------------
% and the properties 
% %----------------------------------------------------------------------------
% \begin{align*}
%     \sum_{\LCT{x}_{e}} \Bigl( \cpsi_{e}(\LCT{x}_{e}) \Bigr)^{2}
%     &= \sum_{\LCT{x}_{e}} \gamma_{e}'(\LCT{x}_{e}) 
%     = \sum_{\LCT{x}_{\upe}} \Bigl( \cpsi_{\upe}(\LCT{x}_{\upe}) \Bigr)^{2}
%     = \sum_{\LCT{x}_{\upe}} \gamma_{\upe}'(\LCT{x}_{\upe}) = 1, 
%     \qquad e \in \setpf, \, \upe \in \upsetpf,\nonumber\\
%     0&\leq \gamma_{e}'(\LCT{x}_{e}) \leq 1,\qquad
%     |\gamma_{e}'(\LCT{x}_{e})|^{1/2} \leq | \gamma_{e}'(\LCT{x}_{e}) |^{1/(\df-2)},
%     \qquad \LCT{x}_{e} \in \setxe, \, e \in \setpf,\,
%     \df \geq 4,
%     \nonumber\\
%     0&\leq \gamma_{\upe}'(\LCT{x}_{\upe}) \leq 1, \qquad
%     |\gamma_{\upe}'(\LCT{x}_{\upe})|^{1/2} \leq | \gamma_{\upe}'(\LCT{x}_{\upe}) |^{1/(\df-2)},
%     \qquad \LCT{x}_{\upe} \in \setxupe, \, 
%     \upe \in \upsetpf, \,
%     \df \geq 4,
% \end{align*}
% %----------------------------------------------------------------------------
% where step $(d)$ follows from the definition of $ \sigupper( |\LCT{f}| ) $ in~XXX,
% and where step $ (e) $ follows from the inequality in~\eqref{sec:3:eqn:13}.
% Then the expression on the right-hand side of the inequality in~\eqref{sec:algsin:eqn:57} is upper bounded by
% %-----------------------------------------------------------------------
% \begin{align*}
%     &\LCT{f}(\bm{0}) \cdot 
%     \Biggl( \prod_{e \in  \setpf} \cpsi_{e}(0) \Biggr) 
%     \cdot \Biggl( \prod_{\upe \in  \upsetpf} \cpsi_{\upe}(0) \Biggr)
%     + 
%     \sum_{\LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 2} |\LCT{f}(\LCTv{x}_{\psetpf})| 
%     \cdot \Biggl( \prod_{e \in  \setpf} \cpsi_{e}(\LCT{x}_{e}) \Biggr) 
%     \cdot \Biggl( \prod_{\upe \in  \upsetpf} \cpsi_{\upe}(\LCT{x}_{e}) \Biggr)
%     \nonumber\\
%     &\overset{(a)}{\leq} 
%     \LCT{f}(\bm{0}) \cdot 
%     \Biggl( 
%         \Biggl( \prod_{e \in  \setpf} \cpsi_{e}(0) \Biggr) 
%         \cdot \Biggl( \prod_{\upe \in  \upsetpf} \cpsi_{\upe}(0) \Biggr)
%         + \bigl| \cpsi_{e_{1}}(\LCT{x}_{e_{1}}')\cdot
%         \cpsi_{e_{2}}(\LCT{x}_{e_{2}}') \bigr| 
%     \Biggr)
%     \nonumber\\
%     &\overset{(b)}{\leq} 
%     \LCT{f}(\bm{0}) \cdot 
%     \Biggl( 
%         \bigl|  \cpsi_{e_{1}}(0)\cdot
%         \cpsi_{e_{2}}(0) \bigr|
%         +  \bigl|  \cpsi_{e_{1}}(\LCT{x}_{e_{1}}')\cdot
%         \cpsi_{e_{2}}(\LCT{x}_{e_{2}}') \bigr|
%      \Biggr)
%     \nonumber\\
%     &\overset{(c)}{\leq} 
%     \LCT{f}(\bm{0}) \cdot 
%     \Biggl( 
%     \bigl| \cpsi_{e_{1}}(0) \bigr|^{2}
%     +
%     \bigl| \cpsi_{e_{1}}(\LCT{x}_{e_{1}}') \bigr|^{2} 
%     \Biggr)^{1/2}
%     \cdot 
%     \Biggl( 
%     \bigl| \cpsi_{e_{2}}(0) \bigr|^{2}
%     +
%     \bigl| \cpsi_{e_{2}}(\LCT{x}_{e_{2}}') \bigr|^{2} 
%     \Biggr)^{1/2}
%     \nonumber\\
%     &\overset{(d)}{\leq} 
%     \LCT{f}(\bm{0}),
% \end{align*}
% %-----------------------------------------------------------------------
% where step $(a)$ follows from the inequality in~\eqref{sec:algsin:eqn:149},
% where step $(b)$ follows from $ 0\leq | \cpsi_{e}(0) | \leq 1 $, $ e \in \setpf $, as indicated by the definition of $ \cpsi_{e} $ in~\eqref{sec:SST:eqn:28},
% and the fact that the edges $ e_{1} $ and $ e_{2} $ are in $ \setpf $,
% where step $(c)$ follows from Cauchy-Schwarz inequality,
% and where step $(d)$ follows from $ \| \cvpsi_{e} \|^{2} = \sum_{\LCT{x}_{e}} | \cpsi_{e}(\LCT{x}_{e}) |^{2} = 1 $ for all $ e \in \setpf $ as defined in~\eqref{sec:SST:eqn:36}--\eqref{sec:SST:eqn:22}.






% Because $ \df \geq 4 $, there exist edges $ e_{1}$, $ e_{2} $, and $ e_{3} $ in $ \setpf $ and associated variables $ \LCT{x}_{e_{1}} $, $\LCT{x}_{e_{2}} $, and $ x_{e_{3}} $ satisfying
% %-----------------------------------------------------------------------
% \begin{align}
%   &\LCT{x}_{e_{1}} \in \set\LCT{x}_{e_{1}} \setminus \{0\}, \,
%   \LCT{x}_{e_{2}} \in \set\LCT{x}_{e_{2}} \setminus \{0\}, \, 
%   x_{e_{3}} \in \setx_{e_{3}} \setminus \{0\},\qquad
%   e_{1} \neq e_{2},\, e_{2} \neq e_{3},\, e_{1} \neq e_{3}, \nonumber\\
%   &\bigl| \cpsi_{e_{1}}(\LCT{x}_{e_{1}}')\cdot
%   \cpsi_{e_{2}}(\LCT{x}_{e_{2}}')\cdot
%   \cpsi_{e_{3}}(x_{e_{3}}) \bigr|^{1-1/(\df-a_{f})}
%   \overset{(a)}{\geq} \max_{ \LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) \geq 3 }\Biggl\{  
%     \prod_{e \in \setpf} 
%     \bigl( |\cpsi_{e}(\LCT{x}_{e})| \cdot |\cpsi_{\upe}(\LCT{x}_{\upe})| \bigr)^{1-1/(\df-a_{f})}
%   \Biggr\}, \label{sec:algsin:eqn:59}
% \end{align}
% %-----------------------------------------------------------------------
% where step $(a)$ follows from the fact that $ |\cpsi_{e}(\LCT{x}_{e})| \leq 1 $ for all $ e \in \setpf $ as defined in~\eqref{sec:SST:eqn:36}--\eqref{sec:SST:eqn:22}. Without loss of generality, we suppose 
% %------------------------------------------------------------------------
% \begin{align*}
%   |\cpsi_{e_{3}}(x_{e_{3}})| \leq 
%   \min\{ |\cpsi_{e_{2}}(\LCT{x}_{e_{2}}')|, 
%   \, |\cpsi_{e_{1}}(\LCT{x}_{e_{1}}')| \}.
% \end{align*}
% %------------------------------------------------------------------------
% Then we have
% %------------------------------------------------------------------------
% \begin{align}
%   \bigl| \cpsi_{e_{1}}(\LCT{x}_{e_{1}}')\cdot
%   \cpsi_{e_{2}}(\LCT{x}_{e_{2}}')\cdot
%   \cpsi_{e_{3}}(x_{e_{3}}) \bigr|^{1-1/(\df-a_{f})}
%   &\leq \bigl| \cpsi_{e_{1}}(\LCT{x}_{e_{1}}')\cdot
%   \cpsi_{e_{2}}(\LCT{x}_{e_{2}}') \bigr|^{(3/2) \cdot (1-1/(\df-a_{f}))} \nonumber\\
%   %--------------------------------------------------------------------
%   &\overset{(a)}{\leq} \bigl| \cpsi_{e_{1}}(\LCT{x}_{e_{1}}')\cdot
%   \cpsi_{e_{2}}(\LCT{x}_{e_{2}}') \bigr|,
%   \label{sec:algsin:eqn:60}
% \end{align}
% %------------------------------------------------------------------------
% where at step $(a)$ we have used $ |\cpsi_{e_{1}}(\LCT{x}_{e_{1}}')|,\, |\cpsi_{e_{2}}(\LCT{x}_{e_{2}} )| \leq 1 $, $ \df - a \geq 3 $ as defined in~\eqref{sec:algsin:eqn:77}, and
% %------------------------------------------------------------------------
% \begin{align*}
%   \frac{3}{2}\cdot \Bigl( 1-\frac{1}{\df-a_{f}} \Bigr) \geq 1,
%   \qquad \df \geq 4.
% \end{align*}
% %------------------------------------------------------------------------
% Similarly, there exist edges $ e_{1} $ and $ e_{2} $ in $ \setpf $ and associated variables $ \LCT{x}_{e_{1}} $ and $\LCT{x}_{e_{2}} $ satisfying
% %-----------------------------------------------------------------------
% \begin{align}
%   & \LCT{x}_{e_{1}} \in \set\LCT{x}_{e_{1}} \setminus \{0\}, \,
%   \LCT{x}_{e_{2}} \in \set\LCT{x}_{e_{2}} \setminus \{0\}, \qquad 
%   e_{1} \neq e_{2}\nonumber\\
%   & \bigl| \cpsi_{e_{1}}(\LCT{x}_{e_{1}}')\cdot
%     \cpsi_{e_{2}}(\LCT{x}_{e_{2}}') \bigr|
%   =
%   \max\Biggl( \max_{ \LCTv{x}_{\psetpf}:\ \wh(\LCTv{x}_{\psetpf}) = 2 }
%   \Biggl\{
%     \biggl(\prod_{e \in  \setpf:\ \LCT{x}_{e} \neq 0} |\cpsi_{e}(\LCT{x}_{e})| \biggr) \cdot \biggl( \prod_{e \in \setpf:\LCT{x}_{\upe} \neq 0}|\cpsi_{\upe}(\LCT{x}_{\upe})| \biggr)
%   \Biggr\},
%     \bigl| \cpsi_{e_{1}}(\LCT{x}_{e_{1}}')\cdot
%     \cpsi_{e_{2}}(\LCT{x}_{e_{2}}') \bigr|
%   \Biggr), \label{sec:algsin:eqn:63}
% \end{align}
% %-----------------------------------------------------------------------
% Here the edges $ e_{1} $ and $ e_{2} $ can be different from the edges $ e_{1} $ and $ e_{2} $.
% Then we have

==> appendices/checkable_cond_graphcover.tex <==
In this appendix, we prove Theorem~\ref{sec:CheckCon:thm:1}.
By the analysis above Theorem~\ref{sec:CheckCon:thm:1}, it is sufficient to prove that~\eqref{sec:CheckCon:eqn:17}, \text{i.e.}, 
%----------------------------------------------------------------------------
\begin{align*}
    \lim_{M \to \infty} \Biggl(
        \int 
        \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
        \dd{\muFSsimple(\cvpsiavgalt)}
    \Biggr)^{1/M}
    = \ZBSPA(\graphN)
\end{align*}
%----------------------------------------------------------------------------
holds under the condition
%---------------------------------------------------------------------------
\begin{align}
    \LCT{u}_{f}(\LCTvxf,0)
    = [\LCTvxf = \bm{0}], \quad 
    \LCTvxf \in \LCTset{X}_{\setpf}, \, f \in \setEfull,
    \label{sec:CheckCon:eqn:22}
\end{align}
%---------------------------------------------------------------------------
where the set $ \LCTset{X}_{\setpf} = \prod_{e} \LCTset{X}_{e} $ and the variables 
%---------------------------------------------------------------------------
\begin{align}
    \LCTv{x}_{\psetpf} &= (\LCT{x}_{\pe})_{\pe \in \psetpf} 
    = ( \LCTv{x}_{\setpf}, \LCTv{x}_{\upsetpf} )
    \in \LCTset{X}_{\psetpf},\quad
    \LCTv{x}_{\setpf} = (\LCT{x}_{e})_{e \in \setpf}, 
    \in \LCTset{X}_{\setpf}, \qquad
    \LCTv{x}_{\upsetpf} 
    = (\LCT{x}_{\upe})_{\upe \in \upsetpf}, 
    \in \LCTset{X}_{\upsetpf}, \nonumber\\
    \LCT{x}_{\pe} &= (\LCT{x}_{e}, \LCT{x}_{\upe}) 
    \in \LCTset{X}_{\pe}, \quad
    \LCT{x}_{e} \in \LCTset{X}_{e},\, \LCT{x}_{\upe} 
    \in \LCTset{X}_{\upe}, 
    \nonumber\\
    \LCTv{x}_{\psetpff} &= (\LCT{x}_{\pe,f})_{\pe \in \psetpf} 
    =  ( \LCTv{x}_{\setpf,f}, \LCTv{x}_{\upsetpf,f} )
    \in \LCTset{X}_{\psetpf}, 
    \quad
    \LCTv{x}_{\setpf,f} = (\LCT{x}_{e,f})_{e \in \setpf}, 
    \in \LCTset{X}_{\setpf}, \qquad
    \LCTv{x}_{\upsetpf,f} 
    = (\LCT{x}_{\upe,f})_{\upe \in \upsetpf}, 
    \in \LCTset{X}_{\upsetpf}, 
    \label{sec:CheckCon:eqn:27}\\
    \LCT{x}_{\pe,f} &= (\LCT{x}_{e,f}, \LCT{x}_{\upe,f}) 
    \in \LCTset{X}_{\pe}, \quad
    \LCT{x}_{e,f} \in \LCTset{X}_{e},\, \LCT{x}_{\upe,f} 
    \in \LCTset{X}_{\upe}. \label{sec:CheckCon:eqn:28}
\end{align}
%---------------------------------------------------------------------------
are defined in Definition~\ref{def:DENFG:LCT:1},
where $ \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt) $ is defined in~\eqref{sec:CheckCon:eqn:8},
and where the functions $ \LCT{u}_{f} $ and $ \LCT{\lambda}_{f} $ are defined in~\eqref{sec:LCT:eqn:2}--\eqref{sec:LCT:eqn:3}.
Note that for each $ f \in \setF $, the largest eigenvalue for the matrix $ \LCTv{C}_{f} $ is $ \LCT{\lambda}_{f}(0) $ and the associated eigenvector is $ \LCTv{u}_{f}(0) $ as shown in~\eqref{sec:LCT:eqn:3}--\eqref{sec:LCT:eqn:7}. In the remaining part of this proof, we assume that $ \LCT{u}_{f} $ satisfies~\eqref{sec:CheckCon:eqn:22}. We have
%-----------------------------------------------------------------------
\begin{align}
    \ZBSPA(\graphN)
    &\overset{(a)}{=} 
    \ZBSPA(\LCT{\graphN},\LCT{\vmu})
    \nonumber\\
    &\overset{(b)}{=} 
    \frac{
        \prod_{f} \Bigl( 
        \sum_{\LCTv{x}_{\psetpf}} 
        \LCT{f}(\LCTv{x}_{\psetpf})
        \prod_{\pe \in \setpf}
        \LCT{\mu}_{\ef}^{(t)}(x_e)
        \cdot 
        \LCT{\mu}_{\upef}^{(t)}(x_{\upe})
        \Bigr)
    }{ 
        \prod_{e} 
        \Bigl( 
            \sum_{\xpe=(x_{e},x_{\upe})} 
            \LCT{\mu}_{\efi}^{(t)}(x_e)
            \cdot
            \LCT{\mu}_{\efj}^{(t)}(x_e)
            \cdot
            \LCT{\mu}_{\upefi}^{(t)}(x_{\upe})
            \cdot
            \LCT{\mu}_{\upefj}^{(t)}(x_{\upe}) 
        \Bigr) 
    } \nonumber\\
    &\overset{(c)}{=} \LCT{g}(\vect{0}) 
    \nonumber\\
    &\overset{(d)}{=}  
    \prod_{f \in \setF} \LCT{f}(\bm{0})
    \nonumber\\
    &\overset{(e)}{=} 
    \prod_{f \in \setF}
    \Biggl( 
        \sum_{\LCTellf \in \LCTset{L}_{f}}
            \LCT{\lambda}_{f}(\LCTellf) \cdot
            \LCT{u}_{f}(\bm{0},\LCTellf) 
        \cdot 
        \overline{ 
            \LCT{u}_{f}
            (\bm{0}, \LCTellf)
        }
    \Biggr) \nonumber\\
    &\overset{(f)}{=} \prod_{f \in \setF} \LCT{\lambda}_{f}(0),
    \label{sec:CheckCon:eqn:18}
\end{align}
%-----------------------------------------------------------------------
where step $(a)$ follows from the property of the SPA fixed-point messages vector in~\eqref{sec:CheckCon:eqn:31},
where step $(b)$ follows from the definition of $ \ZBSPA(\LCT{\graphN},\LCT{\vmu}) $ in Definition~\ref{sec:DENFG:def:3} and the fact that, as defined in item~\ref{def:DENFG:LCT:1:item:2} in Definition~\ref{def:DENFG:LCT:1}, in $ \LCT{\graphN} $ the local function associated with function node $ f $ is $ \LCT{f} $,
where step $(c)$ follows from the expressions of the fixed point messages $ \LCT{\vmu} $ in~\eqref{sec:CheckCon:eqn:7} and Property~\ref{prop:DENFG:LCT:1:item:4}\footnote{{\color{blue}XXXX If we replace the word Property with the word Item, then we need to change it gloally. XXXX}} in Proposition~\ref{prop:DENFG:LCT:1},
where step $ (d) $ follows from the global function $ \LCT{g}(\vx) = \prod_{f} \LCT{f}(\LCTv{x}_{f}) $ of $ \LCT{\graphN} $ as defined in Definition~\ref{def:DENFG:LCT:1},
where step $ (e) $ follows from the decomposition of $ \LCT{f} $ in Property~\ref{prop:DENFG:LCT:1:item:5} in Proposition~\ref{prop:DENFG:LCT:1}, where step $ (f) $ follows from
%-----------------------------------------------------------------------
\begin{align*}
    0
    &\overset{(f)}{=} \sum_{ 
      \LCTvxf 
      \in \LCTsetxpf
    }
    \LCT{u}_{f}(\LCTvxf,0) 
    \cdot 
    \overline{\LCT{u}_{f}
    (\LCTvxf,\ell_{\LCT{f}}')}
    \nonumber\\
    &\overset{(g)}{=}
    \overline{\LCT{u}_{f}
    (\bm{0},\ell_{\LCT{f}}')},
    \qquad 
    \ell_{\LCT{f}}' \in \LCTset{L}_{f} \setminus \{0\}, \,
    f \in \setF,
    \nonumber\\
    1&\overset{(f)}{=} \sum_{ 
      \LCTvxf 
      \in \LCTsetxpf
    }
    \LCT{u}_{f}(\LCTvxf,0) 
    \cdot 
    \overline{\LCT{u}_{f}
    (\LCTvxf,0)}
    \nonumber\\
    &\overset{(g)}{=}
    \overline{\LCT{u}_{f}
    (\bm{0},0)},\, f \in \setF,
\end{align*}
%-----------------------------------------------------------------------
where step $(f)$ follows from the definition of $ \LCT{u}_{f} $ and $ \LCTset{L}_{f} $ in~\eqref{sec:LCT:eqn:5} in Property~9 in Proposition~\ref{prop:DENFG:LCT:1},
and where step $(g)$ follows from the expression of $ \LCT{u}_{f}(\LCTvxf,0) $ in~\eqref{sec:CheckCon:eqn:22}. Steps $ (f) $ and $ (g) $ in the above expressions imply 
%---------------------------------------------------------------------------
\begin{align*}
    \begin{pmatrix}
        \LCT{u}_{f}(\bm{0},0) & \LCT{u}_{f}(\bm{0},1) & \cdots &
        \LCT{u}_{f}(\bm{0},|\LCTset{L}_{f}|)
    \end{pmatrix} = 
     \begin{pmatrix}
        1 & 0 & \cdots & 0
    \end{pmatrix}, \qquad f \in \setF.
\end{align*}
%---------------------------------------------------------------------------

The remaining part of the proof is divided into three parts.
%---------------------------------------------------------------------------
\begin{enumerate}
    \item We rewrite $ \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt) $ in~\eqref{sec:CheckCon:eqn:8} as
    %-------------------------------------------------------------------
    \begin{align}
        \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
        &\overset{(a)}{=}
        \prod_f \left( 
          \sum_{\LCTv{x}_{\psetpff}}
          \sum_{\LCTellf \in \LCTset{L}_{f}}
                \LCT{\lambda}_{f}(\LCTellf) \cdot
                \LCT{u}_{f}(\LCTv{x}_{\setpff},\LCTellf) 
            \cdot 
            \overline{ 
                \LCT{u}_{f}
                (\LCTv{x}_{\upsetpff}, \LCTellf)
            }
          \prod_{\pe \in \psetpf} 
          \cpsi_{\pe,f}(\LCT{x}_{\pe,f}) 
        \right)^{M}
        \nonumber\\
        &\overset{(b)}{=}
        \prod_f \left(
          \sum_{\LCTellf \in \LCTset{L}_{f}}
            \LCT{\lambda}_{f}(\LCTellf) 
            \cdot
            \Biggl( 
                \sum_{\LCTv{x}_{\setpff}}
                \LCT{u}_{f}(\LCTv{x}_{\setpff},\LCTellf) 
                \prod_{e \in \setpf} 
                \cpsi_{e,f}(\LCT{x}_{e,f}) 
            \Biggr)
            \cdot 
            \Biggl( 
                \sum_{\LCTv{x}_{\upsetpff}}
                \overline{ 
                    \LCT{u}_{f}
                    (\LCTv{x}_{\upsetpff}, \LCTellf)
                }
                \prod_{\upe \in \upsetpf} 
                \cpsi_{\upe,f}(\LCT{x}_{\upe,f}) 
             \Biggr)
        \right)^{M}, \label{sec:CheckCon:eqn:10}
    \end{align}
    %-------------------------------------------------------------------
    where step $(a)$ follows from the decomposition of $ \LCT{f} $ in~\eqref{sec:LCT:eqn:2},
    and where step $(b)$ follows from the definition of $ \cpsi_{\pe} $ in~\eqref{sec:SST:eqn:20}, \textit{i.e.}, $ \cpsi_{\pe,f}(\LCT{x}_{\pe,f})=  \cpsi_{e,f}(\LCT{x}_{e,f}) \cdot \cpsi_{\upe,f}(\LCT{x}_{\upe,f}) $ for all $ \LCT{x}_{\pe,f} = (\LCT{x}_{e,f},\LCT{x}_{\upe,f}) \in \LCTset{X}_{\pe} $ which is given in~\eqref{sec:CheckCon:eqn:28} with $ \LCTset{X}_{\pe} =  \LCTset{X}_{e}^{2} $ as defined in item~\ref{def:DENFG:LCT:1:item:5} in Definition~\ref{def:DENFG:LCT:1}, where the variable $ \LCTv{x}_{\psetpff} $ equals $ ( \LCTv{x}_{\setpff}, \LCTv{x}_{\upsetpff} ) $ as specified in~\eqref{sec:CheckCon:eqn:27}, and where the set $ \psetpf = \setpf \times \upsetpf $ is defined in item~\ref{sec:DENFG:def:4:item:2} in Definition~\ref{sec:DENFG:def:4}. Then $ |\ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)| $ satisfies
    %-------------------------------------------------------------------
    \begin{align}
        &|\ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)|
        \nonumber\\
        &\overset{(a)}{\leq}
        \prod_f \left( 
          \sum_{\LCTellf \in \LCTset{L}_{f}}
            \LCT{\lambda}_{f}(\LCTellf) 
            \cdot
            \Biggl| 
                \sum_{\LCTv{x}_{\setpff}}
                \LCT{u}_{f}(\LCTv{x}_{\setpff},\LCTellf) 
                \prod_{e \in \setpf} 
                \cpsi_{e,f}(\LCT{x}_{e,f}) 
            \Biggr|
            \cdot 
            \Biggl| 
                \sum_{\LCTv{x}_{\upsetpff}}
                \overline{ 
                    \LCT{u}_{f}
                    (\LCTv{x}_{\upsetpff}, \LCTellf)
                }
                \prod_{\upe \in \upsetpf} 
                \cpsi_{\upe,f}(\LCT{x}_{\upe,f}) 
             \Biggr|
        \right)^{M} \nonumber\\
        &\overset{(b)}{\leq}
        \prod_f \left( 
            \max_{
               \overset{\vpsi_{f},\vpsi_{f}' 
               \in \sC^{| \LCTsetxf|}}
               { \| \vpsi_{f} \|= \| \vpsi_{f}' \| = 1 }
            }
            \sum_{\LCTellf \in \LCTset{L}_{f}}
            \LCT{\lambda}_{f}(\LCTellf) 
            \cdot
            \Biggl| 
                \sum_{\LCTv{x}_{\setpff}}
                \LCT{u}_{f}(\LCTv{x}_{\setpff},\LCTellf) 
                \cdot \psi_{f}(\LCTv{x}_{\setpff})
            \Biggr|
            \cdot 
            \Biggl| 
                \sum_{\LCTv{x}_{\upsetpff}}
                \overline{ 
                    \LCT{u}_{f}
                    (\LCTv{x}_{\upsetpff}, \LCTellf)
                    \cdot \psi_{f}'(\LCTv{x}_{\upsetpff})
                }
             \Biggr|
        \right)^{M} 
        \nonumber\\
        &\overset{(c)}{\leq}
        \prod_f \left( 
            \max_{\LCTellf \in \LCTset{L}_{f}}
            \LCT{\lambda}_{f}(\LCTellf) 
        \right)^{M}
        \nonumber\\
        &\overset{(g)}{=}
        \prod_f \left( 
            \LCT{\lambda}_{f}(0) 
        \right)^{M} \label{sec:CheckCon:eqn:14}
    \end{align}
    %-------------------------------------------------------------------
    where step $(a)$ follows from $ \LCT{\lambda}_{f}(\LCTellf) \in \sR_{\geq 0} $ for all $ \LCTellf \in \LCTset{L}_{f} $ and $ f \in \setF $ as stated in Property 9 in Proposition~\ref{prop:DENFG:LCT:1},
    where step $ (b) $ follows from 
    %-------------------------------------------------------------------
    \begin{align*}
        \vpsi_{f} = \bigl(\psi_{f}(\LCTv{x}_{\setpff}) \bigr)_{\LCTv{x}_{\setpff} \in \LCTsetxpf} \in \sC^{|\LCTsetxpf|},
        \qquad
        \vpsi_{f}' = \bigl(\psi_{f}'(\LCTv{x}_{\setpff}) \bigr)_{\LCTv{x}_{\setpff} \in \LCTsetxpf} \in \sC^{|\LCTsetxpf|},
        \qquad 
        \|\vpsi_{f}\| = \| \vpsi_{f}' \|=1,
    \end{align*}
    %-------------------------------------------------------------------
    the definition of $ \LCTsetxpf $ in item~\ref{def:DENFG:LCT:1:item:1} in Definition~\ref{def:DENFG:LCT:1}, the definition of $ \cvpsi_{e} $ Definition~\ref{sec:SST:def:3} and the definition of $ \cvpsi_{e,f} $ in~\eqref{sec:SST:eqn:18}, \textit{i.e.}, $ \| \cpsi_{e,f} \| = 1 $ and $ \| \cpsi_{\upe,f} \| = 1 $ for all $ e \in \setpf $ and $ \upe \in \upsetpf $, 
    where step $(c)$ follows from 
    %----------------------------------------------------------------------------
    \begin{align}
        &\max_{
           \vpsi_{f},\vpsi_{f}' 
           \in \sC^{| \LCTsetxf|}
        }
        \sum_{\LCTellf \in \LCTset{L}_{f}}
        \LCT{\lambda}_{f}(\LCTellf) 
        \cdot
        \Biggl| 
            \sum_{\LCTv{x}_{\setpff}}
            \LCT{u}_{f}(\LCTv{x}_{\setpff},\LCTellf) 
            \cdot \psi_{f}(\LCTv{x}_{\setpff})
        \Biggr|
        \cdot 
        \Biggl| 
            \sum_{\LCTv{x}_{\upsetpff}}
            \overline{ 
                \LCT{u}_{f}
                (\LCTv{x}_{\upsetpff}, \LCTellf)
                \cdot \psi_{f}'(\LCTv{x}_{\upsetpff})
            }
        \Biggr|
        \label{sec:CheckCon:eqn:29}\\
        &\qquad \mathrm{s.t.}\quad 
        \|\vpsi_{f}\|= \|\vpsi_{f}'\|=1, 
        \nonumber\\
        &\overset{(d)}{=} \max_{
            \vpsi_{f} \in \sC^{|\LCTsetxf|}
        } \sum_{\LCTellf \in \LCTset{L}_{f}}
        \LCT{\lambda}_{f}(\LCTellf) 
        \cdot
        \Biggl| 
            \sum_{\LCTv{x}_{\setpff}}
            \LCT{u}_{f}(\LCTv{x}_{\setpff},\LCTellf) 
            \cdot \psi_{f}(\LCTv{x}_{\setpff})
        \Biggr|^{2}
        \nonumber\\
        &\qquad \mathrm{s.t.}\quad 
        \|\vpsi_{f}\|=1
        \nonumber\\
        &\overset{(e)}{=} \max_{
            \vpsi_{f} \in \sC^{| \LCTsetxf|}
        } \sum_{\LCTv{x}_{\psetpff}} 
        \LCT{f}(\LCTv{x}_{\setpff}, \LCTv{x}_{\upsetpff})
        \cdot \psi_{f}(\LCTv{x}_{\setpff})
        \cdot \overline{ \psi_{f}(\LCTv{x}_{\upsetpff}) }
        \nonumber\\
        &\qquad \mathrm{s.t.}\quad 
        \|\vpsi_{f}\|=1 \nonumber\\
        &\overset{(f)}{=} \max_{\LCTellf}
        \LCT{\lambda}_{f}(\LCTellf) 
    \end{align}
    %----------------------------------------------------------------------------
    where step $(d)$ follows from the following facts:
    %---------------------------------------------------------------------------
    \begin{enumerate}
        \item the function $  \LCT{\lambda}_{f}(\ellf) $ is nonnegative real-valued for all $ \ellf \in \LCTset{L}_{f} $ as defined in~\eqref{sec:LCT:eqn:3}; 

        \item by Cauchy-Schwarz inequality, the objective function in the optimization problem~\eqref{sec:CheckCon:eqn:29} is maximized when $ \cvpsi_{f}' = \overline{ \cvpsi_{f} } $,
    \end{enumerate}
    %---------------------------------------------------------------------------
    where step $(e)$ follows from the decompostion of $ \LCT{f} $ in~\eqref{sec:LCT:eqn:2}--\eqref{sec:LCT:eqn:3},
    where step $(f)$ follows from Courant–Fischer–Weyl min-max principle of the PSD matrix $ \LCTv{C}_{f} $ defined in~\eqref{sec:LCT:eqn:7}:
    %------------------------------------------------------------------------
    \begin{align*}
        \sum_{\LCTv{x}_{\psetpff}} 
        \LCT{f}(\LCTv{x}_{\setpff}, \LCTv{x}_{\upsetpff})
        \cdot \psi_{f}(\LCTv{x}_{\setpff})
        \cdot \overline{ \psi_{f}(\LCTv{x}_{\upsetpff}) }
        &= \vpsi_{f}^{\tran} \cdot \LCTv{C}_{f} \cdot
        \overline{ \vpsi_{f} }, \nonumber\\
        \max_{\LCTellf}
        \LCT{\lambda}_{f}(\LCTellf) &=\max_{
            \vpsi_{f} \in \sC^{| \LCTsetxf|}
        } \vpsi_{f}^{\tran} \cdot \LCTv{C}_{f} \cdot
        \overline{ \vpsi_{f} }
        \nonumber\\
        &\qquad \mathrm{s.t.}\quad 
        \|\vpsi_{f}\|=1,
    \end{align*}
    %------------------------------------------------------------------------
    and where step $(g)$ follows from the fact that $ \LCT{\lambda}_{f}(0) $ is the largest eigenvalue for $ \LCTv{C}_{f} $ as defined in~\eqref{sec:LCT:eqn:3} for each $ f \in \setF $:
    %-----------------------------------------------------------------------
    \begin{align*}
        \LCT{\lambda}_{f}(0) = \max_{\LCTellf}
        \LCT{\lambda}_{f}(\LCTellf).
    \end{align*}
    %-----------------------------------------------------------------------
    
    \item Similar to the proof of Proposition~\ref{sec:SST:prop:3}, we define
    %-------------------------------------------------------------------
    \begin{align*}
        \LCT{\ell}^{(M)} \defeq ( \LCTellfm )_{f \in \setF, m \in [M]}
        \in \prod_{f} \LCTset{L}_{f}^{M}.
    \end{align*}
    %-------------------------------------------------------------------
    Then it holds that
    %-------------------------------------------------------------------
    \begin{align}
        &\int 
        \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
        \dd{\muFSsimple(\cvpsiavgalt)}
        \nonumber\\
        &\overset{(a)}{=} 
        \int 
        \prod_f \left( 
          \sum_{\LCTellf \in \LCTset{L}_{f}}
            \LCT{\lambda}_{f}(\LCTellf) 
            \cdot
            \Biggl( 
                \sum_{\LCTv{x}_{\setpff}}
                \LCT{u}_{f}(\LCTv{x}_{\setpff},\LCTellf) 
                \prod_{e \in \setpf} 
                \cpsi_{e,f}(\LCT{x}_{e,f}) 
            \Biggr)
            \cdot 
            \Biggl( 
                \sum_{\LCTv{x}_{\upsetpff}}
                \overline{ 
                    \LCT{u}_{f}
                    (\LCTv{x}_{\upsetpff}, \LCTellf)
                }
                \prod_{\upe \in \upsetpf} 
                \cpsi_{\upe,f}(\LCT{x}_{\upe,f}) 
             \Biggr)
        \right)^{M}
        \dd{\muFSsimple(\cvpsiavgalt)}
        \nonumber\\
        &=
        \sum_{\LCT{\ell}^{(M)} \in \prod_{f} \LCTset{L}_{f}^{M} }
        \int 
        \prod_{m=1}^{M} 
        \prod_f
        \Biggl( 
            \sum_{\LCTv{x}_{\setpf,m}}
            \LCT{u}_{f}(\LCTv{x}_{\setpff,m},\LCTellfm) 
            \prod_{e \in \setpf} 
            \cpsi_{e,f}(\LCT{x}_{e,f,m}) 
        \Biggr)
        \cdot 
        \Biggl( 
            \sum_{\LCTv{x}_{\upsetpff,m}}
            \overline{ 
                \LCT{u}_{f}
                (\LCTv{x}_{\upsetpff,m}, \LCTellfm)
            }
            \prod_{\upe \in \upsetpf} 
            \cpsi_{\upe,f}(\LCT{x}_{\upe,f,m}) 
         \Biggr)
        \dd{\muFSsimple(\cvpsiavgalt)}
        \nonumber\\
        &\quad \cdot \Biggl(\prod_{m=1}^{M} 
        \prod_f \LCT{\lambda}_{f}(\LCTellfm) \Biggr) 
        \nonumber\\
        &\overset{(b)}{=} 
        \sum_{\LCT{\ell}^{(M)} \in \prod_{f} \LCTset{L}_{f}^{M} }
        \int 
        \prod_{m=1}^{M} 
        \prod_f
        \Biggl( 
            \sum_{\LCTv{x}_{\setpf,m}}
            \LCT{u}_{f}(\LCTv{x}_{\setpff,m},\LCTellfm) 
            \prod_{e \in \setpf} 
            \cpsi_{e,f}(\LCT{x}_{e,f,m}) 
        \Biggr)
        \prod_{e \in \setEfull}
        \dd{\muFSsimple(\cvpsi_{e})}
        \nonumber\\
        &\quad \cdot 
        \int 
        \prod_{m=1}^{M} 
        \prod_f
        \Biggl( 
            \sum_{\LCTv{x}_{\upsetpff,m}}
            \overline{ 
                \LCT{u}_{f}
                (\LCTv{x}_{\upsetpff,m}, \LCTellfm)
            }
            \prod_{\upe \in \upsetpf} 
            \cpsi_{\upe,f}(\LCT{x}_{\upe,f,m}) 
         \Biggr)
        \prod_{\upe \in \upsetEfull}
        \dd{\muFSsimple(\cvpsi_{\upe})}
        \cdot \Biggl(\prod_{m=1}^{M} 
        \prod_f \LCT{\lambda}_{f}(\LCTellfm) \Biggr) 
        \nonumber\\
        &\overset{(c)}{=}
        \sum_{\LCT{\ell}^{(M)} \in \prod_{f} \LCTset{L}_{f}^{M} }
        \Biggl(\prod_{m=1}^{M} 
        \prod_f \LCT{\lambda}_{f}(\LCTellfm) \Biggr) 
        \cdot
        \Biggl| \int 
        \prod_{m=1}^{M} 
        \prod_f
        \Biggl( 
            \sum_{\LCTv{x}_{\setpf,m}}
            \LCT{u}_{f}(\LCTv{x}_{\setpff,m},\LCTellfm) 
            \prod_{e \in \setpf} 
            \cpsi_{e,f}(\LCT{x}_{e,f,m}) 
        \Biggr)
        \prod_{e \in \setEfull}
        \dd{\muFSsimple(\cvpsi_{e})}
        \Biggr|^{2}, \label{sec:CheckCon:eqn:11}
    \end{align}
    %-------------------------------------------------------------------
    where step $(a)$ follows from the expression of $ \ZSSTM  $ in~\eqref{sec:CheckCon:eqn:10},
    where step $(b)$ follows from fact that the measure for  $ \{ \cvpsi_{e} \}_{e \in \setEfull}$ is independent of the measure for $ \{ \cvpsi_{\upe} \}_{\upe \in \upsetEfull} $, as defined in items~\ref{sec:SST:def:7:item:1} and~\ref{sec:SST:def:7:item:2} in Definition~\ref{sec:SST:def:7},
    and the properties of $ \muFSsimple(\cvpsiavgalt) $ in~\eqref{sec:SST:eqn:29}, 
    and where step $(c)$ follows from similar derivations of the expression in~\eqref{sec:SST:eqn:34} in the proof of Proposition~\ref{sec:SST:prop:3}:
    %------------------------------------------------------------------------
    \begin{align*}
        &\int 
        \prod_{m=1}^{M} 
        \prod_f
        \Biggl(
            \sum_{\LCTv{x}_{\upsetpff,m}}
            \overline{ 
                \LCT{u}_{f}
                (\LCTv{x}_{\upsetpff,m}, \LCTellfm)
            }
            \prod_{\upe \in \upsetpf} 
            \cpsi_{\upe,f}(\LCT{x}_{\upe,f,m})    
        \Biggr)
        \prod_{\upe \in \upsetEfull}
        \dd{\muFSsimple(\cvpsi_{\upe})}
        \nonumber\\
        &\overset{(d)}{=} 
        \Biggl(\int 
        \prod_{m=1}^{M} 
        \prod_f
        \Biggl( 
            \sum_{\LCTv{x}_{\setpf,m}}
            \overline{
                \LCT{u}_{f}(\LCTv{x}_{\setpff,m},\LCTellfm) 
            }
            \prod_{e \in \setpf} 
            \cpsi_{e,f}(\LCT{x}_{e,f,m})
        \Biggr)
        \prod_{e \in \setEfull}
        \dd{\muFSsimple(\cvpsi_{e})}
        \nonumber\\
        &= \overline{ 
        \Biggl(\int 
            \prod_{m=1}^{M} 
            \prod_f
            \Biggl( 
                \sum_{\LCTv{x}_{\setpf,m}}
                \LCT{u}_{f}(\LCTv{x}_{\setpff,m},\LCTellfm) 
                \prod_{e \in \setpf} 
                \overline{ \cpsi_{e,f}(\LCT{x}_{e,f,m}) }
            \Biggr)
            \prod_{e \in \setEfull}
            \dd{\muFSsimple(\cvpsi_{e})}
        }\Biggr)
        \nonumber\\
        &\overset{(e)}{=} \overline{ 
        \Biggl(\int 
        \prod_{m=1}^{M} 
        \prod_f
        \Biggl( 
            \sum_{\LCTv{x}_{\setpf,m}}
            \LCT{u}_{f}(\LCTv{x}_{\setpff,m},\LCTellfm) 
            \prod_{e \in \setpf} 
            \cpsi_{e,f}(\LCT{x}_{e,f,m})
        \Biggr)
        \prod_{e \in \setEfull}
        \dd{\muFSsimple(\cvpsi_{e})}
        \Biggr)}
    \end{align*}
    %------------------------------------------------------------------------
    where step $(d)$ follows from the following facts:
    %---------------------------------------------------------------------------
    \begin{enumerate}

        \item the properties of the SST in Section~\ref{sec:SST} still hold if we conisder applying the LCT and then the SST on a PE-NFG. In order to use the properties of the SST for the resulting PE-NFG, we need to do the following changes:
        %---------------------------------------------------------------------------
        \begin{itemize}
            \item for each $ \pe = (e,\upe) \in \psetEfull $, we replace $ \setxpe $, $ \setxe $, and $ \set{X}_{\upe} $ with $ \LCTset{X}_{\pe} $, $ \LCTsetxe $, and $ \LCTset{X}_{\upe} $, respectively;

            \item for each $ \pe = (e,\upe) \in \psetEfull $, we replace $ \xpe $, $ \xe $, and $ \xupe $ with $ \LCTv{x}_{\pe} $, $ \LCT{x}_{e} $, and $ \LCT{x}_{\upe} $, respectively; 

            \item for each $ f \in \setF $, we replace $ f $, $ u_{f} $, and $ \lambda_{f} $ with $ \LCT{f} $, $ \LCT{u}_{f} $, and $ \LCT{\lambda}_{f} $ which are defined in~\eqref{sec:LCT:eqn:1} and~\eqref{sec:LCT:eqn:2}--\eqref{sec:LCT:eqn:3}, respectively;

            \item for each $ f \in \setF $, we replace $ \vx_{\psetpff} $, $ \vx_{\setpf,f} $, and $ \vx_{\upsetpf,f} $ with $ \LCTv{x}_{\psetpff} $, $ \LCTv{x}_{\setpf,f} $, and $ \LCTv{x}_{\upsetpf,f} $, respectively;

            \item in terms of other variables, e.g., $ \vx_{\pe,m} $, $ x_{e,m} $, $  $, and $ x_{\upe,m} $ for each $ \pe = (e,\upe) \in \psetEfull $ and $ \vx_{\psetpff,m} $, $ \vx_{\setpf,f,m} $, and $ \vx_{\upsetpf,f,m} $ for $ f \in \setF $ with $ m \in \sZpp $, we the apply similar change as above,

        \end{itemize}
        %---------------------------------------------------------------------------

        \item for each $ f \in \setF $, the variables $ \LCTv{x}_{\setpff,m} $ and $ \LCTv{x}_{\upsetpff,m} $ defined in~\eqref{sec:CheckCon:eqn:27} have the same alphabet $\LCTsetxf = \prod_{e \in \setpf} \LCTsetxe =  \prod_{\upe \in \upsetpf} \LCTset{X}_{\upe} = \LCTset{X}_{\upsetpf} $ with $ \LCTsetxe = \LCTset{X}_{\upe} $ for all $ \pe = (e,\upe) \in \psetEfull $ as stated in item~\ref{def:DENFG:LCT:1:item:1} in Definition~\ref{def:DENFG:LCT:1};  

        \item for each $ \pe = (e,\upe) \in \psetEfull $, both $ \cvpsi_{e} $ and $ \cvpsi_{\upe} $ are vectors in $ \sC^{|\LCTsetxe|} $ with $ \|\cvpsi_{e}\| = \|\cvpsi_{\upe}\| =1 $;

        \item for each $ \pe= (e,\upe) \in \psetEfull $, both the measure $ \dd{\muFSsimple(\cvpsi_{e})} $ and the measure $ \dd{\muFSsimple(\cvpsi_{\upe})} $ are independent Fubini-Study measures, \textit{i.e.}, Haar measures over $ \sC^{|\LCTsetxe|} $, which are defined following the similar idea in~\eqref{sec:SST:eqn:30}, 

    \end{enumerate}
    %---------------------------------------------------------------------------
    and where step $(e)$ again follows from the fact that for each $ e \in \setEfull $, the measure $ \dd{\muFSsimple(\cvpsi_{e})} $ is a Fubini-Study measure, \textit{i.e.}, a Haar measure over $ \sC^{|\LCTsetxe|} $. 
    % and where step $(f)$ follows from Assumption~\ref{sec:DENFG:asum:2}, Property 8 in Proposition~\ref{prop:DENFG:LCT:1} and the fact that $ \LCT{\lambda}_{f}(\ellf) \in \sR_{\geq 0} $ for all $ \ellf \in \set{L}_{f} $ and $ f \in \setF $ as defined in~\eqref{sec:LCT:eqn:2}--\eqref{sec:LCT:eqn:3}. }
    Then we have
    %-------------------------------------------------------------------
    \begin{align}
        \int 
        \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
        \dd{\muFSsimple(\cvpsiavgalt)} 
        &\overset{(a)}{\geq}
        \Bigl(\prod_{m=1}^{M} 
        \prod_f \LCT{\lambda}_{f}(0) \Bigr) 
        \cdot
        \Biggl| \int 
        \prod_{m=1}^{M} 
        \prod_f
        \Biggl( 
            \sum_{\LCTv{x}_{\setpf,m}}
            \LCT{u}_{f}(\LCTv{x}_{\setpff,m},0) 
            \prod_{e \in \setpf} 
            \cpsi_{e,f}(\LCT{x}_{e,f,m}) 
        \Biggr)
        \dd{\muFSsimple(\cvpsiavgalt)}
        \Biggr|^{2} \nonumber\\
        &\overset{(b)}{=} 
        \Bigl(
            \prod_f \LCT{\lambda}_{f}(0) 
        \Bigr)^{M}
        \cdot
        \Biggl| \int 
        \prod_{m=1}^{M} 
        \prod_f
        \prod_{e \in \setpf} 
        \cpsi_{e,f}(0) 
        \dd{\muFSsimple(\cvpsiavgalt)}
        \Biggr|^{2} \nonumber\\
        &\overset{(c)}{=} 
        \Bigl(
            \prod_f \LCT{\lambda}_{f}(0) 
        \Bigr)^{M}
        \prod_{e = (f_{i},f_{j}) \in \setEfull}
        \Biggl( 
            \int 
            \prod_{m=1}^{M} 
            \Bigl( 
                \cpsi_{e,f_{i}}(0) \cdot \cpsi_{e,f_{j}}(0) 
            \Bigr)
            \dd{\muFSsimple(\cvpsiavgalt)}
        \Biggr)^{2}
        \nonumber\\
        &\overset{(d)}{=}
        \Bigl(
            \prod_f \LCT{\lambda}_{f}(0) 
        \Bigr)^{M}
        \prod_{e = (f_{i},f_{j}) \in \setEfull}
        \Biggl( 
            \int 
            |\cpsi_{e,f_{i}}(0)|^{2M} 
            \dd{\muFSsimple(\cvpsiavgalt)}
        \Biggr)^{2}
        \nonumber\\
        &\overset{(e)}{=} \Bigl(
            \prod_f \LCT{\lambda}_{f}(0) 
        \Bigr)^{M}
        \cdot
        \prod_{e \in \setEfull}
        \frac{1}{|\set{B}_{\LCTset{X}_e^M}|^{2}} 
        \label{sec:CheckCon:eqn:15}
    \end{align}
    %-------------------------------------------------------------------
    where step $(a)$ follows from the expression of $ \int 
        \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
        \dd{\muFSsimple(\cvpsiavgalt)}  $ in~\eqref{sec:CheckCon:eqn:11} and the fact that $ \LCT{\lambda}_{f}(\LCTellf) \in \sR_{\geq 0} $ for all $ \LCTellf \in \LCTset{L}_{f} $ and $ f \in \setF $ as defined in~\eqref{sec:LCT:eqn:3},
    where step $(b)$ follows from the expression of $ \LCT{u}_{f}(\LCTvxf,0) $ in~\eqref{sec:CheckCon:eqn:22}, 
    where step $(c)$ follows from the fact that the entries in $ \{ \cpsi_{\efi}(0)  \}_{e=(f_{i}, f_{j}) \in \setEfull} $ are independent and the entries in $ \{ \cpsi_{\efj}(0)  \}_{e=(f_{i}, f_{j}) \in \setEfull} $ are independent,  as defined in item~\ref{sec:SST:def:7:item:1} in Definition~\ref{sec:SST:def:7},
    where step $(d)$ follows from the definition of $  \cpsi_{e,f_{i}}(0) $ and $ \cpsi_{e,f_{j}}(0)  $ in~\eqref{sec:SST:eqn:18} and~\eqref{sec:SST:eqn:22}, \textit{i.e.}, $ \cpsi_{e,f_{i}}(0) = \cpsi_{e}(0) = \overline{ \cpsi_{e,f_{j}}(0)  }  $ for $ e = (f_{i},f_{j}) $, $ i < j $,
    and where step $(e)$ follows from~\eqref{sec:SST:eqn:25} in the proof of Proposition~\ref{sec:SST:prop:2}.
    
    \item Combining the results obtained above, we have
    %-------------------------------------------------------------------
    \begin{align*}
        \Bigl(
            \prod_f \LCT{\lambda}_{f}(0) 
        \Bigr)^{M}
        \cdot
        \prod_{e \in \setEfull}
        \frac{1}{|\set{B}_{\set{X}_e^M}|^{2}} 
        \overset{(a)}{\leq}
        \int 
        \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
        \dd{\muFSsimple(\cvpsiavgalt)} 
        \overset{(b)}{\leq}
        \int 
        \prod_f \left( 
            \LCT{\lambda}_{f}(0) 
        \right)^{M}
        \dd{\muFSsimple(\cvpsiavgalt)}
        \overset{(c)}{=}
        \prod_f \left( 
            \LCT{\lambda}_{f}(0) 
        \right)^{M}.
    \end{align*}
    %-------------------------------------------------------------------
    where step $(a)$ follows from~\eqref{sec:CheckCon:eqn:15},
    where step $(b)$ follows from~\eqref{sec:CheckCon:eqn:14},
    where step $(c)$ follows from the fact that $ \dd{\muFSsimple(\cvpsiavgalt)} $ is a Fubini-Study measure, i.e, a Haar measure, satisfying
    %-----------------------------------------------------------------------
    \begin{align*}
        \int 
        \prod_f \left( 
            \LCT{\lambda}_{f}(0) 
        \right)^{M}
        \dd{\muFSsimple(\cvpsiavgalt)}
        =  \prod_f \Biggl( \left( 
            \LCT{\lambda}_{f}(0) 
        \right)^{M} \int 
        \dd{\muFSsimple(\cvpsiavgalt)}
        \Biggr) 
        \overset{(d)}{=} \prod_f \left( 
            \LCT{\lambda}_{f}(0) 
        \right)^{M}.
    \end{align*}
    %-----------------------------------------------------------------------
    where step $(d)$ follows from
    %-----------------------------------------------------------------------
    \begin{align*}
        \dd{\muFSsimple(\cvpsiavgalt)}
        &=\prod_{e \in \setEfull}
        \dd{\muFSsimple(\cvpsi_{e})}
        \cdot 
        \prod_{\upe \in \upsetEfull}
        \dd{\muFSsimple(\cvpsi_{\upe})}, \qquad 
        \int \dd{\muFSsimple(\cvpsi_{e})} = 
        \int \dd{\muFSsimple(\cvpsi_{\upe})} =1, \qquad 
        \pe = (e,\upe) \in \setEfull, \nonumber\\
        \int \dd{\muFSsimple(\cvpsiavgalt)}
        &= \Biggl( \prod_{e \in \setEfull} \int \dd{\muFSsimple(\cvpsi_{e})} \Biggr)
        \cdot \Biggl(\prod_{\upe \in \upsetEfull} \int \dd{\muFSsimple(\cvpsi_{\upe})} \Biggr)
        =1.
    \end{align*}
    %-----------------------------------------------------------------------
    Then we have
    %-------------------------------------------------------------------
    \begin{align*}
        \limsup_{M \to \infty}
        \left( \int 
        \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
        \dd{\muFSsimple(\cvpsiavgalt)} 
        \right)^{1/M}
        \geq \limsup_{M \to \infty} 
        \Biggl(
            \Bigl(
                \prod_f \LCT{\lambda}_{f}(0) 
            \Bigr)
            \cdot
            \prod_{e \in \setEfull}
            \frac{1}{|\set{B}_{\LCTset{X}_e^M}|^{2/M}} 
        \Biggr)
        \overset{(a)}{=}  
        \prod_f \LCT{\lambda}_{f}(0),
    \end{align*}
    %-------------------------------------------------------------------
    where step $(a)$ follows from Lemma~\ref{sec:SST:lem:3}. Moreover, we have
    %-------------------------------------------------------------------
    \begin{align*}
        \limsup_{M \to \infty}
        \Biggl( \int 
        \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
        \dd{\muFSsimple(\cvpsiavgalt)} 
        \Biggr)^{1/M}
        \leq 
        \prod_f 
        \LCT{\lambda}_{f}(0).
    \end{align*}
    %-------------------------------------------------------------------
    Combining the above two inequalities, we obtain
    %-------------------------------------------------------------------
    \begin{align*}
        \limsup_{M \to \infty}
        \Biggl( \int 
        \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
        \dd{\muFSsimple(\cvpsiavgalt)} 
        \Biggr)^{1/M}
        = \prod_f 
        \LCT{\lambda}_{f}(0).
    \end{align*}
    %-------------------------------------------------------------------
\end{enumerate}
%---------------------------------------------------------------------------
Combining with the expression of $ \ZBSPA(\graphN) $ in~\eqref{sec:CheckCon:eqn:18}, we have
%-----------------------------------------------------------------------
\begin{align}
    \lim_{M \to \infty}
    \Biggl( \int 
    \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
    \dd{\muFSsimple(\cvpsiavgalt)} 
    \Biggr)^{1/M}
    =  \ZBSPA(\graphN). \label{sec:CheckCon:eqn:20}
\end{align}
%-----------------------------------------------------------------------
Then we have
%-----------------------------------------------------------------------
\begin{align*}
    \lim_{M \to \infty}
    \ZBM(\LCT{\graphN}) 
    &\overset{(a)}{=}
    \lim_{M \to \infty}
    \left(
        \prod_{e \in \setEfull}
            |\set{B}_{\LCTset{X}_{e}^M}|
    \right)^{2/M}
    \cdot
    \Biggl(
        \int 
         \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
        \dd{\muFSsimple(\cvpsiavgalt)}
    \Biggr)^{1/M} \nonumber\\
    &\overset{(b)}{=}
    \lim_{M \to \infty}
    \left(
        \prod_{e \in \setEfull}
            |\set{B}_{\LCTset{X}_{e}^M}|
    \right)^{2/M}
    \cdot 
    \lim_{M \to \infty}
    \Biggl(
        \int 
         \ZSSTM(\LCTavgalt{\graphN},\cvpsiavgalt)
        \dd{\muFSsimple(\cvpsiavgalt)}
    \Biggr)^{1/M} \nonumber\\
    &\overset{(c)}{=} \ZBSPA(\graphN),
\end{align*}
%-----------------------------------------------------------------------
where step $(a)$ follows from~\eqref{sec:CheckCon:eqn:19},
and where steps $(b)$ and $ (c) $ follow from Lemma~\ref{sec:SST:lem:3} and the expression in~\eqref{sec:CheckCon:eqn:20}.

==> appendices/convergence_tensor_norm.tex <==
Similar to the proof of Lemma~\ref{sec:algsin:lem:8}, we know that the sequence $ \left\{ \log( \Zabsf\left( \Bigl( \vgam_{\psetpf}^{(k)} \Bigr)^{1/\qf} \right) ) \right\}_{k \in \sZpp} $ converges. 
For fixed $ e' \in \setpf $, we consider a vector $ \vgam_{\psetpf,*}^{(k)} $ to be
%----------------------------------------------------------------------------
\begin{align*}
    \gamma_{e,*}^{(k)}(\xe) \defeq
    \begin{cases}
        \gamma_{e}^{(k)}(\xe) + \gamma_{e}^{*}(\xe) & e = e' \\
        \gamma_{e}^{(k)}(\xe) & \text{Otherwise}
    \end{cases}
\end{align*}
%----------------------------------------------------------------------------
Then we have
%----------------------------------------------------------------------------
\begin{align*}
    \left( 
        \left. 
            \nabla_{ \vgam_{\psetpf} } 
            \log( \Zabsfn\Bigl( (\vgam_{\psetpf} )^{1/\qf} \Bigr) )
        \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf,*}^{(k)}  }
    \right)^{\tran}
    \cdot 
    \left( \vgam_{\psetpf}^{(k)} - \vgam_{\psetpf,*}^{(k)} \right)
    = -\sum_{\xep}
    \left. \pdv{}{ \gamma_{e'}(\xep) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
    \cdot \gamma_{e}^{*}(\xe)
    \cdot ( \frac{ \gamma_{e}^{(k)}(\xe) }{ 
     \gamma_{e}^{(k)}(\xe) +  \gamma_{e}^{*}(\xe) } 
\end{align*}
%----------------------------------------------------------------------------
By Proposition~\ref{sec:algsin:prop:5}, we know that the function $ \log( \Zabsfn\Bigl( (\vgam_{\psetpf} )^{1/\qf} \Bigr) ) $ is concave w.r.t. $ \vgam_{\psetpf} $. Thus the following inequality holds
%------------------------------------------------------------------------
\begin{align}
    &\log( \Zabsfn\Bigl( (\vgam_{\psetpf}^{*} )^{1/\qf} \Bigr) )
    \nonumber\\
    &\leq \log( \Zabsfn\Bigl( (\vgam_{\psetpf}^{(k)} )^{1/\qf} \Bigr) )
    + \left( 
        \left. 
            \nabla_{ \vgam_{\psetpf} } 
            \log( \Zabsfn\Bigl( (\vgam_{\psetpf} )^{1/\qf} \Bigr) )
        \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  }
    \right)^{\tran}
    \cdot 
    \left( \vgam_{\psetpf}^{*} - \vgam_{\psetpf}^{(k)} \right) 
    \nonumber\\
    &= \log( \Zabsfn\Bigl( (\vgam_{\psetpf}^{(k)} )^{1/\qf} \Bigr) )
    +
    \sum_{e \in \setpf}
    \sum_{\xe}
    \left. \pdv{}{ \gamma_{e}(\xe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
    \cdot \Bigl( 
        \gamma_{e}^{*}(\xe) - \gamma_{e}^{(k)}(\xe) 
    \Bigr)\nonumber\\
    & \quad
    +
    \sum_{\upe \in \upsetpf}
    \sum_{\xupe}
    \left. \pdv{}{ \gamma_{\upe}(\xupe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
    \cdot \Bigl( 
        \gamma_{\upe}^{*}(\xupe) - \gamma_{\upe}^{(k)}(\xupe) 
    \Bigr)
    , 
    \qquad
    k \in \sZpp, \label{sec:algsin:eqn:104}
\end{align}
%------------------------------------------------------------------------
where the elements in the gradient $ \nabla_{ \vgam_{\psetpf} } 
    \log( \Zabsfn\Bigl( (\vgam_{\psetpf} )^{1/\qf} \Bigr) ) $ are given by
%------------------------------------------------------------------------
\begin{align}
    \left. \pdv{}{ \gamma_{e}(\xe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  }
    &= \frac{1}{\qe}
    \cdot \Biggl( 
    \frac{ 1
    }{ \bigl( \gamma_{e}^{(k)}(\xe) \bigr)^{(q-1)/q} }
    \cdot 
    \frac{ \gamet^{(k+1)}(\xe) }{ \sum_{\xe} 
        ( \gamma_{e}^{(k)}(\xe) )^{1/q} 
        \cdot \gamet^{(k+1)}(\xe) 
    }
    - 1 \Biggr), \label{sec:algsin:eqn:108}\\
    \left. \pdv{}{ \gamma_{\upe}(\xupe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  }
    &= \frac{1}{\qupe}
    \cdot \Biggl( 
    \frac{ 1
    }{ \bigl( \gamma_{\upe}^{(k)}(\xupe) \bigr)^{(q-1)/q} }
    \cdot 
    \frac{ \gamupet^{(k+1)}(\xupe) 
    }{ \sum_{\xe} 
        ( \gamma_{\upe}^{(k)}(\xupe) )^{1/q} 
        \cdot \gamupet^{(k+1)}(\xupe) 
    }
    - 1 \Biggr), \label{sec:algsin:eqn:124}
\end{align}
%------------------------------------------------------------------------
and $ \gamet^{(k+1)} $ and $ \gamupet^{(k+1)} $ are defined in~\eqref{sec:algsin:eqn:90} and~\eqref{sec:algsin:eqn:121}, respectively.  By Remark~\ref{sec:algsin:remk:1} and the fact that $ \gamma_{e}^{(0)}(\xe), \gamma_{\upe}^{(0)}(\xupe) \in \sR_{>0} $ for all $ \xpe \in \setxpe $ and $ \pe \in \psetpf $, we have $ \gamma_{e}^{(k)}(\xe), \gamet^{(k+1)}(\xe), \gamma_{\upe}^{(k)}(\xupe), \gamupet^{(k+1)}(\xupe) \in \sR_{>0} $ for all $ k \in \sZpp $, $ \xpe \in \setxpe $, and $ \pe \in \setpf $. Thus the partial derivatives in~\eqref{sec:algsin:eqn:108} and~\eqref{sec:algsin:eqn:124} are well defined.
Then we have
%------------------------------------------------------------------------
\begin{align}
    &\lim_{k \to \infty} \left. \pdv{}{ \gamma_{e}(\xe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
    \cdot \gamma_{e}^{(k)}(\xe) 
    \nonumber\\
    &=\lim_{k \to \infty}
    \left( \gamma_{e}^{(k)}(\xe) \right)^{1/\qe} 
    \cdot
    \Biggl( 
    \frac{ \gamet^{(k+1)}(\xe) }{ \sum_{\xe} 
        \left( \gamma_{e}^{(k)}(\xe) \right)^{1/\qe} 
        \cdot \gamet^{(k+1)}(\xe) 
    }
    - \bigl( \gamma_{e}^{(k)}(\xe) \bigr)^{(\qe-1)/\qe} \Biggr)
    \nonumber\\
    &\overset{(a)}=  0, \qquad \xe \in \setxe, \, e \in \setpf,
    \label{sec:algsin:eqn:110}
\end{align}
%------------------------------------------------------------------------
where step $(a)$ follows from Lemma~\ref{sec:algsin:lem:4} with the substitution in~\eqref{sec:algsin:eqn:4} and the fact that $ \| \vgam_{e}^{(k)} \|_{q} = 1 $, i.e., $ \{ \gamma_{e}^{(k)}(\xe) \}_{k \in \sZpp} $ is a bounded sequence. Because the sequences $ \{\gamma_{e}^{(k)}(\xe)\}_{k \in \sZpp} $ and  $ \{\gamma_{\upe}^{(k)}(\xupe)\}_{k \in \sZpp} $ are bounded for all $ \xpe \in \setx_{\pe} $ and $ \pe = (e,\upe) \in \psetEfull $, we define the sets
%------------------------------------------------------------------------
\begin{align*}
    \set{S}_{e,1} & \defeq \left\{ \xe \in \setxe  
    \ \left| \ \liminf_{k \to \infty} \gamma_{e}^{(k)}(\xe) > 0 
    \right. \right\}, \qquad
    \set{S}_{e,1}^{\mathrm{c}} \defeq \setxe \setminus \set{S}_{e,1},
    \nonumber\\
    \set{S}_{\upe,1} & \defeq \left\{ \xupe \in \setx_{\upe}  
    \ \left| \ \liminf_{k \to \infty} \gamma_{\upe}^{(k)}(\xupe) > 0 
    \right. \right\}, \qquad 
    \set{S}_{\upe,1}^{\mathrm{c}} \defeq \setxe \setminus \set{S}_{\upe,1},
\end{align*}
%------------------------------------------------------------------------
which implies
%----------------------------------------------------------------------------
\begin{align}
    \liminf_{k \to \infty} \gamma_{e}^{(k)}(\xe)  = 0, \qquad 
    \xe \in \set{S}_{e,1}^{\mathrm{c}}, \qquad 
    \liminf_{k \to \infty} \gamma_{\upe}^{(k)}(\xupe) = 0, \qquad 
    \xupe \in \set{S}_{\upe,1}^{\mathrm{c}}. \label{sec:algsin:eqn:129}
\end{align}
%----------------------------------------------------------------------------
Similar to the derivation of~\eqref{sec:algsin:eqn:110}, we have
%----------------------------------------------------------------------------
\begin{align}
    &\lim_{k \to \infty} \left. \pdv{}{ \gamma_{e}(\xe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
    \nonumber\\
    &=
    \frac{1}{ \qe } \cdot
    \lim_{k \to \infty}
    \bigl( \gamma_{e}^{(k)}(\xe) \bigr)^{-(\qe-1)/\qe}
    \cdot \Biggl( 
    \frac{ \gamet^{(k+1)}(\xe) }{ \sum_{\xe} 
        \left( \gamma_{e}^{(k)}(\xe) \right)^{1/\qe} 
        \cdot \gamet^{(k+1)}(\xe) 
    }
    - \bigl( \gamma_{e}^{(k)}(\xe) \bigr)^{(\qe-1)/\qe} \Biggr)
    \nonumber\\
    &\overset{(a)}{=}   
    0,
    \qquad \xe \in \set{S}_{e,1}, \, e \in \setpf, \label{sec:algsin:eqn:128}
\end{align}
%----------------------------------------------------------------------------
where step $(a)$ follows from Lemma~\ref{sec:algsin:lem:4} with the substitution in~\eqref{sec:algsin:eqn:4} and the fact that because $ \liminf_{k \to \infty} \gamma_{e}^{(k)}(\xe) > 0 $ for $ \xe \in \set{S}_{e,1} $, there exists an $ \epsilon_{e,1} \in \sR_{>0} $ and an integer $ K \in \sZpp $ such that 
$ 0 < \bigl( \gamma_{e}^{(k)}(\xe) \bigr)^{-(\qe-1)/\qe} < \epsilon_{e,1} $ for all $ \xe \in \set{S}_{e,1} $ and $ k \geq K' $. For $ \upe \in \upsetpf $, we obtain the similar results:
%---------------------------------------------------------------------------
\begin{align}
    \lim_{k \to \infty} \left. \pdv{}{ \gamma_{\upe}(\xupe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
    \cdot \gamma_{\upe}^{(k)}(\xupe) 
    &=  0, \qquad \xupe \in \setxupe, \label{sec:algsin:eqn:137}
    \\
    \lim_{k \to \infty} \left. \pdv{}{ \gamma_{\upe}(\xupe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
    &=
    0,
    \qquad \xupe \in \set{S}_{\upe,1}. \label{sec:algsin:eqn:138}
\end{align}
%---------------------------------------------------------------------------
In the following derivations, we suppose that
%------------------------------------------------------------------------
\begin{align*}
    \limsup_{k_{1} \to \infty} 
    \left. \pdv{}{ \gamma_{e}(\xe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{1})}  } 
    \cdot \gamma_{e}^{*}(\xe) \in \sR \cup \{ - \infty, + \infty \}, \qquad 
    \xe \in \set{S}_{e,2}, \, e \in \setpf, \nonumber\\
    \limsup_{k_{1} \to \infty} 
    \left. \pdv{}{ \gamma_{\upe}(\xupe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{1})}  } 
    \cdot \gamma_{\upe}^{*}(\xupe) \in \sR \cup \{ - \infty, + \infty \}, \qquad 
    \xe \in \set{S}_{\upe,2}, \, \upe \in \upsetpf,
\end{align*}
%------------------------------------------------------------------------
where
%----------------------------------------------------------------------------
\begin{align}
    \set{S}_{e,2} & \defeq \left\{ 
        \xe \in \set{S}_{e,1}^{\mathrm{c}}
        \ \left| \ 
        \gamma_{e}^{*}(\xe) > 0
        % \limsup_{k_{1} \to \infty} 
        % \left. \pdv{}{ \gamma_{e}(\xe) }
        % \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
        % \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{1})}  } \neq 0
    \right. \right\}, \label{sec:algsin:eqn:113}\\
    \set{S}_{\upe,2} &\defeq \left\{ 
        \xupe \in \set{S}_{\upe,1}^{\mathrm{c}}
        \ \left| \ 
        \gamma_{\upe}^{*}(\xupe) > 0
        % \limsup_{k_{1} \to \infty} 
        % \left. \pdv{}{ \gamma_{\upe}(\xupe) }
        % \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
        % \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{1})}  } \neq 0
    \right. \right\}. \label{sec:algsin:eqn:136}
\end{align}
%----------------------------------------------------------------------------
Then the inequalities in~\eqref{sec:algsin:eqn:104} implies
%------------------------------------------------------------------------
\begin{align}
    &\log( \Zabsfn\Bigl( (\vgam_{\psetpf}^{*} )^{1/\qf} \Bigr) )
    \nonumber\\
    &\leq \liminf_{k \to \infty} 
    \Biggl( 
        \log( \Zabsfn\Bigl( (\vgam_{\psetpf}^{(k)} )^{1/\qf} \Bigr) )
        +
        \sum_{e \in \setpf}
        \sum_{\xe}
        \left. \pdv{}{ \gamma_{e}(\xe) }
        \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
        \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
        \cdot \Bigl( 
            \gamma_{e}^{*}(\xe) - \gamma_{e}^{(k)}(\xe) 
        \Bigr)
        \nonumber\\
        &\qquad\qquad+
        \sum_{\upe \in \upsetpf}
        \sum_{\xupe}
        \left. \pdv{}{ \gamma_{\upe}(\xupe) }
        \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
        \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
        \cdot \Bigl( 
            \gamma_{\upe}^{*}(\xupe) - \gamma_{\upe}^{(k)}(\xupe) 
        \Bigr)
    \Biggr)
    \nonumber\\
    &\overset{(a)}{=}
    \lim_{k \to \infty} 
    \log( \Zabsfn\Bigl( (\vgam_{\psetpf}^{(k)} )^{1/\qf} \Bigr) )
    + \liminf_{k \to \infty} 
    \Biggl( 
    \sum_{e \in \setpf}
    \sum_{\xe}
    \left. \pdv{}{ \gamma_{e}(\xe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
    \cdot \Bigl( 
        \gamma_{e}^{*}(\xe) - \gamma_{e}^{(k)}(\xe) 
    \Bigr)
    \nonumber\\
    &\quad
    + \sum_{\upe \in \upsetpf}
    \sum_{\xupe}
    \left. \pdv{}{ \gamma_{\upe}(\xupe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
    \cdot \Bigl( 
        \gamma_{\upe}^{*}(\xupe) - \gamma_{\upe}^{(k)}(\xupe) 
    \Bigr)
    \Biggr) 
    \nonumber\\
    &\overset{(b)}{\leq}
    \lim_{k \to \infty} 
    \log( \Zabsfn\Bigl( (\vgam_{\psetpf}^{(k)} )^{1/\qf} \Bigr) )
    + \liminf_{k \to \infty} 
    \Biggl(
        \sum_{e \in \setpf}
        \sum_{\xe \in \set{S}_{e,2}}
        \left. \pdv{}{ \gamma_{e}(\xe) }
        \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
        \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
        \cdot  \gamma_{e}^{*}(\xe)
        \nonumber\\
        & \quad 
        + \sum_{\upe \in \upsetpf}
        \sum_{\xupe \in \set{S}_{\upe,2}}
        \left. \pdv{}{ \gamma_{\upe}(\xupe) }
        \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
        \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
        \cdot  \gamma_{\upe}^{*}(\xupe)
    \Biggr) ,\label{sec:algsin:eqn:116}
\end{align}
%------------------------------------------------------------------------
where step $(a)$ follows from Lemma~\ref{sec:algsin:lem:8} with the substitution in~\eqref{sec:algsin:eqn:4},
and where step $(b)$ follows from the limits in~\eqref{sec:algsin:eqn:110},~\eqref{sec:algsin:eqn:128}--\eqref{sec:algsin:eqn:138}  and the definitions of $ \set{S}_{e,2} $ and $ \set{S}_{\upe,2} $ in~\eqref{sec:algsin:eqn:113} and~\eqref{sec:algsin:eqn:136}, respectively. By the definition of $ \vgam_{\psetpf}^{*} $ in Definition~\ref{sec:algsin:def:2} and the fact that $ \sum_{\xe} \gamma_{e}^{(k)}(\xe) =  \sum_{\xupe} \gamma_{\upe}^{(k)}(\xupe) = 1 $ for all $ \pe \in \psetpf $ and $ k \in \sZpp $ as defined in~\eqref{sec:algsin:eqn:89}, we have
%------------------------------------------------------------------------
\begin{align}
    \lim_{k \to \infty} 
    \log( \Zabsfn\Bigl( (\vgam_{\psetpf}^{(k)} )^{1/\qf} \Bigr) )
    \leq \log( \Zabsfn\Bigl( (\vgam_{\psetpf}^{*} )^{1/\qf} \Bigr) ),
    \label{sec:algsin:eqn:115}
\end{align}
%------------------------------------------------------------------------
which implies
%----------------------------------------------------------------------------
\begin{align}
    &
    \liminf_{k\to \infty} 
    \Biggl( 
    \sum_{e \in \setpf}
    \sum_{\xe \in \set{S}_{e,2}}
    \left. \pdv{}{ \gamma_{e}(\xe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
    \cdot  \gamma_{e}^{*}(\xe)
    \nonumber\\
    &+ \sum_{\upe \in \upsetpf}
    \sum_{\xupe \in \set{S}_{\upe,2}}
    \left. \pdv{}{ \gamma_{\upe}(\xupe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
    \cdot  \gamma_{\upe}^{*}(\xupe)
    \Biggr)
    \geq 0. \label{sec:algsin:eqn:127}
\end{align}
%----------------------------------------------------------------------------
Now we want to show that the limit inferior on the left-hand side of the inequality in~\eqref{sec:algsin:eqn:127} equals zero.
Because of the limits in~\eqref{sec:algsin:eqn:129} and the fact that $ \gamma_{e}^{(k)}(\xe) $ is positive and bounded for all $ \xe \in \setxe $, $ e \in \setpf $, and $ k \in \sZpp $, by the Bolzano–Weierstrass theorem~\cite[Theorem 3.4.8]{Bartle2010}, there exists a subsequence of $ \{ k \}_{k \in \sZpp} $, which is indexed by $ k_{1} \in \sZpp $, such that 
%----------------------------------------------------------------------------
\begin{align*}
    \lim_{k_{1} \to  \infty} \gamma_{e}^{(k_{1})}(\xe) 
    \in \sR_{\geq 0}, \quad 
    \lim_{k_{1} \to  \infty} \gamma_{\upe}^{(k_{1})}(\xupe) 
    \in \sR_{\geq 0}, \qquad 
    \pe = (\xe, \xupe) \in \set{S}_{e',1}^{\mathrm{c}} 
    \times \set{S}_{\upe,1}^{\mathrm{c}},\, 
    \pe = (e,\upe) \in \psetpf.
\end{align*}
%----------------------------------------------------------------------------
We define
%------------------------------------------------------------------------
\begin{align*}
    \set{S}_{e,3} & \defeq \left\{ 
        \xe \in \set{S}_{e,2}
        \ \left| \ 
        \lim_{k_{1} \to  \infty} \gamma_{e}^{(k_{1})}(\xe)
        = 0
    \right. \right\}, \\
    \set{S}_{\upe,3} &\defeq \left\{ 
        \xupe \in \set{S}_{\upe,2}
        \ \left| \ 
        \lim_{k_{1} \to  \infty} \gamma_{\upe}^{(k_{1})}(\xupe)
        = 0
        % \limsup_{k_{1} \to \infty} 
        % \left. \pdv{}{ \gamma_{\upe}(\xupe) }
        % \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
        % \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{1})}  } \neq 0
    \right. \right\}. 
\end{align*}
%------------------------------------------------------------------------
Because both $ \gamma_{e}^{(k_{1})}(\xe) $ and $ \gamma_{\upe}^{(k_{1})}(\xupe) $ are positive-valued for all $ \xe \in \set{S}_{e,2} $ and $ \xupe \in \set{S}_{\upe,2} $ and $ k_{1} \in \sZpp $, 
then there exists a subsequence of $ \{ k_{1} \}_{k_{1} \in \sZpp} $, which is indexed by $ k_{2} \in \sZpp $ such that
%----------------------------------------------------------------------------
\begin{align}
    \frac{ \gamma_{e}^{(k_{2}+1)}(\xe) }{ \gamma_{e}^{(k_{2})}(\xe) }
    <1, \qquad 
    \frac{ \gamma_{\upe}^{(k_{2}+1)}(\xupe) }{ \gamma_{\upe}^{(k_{2})}(\xupe) }
    < 1, \qquad \xpe = (\xe,\xupe) \in \set{S}_{e,3} \times \set{S}_{\upe,3}.
    \label{sec:algsin:eqn:135}
\end{align}
%----------------------------------------------------------------------------
Similar to the proof of~\eqref{sec:algsin:eqn:128}, we have
%----------------------------------------------------------------------------
\begin{align}
    &\liminf_{k_{2}\to \infty} 
    \Biggl( 
    \sum_{e \in \setpf}
    \sum_{\xe \in \set{S}_{e,2}}
    \left. \pdv{}{ \gamma_{e}(\xe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{2})}  } 
    \!\!\!\!\!
    \cdot  \gamma_{e}^{*}(\xe)
    + \sum_{\upe \in \upsetpf}
    \sum_{\xupe \in \set{S}_{\upe,2}}
    \left. \pdv{}{ \gamma_{\upe}(\xupe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{2})}  } 
    \!\!\!\!\!
    \cdot  \gamma_{\upe}^{*}(\xupe)
    \Biggr)
    \nonumber\\
    &= \liminf_{k_{2}\to \infty} 
    \Biggl( 
    \sum_{e \in \setpf}
    \sum_{\xe \in \set{S}_{e,3}}
    \left. \pdv{}{ \gamma_{e}(\xe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{2})}  } 
    \!\!\!\!\!
    \cdot  \gamma_{e}^{*}(\xe)
    + \sum_{\upe \in \upsetpf}
    \sum_{\xupe \in \set{S}_{\upe,3}}
    \left. \pdv{}{ \gamma_{\upe}(\xupe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{2})}  } 
    \!\!\!\!\!
    \cdot  \gamma_{\upe}^{*}(\xupe)
    \Biggr) 
    \label{sec:algsin:eqn:141}\\
    &\geq 0. \label{sec:algsin:eqn:140}
\end{align}
%----------------------------------------------------------------------------
We want to prove that the inequality in~\eqref{sec:algsin:eqn:140} is indeed an equality. We prove it by contradiction.
Suppose that the expression on the left-hand side of the inequality~\eqref{sec:algsin:eqn:140} is positive.
Because both $ \gamma_{e}^{*}(\xe) $ and $ \gamma_{\upe}^{*}(\xupe) $ are positive-valued for all $ \xe \in \set{S}_{e,2} $ and $ \xupe \in \set{S}_{\upe,2} $, the strict inequality in~\eqref{sec:algsin:eqn:140} implies
%------------------------------------------------------------------------
\begin{align}
    &\exists \xe' \in \set{S}_{e,3},\, \mathrm{s.t.}\ 
    \limsup_{k_{2} \to \infty} 
    \left. \pdv{}{ \gamma_{e}(\xe') }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{2})}  } 
    > 0, 
    \label{sec:algsin:eqn:123}\\
    &\text{ or } \exists \xupe' \in \set{S}_{\upe,3},\,  \mathrm{s.t.}\
     \limsup_{k_{2} \to \infty} 
    \left. \pdv{}{ \gamma_{\upe}(\xupe') }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{2})}  } > 0. 
    \label{sec:algsin:eqn:132}
\end{align}
%------------------------------------------------------------------------
%----------------------------------------------------------------------------
\begin{enumerate}
    \item We first consider~\eqref{sec:algsin:eqn:123}, which, by the expression of the partial derivatives in~\eqref{sec:algsin:eqn:108}, implies 
    %------------------------------------------------------------------------
    \begin{align*}
        &\limsup_{k_{2} \to \infty} 
        \bigl( \gamma_{e}^{(k_{2})}(\xe') \bigr)^{-(\qe-1)/\qe}
        \cdot 
        \frac{ \gamet^{(k_{2}+1)}(\xe') }{ \sum_{\xe} 
            ( \gamma_{e}^{(k_{2})}(\xe') )^{1/\qe} 
            \cdot \gamet^{(k_{2}+1)}(\xe') 
        }
        \nonumber\\
        &= \limsup_{k_{2} \to \infty} 
        \frac{ \gamet^{(k_{2}+1)}(\xe') }{ \| \gamet^{(k_{2}+1)}(\xe') \|_{ \qe/(\qe-1) } 
        \cdot 
        \bigl( \gamma_{e}^{(k_{2})}(\xe') \bigr)^{(\qe-1)/\qe} } 
        \cdot 
        \frac{ \| \gamet^{(k_{2}+1)}(\xe') \|_{ \qe/(\qe-1) }  
        }{ \sum_{\xe} 
            ( \gamma_{e}^{(k_{2})}(\xe') )^{1/\qe} 
            \cdot \gamet^{(k_{2}+1)}(\xe') 
        } 
        \nonumber\\
        &\overset{(a)}{=} \limsup_{k_{2} \to \infty} 
        \frac{ \left( \gamma_{e}^{(k_{2}+1)}(\xe') \right)^{(\qe-1)/\qe} 
        }{ \bigl( \gamma_{e}^{(k_{2})}(\xe') \bigr)^{(\qe-1)/\qe} }
        \cdot
        \frac{ 
                \Zabsfn\Bigl( (\vgam_{\psetpf}^{(k_{2}+1)} )^{1/\qe} \Bigr)
        }{  
            \Zabsfn\Bigl( (\vgam_{\psetpf}^{(k_{2})} )^{1/\qe} \Bigr)
        }\nonumber\\
        &\overset{(b)}{=} \limsup_{k_{2} \to \infty} 
        \frac{ \left( \gamma_{e}^{(k_{2}+1)}(\xe') \right)^{(\qe-1)/\qe} 
        }{ \bigl( \gamma_{e}^{(k_{2})}(\xe') \bigr)^{(\qe-1)/\qe} }
        \nonumber\\
        &> 1, \qquad \xe' \in \set{S}_{e,2},
    \end{align*}
    %------------------------------------------------------------------------
    where step $(a)$ follows from the expression of $ \gamma_{e}^{(k_{2}+1)}(\xe) $ in~\eqref{sec:algsin:eqn:89} and the equalities in~\eqref{sec:algsin:eqn:71}--\eqref{sec:algsin:eqn:92} with the substitution in~\eqref{sec:algsin:eqn:4}, 
    and where step $(b)$ follows from Lemma~\ref{sec:algsin:lem:8}, i.e., $ \lim_{k \to \infty} 
        \Zfnorm\Bigl( \vpsi_{\psetpf}^{(k)} \Bigr) $ exists and the fact that $ \Bigl\{ \Zfnorm\Bigl( \vpsi_{\psetpf}^{(k)} \Bigr) \Bigr\}_{ k \in \sZpp } $ is a monotonic sequence.
    For any $ \epsilon_{e} \in \sR_{>0} $ satisfying 
    %------------------------------------------------------------------------
    \begin{align*}
        \limsup_{k_{2} \to \infty} 
        \frac{ \left( \gamma_{e}^{(k_{2}+1)}(\xe') \right)^{(\qe-1)/\qe} 
        }{ \bigl( \gamma_{e}^{(k_{2})}(\xe') \bigr)^{(\qe-1)/\qe} } 
        > 1 +\epsilon_{e},
    \end{align*}
    %------------------------------------------------------------------------
    there exists a subsequence $ \{\gamma_{e}^{(k_{2})}(\xe')\}_{k_{2} \in \sZpp} $ of $ \{\gamma_{e}^{(k_{2})}(\xe')\}_{k_{2} \in \sZpp} $ such that
    %------------------------------------------------------------------------
    \begin{align*}
        \frac{ \left( \gamma_{e}^{(k_{2}+1)}(\xe') \right)^{(\qe-1)/\qe} 
        }{ \bigl( \gamma_{e}^{(k_{2})}(\xe') \bigr)^{(\qe-1)/\qe} } 
        > 1 +\epsilon_{e}, \qquad k_{2} \in \sZpp
    \end{align*}
    %------------------------------------------------------------------------
    which contradicts to~\eqref{sec:algsin:eqn:135}. Thus we have
    %------------------------------------------------------------------------
    \begin{align}
        &\limsup_{k_{2} \to \infty} 
        \left. \pdv{}{ \gamma_{e}(\xe') }
        \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
        \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{2})}  } 
        \cdot  \gamma_{e}^{*}(\xe') = 0. \label{sec:algsin:eqn:133}
    \end{align}
    %------------------------------------------------------------------------

    \item Similarly, by considering~\eqref{sec:algsin:eqn:132}, we also obtain contradictive statements, which proves
    %------------------------------------------------------------------------
    \begin{align}
        &\limsup_{k_{2} \to \infty} 
        \left. \pdv{}{ \gamma_{\upe}(\xupe') }
        \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
        \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{2})}  } 
        \cdot  \gamma_{\upe}^{*}(\xupe') = 0.
        \label{sec:algsin:eqn:134}
    \end{align}
    %------------------------------------------------------------------------
\end{enumerate}
%----------------------------------------------------------------------------
Combining the limit superior in~\eqref{sec:algsin:eqn:133} and~\eqref{sec:algsin:eqn:134} with the
inequalities~\eqref{sec:algsin:eqn:115} and~\eqref{sec:algsin:eqn:116}, we have
%------------------------------------------------------------------------
\begin{align}
    &\lim_{k_{2} \to \infty} 
    \left. \pdv{}{ \gamma_{e}(\xe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{2})}  } 
    \cdot  \gamma_{e}^{*}(\xe) 
    =
    \lim_{k_{2} \to \infty} 
    \left. \pdv{}{ \gamma_{\upe}(\xupe) }
    \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
    \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k_{2})}  } 
    \cdot  \gamma_{\upe}^{*}(\xupe)
    = 0, \nonumber \\
    &\qquad \xpe = (\xe, \xupe) \in \set{S}_{e,3} \times 
    \set{S}_{\upe,3}, \, \pe \in \psetpf,
\end{align}
%------------------------------------------------------------------------
which by the equality in~\eqref{sec:algsin:eqn:141} implies the limit inferior on the left-hand side of the inequality in~\eqref{sec:algsin:eqn:127} equals zero and
%------------------------------------------------------------------------
\begin{align}
    &\log( \Zabsfn\Bigl( (\vgam_{\psetpf}^{*} )^{1/\qf} \Bigr) )
    =
    \lim_{k \to \infty} 
    \log( \Zabsfn\Bigl( (\vgam_{\psetpf}^{(k)} )^{1/\qf} \Bigr) ),
    \label{sec:algsin:eqn:118}\\
    &\log( \sig_{q}(|f|) )
    \overset{(a)}{=}
    \log( \Zabsfn\Bigl( (\vgam_{\psetpf}^{*} )^{1/\qf} \Bigr) )
    \overset{(b)}{=}
    \lim_{k \to \infty} 
    \log( \Zabsfn\Bigl( (\vgam_{\psetpf}^{(k)} )^{1/\qf} \Bigr) ),
    \nonumber
\end{align}
%------------------------------------------------------------------------
where step $(a)$ follows from Proposition~\ref{sec:algsin:prop:6}, 
and where step $(b)$ follows from~\eqref{sec:algsin:eqn:118}.


%  Because the sequences $ \{\gamma_{e}^{(k)}(\xe)\}_{k \in \sZpp} $ and  $ \{\gamma_{\upe}^{(k)}(\xupe)\}_{k \in \sZpp} $ are bounded for all $ \xpe \in \setx_{\pe} $ and $ \pe = (e,\upe) \in \psetEfull $, by the Bolzano–Weierstrass theorem~\cite[Theorem 3.4.8]{Bartle2010}, there exist convergent subsequences $ \{\gamma_{e}^{(k)}(\xe)\}_{k \in \sZpp} $ and  $ \{\gamma_{\upe}^{(k)}(\xupe)\}_{k \in \sZpp} $ indexed by $ k $. 
 
%  Then we have     
%  %------------------------------------------------------------------------
% \begin{align}
%     &\lim_{k \to \infty} \left. \pdv{}{ \gamma_{e}(\xe) }
%     \log( \Zabsfn( (\vgam_{\psetpf} )^{1/\qf} ) )
%     \right|_{ \vgam_{\psetpf} = \vgam_{\psetpf}^{(k)}  } 
%     \nonumber\\
%     &\overset{(a)}{=} 
%     \frac{2}{ \qe } \cdot
%     \lim_{k \to \infty}
%     \bigl( \gamma_{e}^{(k)}(\xe) \bigr)^{-(\qe-1)/\qe}
%     \cdot \Biggl( 
%     \frac{ \gamet^{(k+1)}(\xe) }{ \sum_{\xe} 
%         \left( \gamma_{e}^{(k)}(\xe) \right)^{1/\qe} 
%         \cdot \gamet^{(k+1)}(\xe) 
%     }
%     - \bigl( \gamma_{e}^{(k)}(\xe) \bigr)^{(\qe-1)/\qe} \Biggr)
%     \nonumber\\
%     &\overset{(b)}{=}
%     \frac{2}{\qe} \cdot
%     \left(
%         \lim_{k \to \infty}
%         \bigl( \gamma_{e}^{(k)}(\xe) \bigr)^{-(\qe-1)/\qe}
%     \right)
%     \cdot 
%     \lim_{k \to \infty}
%     \Biggl( 
%     \frac{ \gamet^{(k+1)}(\xe) }{ \sum_{\xe} 
%         \left( \gamma_{e}^{(k)}(\xe) \right)^{1/\qe} 
%         \cdot \gamet^{(k+1)}(\xe) 
%     }
%     - \bigl( \gamma_{e}^{(k)}(\xe) \bigr)^{(\qe-1)/\qe} \Biggr)
%     \nonumber\\
%     &\overset{(c)}{=}0, \qquad \xe \in \set{S}_{e,2}, e \in \setpf,
%     \label{sec:algsin:eqn:111}
% \end{align}
% %------------------------------------------------------------------------
% where step $(a)$ follows from the expression of the partial derivative in~\eqref{sec:algsin:eqn:108}, 
% where step $(b)$ follows from the fact that the limit of product of functions equals the product of limits of the functions provided that the limit of each function is finite,
% and where step $(c)$ follows from the definition of $ \set{S}_{e,2} $ in~\eqref{sec:algsin:eqn:109} and Lemma~\ref{sec:algsin:lem:4} with the substitution in~\eqref{sec:algsin:eqn:4}. Similarly, we have

% %------------------------------------------------------------------------



==> appendices/props_tensor_norm_1.tex <==
The absolute value of function $ Z_{\|f\|} $ defined in~\eqref{sec:algsin:eqn:32} can be written as
%-----------------------------------------------------------------------
\begin{align}
  \Bigl| Z_{\|f\|}(\vpsi_{\setpf},\vpsi_{\upsetpf}) \Bigr|
  &\overset{(a)}{=} 
  \Biggl| 
    \sum_{\ell_f \in \set{L}_f} 
    \lambda_{f}(\ell_f) \cdot 
    \Biggl( 
      \sum_{ \vx_{\setpf} }
      u_{f}(\vx_{\setpf},\ell_f) 
      \cdot \prod_{e \in \setpf} \psi_{e}(\xe) 
    \Biggr)
    \cdot \Biggl( 
      \sum_{ \vx_{\unpair{\setpf}} }
      \overline{u_{f}(\vx_{\unpair{\setpf}},\ell_f)}
      \cdot \prod_{e \in \setpf} \psi_{\upe}(\xupe) 
    \Biggr) 
  \Biggr|
  \nonumber\\
  &\overset{(b)}{\leq} 
  \sum_{\ell_f \in \set{L}_f} 
  \lambda_{f}(\ell_f) \cdot 
  \Biggl| 
    \sum_{ \vx_{\setpf} }
    u_{f}(\vx_{\setpf},\ell_f) 
    \cdot \prod_{e \in \setpf} \psi_{e}(\xe) 
  \Biggr|
  \cdot \Biggl| 
    \sum_{ \vx_{\unpair{\setpf}} }
    \overline{u_{f}(\vx_{\unpair{\setpf}},\ell_f)}
    \cdot \prod_{e \in \setpf} \psi_{\upe}(\xupe) 
  \Biggr|
  \nonumber\\
  &\overset{(c)}{\leq} 
  \max\Biggl(
    \sum_{\ell_f \in \set{L}_f} 
    \lambda_{f}(\ell_f) \cdot 
    \Biggl| 
      \sum_{ \vx_{\setpf} }
      u_{f}(\vx_{\setpf},\ell_f) 
      \cdot \prod_{e \in \setpf} \psi_{e}(\xe) 
    \Biggr|
    \cdot \Biggl| 
      \sum_{ \vx_{\unpair{\setpf}} }
      \overline{u_{f}(\vx_{\unpair{\setpf}},\ell_f)}
      \cdot \prod_{e \in \setpf} \psi_{e}(\xupe) 
    \Biggr|
    ,\nonumber\\
    &\quad \sum_{\ell_f \in \set{L}_f} 
    \lambda_{f}(\ell_f) \cdot 
    \Biggl| 
      \sum_{ \vx_{\setpf} }
      u_{f}(\vx_{\setpf},\ell_f) 
      \cdot \prod_{\pe \in \setpf} \psi_{\upe}(\xe) 
    \Biggr|
    \cdot \Biggl| 
      \sum_{ \vx_{\unpair{\setpf}} }
      \overline{u_{f}(\vx_{\unpair{\setpf}},\ell_f)}
      \cdot \prod_{e \in \setpf} \psi_{\upe}(\xupe) 
    \Biggr|
  \Biggr) 
  \label{sec:algsin:eqn:73}\\
  &\in \sR_{\geq 0}, \nonumber
\end{align}
%-----------------------------------------------------------------------}
where step $(a)$ follows from the fact that for a strict-sense PE-NFG $ N $, each local function $ f \in \setF $ has a decomposition as shown in~\eqref{sec:DENFG:eqn:5},
where step $(b)$ follows from the triangular inequality and
$ \lambda_{f}(\ell_f) \in \sR_{\geq 0} $ for all $ \ell_f $ in $ \set{L}_f $ as shown in~\eqref{sec:DENFG:eqn:8}, 
and where step $(c)$ follows from the Cauchy-Schwarz inequality.
By setting $ \vpsi_{\upsetpf} = \overline{ \vpsi_{\setpf} } $, we have
%-----------------------------------------------------------------------
\begin{align}
  Z_{\|f\|}(\vpsi_{\setpf},\overline{\vpsi_{\setpf}})
  &\overset{(a)}{=} \sum_{\ell_f \in \set{L}_f} 
    \lambda_{f}(\ell_f) \cdot 
    \Biggl( 
      \sum_{ \vx_{\setpf} }
      u_{f}(\vx_{\setpf},\ell_f) 
      \cdot \prod_{e \in \setpf} \psi_{e}(\xe) 
    \Biggr)
    \cdot \Biggl( 
      \sum_{ \vx_{\unpair{\setpf}} }
      \overline{u_{f}(\vx_{\unpair{\setpf}},\ell_f)
      \cdot \prod_{e \in \setpf} \psi_{e}(\xupe) }
    \Biggr) 
  \nonumber\\
  &= \sum_{\ell_f \in \set{L}_f} 
    \lambda_{f}(\ell_f) \cdot 
    \Biggl| 
      \sum_{ \vx_{\setpf} }
      u_{f}(\vx_{\setpf},\ell_f) 
      \cdot \prod_{e \in \setpf} \psi_{e}(\xe) 
    \Biggr|
    \cdot \Biggl| 
      \sum_{ \vx_{\unpair{\setpf}} }
      u_{f}(\vx_{\unpair{\setpf}},\ell_f)
      \cdot \prod_{e \in \setpf} \psi_{e}(\xupe)
    \Biggr|
  \label{sec:algsin:eqn:74}\\
  &\overset{(b)}{\in} \sR_{\geq 0}. \nonumber
\end{align}
%-----------------------------------------------------------------------
where step $(a)$ follows from the fact that for a strict-sense PE-NFG $ N $, each local function $ f \in \setF $ has a decomposition as shown in~\eqref{sec:DENFG:eqn:5}, and
where step $(b)$ follows from $ \lambda_{f}(\ell_f) \in \sR_{\geq 0} $ for all $ \ell_f $ in $ \set{L}_f $ as shown in~\eqref{sec:DENFG:eqn:8}. Combining~\eqref{sec:algsin:eqn:74} with the inequality in~\eqref{sec:algsin:eqn:73}, we know that it is sufficient to solve the optimization problem in~\eqref{sec:algsin:eqn:28} for solving $ \sig_{q}(f) $.

==> appendices/sst_nonnegative_zb_pesnfg.tex <==
Equation~\eqref{sec:DENFG:eqn:9} shows that the Choi-matrix representation of each local function $ f \in \setF $ in the PE-NFG $\graphN$ can be decomposed as follows:
%----------------------------------------------------------------------------
\begin{align*}
    \matr{C}_f &= \sum_{\ell_f \in \set{L}_f} 
    \lambda_{f}(\ell_{f}) \cdot \vect{u}_{f}(\ell_f) 
    \cdot \bigl( \vect{u}_{f}(\ell_f) \bigr)^{\!\Herm},
\end{align*}
%----------------------------------------------------------------------------
where $ \lambda_{f}(\ell_f) \in \sR_{\geq 0} $ is the eigenvalue of $ \matr{C}_{f} $ associated with the right eigenvector $ \vect{u}_{f}(\ell_f) $.
As a result, the function $ \ZSSTf $ can be written as
%------------------------------------------------------------------------
\begin{align}
    \ZSSTf\bigl( \cvpsi_{\psetpff} \bigr) 
    = \sum_{\ell_{f}}
    \lambda_{f}(\ell_{f})
    \cdot
    \Biggl( 
        \vect{u}_{f}(\ell_{f})^{\tran}
        \cdot \bigotimes_{e \in \setpf}
        \cvpsi_{\ef}
    \Biggr)
    \cdot 
    \Biggl( 
        \vect{u}_{f}(\ell_{f})^{ \Herm}
        \cdot \bigotimes_{\upe \in \upsetpf}
        \cvpsi_{\upef}
    \Biggr). \label{expression of ZSSTf in penfg}
\end{align}
%------------------------------------------------------------------------
%----------------------------------------------------------------------------
\begin{definition}
    We make the following definitions.
    \begin{enumerate}
        \item We define
        \begin{align*}
            \vell^{(M)} \defeq ( \ellfm )_{f \in \setF, m \in [M]}
            \in \prod_{f} \set{L}_{f}^{M}, \qquad 
            \vlam_{\setF}\bigl( \vell^{(M)} \bigr)
            \defeq \prod_{m=1}^{M} 
            \prod_f \lambda_{f}(\ellfm).
        \end{align*}
        % where the finite set $ \set{L}_{f} $ and the function $ \lambda_{f} $ are defined in~\eqref{sec:DENFG:eqn:5}--\eqref{sec:DENFG:eqn:8}.

        \item We also define         
        \begin{align*}
            \dd{\muFSsimple\bigl( \cvpsi_{\setEfull} \bigr)} \defeq \prod_{e \in \setEfull}
            \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}, \qquad 
            \dd{\muFSsimple\bigl( \cvpsi_{\upsetEfull} \bigr)} \defeq \prod_{\upe \in \upsetEfull}
            \dd{\muFSsimple\bigl( \cvpsi_{\upe} \bigr)}.
        \end{align*}
    \end{enumerate}
    In this appendix, we use short-hands $ \sum_{\ellf} $, $ \sum_{\vell^{(M)}} $, and $ \prod_{m,f} $ for 
    $ \sum_{\ellf \in \set{L}_{f}} $, 
    $ \sum_{\vell^{(M)} \in \prod_{f} \set{L}_{f}^{M} } $,
    and $ \prod_{m =1}^{M} \prod_{f \in \setF} $, respectively.
    \edefinition
\end{definition}
%----------------------------------------------------------------------------
We obtain
%-------------------------------------------------------------------
\begin{align*}
    \hspace{0.25cm}&\hspace{-0.25cm}
    \Biggl( \prod_e |\set{B}_{\set{X}_e^M}| \Biggr)^{\!\!\!-2} 
    \cdot \bigl( \ZBM(\graphN) \bigr)^{\!M} \nonumber\\
    &\overset{(a)}{=} 
    \int 
    \prod_f \left( 
      \sum_{\ellf}
        \lambda_{f}(\ellf) 
        \cdot
        \Biggl( 
            \vect{u}_{f}(\ellf)^{\tran}
            \cdot \bigotimes_{e \in \setpf} 
            \cvpsi_{e,f}
        \Biggr)
        \cdot 
        \Biggl( 
            \vect{u}_{f}(\ellf)^{\Herm}
            \cdot \bigotimes_{\upe \in \setpf} 
            \cvpsi_{\upe,f}
        \Biggr)
    \right)^{\!\!\! M}
    \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
    \nonumber\\
    &=
    \sum_{ \vell^{(M)} }
    \vlam_{\setF}\bigl( \vell^{(M)} \bigr)
    \cdot
    \int 
    \prod_{m,f}
    \Biggl( 
        \vect{u}_{f}(\ellfm)^{\tran}
        \cdot \bigotimes_{e \in \setpf} 
        \cvpsi_{e,f}
    \Biggr)
    \cdot 
    \Biggl( 
        \vect{u}_{f}(\ellfm)^{\Herm}
        \cdot \bigotimes_{\upe \in \setpf} 
        \cvpsi_{\upe,f}
    \Biggr)
    \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
    \nonumber\\
    &\overset{(b)}{=} 
    \sum_{ \vell^{(M)} }
    \vlam_{\setF}\bigl( \vell^{(M)} \bigr)
    \cdot \left( 
	    \int 
        \prod_{m,f}
	    % \Biggl( 
            \vect{u}_{f}(\ellfm)^{\tran}
            \cdot \bigotimes_{e \in \setpf} 
            \cvpsi_{e,f}
        % \Biggr)
        \dd{\muFSsimple\bigl( \cvpsi_{\setEfull} \bigr)} 
    \right)
    \cdot 
    % \left( 
	    \int 
        \prod_{m,f}
	    % \Biggl( 
            \vect{u}_{f}(\ellfm)^{\Herm}
            \cdot \bigotimes_{\upe \in \setpf} 
            \cvpsi_{\upe,f}
        % \Biggr)
        \dd{\muFSsimple\bigl( \cvpsi_{\upsetEfull} \bigr)} 
    % \right)
    \nonumber\\
    &\overset{(c)}{=}
    \sum_{ \vell^{(M)} }
    \vlam_{\setF}\bigl( \vell^{(M)} \bigr)
    \cdot
    \left| \int 
    \prod_{m,f}
    % \Biggl( 
        \vect{u}_{f}(\ellfm)^{\tran}
        \cdot \bigotimes_{e \in \setpf} 
        \cvpsi_{e,f}
    % \Biggr)
    \dd{\muFSsimple\bigl( \cvpsi_{\setEfull} \bigr)} 
    \right|^{2}
    \nonumber\\
    &\overset{(f)}{\geq} 0,
\end{align*}
%-------------------------------------------------------------------
%----------------------------------------------------------------------------
\begin{itemize}
    \item where step $(a)$ follows from substituting \eqref{expression of ZSSTf in penfg} into the integral in~\eqref{sec:SST:eqn:21} in Proposition~\ref{prop:altenative expression of ZBM by eigenvalue decomposition and SST},

    \item where step $(b)$ follows from Items~\ref{sec:SST:def:7:item:1} and~\ref{sec:SST:def:7:item:2} in Definition~\ref{sec:SST:def:7}, \ie,
    %----------------------------------------------------------------------------
    \begin{align*}
        \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
        =\prod_{e \in \setEfull}
        \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)}
        \cdot 
        \prod_{\upe \in \upsetEfull}
        \dd{\muFSsimple\bigl( \cvpsi_{\upe} \bigr)}, \qquad 
        \int \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)} = 
        \int \dd{\muFSsimple\bigl( \cvpsi_{\upe} \bigr)} =1, \qquad 
        \pe = (e,\upe) \in \setEfull,
    \end{align*}
    %----------------------------------------------------------------------------

    \item where step $(c)$ follows from
    %-----------------------------------------------------------------------
    \begin{align}
        \hspace{0.25cm}&\hspace{-0.25cm}\int 
        \prod_{m,f}
        % \Biggl( 
            \vect{u}_{f}(\ellfm)^{\Herm}
            \cdot \bigotimes_{\upe \in \setpf} 
            \cvpsi_{\upe,f}
        % \Biggr)
        \dd{\muFSsimple\bigl( \cvpsi_{\upsetEfull} \bigr)} 
        \nonumber\\
        &\overset{(d)}{=}
        \int 
        \prod_{m,f}
        % \Biggl( 
            \vect{u}_{f}(\ellfm)^{\Herm}
            \cdot \bigotimes_{e \in \setpf} 
            \cvpsi_{e,f}
        % \Biggr)
        \dd{\muFSsimple\bigl( \cvpsi_{\setEfull} \bigr)}
        \nonumber\\
        &= \overline{ 
            \int 
            \prod_{m,f}
            % \Biggl( 
                \vect{u}_{f}(\ellfm)^{\tran}
                \cdot \bigotimes_{e \in \setpf} 
                \overline{ \cvpsi_{e,f} }
            % \Biggr)
            \dd{\muFSsimple\bigl( \cvpsi_{\setEfull} \bigr)}
        }
        \nonumber\\
        &\overset{(e)}{=}
        \overline{ 
            \int 
            \prod_{m,f}
            % \Biggl( 
                \vect{u}_{f}(\ellfm)^{\tran}
                \cdot \bigotimes_{e \in \setpf} 
                \cvpsi_{e,f}
            % \Biggr)
            \dd{\muFSsimple\bigl( \cvpsi_{\setEfull} \bigr)}
        }, \label{sec:SST:eqn:34}
    \end{align}
    %-----------------------------------------------------------------------
    %----------------------------------------------------------------------------
    % \begin{itemize}
        \item where step $(d)$ follows from  the fact that $ \setxe = \setxupe $ for all $ \pe = (e,\upe) \in \psetpf $ as stated in Item~\ref{sec:DENFG:def:4:item:1} in Definition~\ref{sec:DENFG:def:4},
        
        \item where step $(e)$ follows from the fact that for each $ e \in \setEfull $, the measure $ \muFSsimple\bigl( \cvpsi_{e} \bigr) $ is a Fubini-Study measure, \textit{i.e.}, a Haar measure over $ \sC^{|\setxe|} $, and thus replacing $ \overline{\cvpsi_{e,f}} $ with $ \cvpsi_{e,f} $ for all $ e \in \setpf $ and $ f \in \setF $ does not change the integral's value,
    % \end{itemize}
    %----------------------------------------------------------------------------

    \item where step $(f)$ follows from Assumption~\ref{sec:DENFG:asum:2}: $ \lambda_{f}(\ellf) \in \sR_{\geq 0} $ for all $ \ellf \in \set{L}_{f} $ and $ f \in \setF $.

\end{itemize}
%----------------------------------------------------------------------------




% %---------------------------------------------------------------------------
% \begin{enumerate}

%   \item

%     \item for each $ \pe = (e,\upe) \in \psetEfull $, both $ \cvpsi_{e} $ and $ \cvpsi_{\upe} $ are vectors in $ \sC^{|\setxe|} $ with $ \| \cvpsi_{e} \|_{2} = \|\cvpsi_{\upe}\|_{2} = 1 $ as defined in~\eqref{sec:SST:eqn:28};

%   \item for each $ \pe= (e,\upe) \in \psetEfull $, both the measure $ \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)} $ and the measure $ \dd{\muFSsimple\bigl( \cvpsi_{\upe} \bigr)} $ are independent Fubini-Study measures, \textit{i.e.}, Haar measures over $\{ \cvpsi_{e} \in \sC^{|\setxe|} \ | \ \| \cvpsi_{e} \|_{2} = 1  \} $ as defined in items~\ref{sec:SST:def:7:item:1} and~\ref{sec:SST:def:7:item:2} in Definition~\ref{sec:SST:def:7};

%     \item based on that, it is equivalent to replacing $ \dd{\muFSsimple\bigl( \cvpsi_{\upe} \bigr)} $ with $ \dd{\muFSsimple\bigl( \cvpsi_{e} \bigr)} $ for all $ \pe = (e,\upe) \in \psetEfull $ in the integral,
    
% \end{enumerate}
% %---------------------------------------------------------------------------

==> appendices/sst_snfg.tex <==
The symmetric-subspace transform (SST) provides a different perspective to understand the $M$-covers of S-NFGs or DE-NFGs. While this transformation has been applied in quantum physics~\cite{Wood2015,Harrow2013}, to the best of our knowledge, it is the first time to introduce the SST in the factor-graph literature.

The developments in this section were motivated by the work of Wood \etal~\cite{Wood2015}, where, in terms of the language of the present paper, they transformed a certain integral into the average partition function of some NFGs, with the average taken over double covers. (Although~\cite{Wood2015} focus on double covers, it is clear that their results can be extended to general $M$-covers.) However, in contrast to~\cite{Wood2015}, our approach takes the opposite direction. We express the average partition function of a given NFG in terms of some integral, where the average is over all $M$-covers of the considered NFG.

\section{Reformulation of the function \texorpdfstring{$P_e$}{} as an Integral}
\label{sec:SST:Pe:reformulation:1}

\begin{figure}[t]
	% \subfloat[]{
    % \begin{minipage}[t]{0.3\textwidth}
      \centering
      \begin{tikzpicture}
        \input{figures/head_files_figs.tex}
        \input{figures/sst_examples/snfg/length_large.tex}
        \input{figures/sst_examples/snfg/background_nodes_lines.tex}
        \input{figures/sst_examples/snfg/lines_not_permuted.tex}
        \input{figures/sst_examples/snfg/otb_pe.tex}
        \node[] (var1) at (-0.18*\ldis,-1*\ldis) [label=right: $\cvpsi_{e}$] {};
        \node[state] (Psige) at (0,-1.5*\ldis) [label=below: $ \bigl| \set{B}_{\set{X}_e^M}\! \bigr| \cdot \muFSsimple$] {};
        \input{figures/sst_examples/snfg/otb_back_nodes_lines.tex}
        \begin{pgfonlayer}{background}
          \node[state_dash6] (db1) at (0,0.1*\ldis) [label=below:$P_{e}$] {};
        \end{pgfonlayer}
      \end{tikzpicture}
    % \end{minipage}
    \caption{The NFG for illustrating the SST for S-NFG.\label{sec:SST:fig:10}}
  % }
\end{figure}

%***************************************************************************

In this section, we explore an approach to express the function $P_e$ as an  integral. This integral representation can be utilized to modify the NFG in
Fig.~\ref{sec:SST:fig:9}, resulting in the NFG shown in
Fig.~\ref{sec:SST:fig:10}.

%***************************************************************************


%***************************************************************************

\begin{definition}\label{sec:SST:def:3}
	For the following considerations, we consider an arbitrary edge
	$e = (f_{i}, f_{j}) \in \setEfull$ and a positive integer $M$. We introduce
	the following notation:
	\begin{itemize}

		\item The $2$-norm of a function $\psi_e: \set{X}_e \to \sC$ is defined to be
			$\lVert \psi_e \rVert_{2} \defeq \sqrt{\sum_{\xe} |\psi_e(\xe)|^2}$.

		\item The 2-norm of a vector
			$\vpsi_e = \bigl( \psi_e(\xe) \bigr)_{\xe \in \set{X}_e} \in
			\sC^{|\set{X}_e|}$ is defined to be
			$\lVert \vpsi_e \rVert_{2} \defeq \sqrt{\sum_{\xe} |\psi_e(\xe)|^2} =
			\sqrt{\vpsi_e^\Herm \cdot \vpsi_e}$.

		% \item The vector containing the absolute values of the entries in the vector $ \cvpsi_e $ is defined to be $ |\cvpsi_e| = \bigl( |\cpsi_e(\xe)| \bigr)_{\xe \in \set{X}_e} \in
		% 	\sR_{\geq 0}^{|\set{X}_e|} $.

	\end{itemize}

	Now, let $\cpsi_e: \set{X}_e \to \sC$ be a function with $2$-norm equals one, \textit{i.e.},
	$\lVert \cpsi_e \rVert_{2} = 1$. Based on $\cpsi_e$, we define the function
	$\funcFS_{e,\cpsi_e}: \set{X}_e^{2M} \to \sC$ as follows:
	\begin{align*}
		\funcFS_{e,\cpsi_e}\bigl( \vx_{\efi,[M]}, \vx_{\efj,[M]} \bigr)
		&\defeq
			\bigl| \set{B}_{\set{X}_e^M} \bigr|
			\cdot
			\Biggl(
				 \prod_{m \in [M]}
					 \cpsi_e(x_{\efi,m})
			\Biggr)
			\cdot
			\Biggl(
				 \prod_{m \in [M]}
					 \overline{ \cpsi_e(x_{\efj,m}) }
			\Biggr),
			\qquad \vx_{\efi,[M]}, \vx_{\efj,[M]} \in \set{X}_e^M.
	\end{align*}
	\edefinition
\end{definition}

%***************************************************************************
If we associate the function $\cpsi_e$ with the column vector
%----------------------------------------------------------------------------
\begin{align}
	\cvpsi_e \defeq \bigl( \cpsi_e(\xe) \bigr)_{\xe \in \set{X}_e}
	\in \sC^{|\setxe|},
	\label{sec:SST:eqn:39}
\end{align}
%----------------------------------------------------------------------------
and the
function $\funcFS_{e,\cpsi_e}$ with the matrix $\matrFS_{e,\cpsi_e}$ (with rows
indexed by $\vx_{\efi,[M]}$ and columns indexed by $\vx_{\efj,[M]}$), then we have
\begin{align*}
	\matrFS_{e,\cpsi_e}
		&= \bigl| \set{B}_{\set{X}_e^M} \bigr|
		\cdot
		\bigl( \cvpsi_e^{\otimes M} \bigr)
		\cdot
		\bigl( \cvpsi_e^{\otimes M} \bigr)^{\! \Herm}
		\in \sC^{|\setxe| \times |\setxe|},
\end{align*}
where $\cvpsi_e^{\otimes M}$ represents the $M$-fold Kronecker product of
$\cvpsi_e$ with itself.

%***************************************************************************

% Alternatively, with the introduction of some suitable locally compact
% topological group, it is a Haar measure over that group.

In the following, for every $ e \in \setEfull $, we introduce the so-called Fubini-Study measure in dimension $|\set{X}_e|$ which can be viewed as a, 
in a suitable sense, uniform measure $\muFSsimple$ on functions
$\cpsi_e: \set{X}_e \to \sC_{\geq 0}$ with a $ 2 $-norm of one. This measure is also a Haar measure.
For the purposes of this paper, it is sufficient
to know that a sample $\cvpsi_{e} \in \sC^{|\set{X}_e|}$ from $\muFSsimple$ can be
generated as follows:
\begin{itemize}

\item Let
	\begin{align*}
		\vW_e 
			&\defeq
				 \bigl(
					 (W_{e,\xe,0}, W_{e,\xe,1})
				 \bigr)_{\xe \in \set{X}_e}
					 \in \sR^{|\set{X}_e|} \times \sR^{|\set{X}_e|}
	\end{align*}
	be a length-$2 |\set{X}_e|$ random vector with i.i.d. entries distributed
	according to a normal distribution with mean zero and variance one.

	\item Let $\vw_e$ be a realization of $\vW_e$. Let\footnote{Recall that
		``$\imagunit$'' denotes the imaginary unit.}
	\begin{align*}
		\cvw_e
			&\defeq
				 \vw_e / \lVert \vw_e \rVert_{2}, \nonumber \\
		\cpsi_e(\xe)
			&=
				 \cw_{e,\xe,0} + \imagunit \cw_{e,\xe,1}. 
	 \nonumber
	\end{align*}
	 Because of the bijection between $\cvw$ and $\cvpsi$, we will use, with some slight abuse of notation, the notation $\muFSsimple$ not only for the distribution of $\cvpsi$, but also for the distribution of $\cvw$. In this case, the 2-norm of the function $ \cpsi_e $ is still one, \ie,
	 %------------------------------------------------------------------------
	 \begin{align*}
	 	\sum_{\xe} \bigl| \cpsi_e(\xe) \bigr|^{2} = 1. 
	 \end{align*}
	 %------------------------------------------------------------------------
\end{itemize} 


%***************************************************************************

%---------------------------------------------------------------------------
\begin{lemma}\label{sec:SST:prop:2}

	For all $ \vx_{\efi,[M]}, \vx_{\efj,[M]} \in \set{X}_e^M $, it holds that 
	\begin{align*}
		\int
			\funcFS_{e,\cpsi_e}\bigl( \vx_{\efi,[M]}, \vx_{\efj,[M]} \bigr)
		\dd{\muFSsimple\bigl( \cvpsi_e \bigr)} 
		&= P_e\bigl( \vx_{\efi,[M]}, \vx_{\efj,[M]} \bigr).
	\end{align*}
\end{lemma}
%---------------------------------------------------------------------------
\begin{proof}
	See Appendix~\ref{apx:SST}.
\end{proof}
%---------------------------------------------------------------------------

% {\color{blue}
% Instead of consider the measure of $ \vpsi_{e} $, we can consider the measures of $ |\vpsi| $

% %---------------------------------------------------------------------------
% \begin{definition}
% 	For each $ \xe \in \setxe $ and $ e \in \setEfull $, 
% 	we consider the set $ \set{S}_{e,\xe} \subseteq [0,2\pi] $ and the associated variable $ \theta_{e}(\xe) \in S_{e,\xe} $. Then we define
% 	%-----------------------------------------------------------------------
% 	\begin{alignat*}{3}
% 		\set{S}_{e,\xe} + \pi &\defeq
% 		\Bigl\{ 
% 			\theta_{e}(\xe) \ | \ \theta_{e}(\xe) = \theta_{e}'(\xe) 
% 			\theta_{e}'(\xe) \in S_{e,\xe}
% 		\Bigr\}, \nonumber\\
% 		\vtheta_{e} &\defeq ( \theta_{e}(\xe) )_{\xe \in \setxe} 
% 		\qquad 
% 		&\vtheta &\defeq ( \vtheta_{e} )_{e},
% 		\nonumber\\
% 		\set{S}_{e} &\defeq \prod_{\xe \in \setxe} \set{S}_{e,\xe},
% 		\qquad
% 		& \set{S}_{e} + \pi &= \Bigl\{ \vtheta_{e} \ \left| \
% 		\theta_{e}(\xe) = \theta_{e}'(\xe), \, 
% 		\theta_{e}'(\xe) \in S_{e,\xe},\,
% 		\xe \in \setxe \right. \Bigr\}, 
% 		\nonumber\\		
% 		\set{S}_{\setEfull} &\defeq \prod_{e} \set{S}_{e},
% 		& \set{S}_{\setEfull} + \pi &=  
% 		\prod_{e} ( \set{S}_{e} + \pi ).
% 	\end{alignat*}
% 	%-----------------------------------------------------------------------
% \end{definition}
% %---------------------------------------------------------------------------
% }
% %---------------------------------------------------------------------------
% \begin{remark}	
% 	This remark compares the methods used in~\cite{Vontobel2013} with the methods used in this paper. 
% 	%---------------------------------------------------------------------------
% 	\begin{enumerate}
% 		\item Vontobel in~\cite{Vontobel2013} used the method of types to analyze the behavior of $ \sqrt[M]{ Z\bigl( \hgraphNavg \bigr) } $ to be $ M \to \infty $. In particular, he letted $ \vbeli \in \LMP(\graphN) $ as a pseudomarginal vector consisting of rational elements only. The average number of valid configurations that map down to $ \vbeli $ among all the $M$-covers was denoted by $ \bar{C}_{M}(\vbeli) $. 
% 		In~\cite[Theorem 30]{Vontobel2013}, Vontobel employed the method of types to prove the following expressions as combinatorial characterizations of the Bethe entropy function $ H_{\mathrm{B}} $ and the Bethe free energy function $ \FB $:
% 		%--------------------------------------------------------------------
% 		\begin{align*}
% 			\bar{C}_{M}(\vbeli) &=
% 			\exp\bigl( -M \cdot H_{\mathrm{B}}(\vbeli) + O(M) \bigr), 
% 			\qquad \vbeli \in \set{B}'_{M}, \\
% 			\bigl( \ZBM( \graphN ) \bigr)^{M}&= 
% 			\sum_{\vbeli \in \set{B}'_{M}} 
% 			\exp\bigl( -M \cdot \FB(\vbeli) + O(M) \bigr),
% 		\end{align*}
% 		%-------------------------------------------------------------------
% 		where $ O(\cdot) $ represents standard big-$O$ notation and the set $ \set{B}'_{M} \subseteq \set{B}_{\set{X}^M} $ represents the set of all $M$-cover lift-realizable pseudo-marginal vectors. (For the details of lift-realizable pseudo-marginal vectors, see~\cite{Kelley2007}.)
% 		Based on these characterizations, Vontobel in~\cite[Theorem 33]{Vontobel2013} showed that
% 		%------------------------------------------------------------------------
% 		\begin{align*}
% 			\limsup_{M \to \infty} \ZBM( \graphN )
% 			= \ZB(\graphN).
% 		\end{align*}
% 		%------------------------------------------------------------------------

% 		\item In this paper, we analyze $ Z\bigl( \hgraphNavg \bigr) $, \ie, $  \ZBM( \graphN ) $, by studying the function $ \funcFS_{e,\cpsi_e} $ and examining the asymptotic behavior of the integral in 
% 		%------------------------------------------------------------------------
% 		\begin{align*}
% 			P_e\bigl( \vx_{\efi,[M]}, \vx_{\efj,[M]} \bigr) = 
% 			\int
% 				\funcFS_{e,\cpsi_e}\bigl( \vx_{\efi,[M]}, \vx_{\efj,[M]} \bigr)
% 			\dd{\muFSsimple\bigl( \cvpsi_e \bigr)},
% 			\qquad \vx_{\efi,[M]}, \vx_{\efj,[M]} \in \set{X}_e^M,
% 		\end{align*}
% 		%------------------------------------------------------------------------
% 		as $ M \to \infty $. This approach does not require specific mathematical results derived from the method of types.
% 		Based on this observation, we propose an alternative NFG representing the average $M$-cover of an S-NFG in the following.
% 	\end{enumerate}
% 	\eremark
% \end{remark}
% %---------------------------------------------------------------------------



%***************************************************************************
%***************************************************************************

\section{An Alternative NFG Representing 
the Average \texorpdfstring{$M$}{}-Cover of an S-NFG\label{sec:SST:sunbsec:2}}

%***************************************************************************

In Section~\ref{sec:SST:NFG:average:cover:1}, we introduced the NFG
$\hgraphNavg$, whose partition function equals
$\bigl( \ZBM(\graphN) \bigr)^M$. Now, based on the
results from Section~\ref{sec:SST:Pe:reformulation:1}, we formulate an
alternative NFG, denoted by $\hgraphNavgalt$. The partition function of $\hgraphNavgalt$ also equals
$\bigl( \ZBM(\graphN) \bigr)^M$.

%***************************************************************************

Recall that $P_e\bigl( \vx_{\efi,[M]}, \vx_{\efj,[M]} \bigr)$ represents the exterior
function of the dashed box in Fig.~\ref{sec:SST:fig:8}; in other
words, if we close the dashed box in Fig.~\ref{sec:SST:fig:8}, then we
obtain a single function node representing the function
$P_e\bigl( \vx_{\efi,[M]}, \vx_{\efj,[M]} \bigr)$, as shown in Fig.~\ref{sec:SST:fig:9}.

%***************************************************************************

The NFG $\hgraphNavgalt$ in Fig.~\ref{sec:SST:fig:10} is defined
such that it is the same as the NFG $\hgraphNavg$ in
Fig.~\ref{sec:SST:fig:9}, except for the content of the function $ P_{e} $
for every $e \in \setEfull$. However, the content of the dashed box in
Fig.~\ref{sec:SST:fig:10} is set up in such a way that its exterior function
equals the function $ P_{e} $ in
Fig.~\ref{sec:SST:fig:9} as well as the exterior function of the dashed box in Fig.~\ref{sec:SST:fig:8}. 

By closing the dashed box in Fig.~\ref{sec:SST:fig:10}, a single function node representing the function $P_e$ is formed, as shown in Fig.~\ref{sec:SST:fig:9}. This ensures that the partition function of the NFG in Fig.~\ref{sec:SST:fig:10} equals the partition functions of the NFGs in Figs.~\ref{sec:SST:fig:8} and~\ref{sec:SST:fig:9}. In other words, it can be stated that $Z\bigl( \hgraphNavgalt \bigr) = Z\bigl( \hgraphNavg \bigr) = \bigl( \ZBM(\graphN) \bigr)^M$.\footnote{In terms of NFG language, the
	NFG in Fig.~\ref{sec:SST:fig:10} can be obtained
	by, first applying a closing-the-box operation and
	then an opening-the-box operation~\cite{Loeliger2004} for every $e \in \setEfull$. Note that
	closing-the-box and opening-the-box operations maintain the partition
	function of the NFG.}


% With that, closing the dashed box in
% Fig.~\ref{sec:SST:fig:10} results in a single function node
% representing the function $P_e$, as shown in Fig.~\ref{sec:SST:fig:9}. 




% This guarantees
% that the partition function of the NFG in Fig.~\ref{sec:SST:fig:10}
% equals the partition functions of the NFGs in
% Figs.~\ref{sec:SST:fig:8} and~\ref{sec:SST:fig:9}, \textit{i.e.},
% $Z\bigl( \hgraphNavgalt \bigr) = Z\bigl( \hgraphNavg \bigr) = \bigl( \ZBM(\graphN) \bigr)^M$.\footnote{In terms of NFG language, the
% 	NFG in Fig.~\ref{sec:SST:fig:10} can be obtained
% 	by, first applying a closing-the-box operation and
% 	then an opening-the-box operation~\cite{Loeliger2004a} for every $e \in \setEfull$. Note that
% 	closing-the-box and opening-the-box operations maintain the partition
% 	function of the NFG.}

%***************************************************************************

In the NFG shown in Fig.~\ref{sec:SST:fig:10}, compared to the NFG in Fig.~\ref{sec:SST:fig:8}, the following new elements are introduced for every $ e \in \setEfull $:
\begin{itemize}

\item An edge is added with an associated variable (vector)
	$\cvpsi_e \in \sC^{|\set{X}_e|}$.

\item A function node is added, representing the function
	\begin{align*}
		p_e\bigl( \cvpsi_e \bigr)
			&\defeq
				 \bigl| \set{B}_{\set{X}_e^M} \bigr|
				 \cdot
				 \muFSsimple\bigl( \cvpsi_e \bigr).
	\end{align*}

\item $M$ function nodes representing the function $\cpsi_e$ are added, and $M$ function nodes representing the function $\overline{\cpsi_e}$ are added.  The function $\cpsi_e$ is specified by $\cvpsi_e$ a straightforward manner.

\end{itemize}

%***************************************************************************

%---------------------------------------------------------------------------
\begin{definition}
	\label{sec:SST:def:5}

	We make the following definitions for $ \avgalt{\graphN} $.
	%-----------------------------------------------------------------------
	\begin{enumerate}

		\item We define the set of variables $ \vxavgalt $ to be 
		$ \vxavgalt \defeq ( x_{\ef,m} )_{e \in \setpf, \, f \in \setF, \, m \in [M]} 
		\in \setx{}^{2M} $.

		\item We define the set of vectors $ \cvpsiavgalt $ to be $ \cvpsiavgalt \defeq ( \cvpsi_e )_{e \in \setEfull} $, where $ \cvpsi_{e} $ is defined in~\eqref{sec:SST:eqn:39} for all $ e \in \setEfull $.

		\item We define the measure $ \muFSsimple\bigl( \cvpsiavgalt \bigr) $ to be the product of Fubini-Study measures: 
		$ \muFSsimple\bigl( \cvpsiavgalt \bigr) 
		\defeq \prod_{e} \muFSsimple\bigl( \cvpsi_e \bigr) $.

		\item For each $ e = (f_{i}, f_{j}) \in \setEfull $ such that $ i<j $, we define 
		\begin{align*}
			\cpsi_{\efi}(\xe)
			\defeq \cpsi_{e}(\xe), \qquad
			\cpsi_{\efj}(\xe)
			\defeq \overline{\cpsi_{e}(\xe)}, \qquad
			\xe \in \setxe.
		\end{align*}
	\end{enumerate}
	\edefinition
\end{definition}
%---------------------------------------------------------------------------



With this, the global function of $\hgraphNavgalt$ is
\begin{align}
	g\bigl( \vxavgalt, \cvpsiavgalt \bigr)
		&= \left(
			 \prod_f
				 \prod_{m \in [M]} f(\vx_{\setpff,m})
		 \right)
		 \cdot
		 \left(
			 \prod_{e=(f_{i},f_{j})}
				 	\Biggl( 
					 \bigl| \set{B}_{\set{X}_e^M} \bigr|
					 \cdot
					 \prod_{m \in [M]}
						\bigl( 
							\cpsi_{\efi}(x_{\efi,m})
							\cdot
							\cpsi_{\efj}(x_{\efj,m})
						\bigr)	
					\Biggr)
		 \right) \label{sec:SST:eqn:26} \\
		 &= \Biggl( \prod_f \prod_{m \in [M]} f(\vx_{\setpff,m}) \Biggr)
		 \cdot \prod_{e} 
		 \funcFS_{e,\cpsi_e}\bigl( \vx_{\efi,[M]}, \vx_{\efj,[M]} \bigr), \qquad 
		 \vx_{\efi,[M]}, \vx_{\efj,[M]} \in \set{X}_e^M, \label{sec:SST:eqn:10}
\end{align}
%***************************************************************************
where the last equality follows from the definition of $ \funcFS $ in Definition~\ref{sec:SST:def:3}. Define $ \ZSSTM $ to be the partition function for fixed $ \cvpsiavgalt $:
%----------------------------------------------------------------------------
\begin{align}
	\ZSSTM\bigl( \avgalt{\graphN}, \cvpsiavgalt \bigr) \defeq 
	\sum_{\vxavgalt} g\bigl( \vxavgalt, \cvpsiavgalt \bigr), 
	\label{sec:SST:eqn:43}
\end{align}
%----------------------------------------------------------------------------
where $ \sum_{\vxavgalt} $ represents $ \sum_{ \vxavgalt \in \setx{}^{2M} } $.


%---------------------------------------------------------------------------
\begin{proposition}
	\label{sec:SST:prop:1}
	\label{SEC:SST:PROP:1}

	The partition function of $\hgraphNavgalt$ satisfies
	\begin{align*}
		Z\bigl( \hgraphNavgalt \bigr)
		&= \int \ZSSTM\bigl( \avgalt{\graphN}, \cvpsiavgalt \bigr)
		\dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
		\nonumber\\
		&= 
		\left( \prod_e\bigl| \set{B}_{\set{X}_e^M} \bigr| \right)
	    \cdot  
	    \int \prod_f \Bigl( \ZSSTf\bigl( \cvpsi_{\setpff} \bigr) \Bigr)^{ \! M}
	    \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)} 
	    \\
		&= Z\bigl( \hgraphNavg \bigr),
	\end{align*}
	where for each function node $ f \in \setF $, we define
	%----------------------------------------------------------------------------
	\begin{align}
		\ZSSTf\bigl( \cvpsi_{\setpff} \bigr) 
		\defeq \sum_{\vx_{\setpf}}
	  	f(\vx_{\setpf}) 
	  	\cdot
	  	\prod_{e \in \setpf} 
	  	\cpsi_{e,f}(x_{e}), \label{sec:SST:eqn:42}
	\end{align}
	%----------------------------------------------------------------------------
	and $ \cvpsi_{\setpff} \defeq ( \cvpsi_{\ef} )_{e \in \setpf} $.
\end{proposition}
%***************************************************************************

\begin{proof}
	See Appendix~\ref{apx:property of SST}.
\end{proof}

%***************************************************************************
Consider conditioning on $\cvpsiavgalt$. The simplification $ \prod_f \Bigl( \ZSSTf\bigl( \cvpsi_{\setpff} \bigr) \Bigr)^{ \! M} $ obtained in Proposition~\ref{sec:SST:prop:1} is made possible by decomposing the NFG into $|\setF| \cdot M$ tree-structured components. This decomposition allows us to factorize and separate the partition function into individual components, each corresponding to a tree-structured factor graph consisting of a function node. 

% The simplification that was achieved in the proof of
% Proposition~\ref{sec:SST:prop:1} was thanks to the fact that,
% conditioned on $\cvpsiavgalt$, the NFG decomposes into an NFG with
% $|\setF| \cdot M$ components, where each component is tree-structured.


%***************************************************************************
%***************************************************************************

\section{Combining the Results of this Section}
\label{sec:SST:combining:results:1}
%***************************************************************************

Combining the main results of this section, \ie,
\begin{alignat}{2}
	\text{(Introduction of Section~\ref{sec:SST})} \quad &&
	\ZBM(\graphN)
		&=
			 \sqrt[M]{
				 \Bigl\langle 
					 Z\bigl( \hgraphN \bigr)
				 \Bigr\rangle_{\hgraphN \in \hat{\set{N}}_{M}} }, 
	\label{sec:SST:eqn:expresssion of ZBM} \\
	\text{(Lemma~\ref{sec:SST:lem:1})} \quad &&
	Z\bigl( \hgraphNavg \bigr)
		&= \bigl( \ZBM(\graphN) \bigr)^{\! M}, 
	\label{sec:SST:eqn:23} \\
	\text{(Proposition~\ref{sec:SST:prop:1})} \quad &&
	Z\bigl( \hgraphNavgalt \bigr)
		&= Z\bigl( \hgraphNavg \bigr), 
	\label{sec:SST:eqn:24} \\
	\text{(Proposition~\ref{sec:SST:prop:1})} \quad &&
	Z\bigl( \hgraphNavgalt \bigr)
		&= 
		\left( \prod_e\bigl| \set{B}_{\set{X}_e^M} \bigr| \right)
	    \cdot  
	    \int \prod_f \Bigl( \ZSSTf\bigl( \cvpsi_{\setpff} \bigr) \Bigr)^{ \! M}
	    \dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}, \nonumber
\end{alignat}
we can obtain the expression for $\ZBM(\graphN)$ as follows:
\begin{align}
	\ZBM(\graphN)
	&= 	
	\Biggl( \prod_e \bigl| \set{B}_{\set{X}_e^M} \bigr| \Biggr)^{\!\!\! 1/M}
	\cdot \Biggl(
	\int \prod_f \Bigl( \ZSSTf\bigl( \cvpsi_{\setpff} \bigr) \Bigr)^{ \! M}
	\dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
	\Biggr)^{\!\!\! 1/M}. \label{alternative expression of ZBM in snfg}
\end{align}
% Recall that we are mostly interested in evaluating the limit $\limsup_{M \to \infty} \ZBM(\graphN)$. 
% \begin{lemma}
% 	\label{sec:SST:lem:3}

% 	It holds that
% 	\begin{align*}
% 		\lim_{M \to \infty}
% 			\left(
% 				\prod_e
% 					|\set{B}_{\set{X}_e^M}|
% 			\right)^{\!\! 1/M}
% 			&= 1.
% 	\end{align*}
% \end{lemma}

% %***************************************************************************

% \begin{proof}
% 	Recall from Lemma~\ref{sec:SST:lem:2} that
% 	$|\set{B}_{\set{X}_e^M}| = \binom{|\set{X}_e| + M - 1}{M} = \binom{|\set{X}_e| + M - 1}{|\set{X}_e| - 1} \in O\bigl( M^{|\set{X}_e|-1} \bigr)$, where we have
% 	used the standard big-$O$ notation. This means that $|\set{B}_{\set{X}_e^M}|$
% 	grows only polynomially in $M$, not exponentially in $M$. This allows us to
% 	conclude that
% 	\begin{align*}
% 		\log \left(
% 		\lim_{M \to \infty}
% 		\left(
% 			\prod_e
% 				|\set{B}_{\set{X}_e^M}|
% 		\right)^{\!\! 1/M}
% 		\right)
% 		&= \lim_{M \to \infty}\log
% 		\left(
% 			\left(
% 				\prod_e |\set{B}_{\set{X}_e^M}|
% 			\right)^{\!\! 1/M}
% 		\right) \\
% 		&= \lim_{M \to \infty} \frac{1}{M}
% 		\sum_e \log
% 		\bigl(
% 			|\set{B}_{\set{X}_e^M}|
% 		\bigr) \\
% 		 &= 0.
% 	\end{align*}
% \end{proof}
% %***************************************************************************

\section{SST for DE-NFGs}
\label{sec:SST:DENFG:1}

% \input{figures/sst_examples/denfg/main_pic.tex}
% Comparing
% Figs.~\ref{sec:SST:fig:1} and~\ref{sec:SST:fig:10} for S-NFGs with
% Fig.~\ref{sec:SST:fig:2} for DE-NFGs, 
%***************************************************************************
So far, this section was about the SST for an S-NFGs. The extension to the SST
of a DE-NFGs is, by and large, straightforward. 
We note that the only major change is that for
every edge $e \in \setEfull$, the role of the alphabet $\set{X}_e$ is taken over by
the alphabet $\tset{X}_e = \set{X}_e \times \set{X}_e$. 
% With this, the value of
% $\ZBM(\graphN)$ for a DE-NFG $\graphN$ can be written as (compare
% with~\eqref{alternative expression of ZBM in snfg})
% \begin{align}
% 	\ZBM(\graphN)
% 	=
% 	\Biggl( \prod_e \bigl| \set{B}_{\tset{X}_e^M} \bigr| \Biggr)^{\!\!\! 1/M}
% 	\cdot \Biggl(
% 	\int \prod_f \Bigl( \ZSSTf\bigl( \cvpsi_{\setpff} \bigr) \Bigr)^{ \! M}
% 	\dd{\muFSsimple\bigl( \cvpsiavgalt \bigr)}
% 	\Biggr)^{\!\!\! 1/M}. \label{sec:SST:eqn:3}
% \end{align}
% where
% \begin{align*}
% 	\ZSSTf\bigl( \cvpsi_{\setpff} \bigr)
% 	\defeq 
% 	\sum_{\tvx_{\setpf}}
% 	f(\tvx_{\setpf}) 
% 	\cdot
% 	\prod_{e \in \setpf} 
% 	\cpsi_{e,f}(\txe)
% \end{align*}
% where $\cvpsiavgalt \defeq ( \cvpsi_e )_{e \in \setEfull}$ and where for every
% $e \in \setEfull$, the norm-one vector $\cvpsi_e$ is distributed according to the
% Fubini-Study measure in dimension $|\tset{X}_e|$. Similar
% to Lemma~\ref{sec:SST:lem:3}, we can omit the first factor on the
% right-hand side of~\eqref{sec:SST:eqn:3} in the limit $M \to
% \infty$. (This follows from a straightforward generalization of
% Lemma~\ref{sec:SST:lem:3}.)


==> appendices/the_message_conjugate_penfg.tex <==
It is sufficient to consider the case where $t = 1$. The proof for $t \in \sZ_{\geq 2}$ is similar and is thus omitted.

For $ t =1 $, considering a pair of edge $ \pe \in \psetEfull $ connecting function nodes $ f_{i} $ and $ f_{j} $, we have
%------------------------------------------------------------------------
\begin{align*}
  \overline{\mu_{\upefi}^{(1)}(\zupe)}
  &= \overline{ \bigl( \kappa_{\upefi}^{(1)} \bigr)^{\!-1} } 
    \cdot
        \sum_{\vx_{\psetpfj}: \, \xupe = \zupe}
        \overline{ f_{j}\bigl( \vx_{\psetpfj} \bigr) }
        \cdot
        \overline{ \mu_{\efj}^{(0)}(\xe) }
        \cdot
        \prod_{\pe'\in \psetpfj \setminus \pe}
        \overline{ \mu_{\epfj}^{(0)}(x_{e'}) }
        \cdot 
        \overline{ \mu_{\upepfj}^{(0)}(x_{\upe'}) }
    \nonumber\\
    &\overset{(a)}{=}
    \overline{ \bigl( \kappa_{\upefi}^{(1)} \bigr)^{\!-1} } 
    \cdot
    \sum_{\vx_{\psetpfj}: \, \xupe = \zupe}
    f_{j}(\vx_{\upsetpfj},\vx_{\setpfj})
    \cdot
    \overline{ \mu_{\efj}^{(0)}(\xe)}
    \cdot
    \prod_{\pe'\in \psetpfj \setminus \pe}
    \overline{ \mu_{\epfj}^{(0)}(x_{e'}) }
    \cdot 
    \overline{ \mu_{\upepfj}^{(0)}(x_{\upe'}) }
    \nonumber\\
    &\overset{(b)}{=}
    \overline{ \bigl( \kappa_{\upefi}^{(1)} \bigr)^{\!-1} } 
    \cdot
    \sum_{\vx_{\psetpfj}: \, \xupe = \zupe}
    f_{j}(\vx_{\upsetpfj},\vx_{\setpfj})
    \cdot
    \mu_{\upefj}^{(0)}(\xe)
    \cdot
    \prod_{\pe'\in \psetpfj \setminus \pe}
    \mu_{\upepfj}^{(0)}(x_{e'})
    \cdot 
    \mu_{\epfj}^{(0)}(x_{\upe'})
    \nonumber\\
    &\overset{(c)}{=}
    \overline{ \bigl( \kappa_{\upefi}^{(1)} \bigr)^{\!-1} } 
    \cdot
    \underbrace{
    \sum_{\vx_{\psetpfj}: \, \xe = \zupe }
    f_{j}(\vx_{\setpfj},\vx_{\upsetpfj})
    \cdot
    \mu_{\upefj}^{(0)}(\xupe)
    \cdot
    \prod_{\pe'\in \psetpfj \setminus \pe}
    \mu_{\upepfj}^{(0)}(x_{\upe'})
    \cdot 
    \mu_{\epfj}^{(0)}(x_{e'})
    }_{ \overset{(d)}{=} \kappa_{\efi}^{(1)} \cdot \mu_{\efi}^{(1)}(\zupe) }
    \nonumber\\
    &\overset{(e)}{=}
    \mu_{\efi}^{(1)}(\zupe), \qquad \ze \in \setxe,\, 
    e=(f_{i}, f_{j}) \in \setEfull,\, \upe=(f_{i}, f_{j}) \in \upsetEfull,
\end{align*}
%------------------------------------------------------------------------
where step $(a)$ follows from the fact that the Choi matrix $ \matr{C}_{f_{j}} $ is a PSD matrix:
%--------------------------------------------------------------------
\begin{align*}
    \overline{ f_{j}( \vx_{\psetpfj} ) } = 
    \overline{ f_{j}( \vx_{\setpfj}, \vx_{\upsetpfj} ) }
    = f_{j}( \vx_{\upsetpfj}, \vx_{\setpfj} ),
\end{align*}
%--------------------------------------------------------------------
where step $(b)$ follows from Item~\ref{sec:DENFG:def:4:item:1} in Definition~\ref{sec:DENFG:def:4}: $ \setxe = \setxupe $ for all $ \pe \in \setEfull $, and the initialization of the messages in step 1 in Definition~\ref{sec:DENFG:def:2}:
%--------------------------------------------------------------------
\begin{align*}
    \mu_{\upef}^{(0)}(\xe) = \overline{ \mu_{\ef}^{(0)}(\xe) },
    \qquad \xe \in \setxe,\, e \in \setpf, \, f \in \setF,
\end{align*}
%--------------------------------------------------------------------
where step $(c)$ follows from the fact that because of $ \setxe = \setxupe $ for all $ \pe \in \setEfull $, switching $ \xe $ and $ \xupe $ keeps the expression on the right-hand side unchanged,
where step $(d)$ follows from the update rule of $ \mu_{\efi}^{(1)} $ in~\eqref{sec:DENFG:eqn:10},
and where step $(e)$ follows from the following facts:
%---------------------------------------------------------------------------
\begin{itemize}
  \item from step $(d)$, the message $ \overline{\mu_{\upefi}^{(1)}(\zupe)} $ is proportional to $ \mu_{\efi}^{(1)}(\zupe) $;

  \item both the messages $ \mu_{\efi}^{(1)} $ and $ \mu_{\upefi}^{(1)} $ are normalized: 
  %-------------------------------------------------------------------
  \begin{align*}
    \sum_{x_{e}} \mu_{\efi}^{(t)}(x_{e})
    = \sum_{x_{\upe}} \mu_{\upefi}^{(t)}(x_{\upe}) 
    = 1.
  \end{align*}
  %-------------------------------------------------------------------
\end{itemize}
%---------------------------------------------------------------------------


==> bounds_for_matrix_permanent.tex <==

In this chapter, we study the degree-$M$ Bethe permanent and degree-$M$ Sinkhorn permanent, whose definitions are motivated by the degree-$M$ finite graph covers of the associated S-NFG, as defined in Section~\ref{sec: snfg for permanent of nonnagtive square matrix}. In particular, in Section~\ref{sec:recursions:coefficients:1}, we present the recursions of the coefficients in expressions of the degree-$M$ Bethe permanent and degree-$M$ Sinkhorn permanent. Based on these recursions, in Section~\ref{sec:5}, we prove the main results in Section~\ref{sec:main:constributions:1}, \ie, we bound the permanent via its degree-$M$ Bethe permanent and degree-$M$ Sinkhorn permanent.
Then in Section~\ref{sec:asymptotic:1}, we gives asymptotic expressions for the coefficients in the degree-$M$ Bethe permanent and degree-$M$ Sinkhorn permanent. Finally, in Section~\ref{apx:22}, we focus on the case where $ M = 2 $ and connects some of the results in this chapter with results in other papers.



\section[Recursions for the Coefficients]{Recursions for \texorpdfstring{the \\
              Coefficients
              $\CM{n}( \vgam )$,
              $\CBM{n}( \vgam )$, 
              $\CscSgen{M}{n}( \vgam )$}{}}
\label{sec:recursions:coefficients:1}

%***************************************************************************

In the first part of this section, we prove Lemma~\ref{lem: expression of
  permanents w.r.t. C}. Afterwards, we prove some lemmas that will help us in
the proofs of Theorems~\ref{thm: inequalities for the coefficients}
and~\ref{th:main:permanent:inequalities:1} in the next section. These latter
lemmas are recursions (in $M$) on the coefficients $\CM{n}( \vgam )$,
$\CBM{n}( \vgam )$, and $\CscSgen{M}{n}( \vgam )$. Note that these recursions
on the coefficients $\CM{n}( \vgam )$, $\CBM{n}( \vgam )$, and
$\CscSgen{M}{n}( \vgam )$ are somewhat analogous to recursions for multinomial
coefficients, in particular also recursions for binomial coefficients like the
well-known recursion  
\begin{align*}
  \binom{M}{k} 
  = \binom{M-1}{k-1} 
  + \binom{M-1}{k}.
\end{align*}
(See also the discussion in
Example~\ref{example:pascal:triangle:generalization:1}).

%***************************************************************************

Throughout this section, the positive integer $n$ and the matrix
$\mtheta \in \sR_{\geq 0}^{n \times n}$ are fixed. Recall the definition of
the notation $\vsigma_{[M]}$ in Definition~\ref{sec:1:def:10}.

%***************************************************************************

\begin{definition}
  \label{sec:1:lem:43}

  Consider $M \in \sZpp $ and $ \vgam \in \Gamma_{M,n} $.
  \begin{enumerate}

  \item The coefficient $ \CM{n}( \vgam ) $ is defined to be the
    number of $ \vsigma_{[M]} $ in $ \setS_{[n]}^{M} $ such that
    $ \vsigma_{[M]} $ decomposes $ \vgam $, \ie,
    \begin{align}
      \CM{n}( \vgam )
        &\defeq
           \sum_{ \vsigma_{[M]} \in \setS_{[n]}^{M} }
             \Bigl[ 
               \vgam = \bigl\langle \mP_{\sigma_{m}} \bigr\rangle_{m \in [M]}
             \Bigr]\, ,
               \label{sec:1:eqn:56}
    \end{align}
    where
    $\bigl\langle \mP_{\sigma_{m}} \bigr\rangle_{m \in [M]} \defeq \frac{1}{M}
    \cdot \sum\limits_{m\in [M]} \mP_{\sigma_{m}}$ and where the notation
    $[S]$ represents the Iverson bracket, \ie, $[S] \defeq 1$ if the statement
    $S$ is true and $[S] \defeq 0$ if the statement is false.
    
  \item The coefficient $ \CBM{n}(\vgam) $ is defined to be
    \begin{align*}
      \CBM{n}(\vgam) 
        &\defeq
           (M!)^{ 2n -  n^2} 
           \cdot
           \prod_{i,j}
             \frac{ \bigl(M - M \cdot \gamma(i,j) \bigr)! }
                  { \bigl(M \cdot \gamma(i,j) \bigr)! } .
        % \label{sec:1:eqn:213}
    \end{align*}
    
  \item The coefficient $ \CscSgen{M}{n}(\vgam) $ is defined to be
    \begin{align*}
      \CscSgen{M}{n}(\vgam)
        &\defeq
           M^{-n\cdot M} 
           \cdot
           \frac{ (M!)^{2n} }
                { \prod_{i,j}
                    \bigl( M \cdot \gamma(i,j) \bigr)! 
                }.
        % \label{sec:1:eqn:214}
    \end{align*}

  \end{enumerate}
  Note that for $M = 1$ it holds that
  \begin{align*}
    \Cgen{1}{n}(\vgam) 
      &= \CBgen{1}{n}(\vgam) 
       = \CscSgen{1}{n}(\vgam) 
       = 1\, ,
           \quad \vgam \in \Gamma_{1,n}.
  \end{align*}
  \edefinition
\end{definition}

%***************************************************************************

We are now in a position to prove Lemma~\ref{lem: expression of permanents
  w.r.t. C} in Section~\ref{sec:main:constributions:1}.

%***************************************************************************

\medskip

\noindent
\textbf{Proof of Lemma~\ref{lem: expression of permanents w.r.t. C}}.
\begin{enumerate}

\item The expression in~\eqref{sec:1:eqn:43} follows from
  \begin{align*}
    \bigl( \perm(\mtheta) \bigr)^{\! M}
      &= \Biggl(
           \sum_{\sigma \in \setS_{[n]}} 
             \prod_{i \in [n]}
               \theta\bigl( i, \sigma(i) \bigr)
         \Biggr)^{\!\!\! M} \\
      &\overset{(a)}{=}
         \sum_{\vgam \in \GamMnthe} 
           \mtheta^{ M \cdot \vgam }
           \cdot
           \CM{n}( \vgam )\, , 
  \end{align*}
  where step~$(a)$ follows from expanding the right-hand side of the first
  line, along with using the Birkhoff--von Neumann theorem and
  Eq.~\eqref{sec:1:eqn:56}.

  While it is clear that $\CM{n}( \vgam ) \geq 0$ for all
    $\vgam \in \GamMnthe$, note that the first inequality
    in~\eqref{sec:1:eqn:58} in Theorem~\ref{thm: inequalities for the
      coefficients} (proven later in this thesis) can be used to show that
    $\CM{n}( \vgam ) > 0$ for all $\vgam \in \GamMnthe$.

\item 

    Eq.~\eqref{sec:1:eqn:190} follows from~\cite[Lemma~29]{Vontobel2013},
    where the role of the set $\set{B}'_M$ in~\cite[Lemma~29]{Vontobel2013} is
    played by the set $\Gamma'_{M,n}(\mtheta)$ in this thesis.

    The set $\Gamma'_{M,n}(\mtheta)$ is defined as follows. Namely, as
    mentioned in Section~\ref{sec:free:energy:functions:1}, the paper
    \cite[Section~IV]{Vontobel2013a} shows that the local marginal polytope of
    $\sfN(\mtheta)$ can be parameterized by the set of doubly stochastic
    matrices, more precisely it can be parameterized by
    $\Gamma_{n}(\mtheta)$. For arbitrary $ M \in \sZ_{\geq 1} $, the set
    $\Gamma'_{M,n}(\mtheta) \subseteq \Gamma_{n}(\mtheta)$ is then defined to
    be the parameterization of the set of pseudo-marginal vectors in the local
    marginal polytope that are $M$-cover lift-realizable pseudo-marginal
    vectors. (For the definition of $M$-cover lift-realizable pseudo-marginal
    vectors, see~\cite[Section~VI]{Vontobel2013}.)

    We claim $\Gamma'_{M,n}(\mtheta) = \Gamma_{M,n}(\mtheta)$. Indeed, it
    follows from the construction of pseudo-marginal vectors based on
    $M$-covers that $\Gamma'_{M,n}(\mtheta) \subseteq \Gamma_{M,n}(\mtheta)$,
    and it follows from the construction in the proof
    of~\cite[Lemma~29]{Vontobel2013} that for every element of
    $\Gamma_{M,n}(\mtheta)$ the corresponding pseudo-marginal vector is
    $M$-cover lift-realizable, \ie,
    $\Gamma'_{M,n}(\mtheta) \supseteq \Gamma_{M,n}(\mtheta)$.

\item Eq.~\eqref{sec:1:eqn:168} follows
  from~\cite[Theorem~2.1]{Friedland1979}.

\elemmaproof

\end{enumerate}

%***************************************************************************

The matrices that are introduced in the following definition will turn out to
be useful to formulate the upcoming results.

%***************************************************************************

\begin{definition}    
  \label{sec:1:def:10:part:2}
  \label{sec:1:def:15}

  Consider a matrix $ \vgam \in \Gamma_n $.
  \begin{enumerate}
    
  \item We define
    \begin{align*}
      \setR 
        &\defeq 
           \setR(\vgam)
         \defeq 
           \bigl\{ 
             i \in [n] 
           \bigm|
             \exists j\in [n], \text{ s.t. } 0 < \gamma(i,j) < 1 
           \bigr\}\, , \\
      \setC
        &\defeq 
           \setC(\vgam)
         \defeq
           \bigl\{ 
             j \in [n]
           \bigm|
             \exists i \in [n], \text{ s.t. } 0 < \gamma(i,j) < 1
           \bigr\}\, ,
    \end{align*}
    \ie, the set $\setR$ consists of the row indices of rows where $\vgam$
    contains at least one fractional entry and, similarly, the set $\setC$
    consists of the column indices of columns where $\vgam$ contains at least
    one fractional entry. Based on $\setR$ and $\setC$, we define
    \begin{align*}
      \vgamRCp 
        &\defeq 
           \bigl( \gamma(i,j) \bigr)_{\! (i,j) \in \setR \times \setC}.
    \end{align*}
    On the other hand, the set $[n] \setminus \setR$ consists of the row
    indices of rows where $\vgam$ contains exactly one $1$ and $0$s
    otherwise. Similarly, the set $[n] \setminus \setC$ consists of the
    column indices of columns where $\vgam$ contains exactly one $1$ and $0$s
    otherwise.
  
  \item We define $ r(\vgam) \defeq |\setR|$. One can verify the
    following statements:
    \begin{itemize}

    \item $|\setR| = |\setC|$.

    \item Either $r(\vgam) = 0$ or $r(\vgam) \geq 2$, \ie,
      $r(\vgam) = 1$ is impossible.

    \item If $r(\vgam) = 0$, then
      $\bigl| \setS_{[n]}(\vgam) \bigr| = 1$.

    \item If $r(\vgam) > 0$, then $\vgamRCp \in \Gamma_{r(\vgam)}$, \ie, the
      matrix $\vgamRCp$ is a doubly stochastic matrix of size
      $r(\vgam) \times r(\vgam)$.

  \end{itemize}

  \item Based on the matrix $\vgamRCp$, we define the matrix
    \begin{align*}
      \hvgamRCp
        &\defeq
           \bigl(
             \hgamRCp(i,j)
           \bigr)_{\! (i,j) \in \setR \times \setC}\, ,
    \end{align*}
    where
    \begin{align*}
      \hgamRCp(i,j)
        &\defeq 
          \frac{\gamRCp(i,j) \cdot \bigl( 1- \gamRCp(i,j) \bigr)}
               {\Biggl(
                  \prod\limits_{(i',j') \in \setR \times \setC} 
                     \bigl( 1 - \gamRCp(i',j') \bigr)
                \Biggr)^{\!\!\! 1 / r(\vgam)}
               }.
    \end{align*}
    Note that the permanent of $ \hvgamRCp $ is given by
    \begin{align}
      \perm(\hvgamRCp)
        &= \sum\limits_{\sigma \in \setS_{\setR\to\setC} }
             \prod_{i \in \setR}
               \frac{\gamRCp\bigl(i,\sigma(i) \bigr) 
                     \cdot
                     \Bigl( 1- \gamRCp\bigl(i,\sigma(i) \bigr) \Bigr)
                    }
                 {\Biggl(
                    \prod\limits_{(i',j') \in \setR \times \setC} 
                       \bigl( 1 - \gamRCp(i',j') \bigr)
                  \Biggr)^{\!\!\! 1 / r(\vgam)}
                 } 
        \nonumber \\
        &= \frac{ 
                  \sum\limits_{\sigma \in \setS_{\setR\to\setC} }
                    \prod\limits_{i \in \setR}
                      \gamRCp\bigl(i,\sigma(i) \bigr)
                      \cdot
                      \Bigl( 1- \gamRCp\bigl(i,\sigma(i) \bigr) \Bigr)
                }
                { 
                  \prod\limits_{i \in \setR,j \in \setC}
                    \bigl( 1- \gamRCp(i,j) \bigr) 
                }.
        \label{eqn: permament of hvgamRCp}
    \end{align}

  \end{enumerate}
  \edefinition
\end{definition}

%***************************************************************************

\begin{example}
  \label{example:vgam:1:1}

  Consider the matrix
  \begin{align*}
    \vgam 
       \defeq
         \frac{1}{3}
         \cdot
         \begin{pmatrix}
           3 & 0 & 0 & 0 \\
           0 & 0 & 3 & 0 \\
           0 & 1 & 0 & 2 \\
           0 & 2 & 0 & 1
         \end{pmatrix}
           \in \Gamma_4.
  \end{align*}
  We obtain $\setR = \{ 3, 4 \}$, $\setC = \{ 2, 4 \}$, $r(\vgam) =
  2$, 
  \begin{align*}
    \vgamRCp
      &= \frac{1}{3}
         \cdot
         \begin{pmatrix}
           1 & 2 \\
           2 & 1
         \end{pmatrix}\, ,
    \qquad
    \hvgamRCp
       = \begin{pmatrix}
           1 & 1 \\
           1 & 1
         \end{pmatrix}\, ,
  \end{align*}
  and $\perm(\hvgamRCp) = 2$.
  \eexample
\end{example}

%***************************************************************************

\begin{definition}    
  \label{sec:1:def:10:part:2:add}

  Consider $M \in \sZ_{\geq 2}$, $ \vgam \in \Gamma_{M,n} $, and
  $ \sigma_1 \in \setS_{[n]}(\vgam) $. (The discussion after
    Definition~\ref{sec:1:def:10} ensures that such a $ \sigma_1 $ exists.)
  We define
  \begin{align*}
    \vgam_{\sigma_1}
      &\defeq
         \frac{1}{M-1} 
         \cdot
         \bigl( M \cdot \vgam - \mP_{\sigma_1} \bigr).
  \end{align*}
  Note that $ \vgam_{\sigma_1} \in \Gamma_{M-1,n} $. 
  The matrix
  $\vgam_{\sigma_1}$ can be thought of, modulo normalizations, as being
  obtained by ``peeling off'' the permutation matrix $\mP_{\sigma_1}$ from
  $\vgam$. 
  \edefinition
\end{definition}



%***************************************************************************

\begin{example}
  \label{example:vgam:1:2}

  Consider again the matrix $\vgam \in \Gamma_4$ that was introduced in
  Example~\ref{example:vgam:1:1}. Let $M = 3$. Note that
  $ \vgam \in \Gamma_{3,4} $. If $\sigma_1 \in \setS_{[n]}(\vgam)$ is chosen
  to be
  \begin{align*}
    \sigma_1(1) = 1\, , \ \ 
    \sigma_1(2) = 3\, , \ \ 
    \sigma_1(3) = 2\, , \ \ 
    \sigma_1(4) = 4\, ,
  \end{align*}
  then
  \begin{align*}
    \vgam_{\sigma_1}
       \defeq
         \frac{1}{2}
         \cdot
         \begin{pmatrix}
           2 & 0 & 0 & 0 \\
           0 & 0 & 2 & 0 \\
           0 & 0 & 0 & 2 \\
           0 & 2 & 0 & 0
         \end{pmatrix}
           \in \Gamma_{2,4}.
  \end{align*}
  On the other hand, if $\sigma_1 \in \setS_{[n]}(\vgam)$ is
  chosen to be
  \begin{align*}
    \sigma_1(1) = 1\, , \ \ 
    \sigma_1(2) = 3\, , \ \ 
    \sigma_1(3) = 4\, , \ \ 
    \sigma_1(4) = 2\, ,
  \end{align*}
  then
  \begin{align*}
    \vgam_{\sigma_1}
       \defeq
         \frac{1}{2}
         \cdot
         \begin{pmatrix}
           2 & 0 & 0 & 0 \\
           0 & 0 & 2 & 0 \\
           0 & 1 & 0 & 1 \\
           0 & 1 & 0 & 1
         \end{pmatrix}
           \in \Gamma_{2,4}.
  \end{align*}
  \eexample
\end{example}

%***************************************************************************

The following three lemmas are the key technical results that will allow us to
prove Theorems~\ref{thm: inequalities for the coefficients}
and~\ref{th:main:permanent:inequalities:1} in the next section.

%***************************************************************************

\begin{lemma}
  \label{sec:1:lem:29:copy:2}
  
  Let $ M \in \sZ_{\geq 2} $ and $ \vgam \in \Gamma_{M,n} $. It holds that
  \begin{align*}
     \CM{n}( \vgam )
        &= \sum_{\sigma_1 \in \setS_{[n]}( \vgam )}
             \Cgen{M-1}{n}\bigl( 
                \vgam_{\sigma_1}
        \bigr).
    \end{align*}
\end{lemma}

%***************************************************************************

\begin{proof}
  If $r(\vgam) = 0$, then $\bigl| \setS_{[n]}( \vgam ) \bigr| = 1$ and
  the result in the lemma statement is straightforward. If
  $r(\vgam) \geq 2$, then the result in the lemma statement follows
  from the fact that all permutations in $ \setS_{[n]}(\vgam) $ are distinct
  and can be used as $ \sigma_1 $ in $ \vsigma_{[M]} $ for decomposing the
  matrix $ \vgam $.
\end{proof}

%***************************************************************************

\begin{lemma}
  \label{sec:1:lem:15:copy:2}
  \label{SEC:1:LEM:15:COPY:2}

  Let $M \in \sZ_{\geq 2}$ and $\vgam \in \Gamma_{M,n}$. Based on $\vgam$, we
  define the set $\setR$, the set $\setC$, and the matrix $\hvgamRCp$
  according to Definition~\ref{sec:1:def:15}. Moreover, for any
  $\sigma_1 \in \setS_{[n]}( \vgam )$, we define $\vgam_{\sigma_1}$ according
  to Definition~\ref{sec:1:def:10:part:2:add}. It holds
  that\footnote{Consider
       the case where both $\setR$ and $\setC$ are non-empty sets. Because each entry
      in $ \hvgamRCp $ is positive-valued, we have $\perm(\hvgamRCp) > 0$, and
      so the fraction $1 / \perm(\hvgamRCp)$ is well defined.}
  \begin{align*}
    \CBM{n}(\vgam)
      &= \frac{1}{\perm(\hvgamRCp)}
         \cdot
         \sum_{\sigma_1 \in \setS_{[n]}( \vgam )}
           \CBgen{M-1}{n}
             \bigl( 
               \vgam_{\sigma_1}
             \bigr)\, ,
  \end{align*}
  where we define $\perm(\hvgamRCp) \defeq 1$ if $\setR$ and $\setC$ are
  empty sets.
\end{lemma}

%***************************************************************************

\begin{proof}
  See Appendix~\ref{app:sec:1:lem:15:copy:2}.
\end{proof}

%***************************************************************************

\begin{lemma}
  \label{sec:1:lem:30}
  \label{SEC:1:LEM:30}
  
  Let $M \in \sZ_{\geq 2}$ and $\vgam \in \Gamma_{M,n}$. For any
  $\sigma_1 \in \setS_{[n]}( \vgam )$, we define $\vgam_{\sigma_1}$ according
  to Definition~\ref{sec:1:def:10:part:2:add}. It holds that\footnote{Note
    that $\vgam \in \Gamma_{M,n}$ and so $\perm(\vgam) \geq n! / n^n$ by van
    der Waerden's inequality. With this, the fraction $1 / \perm(\vgam)$ is
    well defined.}
  \begin{align*}
    \CscSgen{M}{n}(\vgam)
      &\!=\! \frac{1}{
           \bigr( \chi(M) \bigl)^{\! n}
           \, \cdot \,
           \perm(\vgam)
         }
        \cdot \!\!\!
        \sum_{\sigma_1 \in \setS_{[n]}( \vgam )} \!\!\!
          \CscSgen{M-1}{n}( \vgam_{\sigma_1} )\, , 
    % \label{sec:1:eqn:176}
  \end{align*}
  where
  \begin{align*}
    \chi(M)
      &\defeq
         \biggl( \frac{M}{M-1} \biggr)^{\!\! M-1}\, ,
  \end{align*}
  which starts at $\bigl. \chi(M) \bigr|_{M = 2} \! = \! 2$
      and increases to $\bigl. \chi(M) \bigr|_{M \to \infty} \! = \! \e$.
\end{lemma}

%***************************************************************************

\begin{proof}
  See Appendix~\ref{apx:23}.
\end{proof}

%***************************************************************************

All objects and quantities in this thesis assume $M \in \sZ_{\geq
  1}$. Interestingly, it is possible to define these objects and quantities
also for $M = 0$, at least formally. However, we will not do this except in
the following example, as it leads to nicer figures (see
Figs.~\ref{fig:pascal:triangle:generalization:1}%
--\ref{fig:pascal:triangle:generalization:3}).

%***************************************************************************

\begin{example}
  \label{example:pascal:triangle:generalization:1}

  The purpose of this example is to visualize the recursions in
  Lemmas~\ref{sec:1:lem:29:copy:2}--\ref{sec:1:lem:30} for the special case
  $n = 2$, \ie, for matrices $\vgam$ of size $2 \times 2$. For,
  $k_1, k_2 \in \sZ_{\geq 0}$, define\footnote{The case $k_1 = k_2 = 0$ is
    special: the matrix $\vgam^{(0,0)}$ has to be considered as some formal
    matrix and the set $\Gamma_{0,2}$ is defined to be the set containing only
    the matrix $\vgam^{(0,0)}$.}
  \begin{align*}
    \vgam^{(k_1,k_2)}
      &\defeq
         \frac{1}{k_1 + k_2} 
         \cdot
         \begin{pmatrix}
           k_1 & k_2 \\
           k_2 & k_1
         \end{pmatrix}
           \in \Gamma_{k_1+k_2,2}.
             \quad
  \end{align*}
  Define
  \begin{align*}
    \Cgen{0}{n}\bigl( \vgam^{(0,0)} \bigr)
      &\defeq
         1\, , \ 
    \CBgen{0}{n}\bigl( \vgam^{(0,0)} \bigr)
       \defeq
         1\, , \ 
    \CscSgen{0}{n}\bigl( \vgam^{(0,0)} \bigr)
       \defeq
         1.
  \end{align*}
  One can the verify that with these definitions, the recursions in
  Lemmas~\ref{sec:1:lem:29:copy:2}--\ref{sec:1:lem:30} hold also for $M = 1$.

%***************************************************************************

  With these definitions in place, we can draw diagrams that can be seen as
  generalizations of Pascal's triangle,\footnote{These generalizations of
    Pascal's triangle are drawn such that $M$ increases from the bottom to the
    top. This is different from the typical drawings of Pascal's triangle
    (where $M$ increases from the top to the bottom), but matches better the
    convention used in Fig.~\ref{fig:combinatorial:characterization:1} and
    similar figures in~\cite{Vontobel2013} (\ie, \cite[Figs.~7
    and~10]{Vontobel2013}), along with better matching the fact that
    $\permbM{M}(\mtheta)$ is based on \emph{liftings} of~$\mtheta$.} see
  Figs.~\ref{fig:pascal:triangle:generalization:1}%
  --\ref{fig:pascal:triangle:generalization:3}. The meaning of these figures
  is as follows. For example, consider the quantity
  $\Cgen{3}{n}\bigl(\vgam^{(1,2)}\bigr)$. According to
  Lemma~\ref{sec:1:lem:29:copy:2}, this quantity can be obtained via
  \begin{align}
    \Cgen{3}{n}\bigl(\vgam^{(1,2)}\bigr)
      &= 1 
           \cdot
           \Cgen{2}{n}\bigl(\vgam^{(1,1)}\bigr)
         +
         1
           \cdot
           \Cgen{2}{n}\bigl(\vgam^{(0,2)}\bigr) \nonumber \\
      &= 1
           \cdot 2
         +
         1
           \cdot 1 \nonumber \\
      &= 3 .
      \label{eq:CM:recursion:special:case:1}
  \end{align}
  The recursion in~\eqref{eq:CM:recursion:special:case:1} is visualized in
  Fig.~\ref{fig:pascal:triangle:generalization:1} as follows. First, the
  vertex/box above the label ``$\Cgen{3}{n}\bigl(\vgam^{(1,2)}\bigr)$''
  contains the value of $\Cgen{3}{n}\bigl(\vgam^{(1,2)}\bigr)$. Second, the
  arrows indicate that $\Cgen{3}{n}\bigl(\vgam^{(1,2)}\bigr)$ is obtained by
  adding $1$ times $\Cgen{2}{n}\bigl(\vgam^{(1,1)}\bigr)$ and $1$ times
  $\Cgen{3}{n}\bigl(\vgam^{(0,2)}\bigr)$.

  Moreover, notice that the value of $\Cgen{3}{n}\bigl(\vgam^{(1,2)}\bigr)$
  equals the number of directed paths from the vertex labeled
  ``$\Cgen{0}{n}\bigl(\vgam^{(0,0)}\bigr)$'' to the vertex labeled
  ``$\Cgen{3}{n}\bigl(\vgam^{(1,2)}\bigr)$''. In general, for
  $k_1, k_2 \in \sZ_{\geq 0}$, the value of
  $\Cgen{k_1+k_2}{n}\bigl(\vgam^{(k_1,k_2)}\bigr)$ equals the number of
  directed paths from the vertex labeled
  ``$\Cgen{0}{n}\bigl(\vgam^{(0,0)}\bigr)$'' to the vertex labeled
  ``$\Cgen{k_1+k_2}{n}\bigl(\vgam^{(k_1,k_2)}\bigr)$''. In this context,
  recall from
  Proposition~\ref{prop:coefficient:asymptotitic:characterization:1} that
  \begin{align*}
    \Cgen{k_1+k_2}{n}\bigl(\vgam^{(k_1,k_2)}\bigr)
      &\approx
         \exp
           \Bigl(
             (k_1 + k_2) \cdot \HG'\bigl( \vgam^{(k_1,k_2)} \bigr)
           \Bigr)\, ,
  \end{align*}
  where the approximation is up to $o(k_1+k_2)$ in the exponent.

%***************************************************************************

  Similar statements can be made for
  $\CBgen{k_1+k_2}{n}\bigl(\vgam^{(k_1,k_2)}\bigr)$ and
  $\CscSgen{k_1+k_2}{n}\bigl(\vgam^{(k_1,k_2)}\bigr)$ in
  Fig.~\ref{fig:pascal:triangle:generalization:2} and
  Fig.~\ref{fig:pascal:triangle:generalization:3}, respectively. Namely, for
  $k_1, k_2 \in \sZ_{\geq 0}$, the value of
  $\CBgen{k_1+k_2}{n}\bigl(\vgam^{(k_1,k_2)}\bigr)$ equals the sum of weighted
  directed paths from the vertex labeled
  ``$\CBgen{0}{n}\bigl(\vgam^{(0,0)}\bigr)$'' to the vertex labeled
  ``$\CBgen{k_1+k_2}{n}\bigl(\vgam^{(k_1,k_2)}\bigr)$'', and \\
  $\CscSgen{k_1+k_2}{n}\bigl(\vgam^{(k_1,k_2)}\bigr)$ equals the sum of
  weighted directed paths from the vertex labeled
  ``$\CscSgen{0}{n}\bigl(\vgam^{(0,0)}\bigr)$'' to the vertex labeled
  ``$\CscSgen{k_1+k_2}{n}\bigl(\vgam^{(k_1,k_2)}\bigr)$''. (Here, the weight
  of a directed path is given by the product of the weights of the directed
  edges in the path.) In this context, recall from
  Proposition~\ref{prop:coefficient:asymptotitic:characterization:1} that
  \begin{align*}
  \CBgen{k_1+k_2}{n}\bigl(\vgam^{(k_1,k_2)}\bigr)
    &\approx
       \exp
         \Bigl(
           (k_1+k_2) \cdot \HBthe\bigl( \vgam^{(k_1,k_2)} \bigr)
         \Bigr)\, , \\
  \CscSgen{k_1+k_2}{n}\bigl(\vgam^{(k_1,k_2)}\bigr)
    &\approx
       \exp
         \Bigl(
           (k_1+k_2) \cdot \HscSthe\bigl( \vgam^{(k_1,k_2)} \bigr)
         \Bigr)\, ,
  \end{align*}
  where the approximation is up to $o(k_1+k_2)$ in the exponent.
  \eexample
\end{example}

%***************************************************************************

\begin{figure}
  \begin{center}
    \input{figures/pascal_triangle1_1.tex}
    \vspace{-0.3cm}
    % \medskip
    \caption{Generalization of Pascal's triangle visualizing the recursion in
      Lemma~\ref{sec:1:lem:29:copy:2}.}
    \label{fig:pascal:triangle:generalization:1}

    \vspace{0.7cm}

    \input{figures/pascal_triangle2_1.tex}
    % \medskip
    \vspace{-0.3cm}
    \caption{Generalization of Pascal's triangle visualizing the recursion in
      Lemma~\ref{sec:1:lem:15:copy:2}.}
    % \medskip
    \label{fig:pascal:triangle:generalization:2}
  
    \vspace{0.7cm}
%   \end{center}
% \end{figure}

% \begin{figure}
%   \centering
  \input{figures/pascal_triangle3_1.tex}
  % \medskip
  \vspace{-0.3cm}
  \caption{Generalization of Pascal's triangle visualizing the recursion in
    Lemma~\ref{sec:1:lem:30}.}
  % \medskip
  \label{fig:pascal:triangle:generalization:3}
  \end{center}
\end{figure}

%***************************************************************************

In the context of Example~\ref{example:pascal:triangle:generalization:1}, note
that for $n = 2$ the matrix
$\matr{1}_{2 \times 2} \defeq \bigl( \begin{smallmatrix} 1 & 1 \\ 1 &
  1 \end{smallmatrix} \bigr)$ achieves the upper bound $2^{n/2} = 2$
in~\eqref{eq:ratio:permanent:bethe:permanent:1}, and with that the matrix
$\matr{1}_{2 \times 2}$ is the ``worst-case matrix'' for $n = 2$ in the sense
that the ratio $\frac{\perm(\mtheta)}{\permb(\mtheta)} = 2$ for
$\mtheta = \matr{1}_{2 \times 2}$ is the furthest away from the ratio
$\frac{\perm(\mtheta)}{\permb(\mtheta)} = 1$ for diagonal
matrices~$\mtheta$. However, this behavior of the all-one matrix for $n = 2$
is atypical. Namely, letting $\matr{1}_{n \times n}$ be the all-one matrix for
$n \in \sZ_{\geq 1}$, one obtains, according to
\cite[Lemma~48]{Vontobel2013a},
\begin{align*}
  \left.
    \frac{\perm(\mtheta)}{\permb(\mtheta)}
  \right|_{\mtheta = \matr{1}_{n \times n}}
    &= \sqrt{\frac{2 \pi n}{\e}}
       \cdot
       \bigl( 1 + o_n(1) \bigr)\, ,
\end{align*}
\ie, the ratio
$\frac{\perm(\matr{1}_{n \times n})}{\permb(\matr{1}_{n \times n})}$ is much
closer to $1$ than to $2^{n/2}$ for large values of $n$. (In the above
expression, the term $o_n(\ldots)$ is based on the usual little-o notation for
a function in $n$.)

%***************************************************************************

In the case of the scaled Sinkhorn permanent, the ``worst-case matrix'' is
given by the all-one matrix not just for $n = 2$, but for all
$n \in \sZ_{\geq 2}$, \ie, the ratio
$\frac{\perm(\mtheta)}{\permscs(\mtheta)} = \e^n \cdot \frac{n!}{n^n}$ for
$\mtheta = \matr{1}_{n \times n}$ is the furthest away from the value of the
ratio $\frac{\perm(\mtheta)}{\permscs(\mtheta)} = \e^n$ for diagonal matrices
$\mtheta$ for all $n \in \sZ_{\geq 2}$.

%***************************************************************************
%***************************************************************************

\ifx\withclearpagecommands\x
\clearpage
\fi

\section{Bounding the Permanent of \texorpdfstring{$\mtheta$}{}}
\label{sec:5}

%***************************************************************************
%***************************************************************************

In this section, we first prove Theorem~\ref{thm: inequalities for the
  coefficients} with the help of Lemmas~\ref{sec:1:lem:15:copy:2}
and~\ref{sec:1:lem:30}, where, in order for Lemmas~\ref{sec:1:lem:15:copy:2}
and~\ref{sec:1:lem:30} to be useful, we need to find lower and upper bounds on
$\perm(\hvgamRCp)$ and on $\perm(\vgam)$, respectively. Afterwards, we use
Theorem~\ref{thm: inequalities for the coefficients} to prove
Theorem~\ref{th:main:permanent:inequalities:1}.

%***************************************************************************
%***************************************************************************

\subsection{\texorpdfstring{Bounding the ratio $\perm(\mtheta) /  
                                                                                     \permbM{M}(\mtheta)$}{}}

%***************************************************************************

In this subsection, we first prove the inequalities in~\eqref{sec:1:eqn:58} in
Theorem~\ref{thm: inequalities for the coefficients} that give bounds on the
ratio $\CM{n}(\vgam) / \CBM{n}(\vgam)$. Then, based on these bounds, we prove
the inequalities in~\eqref{SEC:1:EQN:147} in
Theorem~\ref{th:main:permanent:inequalities:1} that give bounds on the ratio
$\perm(\mtheta) / \permbM{M}(\mtheta)$.

%***************************************************************************

\begin{lemma}
  \label{sec:1:lem:17}

  Consider the setup in Lemma~\ref{sec:1:lem:15:copy:2}. The matrix
  $\hvgamRCp$ satisfies
  \begin{align}
    1
      &\leq  
         \perm(\hvgamRCp)
       \leq
         2^{n/2}.
           \label{sec:1:eqn:145}
  \end{align}
\end{lemma}

%***************************************************************************

\begin{proof}
  It is helpful to first prove that $\permb(\hvgamRCp) = 1$. Indeed,
  \begin{align*}
    \permb(\hvgamRCp)
      &\overset{(a)}{=} 
         \exp
           \biggl(
             - \min_{\vgam \in \Gamma_{|\setR|}(\hvgamRCp)}
                 F_{\mathrm{B},\hvgamRCp}( \vgam )
           \biggr) \\
      &\overset{(b)}{=}
         \exp\bigl( - F_{\mathrm{B},\hvgamRCp}( \vgamRCp ) \bigr) \\
      &\overset{(c)}{=} \exp(0) \\
      &= 1\, ,
  \end{align*}
  where step~$(a)$ follows from the definition of the Bethe permanent in
  Definition~\ref{sec:1:def:16}, where step~$(b)$ follows from the convexity
  of the minimization problem
  $\min_{\vgam \in \Gamma_{|\setR|}(\hvgamRCp)} F_{\mathrm{B},\hvgamRCp}(
  \vgam )$ (which was proven in~\cite{Vontobel2013a}) and from studying the
  KKT conditions for this minimization problem at $\vgam = \vgamRCp$ (the
  details are omitted), and where step~$(c)$ follows from simplifying the
  expression for $F_{\mathrm{B},\hvgamRCp}( \vgamRCp )$.

  With this, the first inequality in~\eqref{sec:1:eqn:145} follows from
  \begin{align*}
    1
      &= \permb(\hvgamRCp)
       \overset{(a)}{\leq}
         \perm(\hvgamRCp)\, ,
  \end{align*}
  where step~$(a)$ follows from the first inequality
  in~\eqref{eq:ratio:permanent:bethe:permanent:1}, and the second inequality
  in~\eqref{sec:1:eqn:145} follows from
  \begin{align*}
    \perm(\hvgamRCp) 
      &\overset{(b)}{\leq}
         \underbrace
         {
           2^{|\setR|/2}
         }_{\leq \ 2^{n/2}} 
         \cdot
         \underbrace{
           \permb(\hvgamRCp)
         }_{= \ 1}
       \leq 
         2^{n/2}\, ,
  \end{align*}
  where step~$(b)$ follows from the second inequality
  in~\eqref{eq:ratio:permanent:bethe:permanent:1}.

  An alternative proof of the first inequality in~\eqref{sec:1:eqn:145} goes
  as follows. Namely, this inequality can be obtained by 
  combining~\eqref{eqn: permament of hvgamRCp} and
  \begin{align*}
    \hspace{4cm}&\hspace{-4cm}
    \sum_{\sigma \in \setS_{\setR \to \setC}}
      \prod_{i \in \setR} 
        \gamRCp\bigl(i,\sigma(i)\bigr)
        \cdot 
        \Bigl( 1 \! - \! \gamRCp\bigl(i,\sigma(i) \bigr) \Bigr) 
      \overset{(a)}{\geq}
         \!\! \prod_{(i,j) \in \setR \times \setC} \!\!
           \bigl( 1 \! - \! \gamRCp(i,j) \bigr)\, ,
  \end{align*}
  where step~$(a)$ follows from~\cite[Corollary~1c of
  Theorem~1]{Schrijver1998}. Note that this alternative proof for the first
  inequality in~\eqref{sec:1:eqn:145} is not really that different from the
  above proof because the first inequality
  in~\eqref{eq:ratio:permanent:bethe:permanent:1} is also based
  on~\cite[Corollary~1c of Theorem~1]{Schrijver1998}
\end{proof}

%***************************************************************************

\noindent
\textbf{Proof of the inequalities in~\eqref{sec:1:eqn:58} in Theorem~\ref{thm:
    inequalities for the coefficients}}.
\begin{itemize}

\item We prove the first inequality in~\eqref{sec:1:eqn:58} by induction on
  $M$. The base case is $M = 1$. From Definition~\ref{sec:1:lem:43}, it
  follows that $\CM{n}(\vgam) = \CBM{n}(\vgam) = 1$ for
  $\vgam \in \Gamma_{M,n}$ and so
  \begin{align*}
    \frac{\CM{n}(\vgam)}
         {\CBM{n}(\vgam)}
      &\geq 1\, ,
         \quad \vgam \in \Gamma_{M,n}\, ,
  \end{align*}
  is indeed satisfied for $M = 1$.

  Consider now an arbitrary $M \in \sZ_{\geq 2}$. By the induction hypothesis,
  we have
  \begin{align}
    \frac{ \Cgen{M-1}{n}(\vgam) }{\CBgen{M-1}{n}(\vgam) }
      &\geq 
        1\, , \qquad \vgam \in \Gamma_{M-1,n}.
    \label{eqn: ineq. used in induction hypothesis w.r.t. cbm}
  \end{align}
  Then we obtain
  \begin{align*}
    \CM{n}( \vgam )
    &\overset{(a)}{=} \sum_{\sigma_1 \in \setS_{[n]}( \vgam )}
         \Cgen{M-1}{n}\bigl( 
            \vgam_{\sigma_1}
    \bigr) 
    \nonumber \\
    &\overset{(b)}{\geq}
    \sum_{\sigma_1 \in \setS_{[n]}( \vgam )}
         \CBgen{M-1}{n}\bigl( 
            \vgam_{\sigma_1}
    \bigr)
    \nonumber \\ 
    &\overset{(c)}{=} \perm(\hvgamRCp) \cdot \CBM{n}(\vgam)
    \nonumber \\
    &\overset{(d)}{\geq} \CBM{n}(\vgam)\, ,
\end{align*}
where step~$(a)$ follows from Lemma~\ref{sec:1:lem:29:copy:2}, where step
$(b)$ follows from the induction hypothesis in~\eqref{eqn: ineq. used in
  induction hypothesis w.r.t. cbm}, where step~$(c)$ follows from
Lemma~\ref{sec:1:lem:15:copy:2}, and where step~$(d)$ follows from
Lemma~\ref{sec:1:lem:17}. 

\item A similar line of reasoning can be used to prove the second inequality
  in~\eqref{sec:1:eqn:58}; the details are omitted.

\end{itemize}
\etheoremproof

%***************************************************************************

\medskip

\noindent
\textbf{Proof of the inequalities in~\eqref{SEC:1:EQN:147} in
  Theorem~\ref{th:main:permanent:inequalities:1}}.
\begin{itemize}

\item We prove the first inequality in~\eqref{SEC:1:EQN:147} by observing that
  \begin{align*}
    \bigl( \perm(\mtheta) \bigr)^{\!M}
      &\overset{(a)}{=} 
         \sum_{\vgam \in \GamMnthe} 
           \mtheta^{ M \cdot \vgam }
           \cdot
           \CM{n}( \vgam )
             \nonumber \\
      &\overset{(b)}{\geq}
         \sum_{\vgam \in \GamMnthe} 
           \mtheta^{ M \cdot \vgam }
           \cdot
           \CBM{n}( \vgam )
             \nonumber \\
      &\overset{(c)}{=}
         \bigl( \permbM{M}(\mtheta) \bigr)^{\!M}\, ,
  \end{align*}
  where step~$(a)$ follows from~\eqref{sec:1:eqn:43}, where step~$(b)$ follows
  from the first inequality in~\eqref{sec:1:eqn:58}, and where step~$(c)$
  follows from~\eqref{sec:1:eqn:190}. The desired inequality is then obtained
  by taking the $M$-th root on both sides of the expression.

\item A similar line of reasoning can be used to prove the second inequality
  in~\eqref{SEC:1:EQN:147}; the details are omitted.

\end{itemize}
\etheoremproof

%***************************************************************************

\medskip

The expression in the following lemma can be used to obtain a slightly
alternative proof of the inequalities in~\eqref{SEC:1:EQN:147} in
Theorem~\ref{th:main:permanent:inequalities:1}. However, this result is also
of interest in itself.

%***************************************************************************

\begin{lemma}
  \label{lemma:ratio:perm:permbM:1}
  \label{LEMMA:RATIO:PERM:PERMBM:1}
  Let $\pmtheta$ be the probability mass function on $\setS_{[n]}$ induced
  by~$\mtheta$ (see Definition~\ref{sec:1:def:10}). It holds that
  \begin{align}
    \frac{\perm(\mtheta)}
         {\permbM{M}(\mtheta)} &= \left( \!
           \sum_{ \vsigma_{[M]} \in \setS_{[n]}^{M} }
             \left(
               \prod_{m \in [M]} \!\!
                 \pmtheta(\sigma_m)
             \right)
             \! \cdot \!
             \frac{\CBM{n}
                     \Bigl(
                       \bigl\langle \mP_{\sigma_{m}} \bigr\rangle_{m \in [M]}
                     \Bigr)}
                  {\CM{n}
                     \Bigl(
                       \bigl\langle \mP_{\sigma_{m}} \bigr\rangle_{m \in [M]}
                     \Bigr)}
         \right)^{\!\!\! -1/M} \!\! .
           \label{eq:ratio:perm:permbM:1}
  \end{align}
  Note that from the first inequality in~\eqref{sec:1:eqn:58}
    in Theorem~\ref{thm: inequalities for the coefficients} it follows that
    $ \CM{n}(\vgam) \geq \CBM{n}(\vgam) > 0 $ for all $ \vgam \in \GamMn $,
    \ie, the ratio appearing in~\eqref{eq:ratio:perm:permbM:1} is well
    defined.
\end{lemma}

%***************************************************************************

\begin{proof}
  See Appendix~\ref{app:proof:lemma:ratio:perm:permbM:1}.
\end{proof}

Based on Lemma~\ref{lemma:ratio:perm:permbM:1}, we  
give an alternative proof of the inequalities in~\eqref{SEC:1:EQN:147} in
  Theorem~\ref{th:main:permanent:inequalities:1} in Appendix~\ref{apx: alternative proof of perm geq permb}.
%***************************************************************************

%***************************************************************************
Note that the first inequality in~\eqref{SEC:1:EQN:147} is tight. Indeed,
choosing the matrix $\mtheta$ to be diagonal with strictly positive diagonal
entries shows that 
\begin{align*}
  \frac{\perm(\mtheta)}{\permbM{M}(\mtheta)} = 1
\end{align*}
for any
$M \in \sZpp$. Furthermore,
\begin{align*}
  \frac{ \perm(\mtheta) }{\permb(\mtheta)} = 
  \liminf_{M \to \infty} \frac{ \perm(\mtheta) }{\permbM{M}(\mtheta)}
  = 1.
\end{align*}

%***************************************************************************

On the other hand, the second inequality in~\eqref{SEC:1:EQN:147} is
\emph{not} tight for finite $M \geq 2$. Indeed, for this inequality to be
tight, all the inequalities
in~\eqref{eq:ratio:perm:permbM:proof:upper:bound:1} in Appendix~\ref{app:proof:lemma:ratio:perm:permbM:1} need to be tight. In
particular, the inequality in step~$(a)$ needs to be tight, which means that
for all $\vsigma_{[M]} \in \setS_{[n]}^{M}$ with
$\prod_{m \in [M]} \pmtheta(\sigma_m) > 0$, it needs to hold that
$\CBM{n}(\ldots) / \CM{n}(\ldots) = (2^{n/2})^{-(M-1)}$. However, this is not
the case for $\vsigma_{[M]} = (\sigma, \ldots, \sigma)$ with
$\sigma \in \setS_{[n]}(\vtheta)$, for which it holds that
$\CBM{n}(\ldots) / \CM{n}(\ldots) = 1$.

%***************************************************************************

Observe that the non-tightness of the second inequality
in~\eqref{SEC:1:EQN:147} for finite $M \geq 2$ is in contrast to the case
$M \to \infty$, where it is known that for
\begin{align*}
  \mtheta = \matr{I}_{(n/2) \times (n/2)} \otimes \bigl( \begin{smallmatrix} 1
  & 1 \\ 1 & 1 \end{smallmatrix} \bigr),
\end{align*}
it holds that
 \begin{align*}
    \frac{\perm(\mtheta)}{ \permb(\mtheta)} 
    = \liminf_{M \to \infty} 
    \frac{\perm(\mtheta)}{\permbM{M}(\mtheta)}
    = 2^{n/2}.
 \end{align*}
 (Here, $n$ is assumed to be even and
$\matr{I}_{(n/2) \times (n/2)}$ is defined to be the identity matrix of size
$(n/2) \times (n/2)$.)

%***************************************************************************

\vspace{0.2 cm}

\noindent
We also give another alternative proof of the inequalities in~\eqref{SEC:1:EQN:147} in
  Theorem~\ref{th:main:permanent:inequalities:1} in Appendix~\ref{apx: alternative prooof of perm geq permb: 2}.
In particular, Lemma~\ref{prop: a special case of Navin conjecture} proven in Appendix~\ref{apx: alternative prooof of perm geq permb: 2} proves the $M_{1}= 1$ case of the following conjecture.
\begin{conjecture}\label{Navin conjecture}
  For any integers $ M_{1} \in \sZpp $ and $ M_{2} \in \sZpp $, it holds that
  \begin{align*}
    \frac{ \bigl( \permbM{M_{1}}(\mtheta) \bigr)^{\! M_{1}} \cdot
    \bigl( \permbM{M_{2}}(\mtheta) \bigr)^{\! M_{2}}
    }{ \bigl( \permbM{M_{1} + M_{2}}(\mtheta) \bigr)^{\! M_{1} + M_{2}}}
    \geq 1.
  \end{align*}
  \econjecture
\end{conjecture}
A useful consequence of Conjecture~\ref{Navin conjecture} is that
\begin{align*}
  \lim_{M \to \infty} 
  \permbM{M}(\mtheta) 
  = \limsup_{M \to \infty} 
  \permbM{M}(\mtheta) 
  =
  \permb(\mtheta)\, ,
\end{align*}
where the first equality follows from Conjecture~\ref{Navin conjecture} and Fekete’s lemma~\cite{Fekete1923} (see, \eg,~\cite[Lemma 11.6]{Lint2001}), and where the second equality follows from~\cite[Theorem 39]{Vontobel2013a}.

%***************************************************************************
%***************************************************************************

\subsection{\texorpdfstring{Bounding the ratio $\perm(\mtheta) /  
                                                                                     \permscsM{M}(\mtheta)$}{}}

%***************************************************************************

In this subsection, we first prove the inequalities in~\eqref{sec:1:eqn:180}
in Theorem~\ref{thm: inequalities for the coefficients} that give bounds on
the ratio $\CM{n}(\vgam) / \CscSgen{M}{n}(\vgam)$. Then, based on these
bounds, we prove the inequalities in~\eqref{sec:1:eqn:200} in
Theorem~\ref{th:main:permanent:inequalities:1} that give bounds on the ratio
$\perm(\mtheta) / \permscsM{M}(\mtheta)$.

%***************************************************************************

\begin{lemma}
  \label{sec:1:lem:36}

  Consider the setup in Lemma~\ref{sec:1:lem:30}. The matrix $\vgam$ satisfies
  \begin{align*}
    \frac{n!}{n^{n}}
      &\leq 
         \perm(\vgam)
       \leq 1.
  \end{align*}
\end{lemma}

%***************************************************************************

\begin{proof}
  The lower bound follows from van der Waerden's inequality proven
  in~\cite[Theorem 1]{Egorychev1981} and~\cite[Theorem 1]{Falikman1981}. The
  upper bound follows from
  \begin{align*}
    \perm(\vgam) 
      &\overset{(a)}{\leq }
         \prod_{i} 
           \Biggl( \sum_{j} \gamma(i,j) \Biggr)
       = 
         \prod_{i} 
           1
       = 1\, ,
  \end{align*}
  where step~$(a)$ follows from the observation that $\perm(\vgam)$ contains a
  subset of the (non-negative) terms in
  $\prod_{i} \bigl( \sum_{j} \gamma(i,j) \bigr)$.
\end{proof}

%***************************************************************************

\noindent
\textbf{Proof of the inequalities in~\eqref{sec:1:eqn:180} in Theorem~\ref{thm:
    inequalities for the coefficients}}.
\begin{itemize}

\item We prove the first inequality in~\eqref{sec:1:eqn:180} by induction on
  $M$. The base case is $M = 1$. From Definition~\ref{sec:1:lem:43}, it
  follows that $\CM{n}(\vgam) = \CscSgen{M}{n}(\vgam) = 1$ for all
  $\vgam \in \Gamma_{M,n}$ and so
  \begin{align*}
    \frac{\CM{n}(\vgam)}
         {\CscSgen{M}{n}(\vgam)}
      &\geq
         1\, , 
           \qquad \vgam \in \Gamma_{M,n}.
  \end{align*}
  (Note that when $M = 1$, then the first inequality in~\eqref{sec:1:eqn:180}
  simplifies to $1$.)

  Consider now an arbitrary $ M \in \sZ_{\geq 2} $. By the induction
  hypothesis, we have
  \begin{align}
    \frac{\Cgen{M-1}{n}(\vgam)}
         {\CscSgen{M-1}{n}(\vgam)} 
      &\! \geq \!
         \Biggl( \!
           \frac{(M \! - \! 1)^{M-1}}
                {(M \! - \! 1)!} \!
         \Biggr)^{\!\!\! n} \!\!
         \cdot \!
         \biggl(
           \frac{ n! }
                { n^{n} }
         \biggr)^{\!\! M-2} \!\!\!\! ,
           \qquad \vgam \in \Gamma_{M-1,n}.
    \label{eqn: ineq. used in induction hypothesis w.r.t. cscsm}
  \end{align}
  Then we obtain
  \begin{align*}
    \CM{n}( \vgam ) 
    &\overset{(a)}{=}
       \sum_{\sigma_1 \in \setS_{[n]}( \vgam )}
         \Cgen{M-1}{n}
           \bigl( 
             \vgam_{\sigma_1}
           \bigr) 
             \nonumber \\
    &\overset{(b)}{\geq}
       \biggl( \frac{(M \! - \! 1)^{M-1}}{(M \! - \! 1)!} \biggr)^{\!\! n}
       \cdot
       \biggl(
         \frac{ n! }{ n^{n} }
       \biggr)^{\!\! M-2} 
       \!\!\!\!\!\!
       \cdot
       \sum_{\sigma_1 \in \setS_{[n]}( \vgam )} \!\!
         \CscSgen{M-1}{n}(\vgam_{\sigma_1})
           \nonumber \\ 
    &\overset{(c)}{=} 
       \biggl( \frac{M^{M}}{M!} \biggr)^{\!\! n}
       \cdot
       \biggl(
         \frac{ n! }{ n^{n} }
       \biggr)^{\!\! M-2} 
       \cdot
       \perm(\vgam)
       \cdot
       \CscSgen{M}{n}(\vgam)
         \nonumber \\
    &\overset{(d)}{\geq}
       \biggl( \frac{M^{M}}{M!} \biggr)^{\!\! n}
       \cdot
       \biggl(
         \frac{ n! }{ n^{n} }
       \biggr)^{\!\! M-1} 
       \cdot 
       \CscSgen{M}{n}(\vgam)\, ,
  \end{align*}
  where step~$(a)$ follows from Lemma~\ref{sec:1:lem:29:copy:2}, where step
  $(b)$ follows from the induction hypothesis 
  in~\eqref{eqn: ineq. used in induction hypothesis w.r.t. cscsm}, 
  where step~$(c)$ follows from
  Lemma~\ref{sec:1:lem:30}, and where step~$(d)$ follows from
  Lemma~\ref{sec:1:lem:36}.

\item A similar line of reasoning can be used to prove the second inequality
  in~\eqref{sec:1:eqn:180}; the details are omitted.

\end{itemize}
\etheoremproof

%***************************************************************************

\medskip

\noindent
\textbf{Proof of the inequalities in~\eqref{sec:1:eqn:200} in
  Theorem~\ref{th:main:permanent:inequalities:1}}.
\begin{itemize}

\item We prove the first inequality in~\eqref{sec:1:eqn:200} by observing that
  \begin{align*}
    \bigl( \perm(\mtheta) \bigr)^{\!M} 
      &\overset{(a)}{=}
         \sum_{\vgam \in \GamMnthe} 
           \mtheta^{ M \cdot \vgam }
         \cdot
         \CM{n}( \vgam )
           \nonumber \\
      &\overset{(b)}{\geq} 
         \biggl( \frac{M^{M}}{M!} \biggr)^{\!\! n}
         \cdot
         \biggl(
           \frac{ n! }{ n^{n} }
         \biggr)^{\!\! M-1} 
         \! \cdot \!\!\!\!\!
         \sum_{\vgam \in \GamMnthe} 
           \mtheta^{ M \cdot \vgam }
         \cdot
         \CscSgen{M}{n}( \vgam )
          \nonumber \\
      &\overset{(c)}{=} 
         \biggl( \frac{M^{M}}{M!} \biggl)^{\!\! n}
         \cdot
         \biggl(
           \frac{ n! }{ n^{n} }
         \biggl)^{\!\! M-1} 
         \cdot 
         \bigl( \permscsM{M}(\mtheta) \bigr)^{\!M}\, ,
  \end{align*}
  where step~$(a)$ follows from~\eqref{sec:1:eqn:43}, where step~$(b)$ follows
  from the first inequality in~\eqref{sec:1:eqn:180}, and where step~$(c)$
  follows from~\eqref{sec:1:eqn:168}. The desired inequality is then obtained
  by taking the $M$-th root on both sides of the expression.

\item A similar line of reasoning can be used to prove the second inequality
  in~\eqref{sec:1:eqn:200}; the details are omitted.

\etheoremproof
\end{itemize}

%***************************************************************************

The expression in the following lemma can be used to obtain a slightly
alternative proof of the inequalities in~\eqref{sec:1:eqn:200} in
Theorem~\ref{th:main:permanent:inequalities:1}. However, this result is also
of interest in itself.

%***************************************************************************

\begin{lemma}
  \label{lemma:ratio:perm:permscM:1}

  Let $\pmtheta$ be the probability mass function on $\setS_{[n]}$ induced
  by~$\mtheta$ (see Definition~\ref{sec:1:def:10}). It holds that
  \begin{align*}
    \frac{\perm(\mtheta)}
         {\permscsM{M}(\mtheta)} 
      &= \left( \!
           \sum_{ \vsigma_{[M]} \in \setS_{[n]}^{M} } \!
             \Biggl(
               \prod_{m \in [M]} \!\!\!
                 \pmtheta(\sigma_m)
             \Biggr)
             \!\! \cdot \!
             \frac{\CscSgen{M}{n}
                     \Bigl(
                       \bigl\langle \mP_{\sigma_{m}} \bigr\rangle_{m \in [M]}
                     \Bigr)}
                  {\CM{n}
                     \Bigl(
                       \bigl\langle \mP_{\sigma_{m}} \bigr\rangle_{m \in [M]}
                     \Bigr)} \!
         \right)^{\!\!\! -1/M} \!\! .
         % \label{eq:ratio:perm:permscM:1}
  \end{align*}
\end{lemma}

%***************************************************************************

\begin{proof}
  The proof of this statement is analogous to the proof of
  Lemma~\ref{lemma:ratio:perm:permbM:1} in
  Appendix~\ref{app:proof:lemma:ratio:perm:permbM:1}; one simply has to
  replace $\permbM{M}(\mtheta)$ and $\CBM{n}(\ldots)$ by
  $\permscsM{M}(\mtheta)$ and $\CscSgen{M}{n}(\ldots)$, respectively.
\end{proof}

%***************************************************************************

\noindent
\textbf{Alternative proof of the inequalities in~\eqref{sec:1:eqn:200} in
  Theorem~\ref{th:main:permanent:inequalities:1}}.

\noindent
Based on Lemma~\ref{lemma:ratio:perm:permscM:1}, an alternative proof of the
inequalities in~\eqref{sec:1:eqn:200} can be given that is very similar to the
alternative proof presented
in Appendix~\ref{apx: alternative proof of perm geq permb}; 
the details are omitted.
\etheoremproof

%***************************************************************************

\medskip

Note that the second inequality in~\eqref{sec:1:eqn:200} is tight. Indeed,
choosing the matrix $\mtheta$ to be diagonal with strictly positive diagonal
entries shows that
\begin{align*}
  \frac{ \perm(\mtheta) }{ \permscsM{M}(\mtheta) }
  = \frac{M^{n}}{(M!)^{n/M}}, \qquad M \in \sZpp.
\end{align*}
Furthermore,
\begin{align*}
  \frac{ \perm(\mtheta) }{\permscs(\mtheta)} 
  = \liminf_{M \to \infty} \frac{ \perm(\mtheta) }{ \permscsM{M}(\mtheta) }
  = \e^n.
\end{align*}

%***************************************************************************

On the other hand, the first inequality in~\eqref{sec:1:eqn:200} is \emph{not}
tight for finite $M \geq 2$. (The proof is similar to the proof of the
non-tightness of the second inequality in~\eqref{SEC:1:EQN:147} for finite
$M \geq 2$.) This is in contrast to the case $M \to \infty$, where it is known
that for $\mtheta$ being equal to the all-one matrix of size $n \times n$ it
holds that
\begin{align*}
  \frac{ \perm(\mtheta) }{ \permscs(\mtheta) } 
  = \liminf_{M \to \infty} 
  \frac{ \perm(\mtheta) }{ \permscsM{M}(\mtheta) }
  = \e^n \cdot \frac{n!}{n^n}.
\end{align*}

%***************************************************************************
%***************************************************************************

\ifx\withclearpagecommands\x
\clearpage
\fi

\section[Asymptotic Expressions for the 
              Coefficients]{Asymptotic Expressions for the 
              Coefficients \texorpdfstring{$\CM{n}( \vgam )$, 
                                   $\CBM{n}( \vgam )$, $\CscSgen{M}{n}( \vgam )$}{}}
\label{sec:asymptotic:1}

%***************************************************************************

In this section, we prove
Proposition~\ref{prop:coefficient:asymptotitic:characterization:1}. Whereas
Definitions~\ref{sec:1:def:18:part:2}, \ref{sec:1:def:16},
and~\ref{sec:1:def:20} give an analytical definition of the entropy functions
$\HG'$, $ \HBthe $, and $ \HscSthe $, the expressions in
Eqs.~\eqref{sec:1:eqn:125}--\eqref{sec:1:eqn:207} in
Proposition~\ref{prop:coefficient:asymptotitic:characterization:1} give a
combinatorial characterization of these entropy functions. The proof of
Proposition~\ref{prop:coefficient:asymptotitic:characterization:1} is based on
standard results of the method of types and considerations that are similar to
the considerations in~\cite[Sections~IV and~VII]{Vontobel2013}. 


%***************************************************************************

% Throughout this section, the positive integer $n$ and the matrix
% $\mtheta \in \sR_{\geq 0}^{n \times n}$ are fixed. In fact, the matrix
% $\mtheta$ is not really needed in this section, and so, for simplicity, we
% assume that the set $\setA(\mtheta)$ (see Definition~\ref{sec:1:def:5}) is the
% largest possible set for any $\mtheta \in \sR_{\geq 0}^{n \times n}$, \ie,
% $\setA(\mtheta) = \setP_{[n]}$, where $\setP_{[n]}$ is the set of
% permutation matrices of size $n \times n$.

%***************************************************************************
\begin{definition}
  \label{sec:1:def:17}

  Fix some $ M \in \sZpp $ and $ \vgam \in \Gamma_{n} $. 
  Recall the definition of the notations
  $\vsigma_{[M]}$ and $\mP_{\vsigma_{[M]}}$ in
  Definition~\ref{sec:1:def:10}. We define the following objects.
  \begin{enumerate}

  \item Let $\mP_{\vsigma_{[M]}} \in \setA(\vgam)^{M}$. The type of
    $ \mP_{\vsigma_{[M]}} $ is defined to be
    \begin{align*}
      \bm{t}_{\mP_{\vsigma_{[M]}}}
        &\defeq 
           \bigl(
             t_{ \mP_{\vsigma_{[M]}} }( \mP_{\sigma} ) 
          \bigr)_{ \! \mP_{\sigma} \in \setA(\vgam) }
           \in \PiA{\vgam}\, ,
    \end{align*}
    where
    \begin{align*}
      t_{\mP_{\vsigma_{[M]}}}( \mP_{\sigma} )
        &\defeq
           \frac{1}{M} 
           \cdot 
           \Bigl| 
             \bigl\{ 
               m \in [M] 
             \bigm|
               \mP_{\sigma_{m}} = \mP_{\sigma} 
             \bigr\}
           \Bigr|.
    \end{align*}

  \item Let $ \set{B}_{\setA(\vgam)^{M}} $ be the set of all the possible types
    $ \mP_{\bm{t}_{ \vsigma_{[M]} }} $:
    \begin{align*}
      \set{B}_{\setA(\vgam)^{M}}
        &\defeq 
           \left\{ 
             \bm{t} 
               \defeq 
                 \Bigl( t( \mP_{\sigma} ) \Bigr)_{ \!\! \mP_{\sigma} \in \setA(\vgam) }
           \ \middle|
             \begin{array}{c}
               \exists \mP_{\vsigma_{[M]}} \in \setA(\vgam)^{M} \\
               \text{s.t.} \ \bm{t}_{\mP_{\vsigma_{[M]}}} = \bm{t}
             \end{array}
           \right\}.
    \end{align*}

  \item Let $ \bm{t} \in \set{B}_{\setA(\vgam)^{M}} $. The type class of
    $ \bm{t} $ is defined to be
    \begin{align*}
      \set{T}_{\bm{t}}
        &\defeq 
           \bigl\{ 
             \mP_{\vsigma_{[M]}} \in \setA(\vgam)^{M}
           \bigm|
             \bm{t}_{\mP_{\vsigma_{[M]}}} = \bm{t}
           \bigr\}.
    \end{align*}

  \end{enumerate}
  \edefinition
\end{definition}

%***************************************************************************

\begin{lemma}
  \label{sec:1:lem:21}

  Consider $ M \in \sZpp $ and $ \vgam \in \Gamma_{n} $. It holds that
  \begin{align*}
    \bigl| \set{B}_{\setA(\vgam)^{M}} \bigr|
      &= \binom{M + |\setA(\vgam)| - 1}{|\setA(\vgam)| - 1} 
           \in O\bigl( M^{|\setA(\vgam)|-1} \bigr)\, , \nonumber \\
    |\set{T}_{\bm{t}}| 
      &= \frac{ M! }
              { \prod\limits_{ \mP_{\sigma} \in \setA(\vgam) } 
                  \bigl( M \cdot t(\mP_{\sigma}) \bigr)! }\, ,
           \quad \bm{t} \in \set{B}_{\setA(\vgam)^{M}}.
  \end{align*}
\end{lemma}
%***************************************************************************

\begin{proof}
  These are standard combinatorial results and so the details of the
  derivation are omitted.
\end{proof}

%***************************************************************************

\noindent
\textbf{Proof sketch of
  Proposition~\ref{prop:coefficient:asymptotitic:characterization:1}}.
\begin{itemize}

\item The expression in~\eqref{sec:1:eqn:125} can be proven as
  follows. Namely, let $\vgam \in \GamMn$. For a large integer $M$, we obtain
  \begin{align*}
    \CM{n}( \vgam )
      &\overset{(a)}{=}
         \sum_{ \vsigma_{[M]} \in \setS_{[n]}^{M} }
           \Bigl[ 
             \vgam = \bigl\langle \mP_{\sigma_{m}} \bigr\rangle_{m \in [M]}
           \Bigr] \\
      &\overset{(b)}{=}
         \sum_{ \bm{t} \in \set{B}_{\setA(\vgam)^{M}} }
           \underbrace
           {
             \sum_{ \mP_{\vsigma_{[M]}} \in \set{T}_{\bm{t}}}
               \Bigl[ 
                 \vgam = \bigl\langle \mP_{\sigma_{m}} \bigr\rangle_{m \in [M]}
               \Bigr]
           }_{\defeq \ (*)} \\
      &\overset{(c)}{=}
         \sum_{ \bm{t} \in \set{B}_{\setA(\vgam)^{M}} \cap \PiA{\vgam}( \vgam )}
           |\set{T}_{\bm{t}}| \\
      &\overset{(d)}{=}
         \sum_{ \bm{t} \in \set{B}_{\setA(\vgam)^{M}} \cap \PiA{\vgam}( \vgam )}
           \exp\bigl( M \cdot \HG( \bm{t} ) + o( M ) \bigr) \\
      &\overset{(e)}{=}
         \max_{ \bm{t} \in \set{B}_{\setA(\vgam)^{M}} \cap \PiA{\vgam}( \vgam )}
           \exp\bigl( M \cdot \HG( \bm{t} ) + o( M ) \bigr) \, ,
  \end{align*}
  where step~$(a)$ follows from the definition of $\CM{n}( \vgam )$
  in~\eqref{sec:1:eqn:56}, where step~$(b)$ follows from the definition of
  $\set{B}_{\setA(\vgam)^{M}}$ and $\set{T}_{\bm{t}}$, where
  step~$(c)$ follows from the observation that $(*)$ equals
  $|\set{T}_{\bm{t}}|$ if 
  $\bm{t} \in \set{B}_{\setA(\vgam)^{M}} \cap \PiA{\vgam}(\vgam)$ and equals zero
  if $\bm{t} \in \set{B}_{\setA(\vgam)^{M}} \setminus \PiA{\vgam}(\vgam)$,
  where step~$(d)$ follows from 
  Stirling's approximation of the factorial function (see, \eg,~\cite{Robbins1955}), 
  Lemma~\ref{sec:1:lem:21}, and the definition of
  $\HG$ in Definition~\ref{sec:1:def:18}, and where step~$(e)$ follows from
  the fact that the size of the set $\set{B}_{\setA(\vgam)^{M}}$ is polynomial
  in $M$ (see Lemma~\ref{sec:1:lem:21}) and therefore can be absorbed in the
  $o(M)$ term in the exponent.
  
  In the limit $M \to \infty$, the set $\set{B}_{\setA(\vgam)^{M}}$ is dense
  in $\PiA{\vgam}( \vgam )$, and so
  \begin{align*}
    \CM{n}( \vgam )
      &= \max_{ \bm{t} \in \PiA{\vgam}( \vgam )}
           \exp\bigl( M \cdot \HG( \bm{t} ) + o( M ) \bigr) \\
      &\overset{(a)}{=}
         \exp\bigl( M \cdot \HG'( \vgam ) + o( M ) \bigr)\, ,
  \end{align*}
  where step~$(a)$ used the definition of $\HG'$ in
  Definition~\ref{sec:1:def:18:part:2}.

\item For the proof of the expression in~\eqref{sec:1:eqn:206},
  see~\cite[Section~VII]{Vontobel2013}.

\item A similar line of reasoning as above can be used to prove the expression
  in~\eqref{sec:1:eqn:207}; the details are omitted.

  \epropositionproof

\end{itemize}

%**************************************************************************
%**************************************************************************

\ifx\withclearpagecommands\x
\clearpage
\fi

\section[Results for the \texorpdfstring{Degree-$2$}{} Case]{Results for the Permanent and the \texorpdfstring{Degree-$2$ Bethe Permanent}{}}
\label{apx:22}

%**************************************************************************

The upcoming proposition, Proposition~\ref{prop:ratio:perm:permbM:2:1}, is the
same as Proposition~2 in~\cite{KitShing2022}. The purpose of this section is
to rederive this proposition based on some of the results that have been
established so far in this thesis.

%**************************************************************************

\begin{proposition}
  \label{prop:ratio:perm:permbM:2:1}
  \label{PROP:RATIO:PERM:PERMBM:2:1}
  Let $\pmtheta$ be the probability mass function on $\setS_{[n]}$ induced
  by~$\mtheta$ (see Definition~\ref{sec:1:def:10}). It holds that
  \begin{align}
    \frac{ \perm(\mtheta) }{ \permbM{2}(\mtheta) }
      &= \Biggl(
            \sum\limits_{ \sigma_1,\sigma_{2} \in \setS_{[n]} } 
              \pmtheta( \sigma_1 )
              \cdot
              \pmtheta( \sigma_{2} ) 
              \cdot
              2^{-c(\sigma_1,\sigma_2)}
         \Biggr)^{\!\!\! -1/2}\, ,
           \label{eq:ratio:perm:permbM:2:result:1}
  \end{align}
  where $c(\sigma_1,\sigma_2)$ is the number of cylces of length larger than
  one in the cycle notation
  expression\footnote{\label{footnote:cycle:notation:example:1}%
    Let us recall the cycle notation for permutations with the help of an
    example. Namely, consider the permutation $\sigma: [7] \to [7]$ defined by
    $\sigma(1) = 1$, $\sigma(2) = 2$, $\sigma(3) = 4$, $\sigma(4) = 3$,
    $\sigma(5) = 6$, $\sigma(6) = 7$, $\sigma(7) = 5$. In terms of cycle
    notation, $\sigma = (1)(2)(34)(567)$. As can be seen from this expression,
    the permutation $\sigma$ contains two cycles of length $1$ (one cycle
    involving only~$1$ and one cycle involving only~$2$), one cycle of length
    $2$ (involving $3$ and $4$), and one cycle of length $3$ (involving $5$,
    $6$, and $7$).} of the permutation ${\sigma_1 \circ \sigma_2^{-1}}$. Here,
  $\sigma_1 \circ \sigma_2^{-1}$ represents the permutation that is obtained
  by first applying the inverse of the permutation $\sigma_2$ and then the
  permutation $\sigma_1$.
  \eproposition
 \end{proposition}

%**************************************************************************

Note that $c(\sigma_1,\sigma_2)$ satisfies\footnote{While the lower bound on
  $c(\sigma_1,\sigma_2)$ is immediately clear, the upper bound on
  $c(\sigma_1,\sigma_2)$ follows from permutations of $[n]$ that contain
  $\lfloor n/2 \rfloor $ cycles of length~$2$.}
\begin{align*}
  0 
    &\leq 
       c(\sigma_1,\sigma_2) 
     \leq 
       \Bigl\lfloor \frac{n}{2} \Bigr\rfloor \, , 
       \qquad \sigma_1,\sigma_{2} \in \setS_{[n]}(\mtheta).
\end{align*}
These bounds on $c(\sigma_1,\sigma_2)$ yield
\begin{align}
  1
    &\overset{(a)}{\leq}
       \frac{ \perm(\mtheta) }{ \permbM{2}(\mtheta) }
     \overset{(b)}{\leq}
       \sqrt{2^{\lfloor n/2 \rfloor}}
     \leq
        2^{n/4}\, ,
          \label{eq:bounds:on"ratio:perm:permbM:2:1}
\end{align}
where the inequality~$(a)$ is obtained by lower bounding the expression
in~\eqref{eq:ratio:perm:permbM:2:result:1} with the help of
$c(\sigma_1,\sigma_2) \geq 0$ and where the inequality~$(b)$ is obtained by
upper bounding the expression in~\eqref{eq:ratio:perm:permbM:2:result:1} with
the help of $c(\sigma_1,\sigma_2) \leq \lfloor n/2 \rfloor$. Note that the
lower and upper bounds in~\eqref{eq:bounds:on"ratio:perm:permbM:2:1} on the
ratio $\perm(\mtheta) / \permbM{2}(\mtheta)$ match exactly the lower and upper
bounds in~\eqref{SEC:1:EQN:147} for $M = 2$.

%**************************************************************************

\begin{remark}
  A variant of Proposition~\ref{prop:ratio:perm:permbM:2:1} (and with that
  of~\cite[Proposition 2]{KitShing2022}), appears in~\cite[Lemma
  4.2]{Csikvari2017}. The setup in~\cite{Csikvari2017} is more special than
  that in~\cite{KitShing2022} in the sense that Csikv{\'a}ri
  in~\cite{Csikvari2017} considered $\{0,1\}$-valued matrices only, not
  arbitrary non-negative matrices. However, the result in~\cite{Csikvari2017}
  is more general than the result in~\cite{KitShing2022} in the sense that
  Csikv{\'a}ri studied matchings of size $k \in [n]$, and not just matchings
  of size $n$ (\ie, perfect matchings).  \eremark
\end{remark}

%***************************************************************************

\noindent
\textbf{Alternative proof Proposition~\ref{prop:ratio:perm:permbM:2:1}.} 
Let us now show how the results in this thesis can be used to rederive
Proposition~\ref{prop:ratio:perm:permbM:2:1}. Namely, we obtain
\begin{align*}
  \frac{\perm(\mtheta)}
       {\permbM{2}(\mtheta)}
    &\overset{(a)}{=}
       \left( \!
         \sum_{ \sigma_1, \sigma_2 \in \setS_{[n]} }
           \pmtheta(\sigma_1)
           \cdot
           \pmtheta(\sigma_2)
           \cdot
           \frac{\CBtwo{n}\Bigl( 
                            \frac{1}{2} 
                            \bigl( 
                              \mP_{\sigma_1} \! + \! \mP_{\sigma_2}
                            \bigr)
                          \Bigr)}
                {\Ctwo{n}\Bigl( 
                           \frac{1}{2} 
                           \bigl( 
                             \mP_{\sigma_1} \! + \! \mP_{\sigma_2}
                           \bigr)
                         \Bigr)}
       \right)^{\!\!\! -1/2} \\
    &\overset{(b)}{=}
       \Biggl( 
         \sum_{ \sigma_1, \sigma_2 \in \setS_{[n]} }
           \pmtheta(\sigma_1)
           \cdot
           \pmtheta(\sigma_2)
           \cdot
           \frac{1}
                {2^{c(\sigma_1,\sigma_2)}}
       \Biggr)^{\!\!\! -1/2}\, ,
\end{align*}
which is the same expression as
in~\eqref{eq:ratio:perm:permbM:2:result:1}. Here, step~$(a)$ follows from
Lemma~\ref{lemma:ratio:perm:permbM:1} for $M = 2$ and step~$(b)$ follows from
\begin{alignat}{2}
  \CBtwo{n}\biggl( 
             \frac{1}{2} 
             \bigl( 
               \mP_{\sigma_1} \! + \! \mP_{\sigma_2} 
             \bigr)
           \biggr)
    &= 1 \, , 
         &&\quad \sigma_1, \sigma_2 \in \setS_{[n]}\, ,
             \label{eq:CBtwo:result:1} \\
  \Ctwo{n}\biggl( 
            \frac{1}{2} 
            \bigl( 
              \mP_{\sigma_1} \! + \! \mP_{\sigma_2} 
            \bigr)
          \biggr)
    &= 2^{c(\sigma_1,\sigma_2)},
         &&\quad \sigma_1, \sigma_2 \in \setS_{[n]}.
             \label{eq:Ctwo:result:1}
\end{alignat}
Eqs.~\eqref{eq:CBtwo:result:1} and~\eqref{eq:Ctwo:result:1} are established in
Appendix~\ref{app:alt:proof:prop:ratio:perm:permbM:2:1}.
\epropositionproof


==> chap1.tex <==
%!TEX root = main.tex



\chapter{Introduction} 
Shannon’s seminal work \cite{sha48} laid down the theoretical foundations of information theory. 




\section{Contributions of this Thesis}
This thesis tries to solve several instances 

In Chapter 2, we .



Chapter 3 does ...

% Via using similar ideas on the outer bounds, we could derive outer bounds for Quadratic Gaussian Distributed Source Coding Problem and Quadratic Gaussian CEO Problem, and present alternative proofs for the optimality of Berger-Tung inner bound in these two settings. To the best of our knowledge, this work has not appeared before.

Chapter 4 is related 

In Chapter 5 we present some interesting future directions and summarize





==> chap2.tex <==
%!TEX root = main.tex
\chapter{ChapterName}
\label{ch:chref}

\section{Introduction}




\section{Main results}








\section{Conclusion and Discussion}
In this chapter, 
% Activate the appendix
% from now on sections are numerated with capital letters
\iffalse
\appendix
\fi

\iffalse






\begin{subappendices}


\end{subappendices}
\fi
	

==> dedication.tex <==
%!TEX root = main.tex
% \noindent 
% Dedicated to \textbf{my parents}.

==> figures/background_nodes_after_lct_proof.tex <==

\foreach{\x} in {0,1}{
    %------------------------------------------------------------------------
    \begin{pgfonlayer}{main}
        \node[] (f3\x) at (-\ldis-2.8*\sdis,2.8*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f4\x) at (-\ldis-2.8*\sdis,-2.8*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f5\x) at (\ldis+2.8*\sdis,2.8*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f6\x) at (\ldis+2.8*\sdis,-2.8*\sdis-5.8*\sdis*\x) [] {};
    \end{pgfonlayer}
    %------------------------------------------------------------------------
}
\node[state] (f7) at (-\ldis,-2.9*\sdis) [label=right: $ \lambda_{f_{i}} $] {};
\node[state] (f8) at (\ldis,-2.9*\sdis) [label=left: $ \lambda_{f_{j}} $] {};

\node[state] (f10) at (-\ldis,0) [label=above: $ u'_{ f_{i} } $] {};
\node[state] (f20) at (\ldis,0) [label=above: $ u'_{ f_{j} } $] {};
\node[state] (f11) at (-\ldis,-5.8*\sdis) 
[label=below: $ \overline{ \LCT{u}_{ f_{i} } } $] {};
\node[state] (f21) at (\ldis,-5.8*\sdis) 
[label=below: $ \overline{ \LCT{u}_{ f_{j} } } $] {};

==> figures/graph_cov_thm/previous_figures/denfg_sincyc.tex <==
\begin{minipage}[t]{0.45\linewidth}
    \centering
    %----------------------
    \begin{tikzpicture}[node distance=2cm, on grid,auto]
      \input{figures/head_files_figs.tex}
      \input{figures/length.tex}
      %----------------------------------------------------------------------------
      \begin{pgfonlayer}{main}
        \node[state] (f1) at (0,0) [label=above: $f_1$] {};
        \node[state] (f2) at (2*\ldis,0) [label=above: $f_2$] {};
        \node[state] (f3) at (0,-2*\ldis) [label=below: $f_3$] {};
      \end{pgfonlayer}
      %----------------------------------------------------------------------------
      \begin{pgfonlayer}{background}
        \draw[double]

          (f1) -- node[above] {$\tvx_{1}$} (f2)
          (f2) -- node[right=.1cm]  {$\tvx_{2}$} (f3) % (q0)  edge [bend left= 10]  node[el,above,pos=0.8] {$a=2$}  (q2)
          (f3) -- node[left=.03cm] 
          { $\tvx_{3}$} (f1);
      \end{pgfonlayer}
      %----------------------------------------------------------------------------
    \end{tikzpicture}
  \end{minipage}

==> figures/graph_cov_thm/previous_figures/denfg_twoedges.tex <==
\begin{minipage}[t]{0.45\linewidth}
  \centering
  %----------------------
  \begin{tikzpicture}[node distance=2cm, on grid,auto]
    \input{figures/length.tex}
    \input{figures/head_files_figs.tex}
    %----------------------------------------------------------------------------
    \begin{pgfonlayer}{main}
      \node[state] (f1) at (0,0) [label=above: $f_1$] {};
      \node[state,right of=f1] (f2) [label=above: $f_2$] {};
      \node[state,left of=f1] (f3) [label=above: $f_3$] {};
    \end{pgfonlayer}
    %----------------------------------------------------------------------------
    \begin{pgfonlayer}{background}
      \draw[double]
        (f1) -- node[above] {$\tvx_{1}$} (f2)
        (f1) -- node[above]  {$\tvx_{2}$} (f3);
    \end{pgfonlayer}
    % ----------------------------------------------------------------------------
  \end{tikzpicture}
  \vspace{0.1 cm}
\end{minipage}

==> figures/graph_cov_thm/previous_figures/snfg_sincyc.tex <==
\begin{minipage}[t]{0.45\linewidth}
    \centering
    %----------------------
    \begin{tikzpicture}[node distance=2cm, on grid,auto]
      \input{figures/head_files_figs.tex}
      \input{figures/length.tex}
      %----------------------------------------------------------------------------
      \begin{pgfonlayer}{main}
        \node[state_large2] (f1) at (0,0) [label=above: $f_1$] {};
        \node[state_large2] (f2) at (2*\ldis,0) [label=above: $f_2$] {};
        \node[state_large2] (f3) at (0,-2*\ldis) [label=below: $f_3$] {};
      \end{pgfonlayer}
      %----------------------------------------------------------------------------
      \begin{pgfonlayer}{background}
        \draw[double]
          (0,\lvaredge) -- node[above] {$ \vx_{\pone} $} (2*\ldis,\lvaredge)
          (0,-\lvaredge) -- (2*\ldis,-\lvaredge)
          (\lvaredge,0) -- (\lvaredge,-2*\ldis)
          (-\lvaredge,0) -- node[left] {$ \vx_{\ptwo} $}  (-\lvaredge,-2*\ldis)

          (2*\ldis-\lvaredge/2,\lvaredge/2) 
          -- (-\lvaredge/2,-2*\ldis+\lvaredge/2)  
          (2*\ldis+\lvaredge/2,-\lvaredge/2) 
          -- node[right,xshift=0.2cm] {$ \vx_{\pthre} $} (\lvaredge/2,-2*\ldis-\lvaredge/2);

          % (f1) -- node[above] {$\vx_{\pone}$} (f2)
          % (f2) -- node[right=.1cm]  {$\vx_{\ptwo}$} (f3) % (q0)  edge [bend left= 10]  node[el,above,pos=0.8] {$a=2$}  (q2)
          % (f3) -- node[left=.03cm] 
          % { $\vx_{\pthre}$} (f1);
      \end{pgfonlayer}
      %----------------------------------------------------------------------------
    \end{tikzpicture}
  \end{minipage}

==> figures/graph_cov_thm/previous_figures/snfg_twoedges.tex <==
\begin{minipage}[t]{0.45\linewidth}
  \centering
  %----------------------
  \begin{tikzpicture}[node distance=2cm, on grid,auto]
    \input{figures/length.tex}
    \input{figures/head_files_figs.tex}
    \node[state_large2] (f1) at (0,0) [label=above: $f_1$] {};
    \node[state_large2] (f2) at (3*\ldis,0) [label=above: $f_2$] {};
    \node[state_large2] (f2) at (-3*\ldis,0) [label=above: $f_3$] {};
    %----------------------------------------------------------------------------
    \begin{pgfonlayer}{background}
      \draw[double]
          (0,\lvaredge) -- node[above] {$ \vx_{\pone} $} (3*\ldis,\lvaredge)
          (0,-\lvaredge) -- (3*\ldis,-\lvaredge)
          (0,\lvaredge) -- node[above] {$ \vx_{\ptwo} $} (-3*\ldis,\lvaredge)
          (0,-\lvaredge) -- (-3*\ldis,-\lvaredge);
    \end{pgfonlayer}
    %----------------------------------------------------------------------------
    % %----------------------------------------------------------------------------
    % \begin{pgfonlayer}{main}
    %   \node[state] (f1) at (0,0) [label=above: $f_1$] {};
    %   \node[state,right of=f1] (f2) [label=above: $f_2$] {};
    %   \node[state,left of=f1] (f3) [label=above: $f_3$] {};
    % \end{pgfonlayer}
    % %----------------------------------------------------------------------------
    % \begin{pgfonlayer}{background}
    %   \draw[double]
    %     (f1) -- node[above] {$\vx_{\pone}$} (f2)
    %     (f1) -- node[above]  {$\vx_{\ptwo}$} (f3);
    % \end{pgfonlayer}
    %----------------------------------------------------------------------------
  \end{tikzpicture}
  \vspace{0.1 cm}
\end{minipage}

==> figures/lct_examples/CTB_dashed_boxes.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{background} 
  \node[state_dash3] (db6) at (-0.9*\ldis,0) [] {};
  \node[state_dash3] (db7) at (0.9*\ldis,0) [] {};
\end{pgfonlayer}
%----------------------------------------------------------------------------

==> figures/lct_examples/penfg/OTB_dashed_boxes.tex <==
\foreach{\x} in {0,1}{
    %------------------------------------------------------------------------
    \begin{pgfonlayer}{background} 
    \node[state_dash1] (db1\x) at (0,\sdis*0.2-5.8*\sdis*\x) [] {};
    \node[state_dash2] (db2\x) 
    at (-\ldis-1.5*\sdis,1.75*\sdis-5.8*\sdis*\x)  [] {};
    \node[state_dash2] (db3\x) 
    at (-\ldis-1.5*\sdis,-1.75*\sdis-5.8*\sdis*\x) [] {};
    \node[state_dash2] (db4\x) 
    at (\ldis+1.5*\sdis,1.75*\sdis-5.8*\sdis*\x) [] {};
    \node[state_dash2] (db5\x) 
    at (\ldis+1.5*\sdis,-1.75*\sdis-5.8*\sdis*\x) [] {};
    \end{pgfonlayer}
    %------------------------------------------------------------------------
}

==> figures/lct_examples/penfg/OTB_dashed_boxes_EVD.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{background} 
  \node[state_dash5] (db1) at (-0.8*\ldis,-2.9*\sdis) [label=above: $f_{i}$] {};
  \node[state_dash5] (db2) at (0.8*\ldis,-2.9*\sdis)  [label=above: $f_{j}$] {};
\end{pgfonlayer}
%----------------------------------------------------------------------------

==> figures/lct_examples/penfg/OTB_dashed_boxes_EVD_after_lct.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{background} 
  \node[state_dash5] (db1) at (-0.8*\ldis,-2.9*\sdis) [label=above: $\LCT{f}_{i}$] {};
  \node[state_dash5] (db2) at (0.8*\ldis,-2.9*\sdis)  [label=above: $\LCT{f}_{j}$] {};
\end{pgfonlayer}
%----------------------------------------------------------------------------

==> figures/lct_examples/penfg/OTB_funs.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{main} 
  % the functions on LHS
  \node[state] (M1) at (-\ldis-2*\sdis,2*\sdis) 
  [label=above: $h_{1}$] {};
  \node[state] (M2) at (-\ldis-\sdis,\sdis) 
  [label=above: $h_{2}$] {};
  \node[state] (M3) at (-\sdis/2,0) 
  [label=above: $h_{3}$] {};
  \node[state] (M4) at (-\ldis-\sdis,-\sdis) 
  [label=below: $h_{4}$] {};
  \node[state] (M5) at (-\ldis-2*\sdis,-2*\sdis) 
  [label=below: $h_{5}$] {};
  % the functions on RHS
  \node[state] (M6) at (\ldis+2*\sdis,2*\sdis) 
  [label=above: $h_{6}$] {};
  \node[state] (M7) at (\ldis+\sdis,\sdis) 
  [label=above: $h_{7}$] {};
  \node[state] (M8) at (\sdis/2,0) 
  [label=above: $h_{8}$] {};
  \node[state] (M9) at (\ldis+\sdis,-\sdis) 
  [label=below: $h_{9}$] {};
  \node[state] (M10) at (\ldis+2*\sdis,-2*\sdis) 
  [label=below: $h_{10}$] {};

  \node[state] (M12) at (-\ldis-2*\sdis,2*\sdis-5.8*\sdis) 
  [label=above: $\overline{h_{1}}$] {};
  \node[state] (M22) at (-\ldis-\sdis,\sdis-5.8*\sdis) 
  [label=above: $\overline{h_{2}}$] {};
  \node[state] (M32) at (-\sdis/2,-5.8*\sdis) 
  [label=above: $\overline{h_{3}}$] {};
  \node[state] (M42) at (-\ldis-\sdis,-\sdis-5.8*\sdis) 
  [label=below: $\overline{h_{4}}$] {};
  \node[state] (M52) at (-\ldis-2*\sdis,-2*\sdis-5.8*\sdis) 
  [label=below: $\overline{h_{5}}$] {};
  % the functions on RHS
  \node[state] (M62) at (\ldis+2*\sdis,2*\sdis-5.8*\sdis) 
  [label=above: $\overline{h_{6}}$] {};
  \node[state] (M72) at (\ldis+\sdis,\sdis-5.8*\sdis) 
  [label=above: $\overline{h_{7}}$] {};
  \node[state] (M82) at (\sdis/2,-5.8*\sdis) 
  [label=above: $\overline{h_{8}}$] {};
  \node[state] (M92) at (\ldis+\sdis,-\sdis-5.8*\sdis) 
  [label=below: $\overline{h_{9}}$] {};
  \node[state] (M102) at (\ldis+2*\sdis,-2*\sdis-5.8*\sdis) 
  [label=below: $\overline{h_{10}}$] {};
  % the variables for OTB
\end{pgfonlayer} 
%----------------------------------------------------------------------------

==> figures/lct_examples/penfg/background_lines.tex <==
\foreach \x in {0,1}{
	\begin{pgfonlayer}{behind} 
		\draw[] 
		(f1\x) -- (f2\x)
		(f1\x) -- (f3\x)
		(f1\x) -- (f4\x)
		(f2\x) -- (f5\x)
		(f2\x) -- (f6\x);
	\end{pgfonlayer}
}
\begin{pgfonlayer}{behind} 
	\draw[] 
	(f10) -- (f11)
	(f20) -- (f21);
\end{pgfonlayer}


==> figures/lct_examples/penfg/background_lines_orignal.tex <==
\begin{pgfonlayer}{background} 
	\foreach \x in {0,1}{
		\draw 
		(f1\x) -- (f2\x)
		(f3\x1) -- (f3\x)
		(f4\x1) -- (f4\x)
		(f5\x1) -- (f5\x)
		(f6\x1) -- (f6\x);
		% (f1) -- (f41)
		% (f2) -- (f51)
		% (f2) -- (f61);
		% \draw 
		% (f1) -- (f2)
		% (f1) -- (f30)
		% (f1) -- (f40)
		% (f2) -- (f50)
		% (f2) -- (f60);
	}
\end{pgfonlayer}

==> figures/lct_examples/penfg/background_nodes.tex <==

\foreach{\x} in {0,1}{
    %------------------------------------------------------------------------
    \begin{pgfonlayer}{main}
        \node[] (f3\x) at (-\ldis-2.8*\sdis,2.8*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f4\x) at (-\ldis-2.8*\sdis,-2.8*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f5\x) at (\ldis+2.8*\sdis,2.8*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f6\x) at (\ldis+2.8*\sdis,-2.8*\sdis-5.8*\sdis*\x) [] {};
    \end{pgfonlayer}
    %------------------------------------------------------------------------
}
\node[state] (f7) at (-\ldis,-2.9*\sdis) [label=right: $ \lambda_{f_{i}} $] {};
\node[state] (f8) at (\ldis,-2.9*\sdis) [label=left: $ \lambda_{f_{j}} $] {};

\node[state] (f10) at (-\ldis,0) [label=above: $ u_{ f_{i} } $] {};
\node[state] (f20) at (\ldis,0) [label=above: $ u_{ f_{j} } $] {};
\node[state] (f11) at (-\ldis,-5.8*\sdis) 
[label=below: $ \overline{ u_{ f_{i} } } $] {};
\node[state] (f21) at (\ldis,-5.8*\sdis) 
[label=below: $ \overline{u_{ f_{j} } } $] {};

==> figures/lct_examples/penfg/background_nodes_after_ctb.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{main}
  \node[] (f30) at (-\ldis-2.9*\sdis, 2.9*\sdis) [] {}; 
  \node[] (f31) at (-\ldis-2.7*\sdis, 2.7*\sdis) [] {}; 

  \node[] (f40) at (-\ldis-2.9*\sdis,-2.9*\sdis) [] {}; 
  \node[] (f41) at (-\ldis-2.7*\sdis,-2.7*\sdis) [] {}; 

  \node[] (f50) at (\ldis+2.9*\sdis,2.9*\sdis) [] {}; 
  \node[] (f51) at (\ldis+2.7*\sdis,2.7*\sdis) [] {}; 

  \node[] (f60) at (\ldis+2.9*\sdis,-2.9*\sdis) [] {};
  \node[] (f61) at (\ldis+2.7*\sdis,-2.7*\sdis) [] {};;
\end{pgfonlayer}
%----------------------------------------------------------------------------

==> figures/lct_examples/penfg/background_nodes_after_ctb_original.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{main}
  \node[] (f30) at (-\ldis-2.9*\sdis, 2.9*\sdis) [] {}; 
  \node[] (f31) at (-\ldis-2.7*\sdis, 2.7*\sdis) [] {}; 

  \node[] (f40) at (-\ldis-2.9*\sdis,-2.9*\sdis) [] {}; 
  \node[] (f41) at (-\ldis-2.7*\sdis,-2.7*\sdis) [] {}; 

  \node[] (f50) at (\ldis+2.9*\sdis,2.9*\sdis) [] {}; 
  \node[] (f51) at (\ldis+2.7*\sdis,2.7*\sdis) [] {}; 

  \node[] (f60) at (\ldis+2.9*\sdis,-2.9*\sdis) [] {};
  \node[] (f61) at (\ldis+2.7*\sdis,-2.7*\sdis) [] {};;
\end{pgfonlayer}
%----------------------------------------------------------------------------

==> figures/lct_examples/penfg/background_nodes_after_lct.tex <==

\foreach{\x} in {0,1}{
    %------------------------------------------------------------------------
    \begin{pgfonlayer}{main}
        \node[] (f3\x) at (-\ldis-2.8*\sdis,2.8*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f4\x) at (-\ldis-2.8*\sdis,-2.8*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f5\x) at (\ldis+2.8*\sdis,2.8*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f6\x) at (\ldis+2.8*\sdis,-2.8*\sdis-5.8*\sdis*\x) [] {};
    \end{pgfonlayer}
    %------------------------------------------------------------------------
}
\node[state] (f7) at (-\ldis,-2.9*\sdis) [label=right: $ \lambda_{f_{i}} $] {};
\node[state] (f8) at (\ldis,-2.9*\sdis) [label=left: $ \lambda_{f_{j}} $] {};

\node[state] (f10) at (-\ldis,0) [label=above: $ u'_{ f_{i} } $] {};
\node[state] (f20) at (\ldis,0) [label=above: $ u'_{ f_{j} } $] {};
\node[state] (f11) at (-\ldis,-5.8*\sdis) 
[label=below: $ \overline{ u'_{ f_{i} } } $] {};
\node[state] (f21) at (\ldis,-5.8*\sdis) 
[label=below: $ \overline{ u'_{ f_{j} } } $] {};

==> figures/lct_examples/penfg/background_nodes_original.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{main}
  \foreach \x/\xin in {1/0,-1/1}{
  \node[] (f1\xin) at (-\ldis, 0.2*\x*\sdis) [] {}; 
  \node[] (f2\xin) at (\ldis, 0.2*\x*\sdis) [] {}; 

  \node[] (f3\xin) at (-\ldis-2.8*\sdis+0.1*\x*\sdis, 2.8*\sdis+0.1*\x*\sdis) [] {}; 
  \node[] (f3\xin1) at (-\ldis+0.1*\x*\sdis, 0.1*\x*\sdis) [] {}; 
  % \node[] (f31) at (-\ldis-2.7*\sdis, 2.7*\sdis) [] {}; 

  \node[] (f4\xin) at (-\ldis-2.8*\sdis+0.1*\x*\sdis,-2.8*\sdis-0.1*\x*\sdis) [] {}; 
  \node[] (f4\xin1) at (-\ldis+0.1*\x*\sdis, -0.1*\x*\sdis) [] {}; 

  % \node[] (f41) at (-\ldis-2.7*\sdis,-2.7*\sdis) [] {}; 

  \node[] (f5\xin) at (\ldis+2.8*\sdis+0.1*\x*\sdis,2.8*\sdis-0.1*\x*\sdis) [] {}; 
  \node[] (f5\xin1) at (\ldis+0.1*\x*\sdis,-0.1*\x*\sdis) [] {}; 
  % \node[] (f51) at (\ldis+2.7*\sdis,2.7*\sdis) [] {}; 

  \node[] (f6\xin) at (\ldis+2.8*\sdis+0.1*\x*\sdis,-2.8*\sdis+0.1*\x*\sdis) [] {};
  \node[] (f6\xin1) at (\ldis+0.1*\x*\sdis,0.1*\x*\sdis) [] {};
  % \node[] (f61) at (\ldis+2.7*\sdis,-2.7*\sdis) [] {};
  }
\end{pgfonlayer}
%----------------------------------------------------------------------------


==> figures/lct_examples/penfg/background_variables.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{main} 
    \node (x1) at (0,-0.22*\sdis) 
    [label=above: $x_{1}$] {}; 
    \node (x3) at (-0.6*\ldis-2.3*\sdis,1.5*\sdis) 
    [label=above: $x_{2}$] {}; 
    \node (x4) at (-0.6*\ldis-2.3*\sdis,-1.5*\sdis) 
    [label=below: $x_{3}$] {};

    \node (x3) at (0.6*\ldis+2.3*\sdis,1.5*\sdis) 
    [label=above: $x_{4}$] {}; 
    \node (x4) at (0.6*\ldis+2.3*\sdis,-1.5*\sdis) 
    [label=below: $x_{5}$] {}; 
\end{pgfonlayer}
%----------------------------------------------------------------------------

%----------------------------------------------------------------------------
\begin{pgfonlayer}{main} 
    \node (x1) at (0,-0.22*\sdis-5.8*\sdis) 
    [label=above: $x_{\upone}$] {}; 
    \node (x3) at (-0.6*\ldis-2.3*\sdis,1.5*\sdis-5.8*\sdis) 
    [label=above: $x_{\uptwo}$] {}; 
    \node (x4) at (-0.6*\ldis-2.3*\sdis,-1.5*\sdis-5.8*\sdis) 
    [label=below: $x_{\upthre}$] {};

    \node (x3) at (0.6*\ldis+2.3*\sdis,1.5*\sdis-5.8*\sdis) 
    [label=above: $x_{\upfor}$] {}; 
    \node (x4) at (0.6*\ldis+2.3*\sdis,-1.5*\sdis-5.8*\sdis) 
    [label=below: $x_{\upfif}$] {}; 
\end{pgfonlayer}
%----------------------------------------------------------------------------

==> figures/lct_examples/penfg/background_variables_EVD_l.tex <==
\node[] (f22) at (-1.1*\ldis,-2*\sdis) [label=right: $ \ell_{f_{i}} $] {};
\node[] (f23) at (1.1*\ldis,-2*\sdis) [label=left: $ \ell_{f_{j}} $] {};

==> figures/lct_examples/penfg/background_variables_EVD_s.tex <==
\node[] (f22) at (-1.2*\ldis,-1.5*\sdis) [label=right: $ \ell_{f_{i}} $] {};
\node[] (f23) at (1.2*\ldis,-1.5*\sdis) [label=left: $ \ell_{f_{j}} $] {};

==> figures/lct_examples/penfg/main_pic.tex <==

\begin{figure}
  \centering
  \captionsetup{font=scriptsize}
  \begin{adjustbox}{minipage=\linewidth,scale=0.98}
  \subfloat[\label{sec:LCT:fig:7}]{
    \begin{minipage}[t]{0.45\linewidth}
      \centering
      \begin{tikzpicture}[on grid, auto, scale=0.98]
        \input{figures/lct_examples/scale_small.tex}
        \input{figures/head_files_figs.tex}
        \input{figures/length.tex}
        \input{figures/lct_examples/penfg/background_nodes_original.tex}

        \node[state_long] (f1) at (-\ldis,0) [label=above: $f_{i}$] {};
        \node[state_long] (f2) at (\ldis,0) [label=above: $f_{j}$] {};
        % draw the lines
        \input{figures/lct_examples/penfg/background_lines_orignal.tex}
        \begin{pgfonlayer}{main} 
          \node (x1) at (0,-0.2*\sdis) 
          [label=above: $\vx_{\pone}$] {}; 
          \node (x3) at (-0.5*\ldis-2.1*\sdis,1.3*\sdis) 
          [label=above: $\vx_{\ptwo}$] {}; 
          \node (x4) at (-0.5*\ldis-2.1*\sdis,-1.3*\sdis) 
          [label=below: $\vx_{\pthre}$] {};

          \node (x3) at (0.5*\ldis+2.1*\sdis,1.3*\sdis) 
          [label=above: $\vx_{\pfor}$] {}; 
          \node (x4) at (0.5*\ldis+2.1*\sdis,-1.3*\sdis) 
          [label=below: $\vx_{\pfif}$] {}; 
        \end{pgfonlayer}
      \end{tikzpicture}
    \end{minipage}
  } 
  \subfloat[\label{sec:LCT:fig:8}]{
    \begin{minipage}[t]{0.45\linewidth}
      \centering
      \begin{tikzpicture}[on grid, auto, scale=0.98]
        \input{figures/lct_examples/scale_small.tex}
        \input{figures/head_files_figs.tex}
        \input{figures/lct_examples/penfg/background_nodes.tex}
        \input{figures/lct_examples/penfg/background_lines.tex}
        \input{figures/lct_examples/penfg/otb_dashed_boxes_evd.tex}
        \input{figures/lct_examples/penfg/background_variables.tex}
        \input{figures/lct_examples/penfg/background_variables_evd_s.tex}
      \end{tikzpicture}
    \end{minipage}
  }\\
  \subfloat[\label{sec:LCT:fig:9}]{
    \begin{minipage}[t]{0.5\linewidth}
      \centering
      \begin{tikzpicture}[on grid, auto, scale=0.98]
        \input{figures/lct_examples/scale_large_pesnfg.tex}
        \input{figures/head_files_figs.tex}
        \input{figures/lct_examples/penfg/background_nodes.tex}
        \input{figures/lct_examples/penfg/background_lines.tex}
        \input{figures/lct_examples/penfg/otb_funs.tex}
        \input{figures/lct_examples/penfg/otb_dashed_boxes.tex}
        \input{figures/lct_examples/penfg/variables_after_lct.tex}
        \input{figures/lct_examples/penfg/background_variables_evd_l.tex}
      \end{tikzpicture}
    \end{minipage}
  }
  %------------------------------------------------------------------------
  \subfloat[\label{sec:LCT:fig:10}]{
    \begin{minipage}[t]{0.45\linewidth}
      \centering
      \begin{tikzpicture}[on grid, auto, scale=0.98]
        \input{figures/lct_examples/scale_large_pesnfg.tex}
        \input{figures/head_files_figs.tex}
        \input{figures/lct_examples/penfg/background_nodes.tex}
        \input{figures/lct_examples/penfg/background_lines.tex}
        \input{figures/lct_examples/penfg/otb_funs.tex}
        \input{figures/lct_examples/penfg/ctb_dashed_boxes.tex}
        \input{figures/lct_examples/penfg/variables_before_lct.tex}
        \input{figures/lct_examples/penfg/variables_after_lct.tex}
        \input{figures/lct_examples/penfg/background_variables_evd_l.tex}
        % \foreach{\x} in {0,1}{
            %------------------------------------------------------------------------
            \begin{pgfonlayer}{background} 
              \node[] (lctfi) at (-\ldis,1.6*\sdis) 
              [label=above: $u'_{f_{i}}$] {};
              \node[] (lctfj) at (\ldis,1.6*\sdis) 
              [label=above: $u'_{f_{j}}$] {};
              \node[] (lctfi) at (-\ldis,-7.4*\sdis) 
              [label=below: $\overline{u'_{f_{i}}}$] {};
              \node[] (lctfj) at (\ldis,-7.4*\sdis) 
              [label=below: $\overline{u'_{f_{j}}}$] {};
            \end{pgfonlayer}
            %-------------------------------------------------------------------------9.2*\sdis*\x+
        % }
      \end{tikzpicture}
    \end{minipage}
  }\\
  \subfloat[\label{sec:LCT:fig:11}]{
    \begin{minipage}[t]{0.45\linewidth}
      \centering
      \begin{tikzpicture}[on grid, auto, scale=0.98]
        \input{figures/lct_examples/scale_small.tex}
        \input{figures/head_files_figs.tex}
        \input{figures/lct_examples/penfg/background_nodes_after_lct.tex}
        \input{figures/lct_examples/penfg/background_lines.tex}
        \input{figures/lct_examples/penfg/variables_after_lct_clb.tex}
        \input{figures/lct_examples/penfg/otb_dashed_boxes_evd_after_lct.tex}
        \input{figures/lct_examples/penfg/background_variables_evd_s.tex}
      \end{tikzpicture}
    \end{minipage}
  }
  \subfloat[\label{sec:LCT:fig:12}]{
    \begin{minipage}[t]{0.45\linewidth}
      \centering
      \begin{tikzpicture}[on grid, auto, scale=0.98]
        \input{figures/lct_examples/scale_small.tex}
        \input{figures/head_files_figs.tex}
        \input{figures/lct_examples/penfg/background_nodes_original.tex}
        \node[state_long] (f1) at (-\ldis,0) [label=above: $\LCT{f}_{i}$] {};
        \node[state_long] (f2) at (\ldis,0) [label=above: $\LCT{f}_{j}$] {};
        % draw the lines
        \input{figures/lct_examples/penfg/background_lines_orignal.tex}
        %----------------------------------------------------------------------
        \begin{pgfonlayer}{main} 
            \node (x1) at (0,-0.2*\sdis) 
            [label=above: $\vx_{\pone}$] {}; 
            \node (x3) at (-0.5*\ldis-2.1*\sdis,1.3*\sdis) 
            [label=above: $\LCTv{x}_{\ptwo}$] {}; 
            \node (x4) at (-0.5*\ldis-2.1*\sdis,-1.3*\sdis) 
            [label=below: $\LCTv{x}_{\pthre}$] {};

            \node (x3) at (0.5*\ldis+2.1*\sdis,1.3*\sdis) 
            [label=above: $\LCTv{x}_{\pfor}$] {}; 
            \node (x4) at (0.5*\ldis+2.1*\sdis,-1.3*\sdis) 
            [label=below: $\LCTv{x}_{\pfif}$] {}; 
        \end{pgfonlayer}
        %----------------------------------------------------------------------
      \end{tikzpicture}
    \end{minipage}
  }
  % %------------------------------------------------------------------------
  % \subfloat[]{
  %   \begin{minipage}[t]{0.45\linewidth}
  %     \centering
  %     \begin{tikzpicture}[on grid, auto, scale=0.98]
  %       \input{figures/lct_examples/scale_small.tex}
  %       \input{figures/head_files_figs.tex}
  %       \input{figures/lct_examples/background_nodes_after_ctb.tex}
  %       \input{figures/lct_examples/background_lines_DENFG.tex}
  %       \input{figures/lct_examples/variables_after_lct_DENFG.tex}
  %     \end{tikzpicture}
  %   \end{minipage}
  % }
  %------------------------------------------------------------------------
  \end{adjustbox}
  \caption{Left: Exemplifying the LCT for a part of an example
  PE-NFG.\label{sec:LCT:fig:2}}
\end{figure}



==> figures/lct_examples/penfg/variables_after_lct.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{main} 
    \node (x1) at (0,-0.22*\sdis) 
    [label=above: $\LCT{x}_{1}$] {}; 
    \node (x3) at (-0.5*\ldis-2.3*\sdis,1.5*\sdis) 
    [label=above: $\LCT{x}_{2}$] {}; 
    \node (x4) at (-0.5*\ldis-2.3*\sdis,-1.5*\sdis) 
    [label=below: $\LCT{x}_{3}$] {};

    \node (x3) at (0.5*\ldis+2.3*\sdis,1.5*\sdis) 
    [label=above: $\LCT{x}_{4}$] {}; 
    \node (x4) at (0.5*\ldis+2.3*\sdis,-1.5*\sdis) 
    [label=below: $\LCT{x}_{5}$] {}; 
\end{pgfonlayer}
%----------------------------------------------------------------------------

%----------------------------------------------------------------------------
\begin{pgfonlayer}{main} 
    \node (x1) at (0,-0.22*\sdis-5.8*\sdis) 
    [label=above: $\LCT{x}_{\upone}$] {}; 
    \node (x3) at (-0.5*\ldis-2.3*\sdis,1.5*\sdis-5.8*\sdis) 
    [label=above: $\LCT{x}_{\uptwo}$] {}; 
    \node (x4) at (-0.5*\ldis-2.3*\sdis,-1.5*\sdis-5.8*\sdis) 
    [label=below: $\LCT{x}_{\upthre}$] {};

    \node (x3) at (0.5*\ldis+2.3*\sdis,1.5*\sdis-5.8*\sdis) 
    [label=above: $\LCT{x}_{\upfor}$] {}; 
    \node (x4) at (0.5*\ldis+2.3*\sdis,-1.5*\sdis-5.8*\sdis) 
    [label=below: $\LCT{x}_{\upfif}$] {}; 
\end{pgfonlayer}
%----------------------------------------------------------------------------

==> figures/lct_examples/penfg/variables_after_lct_clb.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{main} 
    \node (x1) at (0,-0.22*\sdis) 
    [label=above: $\LCT{x}_{1}$] {}; 
    \node (x3) at (-0.57*\ldis-2.3*\sdis,1.4*\sdis) 
    [label=above: $\LCT{x}_{2}$] {}; 
    \node (x4) at (-0.57*\ldis-2.3*\sdis,-1.4*\sdis) 
    [label=below: $\LCT{x}_{3}$] {};

    \node (x3) at (0.57*\ldis+2.3*\sdis,1.4*\sdis) 
    [label=above: $\LCT{x}_{4}$] {}; 
    \node (x4) at (0.57*\ldis+2.3*\sdis,-1.4*\sdis) 
    [label=below: $\LCT{x}_{5}$] {}; 
\end{pgfonlayer}
%----------------------------------------------------------------------------

%----------------------------------------------------------------------------
\begin{pgfonlayer}{main} 
    \node (x1) at (0,-0.22*\sdis-5.8*\sdis) 
    [label=above: $\LCT{x}_{\upone}$] {}; 
    \node (x3) at (-0.57*\ldis-2.3*\sdis,1.4*\sdis-5.8*\sdis) 
    [label=above: $\LCT{x}_{\uptwo}$] {}; 
    \node (x4) at (-0.57*\ldis-2.3*\sdis,-1.4*\sdis-5.8*\sdis) 
    [label=below: $\LCT{x}_{\upthre}$] {};

    \node (x3) at (0.57*\ldis+2.3*\sdis,1.4*\sdis-5.8*\sdis) 
    [label=above: $\LCT{x}_{\upfor}$] {}; 
    \node (x4) at (0.57*\ldis+2.3*\sdis,-1.4*\sdis-5.8*\sdis) 
    [label=below: $\LCT{x}_{\upfif}$] {}; 
\end{pgfonlayer}
%----------------------------------------------------------------------------

==> figures/lct_examples/penfg/variables_before_lct.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{main} 
    \node (x3) at (-0.5*\ldis-0.22*\sdis,-0.22*\sdis) 
    [label=above: $x_{1}$] {};
    \node (x4) at (-0.5*\ldis-1.1*\sdis,0.4*\sdis) 
    [label=above: $x_{2}$] {}; 
    \node (x5) at (-0.5*\ldis-1.1*\sdis,-0.4*\sdis) 
    [label=below: $x_{3}$] {}; 

    \node (x6) at (0.5*\ldis+0.22*\sdis,-0.22*\sdis) 
    [label=above: $x_{4}$] {};
    \node (x7) at (0.5*\ldis+1.1*\sdis,0.4*\sdis) 
    [label=above: $x_{5}$] {}; 
    \node (x8) at (0.5*\ldis+1.1*\sdis,-0.4*\sdis) 
    [label=below: $x_{6}$] {}; 
\end{pgfonlayer}
%----------------------------------------------------------------------------

%----------------------------------------------------------------------------
\begin{pgfonlayer}{main} 
    \node (x3) at (-0.5*\ldis-0.22*\sdis,-0.22*\sdis-5.8*\sdis) 
    [label=above: $x_{\upone}$] {};
    \node (x4) at (-0.5*\ldis-1.1*\sdis,0.4*\sdis-5.8*\sdis) 
    [label=above: $x_{\uptwo}$] {}; 
    \node (x5) at (-0.5*\ldis-1.1*\sdis,-0.4*\sdis-5.8*\sdis) 
    [label=below: $x_{\upthre}$] {}; 

    \node (x6) at (0.5*\ldis+0.22*\sdis,-0.22*\sdis-5.8*\sdis) 
    [label=above: $x_{\upfor}$] {};
    \node (x7) at (0.5*\ldis+1.1*\sdis,0.4*\sdis-5.8*\sdis) 
    [label=above: $x_{\upfif}$] {}; 
    \node (x8) at (0.5*\ldis+1.1*\sdis,-0.4*\sdis-5.8*\sdis) 
    [label=below: $x_{\upsix}$] {}; 
\end{pgfonlayer}
%----------------------------------------------------------------------------

==> figures/lct_examples/scale_large_pesnfg.tex <==
% the distance between h and x
\pgfmathsetmacro{\ldis}{1.5} 
\pgfmathsetmacro{\sdis}{1} 

==> figures/length.tex <==
% the distance between h and x
\pgfmathsetmacro{\ldis}{1} 
\pgfmathsetmacro{\sdis}{0.5} 
\pgfmathsetmacro{\lvaredge}{0.1} 

==> figures/penfg_example_main.tex <==
\begin{figure}[h]
  \centering
  \captionsetup{font=scriptsize}
  \subfloat{
    \input{figures/penfg_example.tex}
  } 
  \subfloat{
    \input{figures/penfg_example_paired_edge.tex}
  } 
  \caption{PE-NFGs in Example~\ref{sec:DENFG:exp:1}.\label{sec:DENFG:fig:1}}
\end{figure}

==> figures/proof_lower_bound/background_nodes_after_lct_proof.tex <==

\foreach{\x} in {0,1}{
    %------------------------------------------------------------------------
    \begin{pgfonlayer}{main}
        \node[] (f3\x) at (-\ldis-2*\sdis,2*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f4\x) at (-\ldis-2*\sdis,-2*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f5\x) at (\ldis+2*\sdis,2*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f6\x) at (\ldis+2*\sdis,-2*\sdis-5.8*\sdis*\x) [] {};
    \end{pgfonlayer}
    %------------------------------------------------------------------------
}
% de[state] (f8) at (\ldis,-2.9*\sdis) [label=left: $ \lambda_{f_{j}} $] {};

\node[state] (f10) at (-\ldis,0) 
[label={[xshift=0.1*\sdis cm] $ \LCT{L}_{ f_{i} } $ }] {};
\node[state] (f20) at (\ldis,0) 
[label={[xshift=0-.1*\sdis cm] $ \LCT{L}_{ f_{j} } $ }] {};
\node[state] (f11) at (-\ldis,-5.8*\sdis) 
[label={[xshift=0.1*\sdis cm,yshift=-1.2*\sdis cm] $ \overline{ \LCT{L}_{ f_{i} } } $ }] {};
\node[state] (f21) at (\ldis,-5.8*\sdis) 
[label={[xshift=-0.1*\sdis cm,yshift=-1.2*\sdis cm] $ \overline{ \LCT{L}_{ f_{j} } } $ }] {};

==> figures/proof_lower_bound/background_nodes_after_lct_proof_s.tex <==

\foreach{\x} in {0,1}{
    %------------------------------------------------------------------------
    \begin{pgfonlayer}{main}
        \node[] (f3\x) at (-\ldis-2.5*\sdis,2.5*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f4\x) at (-\ldis-2.5*\sdis,-2.5*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f5\x) at (\ldis+2.5*\sdis,2.5*\sdis-5.8*\sdis*\x) [] {}; 
        \node[] (f6\x) at (\ldis+2.5*\sdis,-2.5*\sdis-5.8*\sdis*\x) [] {};
    \end{pgfonlayer}
    %------------------------------------------------------------------------
}
% de[state] (f8) at (\ldis,-2.9*\sdis) [label=left: $ \lambda_{f_{j}} $] {};

\node[state] (f10) at (-\ldis,0) 
[label={[xshift=0.1*\sdis cm] $ \LCT{L}_{ f_{i} } $ }] {};
\node[state] (f20) at (\ldis,0) 
[label={[xshift=0-.1*\sdis cm] $ \LCT{L}_{ f_{j} } $ }] {};
\node[state] (f11) at (-\ldis,-5.8*\sdis) 
[label={[xshift=0.1*\sdis cm,yshift=-1*\ldis cm] $ \overline{ \LCT{L}_{ f_{i} } } $ }] {};
\node[state] (f21) at (\ldis,-5.8*\sdis) 
[label={[xshift=-0.1*\sdis cm,yshift=-1*\ldis cm] $ \overline{ \LCT{L}_{ f_{j} } } $ }] {};

==> figures/proof_lower_bound/background_variables_EVD_l.tex <==

\node[] (f22) at (-1.1*\ldis,-2.9*\sdis) [label=right: $ \LCT{\ell}_{f_{i}} $] {};
\node[] (f23) at (1.1*\ldis,-2.9*\sdis) [label=left: $ \LCT{\ell}_{f_{j}} $] {};

\node[] (f22) at (-1.1*\ldis,-0.6*\sdis) [label=right: $ \LCT{\ell}_{f_{i},1}' $] {};
\node[] (f22) at (1.1*\ldis,-0.6*\sdis) [label=left: $ \LCT{\ell}_{f_{j},1}' $] {};

\node[] (f22) at (-1.1*\ldis,-5.2*\sdis) [label=right: $ \LCT{\ell}_{f_{i},2}' $] {};
\node[] (f22) at (1.1*\ldis,-5.2*\sdis) [label=left: $ \LCT{\ell}_{f_{j},2}' $] {};

==> figures/proof_lower_bound/background_variables_EVD_l0.tex <==
\node[] (f22) at (-1.1*\ldis,-2.9*\sdis) [label=right: $ \LCT{\ell}_{f_{i}}\equal0 $] {};
\node[] (f23) at (1.1*\ldis,-2.9*\sdis) [label=left: $ \LCT{\ell}_{f_{j}}\equal 0 $] {};

==> figures/proof_lower_bound/background_variables_EVD_s.tex <==
\node[] (f22) at (-1.2*\ldis,-2.9*\sdis) [label=right: $ \LCT{\ell}_{f_{i}} $] {};
\node[] (f23) at (1.2*\ldis,-2.9*\sdis) [label=left: $ \LCT{\ell}_{f_{j}} $] {};

==> figures/proof_lower_bound/function_otb_lct.tex <==
\node[state] (f32) at (-\ldis,-1.9*\sdis) 
[label={[xshift=0.6*\sdis cm, yshift=-0.1*\sdis cm] $ \LCT{U}_{L,f_{i}} $} ] {};
\node[state] (f33) at (-\ldis,-3.8*\sdis) 
[label={[xshift=0.6*\sdis cm, yshift=-1.1*\sdis cm] $ \overline{\LCT{U}_{L,f_{i}}} $} ] {};

\node[state] (f43) at (\ldis,-1.9*\sdis) 
[label={[xshift=-0.6*\sdis cm, yshift=-0.1*\sdis cm] $ \LCT{U}_{L,f_{j}} $} ] {};
\node[state] (f45) at (\ldis,-3.8*\sdis) 
[label={[xshift=-0.6*\sdis cm, yshift=-1.1*\sdis cm] $ \overline{\LCT{U}_{L,f_{j}}} $}] {};

==> figures/proof_lower_bound/head_files_figs.tex <==
\tikzstyle{state}=[shape=rectangle,fill=white, draw, minimum width=0.2cm, minimum height = 0.2cm,outer sep=-0.3pt]
% the smallest dashed boxes for OTB
\tikzstyle{state_dash1}=[shape=rectangle, draw, dashed, minimum width=1.8*\sdis cm, minimum height = \ldis cm,outer sep=-0.3pt]
% the large dashed boxes for OTB
\tikzstyle{state_dash2}=[shape=rectangle, draw, dashed, minimum width=2*\sdis cm, minimum height = 2*\sdis cm,outer sep=-0.3pt]
% the largest dashed boxes for CTB
% the largest dashed boxes for CTB in S-NFG
\tikzstyle{state_dash3}=[shape=rectangle, draw, dashed, minimum width= 3*\sdis cm, minimum height = 3.3*\sdis cm,outer sep=-0.3pt]

% the largest dashed boxes for CTB in PEs-NFG
\tikzstyle{state_dash4}=[shape=rectangle, draw, dashed, minimum width= 2.5*\sdis cm, minimum height = 3.4*\sdis cm,outer sep=-0.3pt]

% the dashed boxes for OTB of local functions in PEs-NFG
\tikzstyle{state_dash5}=[shape=rectangle, draw, dashed, minimum width= 2.6*\sdis cm, minimum height = 4*\ldis cm,outer sep=-0.3pt]

% the dashed boxes for SST in OTB of local functions in S-NFG

\tikzstyle{state_dash6}=[shape=rectangle, draw, dashed, minimum width= 2.9*\sdis cm, minimum height = 9*\sdis cm,outer sep=-0.3pt]


% for illustrating the quantum information processing system
\tikzstyle{state_long}=[shape=rectangle,draw ,  fill =white, minimum width=0.7cm, minimum height = 0.8cm,outer sep=0pt]

\tikzset{dot/.style={circle,fill=#1,inner sep=0,minimum size=3pt}}

\tikzstyle{state_large}=[shape=rectangle,draw, fill =white, minimum width= 1*\ldis cm, minimum height = 2.4*\ldis cm,outer sep=0pt]

% for graph cover
\tikzstyle{state_large2}=[shape=rectangle,draw, fill =white, minimum width= 0.6*\ldis cm, minimum height = 0.6*\ldis cm,outer sep=0pt]
% for illustrat

==> figures/proof_lower_bound/scale_large_pesnfg.tex <==
% the distance between h and x
\pgfmathsetmacro{\ldis}{1.5} 
\pgfmathsetmacro{\sdis}{0.8} 

==> figures/proof_lower_bound/scale_large_pesnfg_lower_bound.tex <==
% the distance between h and x
\pgfmathsetmacro{\ldis}{1.5} 
\pgfmathsetmacro{\sdis}{0.8} 

==> figures/proof_lower_bound/variables_after_lct_clb_2.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{main} 
    \node (x1) at (0,-0.22*\sdis) 
    [label=above: $\LCT{x}_{1}$] {}; 
    \node (x3) at (-0.57*\ldis-2.3*\sdis,1.4*\sdis) 
    [label=above: $\LCT{x}_{2}$] {}; 
    \node (x4) at (-0.57*\ldis-2.3*\sdis,-1.4*\sdis) 
    [label=below: $\LCT{x}_{3}$] {};

    \node (x3) at (0.57*\ldis+2.3*\sdis,1.4*\sdis) 
    [label=above: $\LCT{x}_{4}$] {}; 
    \node (x4) at (0.57*\ldis+2.3*\sdis,-1.4*\sdis) 
    [label=below: $\LCT{x}_{5}$] {}; 
\end{pgfonlayer}
%----------------------------------------------------------------------------

%----------------------------------------------------------------------------
\begin{pgfonlayer}{main} 
    \node (x1) at (0,-0.22*\sdis-5.8*\sdis) 
    [label=above: $\LCT{x}_{\upone}$] {}; 
    \node (x3) at (-0.57*\ldis-2.3*\sdis,1.4*\sdis-5.8*\sdis) 
    [label=above: $\LCT{x}_{\uptwo}$] {}; 
    \node (x4) at (-0.57*\ldis-2.3*\sdis,-1.4*\sdis-5.8*\sdis) 
    [label=below: $\LCT{x}_{\upthre}$] {};

    \node (x3) at (0.57*\ldis+2.3*\sdis,1.4*\sdis-5.8*\sdis) 
    [label=above: $\LCT{x}_{\upfor}$] {}; 
    \node (x4) at (0.57*\ldis+2.3*\sdis,-1.4*\sdis-5.8*\sdis) 
    [label=below: $\LCT{x}_{\upfif}$] {}; 
\end{pgfonlayer}
%----------------------------------------------------------------------------

==> figures/proof_lower_bound/variables_after_lct_clb_3.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{main} 
    \node (x1) at (0,-0.22*\sdis) 
    [label=above: $\LCT{x}_{1}$] {}; 
    \node (x3) at (-0.57*\ldis-2.8*\sdis,1.5*\sdis) 
    [label=above: $\LCT{x}_{2}$] {}; 
    \node (x4) at (-0.57*\ldis-2.8*\sdis,-1.5*\sdis) 
    [label=below: $\LCT{x}_{3}$] {};

    \node (x3) at (0.57*\ldis+2.8*\sdis,1.5*\sdis) 
    [label=above: $\LCT{x}_{4}$] {}; 
    \node (x4) at (0.57*\ldis+2.8*\sdis,-1.5*\sdis) 
    [label=below: $\LCT{x}_{5}$] {}; 
\end{pgfonlayer}
%----------------------------------------------------------------------------

%----------------------------------------------------------------------------
\begin{pgfonlayer}{main} 
    \node (x1) at (0,-0.22*\sdis-5.8*\sdis) 
    [label=above: $\LCT{x}_{\upone}$] {}; 
    \node (x3) at (-0.57*\ldis-2.8*\sdis,1.5*\sdis-5.8*\sdis) 
    [label=above: $\LCT{x}_{\uptwo}$] {}; 
    \node (x4) at (-0.57*\ldis-2.8*\sdis,-1.5*\sdis-5.8*\sdis) 
    [label=below: $\LCT{x}_{\upthre}$] {};

    \node (x3) at (0.57*\ldis+2.8*\sdis,1.5*\sdis-5.8*\sdis) 
    [label=above: $\LCT{x}_{\upfor}$] {}; 
    \node (x4) at (0.57*\ldis+2.8*\sdis,-1.5*\sdis-5.8*\sdis) 
    [label=below: $\LCT{x}_{\upfif}$] {}; 
\end{pgfonlayer}
%----------------------------------------------------------------------------

==> figures/sst_examples/denfg/OTB_back_nodes_lines.tex <==
% For illustrate SST
\begin{pgfonlayer}{behind}
  \foreach \x in {0,1}{
    \node[state] (eqn\x) at (0,\x*2*\ldis) [] {$=$};
  }
\end{pgfonlayer}

\begin{pgfonlayer}{background}
  \draw[] (eqn1) -- (Psige);
\end{pgfonlayer}

==> figures/sst_examples/denfg/OTB_pe.tex <==
\begin{pgfonlayer}{behind}
  \foreach \x in {0,1}{
    \node[state] (psi\x) at (-\sdis,\x*2*\ldis) [label=below: $\cpsi_{e}$] {};
    \node[state] (cpsi\x) at (\sdis,\x*2*\ldis) [label=below: $\overline{\cpsi_{e}}$] {};
  }  
\end{pgfonlayer}


==> figures/sst_examples/denfg/background_nodes_lines.tex <==
\foreach \x in {0,1}{
  %----------------------------------------------------------------------------
  \begin{pgfonlayer}{main}
    \node[state] (f1\x) at (-\ldis,\x*2*\ldis) [label=above: $f_{i,\x}$] {};
    \node[state] (f2\x) at (\ldis,\x*2*\ldis) [label=above: $f_{j,\x}$] {};
    \node[] (f3\x) at (-2*\ldis,\ldis+\x*2*\ldis) [] {}; 
    \node[] (f4\x) at (-2*\ldis,-\ldis+\x*2*\ldis) [] {}; 
    \node[] (f5\x) at (2*\ldis,\ldis+\x*2*\ldis) [] {}; 
    \node[] (f6\x) at (2*\ldis,-\ldis+\x*2*\ldis) [] {}; 
  \end{pgfonlayer}
  %----------------------------------------------------------------------------
  \begin{pgfonlayer}{background}
    \draw[double]
      (f1\x) -- (f3\x)
      (f1\x) -- (f4\x)
      (f2\x) -- (f5\x)
      (f2\x) -- (f6\x);
  \end{pgfonlayer}
  %----------------------------------------------------------------------------
}


==> figures/sst_examples/denfg/length.tex <==
% the distance between h and x
\pgfmathsetmacro{\ldis}{1} 
\pgfmathsetmacro{\sdis}{0.5} 

==> figures/sst_examples/denfg/lines_not_permuted.tex <==
\foreach \x in {0,1}{
  %----------------------------------------------------------------------------
  \begin{pgfonlayer}{behind}
    \draw[double]
      (f1\x) -- (f2\x);
  \end{pgfonlayer}
  %----------------------------------------------------------------------------
}

==> figures/sst_examples/denfg/main_pic.tex <==
\begin{figure}[t]
  \captionsetup{font=scriptsize}
  \subfloat[]{
    \begin{minipage}[t]{0.9\textwidth}
      \centering
      \begin{tikzpicture}[node distance=2cm, on grid,auto]
        \input{figures/head_files_figs.tex}
        \input{figures/sst_examples/denfg/length.tex}
        \input{figures/sst_examples/denfg/pic_1.tex}
      \end{tikzpicture}
    \end{minipage}
  }

  \subfloat[]{
    \begin{minipage}[t]{0.45\textwidth}
      \centering
      \begin{tikzpicture}[node distance=2cm, on grid,auto]
        \input{figures/head_files_figs.tex}
        \input{figures/sst_examples/denfg/length.tex}
        \input{figures/sst_examples/denfg/background_nodes_lines.tex}
        \input{figures/sst_examples/denfg/lines_not_permuted.tex}
      \end{tikzpicture}
    \end{minipage}
  }
  \subfloat[]{
    \begin{minipage}[t]{0.45\textwidth}
      \centering
      \begin{tikzpicture}[node distance=2cm, on grid,auto]
        \input{figures/head_files_figs.tex}
        \input{figures/sst_examples/denfg/length.tex}
        \input{figures/sst_examples/denfg/background_nodes_lines.tex}
        %--------------------------------------------------------------------
        \begin{pgfonlayer}{background} 
          \foreach \x in {0,1}{
            \coordinate (f7\x) at (-1*0.5*\ldis,\x*2*\ldis) ; 
            \coordinate (f8\x) at (0.5*\ldis,\x*2*\ldis) ; 
          }
          \draw[double]
            (f10) -- (f70) -- (f81) -- (f21); 
        \end{pgfonlayer}
        %--------------------------------------------------------------------
        \begin{pgfonlayer}{behind}
          \draw[double] 
          (f11) -- (f71) -- (f80) -- (f20);
        \end{pgfonlayer}
      \end{tikzpicture}
    \end{minipage}
  }

  \subfloat[]{
    \begin{minipage}[t]{0.45\textwidth}
      \centering
      \begin{tikzpicture}[node distance=2cm, on grid,auto]
        \input{figures/head_files_figs.tex}
        \input{figures/sst_examples/denfg/length.tex}
        \input{figures/sst_examples/denfg/background_nodes_lines.tex}
        \input{figures/sst_examples/denfg/lines_not_permuted.tex}
        \input{figures/sst_examples/denfg/node_pe_sige.tex}
      \end{tikzpicture}
    \end{minipage}
  }
  \subfloat[]{
    \begin{minipage}[t]{0.45\textwidth}
      \centering
      \begin{tikzpicture}[node distance=2cm, on grid,auto]
        \input{figures/head_files_figs.tex}
        \input{figures/sst_examples/denfg/length.tex}
        \input{figures/sst_examples/denfg/background_nodes_lines.tex}
        \input{figures/sst_examples/denfg/lines_not_permuted.tex}
        \input{figures/sst_examples/denfg/node_pe_sige.tex}
      \end{tikzpicture}
    \end{minipage}
  }

  \subfloat[]{
    \begin{minipage}[t]{0.3\textwidth}
      \centering
      \begin{tikzpicture}[node distance=2cm, on grid,auto]
        \tikzstyle{state_dash4}=[shape=rectangle, draw, dashed, minimum width= 1.4*\ldis cm, minimum height = 4.5*\ldis  cm,outer sep=-0.3pt]
        \input{figures/head_files_figs.tex}
        \input{figures/sst_examples/denfg/length.tex}
        \input{figures/sst_examples/denfg/background_nodes_lines.tex}
        \input{figures/sst_examples/denfg/lines_not_permuted.tex}
        \input{figures/sst_examples/denfg/node_pe_sige.tex}
        \begin{pgfonlayer}{background}
          \node[state_dash6] (db1) at (0,0.1*\ldis) [label=below:$P_{e}$] {};
          \node[] (var1) at (-0.18*\ldis,-1*\ldis) [label=right: $\sigma_{e}$] {};
           \node[state] (Psige) at (0,-1.5*\ldis) [label=below: $p_{\Sigma(e)}$] {};
        \end{pgfonlayer}
        \input{figures/sst_examples/denfg/otb_back_nodes_lines.tex}
      \end{tikzpicture}
    \end{minipage}
  }
  \subfloat[]{
    \begin{minipage}[t]{0.3\textwidth}
      \centering
      \begin{tikzpicture}[node distance=2cm, on grid,auto]
        \input{figures/head_files_figs.tex}
        \input{figures/sst_examples/denfg/length.tex}
        \input{figures/sst_examples/denfg/background_nodes_lines.tex}
        \input{figures/sst_examples/denfg/lines_not_permuted.tex}
        % \input{figures/sst_examples/denfg/otb_pe.tex}
        \begin{pgfonlayer}{above}
          \node[state_large] (db1) at (0,1*\ldis) [label=below:$P_{e}$] {};
        \end{pgfonlayer}
      \end{tikzpicture}
    \end{minipage}
  }
  \subfloat[]{
    \begin{minipage}[t]{0.3\textwidth}
      \centering
      \begin{tikzpicture}[node distance=2cm, on grid,auto]
        \input{figures/head_files_figs.tex}
        \input{figures/sst_examples/denfg/length.tex}
        \input{figures/sst_examples/denfg/background_nodes_lines.tex}
        \input{figures/sst_examples/denfg/lines_not_permuted.tex}
        % \input{figures/sst_examples/denfg/otb_pe.tex}
        \node[] (var1) at (-0.18*\ldis,-1*\ldis) [label=right: $\cvpsi_{e}$] {};
        \node[state] (Psige) at (0,-1.5*\ldis) [label=below: $\muFSsimple$] {};
        \input{figures/sst_examples/denfg/otb_back_nodes_lines.tex}
      \end{tikzpicture}
    \end{minipage}
  }
  \caption{Partial DE-NFGs illustrating the SST.  (See main text for details.)\label{sec:SST:fig:2}}
\end{figure}


==> figures/sst_examples/denfg/node_pe_sige.tex <==
% For illustrate SST
\tikzstyle{state_large}=[shape=rectangle,draw, fill =white, minimum width=1*\ldis cm, minimum height = 2.4*\ldis cm,outer sep=0pt]
\begin{pgfonlayer}{main}
  \node[state_large] (Pe) at (0,\ldis) [] {$P_{e,\sigma_e}$};
\end{pgfonlayer}

==> figures/sst_examples/denfg/pic_1.tex <==
%----------------------------------------------------------------------------
\begin{pgfonlayer}{behind}
  \node[state] (f1) at (-\ldis,0) [label=above: $f_{i}$] {};
  \node[state] (f2) at (\ldis,0) [label=above: $f_{j}$] {};
  \node[] (f3) at (-2*\ldis,\ldis) [] {}; 
  \node[] (f4) at (-2*\ldis,-\ldis) [] {}; 
  \node[] (f5) at (2*\ldis,\ldis) [] {}; 
  \node[] (f6) at (2*\ldis,-\ldis) [] {}; 
\end{pgfonlayer}
%----------------------------------------------------------------------------
\begin{pgfonlayer}{background}
  \draw[double]
    (f1) --  (f2)
    (f1) -- (f3)
    (f1) -- (f4)
    (f2) -- (f5)
    (f2) -- (f6);
\end{pgfonlayer}
%----------------------------------------------------------------------------

==> graph_cover_thm_denfg.tex <==
In this section, we present a proof for Conjecture~\ref{sec:GraCov:conj:1}, \ie, the graph-cover theorem, for the DE-NFGs satisfying an easily checkable condition. In Conjecture~\ref{sec:GraCov:conj:1}, we conjecture that for some DE-NFG $ \graphN $, the limit in~\eqref{sec:CheckCon:eqn:25} holds
% %---------------------------------------------------------------------------
% \begin{align}
%     \limsup_{M \to \infty} \ZBM(\graphN) = \ZBSPA^{*}(\graphN). 
    
% \end{align}
%---------------------------------------------------------------------------
% where $ \ZBM(\graphN) $ is defined in Definition~\ref{sec:GraCov:def:2} and $ \ZBSPA^{*}(\graphN) $ is defined in Definition~\ref{sec:DENFG:def:3}.
% Although the expression of $\ZBM(\graphN)$ 
% in Proposition~\ref{prop:altenative expression of ZBM by eigenvalue decomposition and SST}, thanks to the SST, is
% interesting, it is generally challenging to analyze this expression in the limit 
% $M \to \infty$. However, if we apply the SST after applying the LCT to every $M$-cover of $\graphN$, we obtain expressions that are easier to analyze.
%***************************************************************************
This section is organized as follows.

\begin{enumerate}

  \item \textbf{Application of the LCT}: We begin by applying the LCT to a DE-NFG $ \graphN $, based on an SPA fixed point that achieves $ \ZBSPA^{*}(\graphN) $. The resulting factor graph is denoted by $ \LCT{\graphN} $. Recall in Proposition~\ref{prop:DENFG:LCT:1}, we establish that $ \ZBM(\graphN) = \ZBM\bigl( \LCT{\graphN} \bigr) $ for any $ M \in \sZpp $.

  % \item \textbf{Application of the SST}: Next, we apply the SST to $ \LCT{\graphN} $, leading to a factor graph denoted by $ \LCTavgalt{\graphN}$. Following the similar idea as in Section~\ref{sec:SST}, we obtain $ \ZBM\bigl( \LCT{\graphN} \bigr) = \sqrt[M]{Z\bigl( \LCTavgalt{\graphN}\bigr)} $. 

  \item \textbf{Limit Evaluation}: In order to establish the limit stated in~\eqref{sec:CheckCon:eqn:25}, we need to evaluate $ \ZBM(\graphN) $ as $ M \to \infty $. We propose a checkable sufficient condition based on the local functions in the LCT-transformed DE-NFG  $ \LCT{\graphN} $, which ensures that $ \lim_{M \to \infty}\ZBM\bigl( \LCT{\graphN} ) = \ZBSPA^{*}( \graphN ) $.
\end{enumerate}
%***************************************************************************
%***************************************************************************


The considered setup is given as follows.
%---------------------------------------------------------------------------
\begin{itemize}
    \item Consider an arbitrary DE-NFG $\graphN$.

    \item Assume that among all fixed-point SPA message vectors for $\graphN$, we obtain a vector $\vmu$ that achieves the maximum value of $\ZBSPA(\graphN,\vmu)$, \ie,
    %-----------------------------------------------------------------------
    \begin{align*}
         \ZBSPA(\graphN,\vmu) = \ZBSPA^{*}(\graphN) \in \sR_{\geq 0}, \qquad 
         Z_{e}(\vmu) >0, \qquad e \in \setEfull.
    \end{align*}
    %-----------------------------------------------------------------------
    (See also Definition~\ref{sec:DENFG:def:3} and Remark~\ref{sec:DENFG:remk:1}.) 

    \item We apply the LCT w.r.t. $\vmu$ on $\graphN$, resulting in a new DE-NFG denoted as $ \LCT{\graphN} $. We recall the properties of $ \LCT{\graphN} $, which are summarized in Proposition~\ref{prop:DENFG:LCT:1}, 
    as follows.
    %----------------------------------------------------------------------------
    \begin{itemize}

       \item It holds that $ Z\bigl( \LCT{\graphN} \bigr) = Z(\graphN) $.

       \item The fixed-point SPA message vector $\vmu$ induces an SPA fixed-point message vector
        $\LCTv{\mu} = \bigl( \LCTv{\mu}_{\ef} \bigr)_{ e \in \setpf,\, f \in \setF}$ for
        $\LCT{\graphN}$, which has a simple structure:
        %-------------------------------------------------------------------
        \begin{align*}
            \LCTv{\mu}_{\ef}
            = \begin{pmatrix}
                1, & 0, & \cdots & 0
            \end{pmatrix}^{\!\! \tran}
            \in \sR^{|\LCTtset{X}_{e}|},
            \qquad
            e \in \setpf,\, f \in \setF.  \nonumber
        \end{align*}
        %-------------------------------------------------------------------
       % \item There is a bijection between the set of fixed-point SPA message vectors for $ \graphN $ and the set of fixed-point SPA message vectors for $\LCT{\graphN}$. Therefore, following the definition of $ \ZBSPA^{*} $ in Definition~\ref{sec:DENFG:def:3}, we obtain
       This simple structure implies
        %-----------------------------------------------------------------------
        \begin{align}
            \ZBSPA^{*}(\graphN)
            % = \ZBSPA^{*}\bigl( \LCT{\graphN} \bigr)
            = \ZBSPA(\graphN,\vmu)
            = \ZBSPA(\LCT{\graphN}, \LCTv{\mu})
            =
            \prod_{f} \LCT{f}(\bm{0}) \in \sR_{\geq 0},
            \label{sec:CheckCon:eqn:31}
        \end{align}
        where the last inequality follows from Remark~\ref{sec:DENFG:remk:1}. 
   \end{itemize}
   %----------------------------------------------------------------------------
    
    \item For each $ M \in \sZpp $, we consider a degree-$M$ finite graph cover, 
    denoted as $ \hLCTgraphN $, of $ \LCT{\graphN} $. This graph cover is specified by a collection of permutations 
    $ \vsigma = (\sigma_e)_{e \in \setEfull} 
    \in \set{S}^{|\setEfull|}_{M} $.

    The collection of vectors given by
    %-----------------------------------------------------------------------
    \begin{align*}
        \hat{\LCTv{\mu}}_{(e,m),(f_{i},m)}=
        \hat{\LCTv{\mu}}_{(e,m),(f_{j},\sigma_{e}(m))}
        = \begin{pmatrix}
            1, & 0, & \cdots & 0
        \end{pmatrix}^{\!\!\! \tran},
        \,\, m \in [M],\, e = (f_{i},f_{j}) \in \setEfull
    \end{align*}
    %-----------------------------------------------------------------------
    represents a collection of fixed-point SPA message vectors for $ \hLCTgraphN $.
    Here, $ \hat{\LCTv{\mu}}_{(e,m),(f_{i},m')} $ denotes the SPA message vector from edge $ (e,m) $ to local function $ (f_{i},m') $ for $ m, m' \in [M] $.
    (Because an $M$-cover of $\hLCTgraphN$ looks locally the same as the base graph $\LCT{\graphN}$, the SPA fixed-point vector $ \LCTv{\mu}$ for $\LCT{\graphN}$ yields an SPA fixed point vector $\hat{\LCTv{\mu}}$ for $\hLCTgraphN$ simply by repeating every message $M$ times.\footnote{This observation was the original motivation for the graph cover analysis of message-passing iterative decoders~\cite{Koetter2003,Koetter2007}.}) 


    \item The degree-$M$ Bethe partition functions of $ \graphN $ and 
        $ \LCT{\graphN} $ are equal, \ie,
    %-----------------------------------------------------------------------
    \begin{align*}
        \ZBM(\graphN) 
        &\overset{(a)}{=} \sqrt[M]{
          \bigl\langle
             Z\bigl( \hgraphN \bigr)
           \bigr\rangle_{ \hgraphN \in \hat{\set{N}}_{M}}
        }
        \overset{(b)}{=} \sqrt[M]{
            \Bigl\langle
                Z\bigl( \hLCTgraphN \bigr)
            \Bigr\rangle_{ \hLCTgraphN \in \hLCT{\set{N}}_{M} }
        }
        \overset{(c)}{=} \ZBM\bigl( \LCT{\graphN} \bigr) ,\quad M \in \sZpp,  \nonumber
    \end{align*}
    %----------------------------------------------------------------------
    where step $(a)$ follows from the definition of the function $ \ZBM $ in Definition~\ref{sec:GraCov:def:2}, where step $(b)$ follows from Proposition~\ref{prop:DENFG:LCT:1},
    and where step $(c)$ again follows from~Definition~\ref{sec:GraCov:def:2}.

    \item In the following, we evaluate $ \ZBM\bigl( \LCT{\graphN} \bigr) $ as $ M \to \infty $.

    % %----------------------------------------------------------------------------
    % \begin{itemize}
    %     \item 
    %     \item 

    %     % \item Following the similar idea of Lemmas~\ref{sec:SST:lem:1} and~\ref{sec:SST:lem:6}, the $M$-th power of the degree-$M$ Bethe partition can be written as
    %     % \begin{align*}
    %     %     \ZBM(\graphN) 
    %     %     = Z\bigl( \hgraphNavg \bigr) 
    %     %     =
    %     %      \sum_{ \LCTvxsM, \LCTvxlM }
    %     %       \Biggl( 
    %     %         \prod_{m \in [M]} \prod_{f} 
    %     %         \LCT{f}( \LCTtv{x}_{\setpf,f,m}) 
    %     %       \Biggr) 
    %     %       \cdot \prod_{e = (f_{i},f_{j})} 
    %     %       P_{e}(\LCTtv{x}_{\efi,[M]}, \LCTtv{x}_{\efj,[M]})
    %     % \end{align*}
    
    % \end{itemize}
    % %---------------------------------------------------------------------------- 
    (Note that the order of operations, namely constructing a graph cover and applying the LCT, does not affect the resulting degree-$M$ Bethe partition function. In other words, changing the order of these two operations does not alter the outcome.)
\end{itemize}

%---------------------------------------------------------------------------
\begin{theorem}\label{sec:CheckCon:thm:1}
  \label{SEC:CHECKCON:THM:1}
  \index{Graph-cover theorem!for special DE-NFG}
  Consider a DE-NFG $ \graphN $, along with its associated LCT-transformed DE-NFG $ \LCT{\graphN} $. If 
  the following checkable inequality is satisfied:
  %-----------------------------------------------------------------------
  \begin{align}
    \frac{3}{2}
    \cdot \ZBSPA^{*}(\graphN)
    &>
    \prod_{f}
     \left( 
        \sum_{\LCTtv{x}_{\setpf}}
        |\LCT{f}( \LCTtv{x}_{\setpf} )|
    \right)
    % \Biggr),
    % \sum_{ \LCTvxs, \LCTvxl }
    % \bigl|G_{ \LCTzero{\graphN}, 1 }( \LCTvxs, \LCTvxl )\bigr|,
    \label{sec:CheckCon:eqn:70}
  \end{align}
  %-----------------------------------------------------------------------
  then we have
  %-----------------------------------------------------------------------
  \begin{align*}
    \lim_{M \to \infty}
    \ZBM(\graphN)
    = \lim_{M \to \infty}
    \ZBM(\LCT{\graphN})
    = \ZBSPA^{*}(\graphN). 
  \end{align*}
  %-----------------------------------------------------------------------
  % {\color{red}(whether $\limsup$ or $ \liminf $, we will come back later)}
\end{theorem}
%---------------------------------------------------------------------------
%---------------------------------------------------------------------------
\begin{proof}
  See Appendix~\ref{apx:check_graph_thm}.
\end{proof}
%---------------------------------------------------------------------------


==> index.tex <==
%!TEX root = main.tex
% Sample index entry LaTeX code:
\begin{itemize}[label={}]

\item Bethe free energy function 
  \subitem for S-NFG, \pageref{sec:SNFG:def:1}
  \subitem for S-NFG associated with the matrix permanent, \pageref{sec:SNFG:def:1}

\item Bethe partition function 
  \subitem for S-NFG, \pageref{sec:SNFG:eqn:4}
  \subitem for S-NFG associated with the matrix permanent, \pageref{sec:1:eqn:192}
 
\indexspace
  \item Degree-$M$ Bethe permanent, \pageref{def:matrix:degree:M:cover:1}

\indexspace
  \item Degree-$M$ (scaled) Sinkhorn permanent, \pageref{def:Sinkhorn:degree:M:cover:1}

\indexspace
  \item DE-NFG, \pageref{sec:DENFG:def:4}

\indexspace
  \item Finite graph covers, \pageref{sec:GraCov:def:1}

\indexspace
  \item Graph-cover theorem
  \subitem for S-NFG, \pageref{sec:GraCov:thm:1}
  \subitem for S-NFG associated with the matrix permanent, \pageref{sec:1:thm:8}
  \subitem for special DE-NFG, \pageref{sec:CheckCon:thm:1}

\indexspace
  \item Gibbs free energy function,
  \subitem for S-NFG associated with the matrix permanent, \pageref{sec:1:def:18}, \pageref{sec:1:def:18:part:2}

\indexspace
\item LCT
  \subitem for S-NFG, \pageref{sec:LCT:def:1}
  \subitem for DE-NFG, \pageref{def:DENFG:LCT:1}
 
\indexspace
  \item Partition function
  \subitem for S-NFG \pageref{partition function of snfg},
  \subitem for S-NFG associated with the matrix permanent, \pageref{partition function of N theta}, \pageref{sec:1:def:18:part:2}
  \subitem for DE-NFG \pageref{partition function of denfg},

\indexspace
  \item Permanent of a non-negative square matrix, \pageref{chapt:intro:permanent}

\indexspace
  \item Pseudo-dual Bethe partition function
    \subitem for S-NFG, \pageref{sec:SNFG:def:2}
    \subitem for DE-NFG, \pageref{sec:DENFG:def:3}

\indexspace
  \item Scaled Sinkhorn free energy function
  \subitem for S-NFG associated with the matrix permanent, \pageref{sec:1:def:20}

\indexspace
\item S-NFG
  \subitem general definition, \pageref{def: def of snfg}
  \subitem definition associated with the matrix permanent, \pageref{def: details of S-NFG of permanent}


\indexspace
\item SPA
  \subitem for S-NFG, \pageref{sec:SNFG:def:4}
  \subitem for DE-NFG, \pageref{sec:DENFG:def:2}

\indexspace
\item SST
  \subitem for S-NFG, \pageref{sec:SST:def:5}
  \subitem for DE-NFG, \pageref{sec:SST:DENFG:1}

\end{itemize}
% \begin{xltabular}{\textwidth}{L|R}
%   % \multicolumn{2}{l}{\textbf{\Large Mathematics}}
%   % \\
%   \hline
%   DE-FG & double-edge factor graph
%   \\ \hline 
%   DE-NFG & double-edge normal factor graph
%   \\ \hline 
%   LBP & loopy belief propagation 
%   \\ \hline
%   LCT & loop calculus transform
%   \\ \hline 
%   LCT & loop calculus transform
%   \\ \hline 
%   NFG & normal factor graph
%   \\ \hline 
%   PSD & positive semi-definite
%   \\ \hline
%   S-FG & standard factor graph
%   \\ \hline
%   S-NFG & standard normal factor graphs
%   \\ \hline
%   SPA & sum-product algorithm 
%   \\ \hline
%   SST & symmetric-subspace transform
%   \\ \hline 
% \end{xltabular}

==> introduction.tex <==
Standard factor graphs (S-FGs)~\cite{Kschischang2001, Forney2001,Loeliger2004}, \ie, factor graphs with local functions taking on
non-negative real values, are used for representing statistical models.\footnote{In this thesis, we consider the factor graphs in both the classical case and the quantum case. In the classical case, we consider S-FGs, whereas in the quantum case, we consider double-edges factor graphs.} They have wide applications in different areas including statistical mechanics (see, \textit{e.g.},~\cite{Mezard2009}), coding theory (see, \textit{e.g.}, \cite{Richardson2008}), and communications (see, \textit{e.g.}, \cite{Wymeersch2007}). Many typical inference problems in these areas are equivalent to computing the marginals and the partition functions of the global functions represented by the S-FGs. Because the exact 
computation of the partition functions is generally challenging, in order to approximate these quantities efficiently, a popular choice is the sum-product algorithm (SPA), also known as loopy belief propagation (LBP). The SPA is a heuristic algorithm and has been successfully used for approximating the marginal functions and the partition functions for many classes of S-FGs.
  

%***************************************************************************
There are various characterizations of the pseudo-marginal functions obtained via an SPA fixed point. When an S-FG is cycle-free, \ie, tree-structured, the pseudo-marginal
functions evaluated at the SPA fixed point are the exact marginal functions of the global function represented by the S-FG~\cite{Mezard2009}. As for the S-FGs with cycles, the SPA often provides a surprisingly good approximation of the associated marginals and partition functions. Motivated by Bethe's famous approximation method for magnets~\cite{Bethe1935},
Yedidia \etal~in~\cite{Yedidia2005} defined the Bethe free energy function for an S-FG and~gave a theoretical justification of the SPA by showing that, roughly speaking, the SPA's fixed points correspond to the Bethe free energy function's stationary points. Because of this connection between the SPA and the Bethe free energy function, the approximation of the partition function in the Bethe approach can be solved with the help of the SPA, and it is often called the Bethe approximation of the partition function, or simply the Bethe partition
function. In~\cite{Chertkov2006, Chernyak2007}, Chertkov and Chernyak
presented a technique they called loop calculus that yields an expression
relating the partition function to the Bethe partition function. 
This expression provides an exact representation
of the partition function as a sum of terms, with the first term
corresponding to the Bethe partition function and higher-order
terms obtained by adding so-called loop corrections. Based on the concepts from information geometry,
Mori in~\cite{Mori2015} extended the results obtained by Chertkov and Chernyak to S-FGs with non-binary
alphabets by applying a local linear transformation in these S-FGs. Similar ideas also appear in \cite{Altieri2017,Angelini2022}.

%***************************************************************************

Finite graph covers of S-FGs are a useful theoretical tool~\cite{Koetter2007,
Vontobel2013,Ruozzi2013,Shams2019,Ruozzi2009} for understanding the SPA and the Bethe partition function. 
%----------------------------------------------------------------------------
\begin{itemize}
  \item Ruozzi \etal~in~\cite{Ruozzi2009} 
  used graph covers to characterize the behavior of the max-product
  algorithm for Gaussian graphical models. (For Gaussian graphical models, the
  max-product algorithm is essentially equivalent to the sum-product algorithm.)
  Similarly, in order to understand SPA's behavior, Koetter \etal~studied
  the finite graph covers of the S-FGs representing low-density parity-check (LDPC) 
  codes in~\cite{Koetter2007}.

  \item A combinatorial characterization of an S-FG's Bethe partition function in terms of the associated finite graph covers' partition functions was given in~\cite{Vontobel2013}. Leveraging this result, Ruozzi \etal~in~\cite{Ruozzi2012} and Csikv\'{a}ri \etal~in~\cite{Csikvari2022} 
  proved that the partition functions is lower bounded by the Bethe partition functions
  for certain classes of S-FGs, in particular solving a conjecture by Sudderth
  \etal\ about log-supermodular graphical
  models~\cite{E.B.Sudderth2007}. 
\end{itemize}
%----------------------------------------------------------------------------
 

In this thesis, we also use the finite graph cover to study the SPA and the relationship between the Bethe partition function and partition function for factor graphs representing classical and quantum information processing systems.
%----------------------------------------------------------------------------
\begin{itemize}
  \item Vontobel in~\cite{Vontobel2013a} introduced a class of S-FGs such that each S-FG's partition function is equal to the permanent of a non-negative square matrix.  
  Gurvits~\cite{Gurvits2011} proved that for this class of S-FGs, each S-FG's partition function is lower bounded by the associated Bethe partition function. Similar to~\cite{Ruozzi2012,Csikvari2022}, we show that there is a combinatorial characterization of this lower bound in terms of the finite graph covers. The detailed discussion of this characterization is in Section~\ref{sec: degree M charactertion of Bethe and Sinkhorn permanent}.

  \item Recently, Cao and Vontobel in~\cite{Cao2017} introduced more general factor graphs, namely double-edge factor graphs (DE-FGs), in order to representing quantities of interest in quantum information processing. A natural question is that whether
  there is also a combinatorial characterization of a DE-FG's Bethe partition function in terms of the associated finite graph covers. Such characterization can be viewed as a generalization of the combinatorial characterization proven in~\cite{Vontobel2013} for S-FGs. The detailed discussion of the combinatorial characterization of a DE-FG's Bethe partition function is in Section~\ref{intro: characterize ZB for DE-FG}.
\end{itemize}
%----------------------------------------------------------------------------

\section[Finite-Graph-Cover-Based Bounds on the Permanent]{\texorpdfstring{Degree-$M$}{} Bethe and Sinkhorn Permanent Based Bounds on the Permanent of a Non-negative Matrix}\label{sec: degree M charactertion of Bethe and Sinkhorn permanent}

In this section, we present finite-graph-cover-based bounds on the permanent of a nonnegative, square matrix. We first introduce the permanent of a non-negative square matrix in Section~\ref{chapt:intro:permanent}. Then in Section~\ref{chapt:intro:Bethe permanent}, we discuss the Bethe permanent, which is known as an S-FG based approximation of the matrix permanent. Based on the degree-$M$ finite graph covers of the S-FG, in Section~\ref{chapt: permanent: combinartorial chara of ZB and ZscC}, we introduce the degree-$M$ Bethe permanent and show that the degree-$M$ Bethe permanent provides a combinatorial characterization of the Bethe permanent. In Section~\ref{sec:main:constributions:1}, we present the degree-$M$ Bethe permanent based bounds on the matrix permanent. Moreover, we show that similar results also hold for the (scaled) Sinkhorn permanent~\cite{N.Anari2021}, which is another S-FG based approximation of the matrix permanent.

\subsection{The permanent of a square matrix}
\label{chapt:intro:permanent}

For any $n \in \sZpp$, define $[n] \defeq \{ 1, 2, \ldots, n \}$ and let
$\setS_{[n]}$ be the set of all $n!$ bijections from $[n]$ to $[n]$. Recall
the definition of the permanent of a real square matrix (see, \eg,
\cite{Minc1984}).

%***************************************************************************

\begin{definition}\label{sec:1:def:13}
  Let $n \in \sZpp$ and let
  $ \mtheta \defeq \bigl( \theta(i,j) \bigr)_{\! i,j\in [n]}$ be a real matrix of
  size $n \times n$. The permanent of $ \mtheta $ is defined to be
  \begin{align}
    \perm(\mtheta)
      &\defeq
         \sum_{\sigma \in \setS_{[n]}} 
           \prod_{i \in [n]}
             \theta\bigl( i, \sigma(i) \bigr) .
               \label{eq:def:permanent:1} \\[-1.00cm] \nonumber
  \end{align}
  \edefinition
\end{definition}

%***************************************************************************

In this thesis, we consider only the matrix $\mtheta$ such that there is at least one
$\sigma \in \setS_{[n]}$ such that
$\prod_{i \in [n]} \theta\bigl( i, \sigma(i) \bigr) \neq 0$.

%In this thesis, we consider only matrices $\mtheta$ where
%$\perm(\mtheta) \neq 0$.

%***************************************************************************

Computing the exact permanent is in the complexity class \#P, where \#P is the
set of the counting problems associated with the decision problems in the
class NP. Notably, already the computation of the permanent
of matrices that contain only zeros and ones is \#P-complete~\cite{Valiant1979}.

%***************************************************************************

\subsection{The Bethe Permanent and the (Scaled) Sinkhorn Permanent of a non-negative square matrix}
\label{chapt:intro:Bethe permanent}

While being able to compute the exact permanent of a matrix might be desirable
in some circumstances, many applications require only a good approximation of
the permanent. In this thesis, we focus on the important special
case of approximating the permanent of a non-negative real matrix, \ie, a
matrix where all entries are non-negative real numbers. In particular, we
study two graphical-model-based methods for approximating the permanent of a
non-negative matrix. The first method is motivated by Bethe-approximation /
SPA based methods proposed in~\cite{Chertkov2008,
  Huang2009} and studied in more detail in~\cite{Vontobel2013a}. The second
method is motivated by Sinkhorn's matrix scaling algorithm~\cite{Linial2000}.

%***************************************************************************

The main idea of these methods is to construct an S-FG~\cite{Forney2001, Loeliger2004} whose partition
function equals the permanent.
Consequently, the permanent can be obtained by
finding the minimum of the Gibbs free energy function associated with the
factor graph. However, because finding the minimum of the Gibbs free energy
function is in general intractable unless $n$ is small, one considers the
minimization of some functions that suitably approximate the Gibbs free energy
function.

%***************************************************************************

A first approximation of the Gibbs free energy function is given by the Bethe
free energy function~\cite{Yedidia2005}; the resulting approximation of
$\perm(\mtheta)$ is called the Bethe permanent and denoted by
$ \permb(\mtheta)$. Vontobel~\cite{Vontobel2013a} showed that for the relevant
factor graph, the Bethe free energy function is convex and that the SPA
converges to its minimum.
(This is in contrast to the situation for factor
graphs in general, where the Bethe free energy function associated with a
factor graph is not convex and the SPA is not guaranteed to converge to its
minimum.) The Bethe permanent $\permb(\mtheta)$ satisfies
\begin{align}
  1 
    &\leq 
       \frac{\perm(\mtheta)}{ \permb(\mtheta)} 
     \leq 
        2^{n/2}.
        \label{eq:ratio:permanent:bethe:permanent:1}
\end{align}
The first inequality in~\eqref{eq:ratio:permanent:bethe:permanent:1} was
proven by Gurvits~\cite{Gurvits2011} with the help of an inequality of
Schrijver~\cite{Schrijver1998}. Later on, an alternative proof based on
results from real stable polynomials was given by Straszak and Vishnoi
in~\cite{Straszak2019} and Anari and Gharan in~\cite{Anari2021}. The second
inequality in~\eqref{eq:ratio:permanent:bethe:permanent:1} was conjectured by
Gurvits~\cite{Gurvits2011} and proven by Anari and
Rezaei~\cite{Anari2019}. Both inequalities
in~\eqref{eq:ratio:permanent:bethe:permanent:1} are the best possible given
only the knowledge of the size of the matrix~$\mtheta$.


A second approximation of the Gibbs free energy function is given by the
Sinkhorn free energy function; the resulting approximation of $\perm(\mtheta)$
is called the Sinkhorn permanent and denoted by $\perms(\mtheta)$. (The
Sinkhorn free energy function was formally defined in~\cite{Vontobel2014}
based on some considerations in~\cite{Huang2009}. Note that
  $\perms(\mtheta)$ appears already in~\cite{Linial2000} as an approximation
  of $\perm(\mtheta)$ without being called the Sinkhorn permanent.) The
Sinkhorn free energy function is easily seen to be convex and it can be
efficiently minimized with the help of Sinkhorn's matrix scaling
algorithm~\cite{Linial2000}, thereby motivating its name. In this thesis, we
will actually work with the scaled Sinkhorn permanent
$\permscs(\mtheta) \defeq \e^{-n} \cdot \perms(\mtheta)$, a variant of the
Sinkhorn permanent $\perms(\mtheta)$ that was introduced
in~\cite{Anari2021}. The scaled Sinkhorn permanent $\permscs(\mtheta)$
satisfies
\begin{align}
  \e^n \cdot \frac{n!}{n^n}
    &\leq 
       \frac{\perm(\mtheta)}{\permscs(\mtheta)}
     \leq 
       \e^n .
         \label{eq:ratio:permanent:scaled:Sinkhorn:permanent:1}
\end{align}
The first inequality in~\eqref{eq:ratio:permanent:scaled:Sinkhorn:permanent:1}
follows from van der Waerden's inequality proven by
Egorychev~\cite{Egorychev1981} and Falikman~\cite{Falikman1981}, whereas the
second equality follows from a relatively simple to prove inequality. Both
inequalities~\eqref{eq:ratio:permanent:scaled:Sinkhorn:permanent:1} are the
best possible given only the knowledge of the size of the
matrix $\mtheta$. Note that the value on the LHS
of~\eqref{eq:ratio:permanent:scaled:Sinkhorn:permanent:1} is approximately
$\sqrt{2 \pi n}$.

%***************************************************************************

\subsection{A Combinatorial Characterization of the Bethe Permanent and the (Scaled) Sinkhorn Permanent}
\label{chapt: permanent: combinartorial chara of ZB and ZscC}

While the definition of $\perm(\mtheta)$ in~\eqref{eq:def:permanent:1} clearly
has a combinatorial flavor (\eg, counting weighted perfect matchings in a
complete bipartite graph with two times $n$ vertices), it is, a priori, not
clear if a combinatorial characterization can be given for $\permb(\mtheta)$
and $\permscs(\mtheta)$. However, this is indeed the case.

%***************************************************************************

Namely, using the results in~\cite{Vontobel2013}, a finite-graph-cover-based
combinatorial characterization was given for $\permb(\mtheta)$
in~\cite{Vontobel2013a}. Namely,
\begin{align*}
  \permb(\mtheta)
    &= \limsup_{M \to \infty} \,
         \permbM{M}(\mtheta)\, ,
           % \label{eq:bethe:perm:as:limit:1}
\end{align*}
where the degree-$M$ Bethe permanent is defined to be
\begin{align*}
  \permbM{M}(\mtheta)
    &\defeq
      \sqrt[M]{
        \bigl\langle
          \perm( \mtheta^{\uparrow \mP_{M}} )
        \bigr\rangle_{\mP_{M} \in \tPsi_{M} }
     } \, , 
       % \label{eq:def:degree:M:Bethe:permanent:1}
\end{align*}
where the angular brackets represent an arithmetic average and where
$\mtheta^{\uparrow \mP_{M}}$ represents a degree-$M$ cover of $\mtheta$
defined by a collection of permutation matrices $\mP_{M}$. (See
Definition~\ref{def:matrix:degree:M:cover:1} for the details.)

%***************************************************************************

In this thesis we offer a combinatorial characterization of the scaled Sinkhorn
permanent $\permscs(\mtheta)$. Namely,
\begin{align*}
  \permscs(\mtheta)
    &= \limsup_{M \to \infty} \, 
         \permscsM{M}(\mtheta)\, , 
           % \label{eq:scaled:Sinkhorn:permanent:as:limit:1}
\end{align*}
where $\permscs(\mtheta)$ was defined
in~\cite{N.Anari2021}, and where
the degree-$M$ scaled Sinkhorn permanent is defined to be \\[-0.35cm]
\begin{align}
  \permscsM{M}(\mtheta)
    &\defeq 
       \sqrt[M]{
         \perm
           \bigl(
             \langle
               \mtheta^{\uparrow \mP_{M}}
             \rangle_{\mP_{M} \in \tPsi_{M} }
           \bigr)
       } \nonumber \\
    &= \sqrt[M]{
         \perm( \mtheta \otimes \mU_{M,M})
       } \, ,\nonumber
\end{align}
where $\otimes$ denotes the Kronecker product of two matrices and where
$ \mU_{M,M} $ is the matrix of size $M \times M$ with all entries equal to
$1/M$.  (See Definition~\ref{def:Sinkhorn:degree:M:cover:1} and
Proposition~\ref{sec:1:prop:14} for the details.)~\footnote{Note that the quantity
  $\sqrt[M]{ \perm( \mtheta \otimes \mU_{M,M}) }$ appears in the literature at
  least as early as~\cite{Bang1976,Friedland1979}. These papers show that for
  $M = 2^s$, $s \in \sZp$, it holds that
  $\sqrt[M]{ \perm( \mtheta \otimes \mU_{M,M}) } \leq \perm(\mtheta)$, which,
  in our notation, implies $1 \leq \perm(\mtheta) / \permscsM{M}(\mtheta)$ for
  $M = 2^s$, $s \in \sZp$.}%
~\footnote{Barvinok~\cite{Barvinok2010} considered combinatorial expressions
  in the same spirit as $\sqrt[M]{ \perm( \mtheta \otimes \mU_{M,M}) }$, but
  the details and the limit are different.}

%***************************************************************************

\begin{figure}[t]
  \begin{center}
    \hspace{-2.25cm}\input{figures/relate_z_zbm_zb.tex}
    \hspace{-1.75cm}\input{figures/relate_z_permscsm_permscs.tex}
  \end{center}
  \caption{Combinatorial characterizations of the 
    Bethe and scaled Sinkhorn permanents.}
  \label{fig:combinatorial:characterization:1}
  \vspace{0.00cm} % see if this space is needed in the end
\end{figure}

%***************************************************************************

%***************************************************************************

These combinatorial characterizations of the Bethe and scaled Sinkhorn
permanent are summarized in Fig.~\ref{fig:combinatorial:characterization:1}.

%***************************************************************************

Besides the quantities $\permbM{M}(\mtheta)$ and $\permscsM{M}(\mtheta)$ being
of inherent interest, they are particularly interesting toward understanding
the ratios \\ $\perm(\mtheta) / \permb(\mtheta)$ and
$\perm(\mtheta) / \permscs(\mtheta)$ for general non-negative matrices or for
special classes of non-negative matrices.

%***************************************************************************

For example, as discussed in~\cite[Sec.~VII]{Vontobel2013}, one can consider
the equation
\begin{align*}
  \hspace{-0.25cm}
  \frac{\perm(\mtheta)}{\permb(\mtheta)}
    &= \frac{\perm(\mtheta)}{\permbM{2}(\mtheta)}
       \!\cdot\!
       \frac{\permbM{2}(\mtheta) }{\permbM{3}(\mtheta)}
       \!\cdot\!
       \frac{\permbM{3}(\mtheta) }{\permbM{4}(\mtheta)}
       \!\cdots .
         % \label{eq:Z:ratios:long:1}
\end{align*}
If one can give bounds on the ratios appearing on the RHS of this equation,
then one obtains bounds on the ratio on the LHS of this equation.

% In fact, one of the main results of the present thesis is in this spirit. In
% particular, from the results in this thesis it follows that XXXXX
% \begin{align}
%   LBXXXXX
%     &\leq 
%        \frac{\permbM{M}(\mtheta)}{\permbM{M+1}(\mtheta)}
%      \leq
%        UBXXXXX .
% \end{align}
% XXXXX Also $(M \! - \! 1)/M$ ranges from $0$ to $1$, with $1/2$ achieved for
% $M = 2$. XXXXX also similar strategy for other graphical models XXXXX

%***************************************************************************

Alternatively, one can consider the equation
\begin{align}
  \underbrace{
    \frac{\perm(\mtheta)}
         {\permb(\mtheta)}
  }_{\text{\ding{192}}}
    &= \underbrace{
         \frac{\perm(\mtheta)}
              {\permbM{2}(\mtheta)}
       }_{\text{\ding{193}}}
       \cdot
       \underbrace{
         \frac{\permbM{2}(\mtheta)}
              {\permb(\mtheta)}
       }_{\text{\ding{194}}} .
         \label{eq:perm:ratios:1}
\end{align}
Based on numerical and analytical results, Ng and Vontobel~\cite{KitShing2022}
concluded that it appears that for many classes of matrices of interest, the
ratio~\ding{193} behaves similarly to the ratio~\ding{194}. Therefore,
understanding the ratio~\ding{193} goes a long way toward understanding the
ratio~\ding{192}. (Note that the ratio~\ding{193} is easier to analyze than
the ratio~\ding{192} for some classes of matrices of interest.)

%***************************************************************************

Results similar in spirit to the above results were given for the Bethe
approximation of the partition function of other graphical models (see, \eg,
\cite{Ruozzi2012,Vontobel2016,Csikvari2022}).

\subsection{Main Contributions}
\label{sec:main:constributions:1}

%***************************************************************************

Let $n, M \in \sZpp$, let $\mtheta$ be a fixed non-negative matrix of size
$n \times n$, and let $\GamMn$ be the set of doubly stochastic matrices of
size $n \times n$ where all entries are integer multiples of $1/M$. Moreover,
for $\vgam \in \GamMn$, let
$\mtheta^{ M \cdot \vgam } \defeq \prod_{i,j \in [n]} \bigl( \theta(i,j)
\bigr)^{\! M \cdot \gamma(i,j)}$. (Note that in this expression, all exponents
are non-negative integers.) Throughout this thesis, we consider $ \mtheta $
such that $ \perm(\mtheta) $, $ \permbM{M}(\mtheta) $, and
$ \permscsM{M}(\mtheta) $ are positive real-valued.

%***************************************************************************

\begin{lemma}
  \label{lem: expression of permanents w.r.t. C}

  There are collections of non-negative real numbers \\
  \mbox{$\bigl\{ \CM{n}( \vgam ) \bigr\}_{\vgam \in \GamMn}$,\!
  $\bigl\{ \CBM{n}( \vgam ) \bigr\}_{\vgam \in \GamMn}$,\!
  $\bigl\{ \CscSgen{M}{n}( \vgam ) \bigr\}_{\vgam \in \GamMn}$} such that
  \begin{align}
    \bigl( \perm(\mtheta) \bigr)^{\! M} 
      &= \sum_{\vgam \in \GamMn} 
           \mtheta^{ M \cdot \vgam }
           \cdot
           \CM{n}( \vgam )\, , 
             \label{sec:1:eqn:43} \\
    \bigl( \permbM{M}(\mtheta) \bigr)^{\! M} 
      &= \sum_{\vgam \in \GamMn} 
           \mtheta^{ M \cdot \vgam }
           \cdot
           \CBM{n}( \vgam )\, ,
             \label{sec:1:eqn:190}  \\
    \bigl( \permscsM{M}(\mtheta) \bigr)^{\! M}
      &= \sum_{\vgam \in \GamMn}
           \mtheta^{ M \cdot \vgam } \cdot \CscSgen{M}{n}( \vgam ).
             \label{sec:1:eqn:168} \\[-0.75cm] \nonumber
  \end{align}
  \elemma
\end{lemma}

%***************************************************************************

With the help of the inequalities
  in~\eqref{eq:ratio:permanent:bethe:permanent:1}
  and~\eqref{eq:ratio:permanent:scaled:Sinkhorn:permanent:1}, along with some
  results that are established in this thesis, we can make the following
  statement about the coefficients $\CM{n}( \vgam )$, $\CBM{n}( \vgam )$, and
  $\CscSgen{M}{n}( \vgam )$ in Lemma~\ref{lem: expression of permanents
    w.r.t. C}.

%***************************************************************************

\begin{theorem}
  \label{thm: inequalities for the coefficients}

  For every $\vgam \in \GamMn$, the coefficients $\CM{n}( \vgam )$,
  $\CBM{n}( \vgam )$, and $\CscSgen{M}{n}( \vgam )$ satisfy
  \begin{align}
    1 
      &\leq 
         \frac{ \CM{n}(\vgam) }{\CBM{n}(\vgam) }
       \leq
         \Bigl( 2^{n/2} \Bigr)^{\! M-1}\, ,
           \label{sec:1:eqn:58} \\
    \Biggl( \frac{M^{M}}{M!} \Biggr)^{\!\!\! n}
    \cdot
    \biggl(
      \frac{ n! }{ n^{n} }
    \biggr)^{\!\! M-1} 
      &\leq
         \frac{\CM{n}(\vgam)}{\CscSgen{M}{n}(\vgam)} 
       \leq 
         \Biggl( \frac{M^{M}}{M!} \Biggr)^{\!\! n}.
           \label{sec:1:eqn:180}
  \end{align}
  \etheorem
\end{theorem}

%***************************************************************************
Combining Lemma~\ref{lem: expression of permanents w.r.t. C} and
Theorem~\ref{thm: inequalities for the coefficients}, we can make the
following statement.

%***************************************************************************

\begin{theorem}
  \label{th:main:permanent:inequalities:1}
  \label{TH:MAIN:PERMANENT:INEQUALITIES:1}
  It holds that
  \begin{align}
    1 
      &\leq
         \frac{\perm(\mtheta)}{\permbM{M}(\mtheta)}
       \leq
         \Bigl( 2^{n/2} \Bigr)^{\!\! \frac{M-1}{M}}
           \label{SEC:1:EQN:147}, \\
    \frac{M^{n}}{(M!)^{n/M}}
    \cdot
    \biggl( \frac{n!}{n^{n}} \biggr)^{\!\! \frac{M-1}{M}}
      &\leq
         \frac{ \perm(\mtheta) }{ \permscsM{M}(\mtheta) }
       \leq
         \frac{M^{n}}{(M!)^{n/M}}.
           \label{sec:1:eqn:200}
  \end{align}
  Note that in the limit $M \to \infty$ we recover the inequalities
  in~\eqref{eq:ratio:permanent:bethe:permanent:1}
  and~\eqref{eq:ratio:permanent:scaled:Sinkhorn:permanent:1}.
  \etheorem
\end{theorem}

%***************************************************************************
Finally, we discuss the following asymptotic characterization of the
coefficients $\CM{n}( \vgam )$, $\CBM{n}( \vgam )$, and
$\CscSgen{M}{n}( \vgam )$.

%***************************************************************************

\begin{proposition}
  \label{prop:coefficient:asymptotitic:characterization:1}
  
  Let $\vgam \in \GamMn$. It holds that
  \begin{align}
    \CM{n}( \vgam )
      &= \exp\bigl( M \cdot \HG'(\vgam) + o(M) \bigr)\, ,
           \label{sec:1:eqn:125} \\
    \CBM{n}( \vgam )
      &= \exp\bigl( M \cdot \HBthe(\vgam) + o(M) \bigr)\, ,
           \label{sec:1:eqn:206}  \\
    \CscSgen{M}{n}( \vgam )
      &= \exp\bigl( M \cdot \HscSthe(\vgam) + o(M) \bigr)\, ,
           \label{sec:1:eqn:207}
  \end{align}
  where $\HG'(\vgam)$, $\HBthe(\vgam)$, and $\HscSthe(\vgam)$ are the
  modified Gibbs entropy function, the Bethe entropy function, and the
  scaled Sinkhorn entropy function, respectively, as defined in Section~\ref{sec:free:energy:functions:1}.

  \vspace{-0.02 cm}
  \eproposition
\end{proposition}

%***************************************************************************

Let us put the above results into some context:
\begin{itemize}

  \item The first inequality in~\eqref{sec:1:eqn:58} proves the first (weaker)
    conjecture in~\cite[Conjecture 52]{Vontobel2013a}.

  \item Smarandache and Haenggi~\cite{Smarandache2015} claimed a proof of the
    second (stronger) conjecture
    in~\cite[Conjecture~52]{Vontobel2013a},\footnote{The second
        (stronger) conjecture in~\cite[Conjecture~52]{Vontobel2013a} stated that
        for each $ \mP_{M} \in \tPsi_{M} $, there is a collection of
        non-negative real numbers
        $\bigl\{ C_{\mathrm{B},M,n,\mP_{M}}( \vgam ) \bigr\}_{\vgam \in \GamMn}$
        such that
        \begin{align*}
          \perm( \mtheta^{\uparrow \mP_{M}} ) = \sum_{\vgam \in \GamMn}
        \mtheta^{ M \cdot \vgam } \cdot C_{\mathrm{B},M,n,\mP_{M}}( \vgam )\, ,
        \end{align*}
        and that for every $ \vgam \in \GamMn $, it holds that
        $ \CM{n}(\vgam) / C_{\mathrm{B},M,n,\mP_{M}}( \vgam ) \geq 1.  $}
    which would imply the first (weaker) conjecture in~\cite[Conjecture
    52]{Vontobel2013a}. However, the proof in~\cite{Smarandache2015} is
    incomplete.

  \item The first inequality in~\eqref{SEC:1:EQN:147} proves the first (weaker)
    conjecture in~\cite[Conjecture 51]{Vontobel2013a}.

  \item The proof of the first inequality in~\eqref{sec:1:eqn:58}, and with that
    the proof of the first inequality in~\eqref{SEC:1:EQN:147}, uses an
    inequality of 
    Schrijver~\cite{Schrijver1998}. By now, there are various
    proofs of Schrijver's inequality and also various proofs of the first
    inequality in~\eqref{eq:ratio:permanent:bethe:permanent:1} available in the
    literature, however, the ones that we are aware of are either quite involved
    (like Schrijver's original proof of his inequality) or use reasonably
    sophisticated machinery like real stable polynomials. Given the established
    veracity of the first inequality in~\eqref{SEC:1:EQN:147}, it is hoped that
    a more basic proof for this inequality, and with that of the first
    inequality in~\eqref{eq:ratio:permanent:bethe:permanent:1}, can be
    found. Similar statements can be made for the other inequalities
    in~\eqref{SEC:1:EQN:147} and~\eqref{sec:1:eqn:200}.

    In fact, for $M = 2$, a basic proof of the inequalities
    in~\eqref{SEC:1:EQN:147} is available: it is based
    on~\cite[Proposition~2]{KitShing2022} (which appears in this thesis as
    Proposition~\ref{prop:ratio:perm:permbM:2:1}), along with the observation
    that the quantity $c(\sigma_1,\sigma_2)$ appearing therein is bounded as
    $0 \leq c(\sigma_1,\sigma_2) \leq n/2$. Another basic proof of the first
    inequality in~\eqref{SEC:1:EQN:147} is based on a straightforward
    generalization of the result in~\cite[Lemma 4.2]{Csikvari2017} from
    $\{0,1\}$-valued matrices to arbitrary non-negative matrices and then
    averaging over $2$-covers.

    Moreover, for the case where $\mtheta$ is proportional to the all-one matrix
    and where $M \in \sZpp$ is arbitrary, a basic proof of the first inequality
    in~\eqref{SEC:1:EQN:147} was given in~\cite[Appendix~I]{Vontobel2013a}.
    However, presently it is not clear how to generalize this proof to other
    matrices $\mtheta$.

  \item For $M = 2$, the lower and upper bounds in~\eqref{SEC:1:EQN:147} are
    exactly the square root of the lower and upper bounds
    in~\eqref{eq:ratio:permanent:bethe:permanent:1}, respectively, thereby
    corroborating some of the statements made after~\eqref{eq:perm:ratios:1}.

  \item Although we take advantage of special properties of the factor graphs
    under consideration, potentially the techniques in this thesis can be
    extended toward a better understanding of the Bethe approximation of the
    partition function of other factor graphs. (For more on this topic, see the discussion in Chapter~\ref{chapt: summary and outlook}.)

\end{itemize}



\section[The Graph Covers for DE-FGs]{Characterizing the Bethe Partition Function of \\Double-Edges Factor Graphs via Graph Covers}
\label{intro: characterize ZB for DE-FG}

The above results are for factor graphs called S-FGs, \ie,
for factor graphs with local functions taking on non-negative real
values. Recently, some papers have considered more general factor graphs,
namely factor graphs where the local functions take on complex values, in
particular toward representing quantities of interest in quantum information
processing~\cite{Loeliger2012, Loeliger2017, Loeliger2020, Mori2015a}. (For connections of these factor graphs to other graphical notations in physics, see~\cite[Appendix~A]{Loeliger2017}.) The structure of these factor graphs is not completely arbitrary, and so, toward formalizing such factor graphs, Cao and Vontobel~\cite{Cao2017} introduced DE-FGs, where local functions take on complex values and have to satisfy some positive semi-definiteness constraints. DE-FGs have the property~\cite{Cao2017} that the partition function is a
non-negative real number. However, because the partition function is the sum of complex numbers (notably, the real and the imaginary parts of these complex numbers can have a positive or negative sign), approximating the partition function is, in general, much more challenging for DE-FGs than for S-FGs. This problem is known as the numerical sign problem in applied mathematics and theoretical physics~(see, \textit{e.g.}, \cite{LohJr.1990}).

DE-FGs are closely related to tensor networks~\cite{Cirac2009,Coecke2010,Robeva2019,Alkabetz2021}, which is one of the central topics in theoretical physics~\cite{Cowen2015}.
Alkabetz and Arad in~\cite{Alkabetz2021} showed how to map a projected-entangled-pair-state (PEPS) tensor network to a DE-FG. It is straightforward to define the SPA for a DE-FG, along with defining the Bethe partition function based on the SPA fixed-point messages.\footnote{Similar to the definition of the Bethe partition function in~\cite[Def.~8]{Cao2017}, in this thesis, the Bethe partition function is formulated based on the so-called pseudo-dual Bethe
free energy function for S-FGs. Although
generalizing the primal Bethe free energy function from S-FGs to DE-FGs is
formally straightforward, it poses challenges because of the
multi-valuedness of the complex logarithm and is left for future research.}
Similar to the S-FG case, the SPA on a DE-FG can be used to approximate the induced marginals and partition function. Alkabetz and Arad in~\cite{Alkabetz2021} further connected the SPA on a DE-FG to tensor network contractions. Motivated by this connection, Tindall and Fishman~\cite{Tindall2023} related the SPA to known tensor network gauging methods. Moreover, Tindall \etal~in~\cite{Tindall2024} showed that for the kicked Ising quantum system that was studied in~\cite{Kim2023}, the SPA-based approximation results are more accurate and precise than the results obtained from the quantum processor and many other classical methods. These promising results motivate us to study the SPA for a DE-FG.
%***************************************************************************

% Motivated by the DE-FGs in~\cite{Cao2017}, we introduce paired-edges factor graphs (DE-FGs) in this thesis. Here's a comparison between DE-FGs and DE-FGs:
% %---------------------------------------------------------------------------
% \begin{itemize}

%     \item In DE-FGs, a double edge is used to represent a pair of variables. In DE-FGs, instead of a double edge, a pair of edges is used to represent the same pair of variables. 

%     \item Due to the difference in the representation of each pair of variables, the SPA for DE-FGs is different from the SPA for DE-FGs. 

%     \item In the DE-FGs considered in the previous work (Cao \etal~\cite{Cao2017}), the local functions are subject to positive semi-definiteness constraints.
%     In this thesis, two types of DE-FGs are considered: strict-sense DE-FGs and weak-sense DE-FGs.
%     %----------------------------------------------------------------------------
%     \begin{itemize}
%       \item Strict-sense DE-FGs: The local functions in strict-sense DE-FGs need to satisfy the same positive semi-definiteness constraints as in DE-FGs.

%       \item Weak-sense DE-FGs: The local functions in weak-sense DE-FGs need to satisfy some Hermitian constraints, which are weaker than the positive semi-definiteness constraints required for strict-sense DE-FGs.
%     \end{itemize}
%     %---------------------------------------------------------------------------


% \end{itemize}
% %---------------------------------------------------------------------------


% \begin{align*}
% \ZBSPA(\graphN,\vmu)
%   &\defeq \frac{\prod\limits_f 
%     \Bigl( 
%     \sum\limits_{\vx_{\setpf}}
%       f(\tvx_{\setpf})
%           \cdot
%           \prod_{e \in \setpf}
%           \mu_{\ef}(\txe) 
%     \Bigr)}{\prod\limits_{e = (f_{i}, f_{j})} 
%     \Bigl( \sum\limits_{\txe}
%             \mu_{\efi}(\txe)
%             \cdot
%             \mu_{\efj}(\txe) 
%     \Bigr)}
% \end{align*}
% where $ f $ represents the function node and also the associated local function,  
% $ e $ represents the edge connecting function nodes $ f_{i} $ and $ f_{j} $, and the functions $ Z_{f} $ and $ Z_{e} $ are given by
% \begin{alignat*}{2}
%     Z_f(\vmu)
%     &\defeq
%             \qquad f \in \setF, \nonumber \\                
%     Z_{e}(\vmu)
%       &\defeq
%         \sum_{\txe}
%             \mu_{\efi}(\txe)
%             \cdot
%             \mu_{\efj}(\txe)
%             , \qquad e = (f_{i}, f_{j}) \in \setEfull.
% \end{alignat*}
% The details will be given in Section~\ref{sec:DENFG}.

One can prove that if the fixed-point messages satisfy some positive semi-definiteness constraints, the Bethe partition function is a non-negative real number for the DE-FG considered in~\cite{Cao2017}. Given this, we wonder if there is a characterization of a DE-FG's Bethe partition function in terms of its finite graph covers' partition functions, which is analogous to the result for S-FGs in~\cite{Vontobel2013}. Numerical calculations that we performed for small DE-FGs suggested that such a result
should also holds. However, proving such a result for DE-FGs turns out to be
much more challenging than that for S-FGs. The reason is that the method
of types, which was the main ingredient in the proof for the case of S-FGs,
works essentially only for approximating sums of non-negative real
values, as shown in~\cite{Vontobel2013}. The difficulty of approximating the sum of complex numbers can be illustrated by the following example.
\begin{example}
  For any positive-valued integer $ M $ and any complex number $ \alpha $, we define
  \begin{align*}
    Z_{M} \defeq 
    \sum_{\ell = 0}^{M} c_{M,\ell},
  \end{align*}
  where
  \begin{align*}
    c_{M,\ell} = \binom{M}{ \ell } 
    \cdot ( 1 - \alpha )^{M - \ell}
    \cdot \alpha^{ \ell }.
  \end{align*}
  One can verify that $ Z_{M} = 1 $ for any positive-valued integer $ M $ and any complex number $ \alpha $.

  If $ \alpha $ is a non-negative number satisfying $ 0 \leq \alpha \leq 1 $, then $ c_{M,\ell} $ is non-negative-valued for all $ \ell \in \{0,\ldots,M\} $ and we obtain
  \begin{align*}
    \max_{ \ell \in \{0,\ldots,M\} } c_{M,\ell} 
    \leq Z_{M}
    \leq (M+1) \cdot \max_{ \ell \in \{0,\ldots,M\} } c_{M,\ell}, 
  \end{align*}
  which implies
  \begin{align*}
    \frac{1}{M} \cdot 
    \log( \max_{ \ell \in \{0,\ldots,M\} } c_{M,\ell} )
    &\leq 
    \frac{1}{M} \cdot \log(Z_{M})
    \nonumber\\
    &\leq 
    \frac{1}{M} 
    \cdot \log(M+1)
    +
    \frac{1}{M} 
    \cdot \log( \max_{ \ell \in \{0,\ldots,M\} } c_{M,\ell} ).
  \end{align*}
  In the limit $ M \to \infty $, we get
  \begin{align}
    \lim_{ M \to \infty }
    \frac{1}{M} \cdot \log(Z_{M})
    = 
    \lim_{ M \to \infty }
    \frac{1}{M} \cdot 
    \log( \max_{ \ell \in \{0,\ldots,M\} } c_{M,\ell} ).
    \label{eqn: limit of 1 M log ZM}
  \end{align}
  For simplicity of exposition, suppose that there exists a positive-valued integer $ M $ such that $ \alpha \cdot M \in \sZpp $, then for such $ \alpha $, 
  we have
  \begin{align}
    \max_{ \ell \in \{0,\ldots,M\} } c_{M,\ell}
    = c_{M,\alpha \cdot M}
    = \underbrace{
      \binom{M}{\alpha \cdot M} 
    }_{ \overset{(a)}{=} \exp( M \cdot h(\alpha) + o(M) ) }
    \underbrace{ (1-\alpha)^{ M (1-\alpha) }
    \cdot \alpha^{ M \alpha }
    }_{ = \exp( -M \cdot h(\alpha) ) }
    = \exp( o(M) ),
    \label{eqn: Cml is a little o function wrt M}
  \end{align}
  where $ h(\alpha) \defeq -\alpha \cdot \log( \alpha ) 
  - (1-\alpha) \cdot \log( 1 - \alpha ) $,
  where $ o(M) $ is the usual little-$o$ notation for a function in $M$,
  and where step $(a)$ follows from Stirling approximation (see, \eg,~\cite{Robbins1955}).
  Plugging~\eqref{eqn: Cml is a little o function wrt M} into~\eqref{eqn: limit of 1 M log ZM}, we obtain
  \begin{align*}
    \lim_{ M \to \infty }
    \frac{1}{M} \cdot 
    \log( \max_{ \ell \in \{0,\ldots,M\} } c_{M,\ell} )
    =\lim_{ M \to \infty }
    \frac{o(M)}{M} = 0
    = 
    \lim_{ M \to \infty }
    \frac{1}{M} \cdot \log(Z_{M}),
  \end{align*}
  where the last equality follows from the fact that $ Z_{M} = 1 $ for all positive-valued integer $ M $.
  We can see that for the case $ 0 \leq \alpha \leq 1 $, all the terms in $ Z_{M} $ are non-negative-valued and are added up constructively, and we can approximate $ Z_{M} $ by the term with the largest magnitude. Following the similar idea, Vontobel~\cite{Vontobel2013} used the method of types to characterize an S-FG's Bethe partition function in terms of its finite graph covers.

  However, if $ \alpha $ is a complex-valued number with non-zero imaginary part, the terms in $ Z_{M} $ can be complex-valued and these terms are added up constructively and destructively. In this case,
  we cannot approximate $ \lim_{ M \to \infty } M^{-1} \cdot \log(Z_{M}) $ following the same idea as in the case $ 0 \leq \alpha \leq 1 $, as the term with the largest magnitude gives a bad estimate of $ Z_{M} $. 
\end{example}
% and the $M$-th power of $ (a-b) $ are given by
% \begin{align*}
%   (a+b)^{M} &= 
%   \sum_{ k = 0 }^{M} \binom{ M }{ k } \cdot a^{k} \cdot b^{M-k}, 
%   \nonumber\\
%   (a-b)^{M} &= \sum_{ k = 0 }^{M} \binom{ M }{ k } \cdot a^{k} \cdot (-b)^{M-k}, 
% \end{align*}


%  we need to develop a novel proof approach for the case
% of DE-FGs; this novel proof approach is the main result of this thesis besides
% the statement itself. (Currently, the characterization of a DE-FG's Bethe partition function in terms of its finite graph covers is for the strict-sense DE-FGs
% satisfying an (easily checkable) condition. However, based on the numerical
% results, we suspect that the characterization holds more
% broadly.)

\subsection{Main Contributions}

We develop a novel approach to prove the combinatorial characterization of the Bethe partition functions for a certain class of DE-FGs. This novel proof approach is one of the main results in this thesis besides
the statement itself. (Currently, the combinatorial characterization of a DE-FG's Bethe partition function in terms of its finite graph covers is for the strict-sense DE-FGs
satisfying an (easily checkable) condition. However, based on the numerical
results, we suspect that the characterization holds more
broadly.) 

%***************************************************************************

Our proof approach consists of three main ingredients:
\begin{itemize}

  \item In the first step, we apply the loop-calculus transform (LCT)\footnote{The loop-calculus transform can be seen as a particular instance of a holographic
  transform~\cite{AlBashabsheh2011}.} to a DE-FG based on a
  fixed point of the SPA. (If the SPA has multiple fixed points,
  we assume that it is the fixed point with the largest Bethe partition
  function value.) The benefit of the loop-calculus transform is that the
  transformed SPA fixed-point messages have an elementary form, which is independent of the edge and the direction of a message. Note that the LCT leaves the partition function of the DE-FG unchanged.

  \item In the second step, for any positive-valued integer $M$, we to express the average of the associated $M$-covers' partition functions in terms of the partition function of its associated average degree-$M$ cover. 

  \item In the third step, we let $M \to \infty$ and evaluate the partition function of average degree-$M$ cover of the loop-calculus transformed DE-FG. So far, we can relate the associated $M$-covers' average partition function to the Bethe partition function when some (easily checkable) conditions are satisfied. However, we suspect that it holds more generally. We leave it as an open problem to broadly characterize when the relevant function has a global maximum at the point of interest. 

\end{itemize}

Based on the average degree-$M$ cover of DE-FG, we further develop the symmetric-subspace transform (SST) for DE-FG, which allows one to express the partition function of the average degree-$M$ cover in terms of some integral.
The LCT and the SST should be of interest in other research topics besides characterizing the partition function. The reasons are listed as follows.
%----------------------------------------------------------------------------
\begin{enumerate}
  \item The LCT defined in this thesis does not have any restriction on the associated SPA fixed-point messages, \ie, this transform works for complex-valued SPA fixed-point messages as well. In contrast, the LCT defined in~\cite{Mori2015} required the associated messages to be nonzero-valued, \ie, our proposed transform is a generalization of the transform in~\cite{Mori2015}.
  
  \item The SST defined in this thesis is applicable for both S-FGs and DE-FGs. To the best of our knowledge, it is the first time to introduce this transform in factor-graph literature, although it has wide applications in quantum physics~\cite{Wood2015,Harrow2013}.
\end{enumerate}
%----------------------------------------------------------------------------

\section{Structure of this Thesis}

This thesis is structured as follows. Chapter~\ref{chapt: preliminaries} reviews the basic definitions and notations that are frequently used in this thesis. In particular, Chapter~\ref{chapt: preliminaries} introduces the S-FGs, a special class of S-FGs that each S-FG's partition function is equal to the permanent of a non-negative square matrix, the DE-FGs, and the finite graph covers for these factor graphs. Chapter~\ref{chapt: finite graph cover based bound for matrix permanent} proves degree-$M$-Bethe-permanent-based bounds on the permanent of a non-negative matrix and also proves similar results for another approximation of the permanent known as the (scaled) Sinkhorn permanent. Chapters~\ref{chapt: LCT} and~\ref{chapt:SST} introduces the LCT and the SST, respectively, for both S-FGs and DE-FGs. Chapter~\ref{chapt: graph cover thm for DENFG} proves the graph-cover theorem for a class of DE-FGs satisfying an easily checkable conditions. Various (longer) proofs have been collected in the appendices.



==> lct.tex <==
Loop calculus, as defined by Chertkov and Chernyak~\cite{Chertkov2006,
  Chernyak2007} and further developed by Mori~\cite{Mori2015}, can be
formulated as a certain holographic transform~\cite{AlBashabsheh2011} applied
to an S-NFG, and will henceforth be called the loop-calculus transform
(LCT). After applying the LCT to an S-NFG, the partition function equals the sum of the Bethe partition function and some correction terms, where the sum of the correction terms are related to a weighted sum over all generalized loops in the S-NFG. 

In this chapter, we introduce the LCT for both S-NFGs and DE-NFGs. 
The LCT for DE-NFGs has been discussed by Cao in~\cite[Theorem 2.21]{Cao2021}. Let us make a comparison between the LCT proposed in~\cite{Mori2015,Cao2021} and our proposed LCT.
%----------------------------------------------------------------------------
\begin{itemize}
  \item Mori in~\cite{Mori2015} considered S-NFGs and defined
  the LCT based on the SPA fixed-point message vector that consists of positive-valued entries only. Note that he did not define the LCT for the SPA fixed-point message vector that consists of at least one zero-valued entry.

  \item Cao in~\cite{Cao2021} considered DE-NFGs and defined the LCT for DE-NFGs based on the SPA fixed-point message vector 
  where the entries are allowed to take values in the field of complex numbers.
  However, he only
  stated the constraints that the LCT has to satisfy, 
  and he did not provide explicit expressions that enable us to applying the LCT 
  for DE-NFGs.

  \item In this section, we explicitly define the LCT for both S-NFGs and DE-NFGs. Our proposed LCT is defined based on the SPA fixed-point message vector whose entries can take values in the field of complex numbers, \ie, the SPA fixed-point message vector is allowed to have zero-valued entries. Our proposed LCT generalizes the results in~\cite{Mori2015,Cao2021}.

  \item In Chapter~\ref{CHAPT: GCT DENFG}, we use the LCT for DE-NFGs to prove the graph-cover theorem, \ie, Conjecture~\ref{sec:GraCov:conj:1} for a class of DE-NFGs that satisfy an easily checkable condition.
\end{itemize}
%----------------------------------------------------------------------------

%***************************************************************************
%***************************************************************************

\section{LCT for S-NFGs}
\label{sec:LCT:SNFG:1}

% In the following, we first give a high-level introduction of our proposed LCT for S-NFGs with the help of Fig.~\ref{sec:LCT:fig:1}.


%***************************************************************************

Before giving the general definition of the LCT for S-NFGs, we consider a
specific S-NFG $\graphN$ and assume that a part of it looks as shown in
Fig.~\ref{sec:LCT:fig:3}. Let
$\vmu $ be some SPA
fixed-point message vector for $\graphN$. The LCT is a sequence of
modifications to the original S-NFG that leave the partition function
unchanged. This is done by applying opening-the-box and closing-the box
operations~\cite{Loeliger2004} as follows.
\begin{enumerate}

\item The S-NFG in Fig.~\ref{sec:LCT:fig:4} is obtained from the S-NFG
  in Fig.~\ref{sec:LCT:fig:3} by applying suitable opening-the-box
  operations~\cite{Loeliger2004}. Importantly, the new function nodes $h_i$
  are based on $\vmu$ and are defined in such a way that the partition function remains unchanged.

  For example, for the edge $1$ that connects the function nodes $f_{i}$ and $f_{j}$, as shown in Fig.~\ref{sec:LCT:fig:3}, we
  introduce the function nodes $h_3$ and $h_8$ with the local functions
  $h_3: \set{X}_{1} \times \LCTset{X}_{1} \to \sC$ and
  $h_8: \set{X}_{1} \times \LCTset{X}_{1} \to \sC$, where
  $\LCTset{X}_{1} \defeq \set{X}_{1} $. The partition function of the S-NFG remains unchanged because $h_3$ and $h_8$ are
  defined such that the following equalities hold
  \begin{align*}
    \sum_{\LCT{x}_{1} \in \LCTset{X}_{1}} 
    h_3(x_{1,f_{i}}, \LCT{x}_{1}) \cdot h_8(x_{1,f_{j}}, \LCT{x}_{1}) =
    [x_{1,f_{i}} \! = \! x_{1,f_{j}}], \qquad 
    x_{1,f_{i}}, x_{1,f_{j}} \in \set{X}_{1}.
  \end{align*}

\item The S-NFG in Fig.~\ref{sec:LCT:fig:5} is essentially the same as
  the S-NFG in Fig.~\ref{sec:LCT:fig:4}.
  
\item The S-NFG in Fig.~\ref{sec:LCT:fig:6} is obtained from the S-NFG
  in Fig.~\ref{sec:LCT:fig:5} by applying suitable closing-the-box
  operations~\cite{Loeliger2004} to the S-NFG in
  Fig.~\ref{sec:LCT:fig:5}. Consider the dashed boxes on the left-hand side in Fig.~\ref{sec:LCT:fig:5}. Its exterior function is defined to be the sum, over the internal variables, of the product of the internal local functions. Replacing this dashed box by a single function node that represents this exterior function is known as closing-the-box operation~\cite{Loeliger2004}.
  For example, the local function
  $\LCT{f}_{i}$ with the set of adjacent edges $\setpfi = \{1,2,3\}$ is
  defined to be
  \begin{align*}
    \LCT{f}_{i}(\LCT{x}_{1}, \LCT{x}_{2}, \LCT{x}_{3})
      &\defeq \!\!\!\!\! 
      \sum_{
          x_{1,f_{i}} \in \set{X}_{1}, x_{2,f_{i}} \in  \set{X}_{2}, 
          x_{3,f_{i}} \in \set{X}_{2}
        } \!\!\!\!\!\!\!
            f_{i}(x_{1,f_{i}}, x_{2,f_{i}}, x_{3,f_{i}})
            \cdot
            h_3(x_{1,f_{i}}, \LCT{x}_{1})
            \nonumber\\
            &\hspace{3.5 cm}
            \cdot
            h_2(x_{2,f_{i}}, \LCT{x}_{2})
            \cdot
            h_4(x_{3,f_{i}}, \LCT{x}_{3}).
  \end{align*}
  The partition function of the S-NFG remains unchanged due to the way that $\LCT{f}$ is defined.
  
\end{enumerate}

%***************************************************************************

Let us now give the general definition of the LCT for an S-NFG $\graphN$ that
we use in this thesis, along with stating its main properties.


%***************************************************************************

\begin{definition}
  \label{sec:LCT:def:1}
  \index{LCT!for S-NFG}
  Consider some S-NFG $\graphN$ and let
  $\vmu $ be some SPA
  fixed-point message vector. 
  In the following, for each $ e = (f_{i}, f_{j}) \in \setEfull $, we use the
  short-hand notation $Z_e$ for $Z_e(\vmu)$, where
  (see~\eqref{sec:SNFG:eqn:6})
  \begin{align*}
    Z_e
      = \sum_{x_e} \mu_{\efi}(\xe) \cdot \mu_{\efj}(\xe).
  \end{align*}
  (Recall that in Assumption~\ref{asmp: assume messages are non-negative}, we assume that $ Z_e(\vmu) >0 $ for all $ e \in \setEfull $.) 
  We apply the following steps.
  \begin{enumerate}
  
  \item (generalization of the first step above) For every edge $e \in
    \setEfull$, we do the following.
  
    \begin{itemize}

    \item For every edge $e \in \setE$, we pick a special element of
      $\set{X}_e$. In order to simplify the notation, and without loss of
      generality, this special element will be called $0$ for all edges, \ie, we suppose that $ 0 \in \setxe $.
  
    \item We define the alphabet
      $\LCTset{X}_{e} \defeq \set{X}_e$.\footnote{The set $ \LCTset{X}_{e} $ can be different from $ \set{X}_e $. Essentially, the only requirement is that 
      $ |\LCTset{X}_{e}| = |\set{X}_e|$. In this thesis, we use the definition $ \LCTset{X}_{e} \defeq \set{X}_e $ for simplicity.}
  
    \item The edge $e$ (with associated variable $x_e$) connecting $f_{i}$ to $f_{j}$
      is replaced by the following alternating sequence of edges and function
      nodes: an edge with associated variable $x_{e,f_{i}} \in \set{X}_e$, a
      function node $M_{\efi}$, an edge with associated variable
      $\LCT{x}_e \in \LCTset{X}_{e}$, a function node $M_{\efj}$, and an edge
      with associated variable $x_{e,f_{j}} \in \set{X}_e$. Here:
      \begin{itemize}
  
      \item The function node $M_{\efi}$ is associated with the local function
        \begin{align*}
          M_{\efi}: \set{X}_e \times \LCTset{X}_{e} \to \sR;
        \end{align*}
      
      \item The function node $M_{\efj}$ is associated with the local function
        \begin{align*}
          M_{\efj}: \set{X}_e \times \LCTset{X}_{e} \to \sR.
        \end{align*}
  
      \end{itemize}
      In order to ensure that the partition function of the resulting factor graph equals the
      partition function of the original S-NFG, the local functions $M_{\efi}$
      and $M_{\efj}$ have to satisfy
      \begin{alignat}{2}
        \sum_{\LCT{x}_e}
          M_{\efi}(x_{\efi}, \LCT{x}_e)
          \cdot
          M_{\efj}(x_{\efj}, \LCT{x}_e) 
          &= [x_{\efi} \! = \!  x_{\efj}],
                \qquad x_{e,f_i}, x_{e,f_{j}} \in \set{X}_e,
                  \label{sec:LCT:exp:1}
      \end{alignat}
      where $ \sum_{\LCT{x}_e} $ represents $ \sum_{\LCT{x}_e \in \LCTset{X}_{e}} $ for simplicity.
      Note that~\eqref{sec:LCT:exp:1} implies\footnote{Let
        $\matr{M}_1$ and $\matr{M}_2$ be square matrices satisfying
        $\matr{M}_1 \cdot \matr{M}_2^\tran = \matr{I}$, where $\matr{I}$ is
        the identity matrix of the corresponding size. From linear algebra it
        is well known that this implies
        $\matr{M}_2^\tran \cdot \matr{M}_1 = \matr{I}$. Transposing both
        sides, one obtains $\matr{M}_1^\tran \cdot \matr{M}_2 = \matr{I}$.}
      \begin{alignat}{2}
        \sum_{x_e}
          M_{\efi}(\xe, \LCT{x}_{e,f_{i}})
          \cdot
          M_{\efj}(\xe, \LCT{x}_{e,f_{j}})
          &= \bigl[ \LCT{x}_{e,f_{i}} \! = \!  \LCT{x}_{e,f_{j}} \bigr]
          \qquad \LCT{x}_{e,f_{i}}, \LCT{x}_{e,f_{j}} \in \LCTset{X}_{e}.
          \label{sec:LCT:exp:2}
      \end{alignat}
  
    \item Let $\zeta_{\efi}$ and $\zeta_{\efj}$ be some arbitrary nonzero
      real-valued constants. At the heart of the LCT are the following definitions for 
      $M_{\efi}$ and $M_{\efj}$:
      \begin{alignat}{2}
        M_{\efi}(\xe,\LCT{x}_e)
          &= \zeta_{\efi}
               \cdot
               \mu_{\efi}(\xe),
                 \qquad x_e \in \set{X}_e, \ \LCT{x}_e = 0,
                     \label{sec:LCT:exp:3} \\
        M_{\efj}(\xe,\LCT{x}_e)
          &= \zeta_{\efj}
               \cdot
               \mu_{\efj}(\xe),
                 \qquad x_e \in \set{X}_e, \ \LCT{x}_e = 0.
                     \label{sec:LCT:exp:4}
      \end{alignat}
      Evaluating~\eqref{sec:LCT:exp:2} for $\LCT{x}_{\efi} = 0$ and
      $\LCT{x}_{\efj} = 0$, yields the following constraints on $\zeta_{\efi}$
      and $\zeta_{\efj}$:
      \begin{align}
        \zeta_{\efi}
        \cdot
        \zeta_{\efj}
          &= Z_e^{-1}.
               \label{sec:LCT:exp:5}
      \end{align}
      % where we use $Z_e$ for $Z_{e}(\vmu)$ as defined in~\eqref{sec:SNFG:eqn:6} for simplicity.
      
  
    \item A possible choice for the remaining function values of $M_{\efi}$ and
      $M_{\efj}$ is given as follows:
      \begin{align}
        &\hspace*{-1.6 cm}
        M_{\efi}(\xe,\LCT{x}_e)
          \defeq \zeta_{\efi}
                \cdot
                \chi_{\efi}
          \nonumber\\
          &\hspace*{-1.5 cm} \cdot
              \begin{cases}
                  - \mu_{\efj}(\LCT{x}_e)
                    & x_e = 0, \ 
                       \LCT{x}_e \in \LCTset{X}_{e}\setminus\{0\} \\
                  \delta_{\efi} 
                    \cdot
                    [x_e \!=\! \LCT{x}_e] 
                  +
                  \epsilon_{\efi}
                    \cdot
                    \mu_{\efi}(\xe) 
                    \cdot 
                    \mu_{\efj}(\LCT{x}_e)
                    & x_e \in \set{X}_e \setminus \{ 0 \}, \ 
                       \LCT{x}_e \in \LCTset{X}_{e}\setminus\{0\}
                \end{cases} 
        \label{sec:LCT:eqn:14},\\
        &\hspace*{-1.6 cm}
        M_{\efj}(\xe,\LCT{x}_e)
          \defeq 
          \zeta_{\efj}
                \cdot
                \chi_{\efj}
          \nonumber\\
          &\hspace*{-1.5 cm} 
            \cdot
                \begin{cases}
                  - \mu_{\efi}(\LCT{x}_e)
                    & x_e = 0, \ 
                       \LCT{x}_e \in \LCTset{X}_{e}\setminus\{0\} \\
                  \delta_{\efj} 
                    \cdot
                    [x_e \!=\! \LCT{x}_e] 
                  +
                  \epsilon_{\efj}
                    \cdot
                    \mu_{\efj}(\xe) 
                    \cdot 
                    \mu_{\efi}(\LCT{x}_e)
                    & x_e \in \set{X}_e \setminus \{ 0 \}, \ 
                       \LCT{x}_e \in \LCTset{X}_{e}\setminus\{0\}
                \end{cases},
            \label{sec:LCT:eqn:15}
      \end{align}
      where $\chi_{\efi}$ and $\chi_{\efj}$ are real-valued constants satisfying
      \begin{align}
        \chi_{\efi}
        \cdot
        \chi_{\efj}
          &= 1,
               \label{sec:LCT:exp:6}
      \end{align}
      where $\delta_{\efi}$, $\delta_{\efj}$ are real-valued constants satisfying
      \begin{align}
        \delta_{\efi} 
          \cdot
          \delta_{\efj}
          &= Z_e,
               \label{sec:LCT:exp:7}
      \end{align}
      where for $ \beli_e(0) \neq 1 $, the constants $\delta_{\efi}$, $\delta_{\efj}$, $\epsilon_{\efi}$, and
      $\epsilon_{\efj}$ satisfy
      \begin{align}
        \delta_{\efi} 
        + 
        Z_e
          \cdot 
          \bigl( 1 - \beli_e(0) \bigr)
          \cdot
          \epsilon_{\efi}
          &= \mu_{\efj}(0),
               \label{sec:LCT:exp:8} \\
        \delta_{\efj} 
        + 
        Z_e
          \cdot 
          \bigl( 1 - \beli_e(0) \bigr)
          \cdot
          \epsilon_{\efj}
          &= \mu_{\efi}(0),
               \label{sec:LCT:exp:9}
      \end{align}
      where for $ \beli_e(0) = 1 $, the constants $\delta_{\efi}$, $\delta_{\efj}$ satisfy~\eqref{sec:LCT:exp:8} and~\eqref{sec:LCT:exp:9}, respectively, and the constants $\epsilon_{\efi}$ and
      $\epsilon_{\efj}$ satisfy
      \begin{align}
        1
        +
        \delta_{\efi}
          \cdot
          \epsilon_{\efj}
        +
        \delta_{\efj} 
          \cdot
          \epsilon_{\efi} &= 0, 
          \label{extra constraint on epsilon for beli = [x = 0]}
      \end{align}
      and where $\beli_e(0) = \mu_{\efi}(0) \cdot \mu_{\efj}(0) / Z_e$ (see
      Definition~\ref{def:belief at SPA fixed point for S-NFG}). 
      The proof showing that the above gives a valid
      choice for $M_{\efi}$ and $M_{\efj}$ is given in
      Appendix~\ref{apx:LCT SNFGs}.
      

      Let $ \matr{M}_{\efi} $ and $ \matr{M}_{\efj} $ to be the matrices associated with $ M_{\efi} $ and $ M_{\efi} $, respectively, 
      with rows indices $ \xe $ and column indices $ \LCT{x}_e $.
      If $ \mu_{\efi}(0) = \mu_{\efj}(0) = 1 $ and $\mu_{\efi}(\xe) = \mu_{\efj}(\xe) = 0$ for $ \xe \in \setxe \setminus \{0\} $, then from~\eqref{sec:LCT:eqn:14} and~\eqref{sec:LCT:eqn:15}, the matrices $ \matr{M}_{\efi} $ and $ \matr{M}_{\efj} $ become
      %--------------------------------------------------------------------
      \begin{align*}
          \matr{M}_{\efi} = \matr{M}_{\efj} = \matr{I},
      \end{align*}
      %--------------------------------------------------------------------
      where $ \matr{I} $ is the identity matrix of size $ |\setxe| \times |\LCTset{X}_{e}| $.
      To sum up, in this case, the LCT is to set “0” in the associated off-diagonal entries in the matrices $ \matr{M}_{\efi} $ and $ \matr{M}_{\efj} $.


            % suppose that the row $ \matr{M}_{\efi}(\ze,:) $ is at the $ (i_{\ze}-1) $-th row in the matrix $ \matr{M}_{\efi} $ with $ i_{\ze} > 1 $. 
            % the expressions for
            % $ M_{\efi}(\ze,:) $, $ M_{\efi}(:,i_{\ze}-1) $, 
            % $ M_{\efj}(\ze,:) $, and $ M_{\efj}(:,i_{\ze}-1) $ becomes
            % %--------------------------------------------------------------------
            % \begin{align*}
            %     M_{\efi}(\ze,\LCT{x}_e) &= 
            %     \zeta_{\efj}
            %     \cdot
            %     \chi_{\efj}
            %     \cdot [ \LCT{x}_e = i_{\ze}-1 ], 
            %     \qquad ( \LCT{x}_e \in \LCTset{X}_{e} ), \nonumber\\
            %     M_{\efi}(\xe,i_{\ze}-1) &= 
            %     \zeta_{\efj}
            %     \cdot
            %     \chi_{\efj}
            %     \cdot [ \xe = \ze ], 
            %     \qquad ( \xe \in \setxe ),\nonumber\\
            %     M_{\efj}(\ze,\LCT{x}_e) &= M_{\efi}(\ze,\LCT{x}_e), \qquad 
            %     ( \LCT{x}_e \in \LCTset{X}_{e} ), \nonumber\\
            %     M_{\efj}(\xe,i_{\ze}-1) &= M_{\efi}(\xe,i_{\ze}-1), \qquad 
            %     ( \xe \in \setxe ).
            % \end{align*}
            % %--------------------------------------------------------------------
  
      Note that when $|\set{X}_e| = 2$, say $\set{X}_e = \{ 0, 1 \}$, and,
      correspondingly, $\LCTset{X}_{e} = \{ 0, 1 \}$, the function values of
      $M_{\efi}(1,1)$ and $M_{\efj}(1,1)$ are uniquely fixed:
        \begin{align*}
            M_{\efi}(1,1)
            &= \zeta_{\efi}
            \cdot
            \chi_{\efi}
            \cdot
            \mu_{\efj}(0), \\
            M_{\efj}(1,1)
            &= \zeta_{\efj}
            \cdot
            \chi_{\efj}
            \cdot
            \mu_{\efi}(0),
        \end{align*}
      \ie, although different choices are possible for $\delta_{\efi}$,
      $\delta_{\efj}$, $\epsilon_{\efi}$, and $\epsilon_{\efj}$, they all
      lead to the same function values for $M_{\efi}(1,1)$ and
      $M_{\efj}(1,1)$.
  
    \end{itemize}
  
  \item (generalization of the second step above) Nothing is done in this step.
  
  \item (generalization of the third step above) For every function node
    $f \in \setF$, we do the following.
    \begin{itemize}
  
    \item Let 
      $\LCTvxf \defeq ( \LCT{x}_e )_{e \in \setpf} \in \LCTsetx_{\setpf}$ and 
      $ \LCTsetx_{\setpf} \defeq \prod_{e \in \setpf} \LCTset{X}_{e} $.
  
    % \item Assume that $\setpf = \{ e_1, \ldots, e_{|\setpf|} \}$.
  
    \item Define
      \begin{align}
        \LCT{f}(\LCTvxf)
          &\defeq \sum_{\vx_{\setpf}}
            f(\vx_{\setpf})
            \cdot
            \prod_{e \in \setpf}
            M_{\ef}(x_{e}, \LCT{x}_e), \qquad 
            \LCTvxf \in \LCTsetx_{\setpf}.
        \label{sec:LCT:exp:10}
      \end{align}
  
    \item Finally, the LCT $\LCT{\graphN}$ of $\graphN$ based on $\vmu$ is
      defined to be the NFG with function node set $\setF$, edge set $\setE$,
      edge-function node incidence as for $\graphN$, where for every function
      node $f \in \setF$, the associated local function is $\LCT{f}$,
      and where for every edge $e \in \setE$, the associated variable 
      is $\LCT{x}_e$ and the associated alphabet is $ \LCTset{X}_{e} $.
      With this, the global function of $\LCT{\graphN}$ is defined to be the mapping
      \begin{align*}
          \LCT{g}: \prod_{e} \LCTset{X}_{e} &\to \sR, \nonumber\\
          \LCTv{x} &\mapsto \prod_f \LCT{f}(\LCTvxf).
      \end{align*}

      % \footnote{Note that we use the same labels to denote
      %   vertices and edges in $\LCT{\graphN}$ as in $\graphN$. However, now the
      %   local function associated with function node $f \in \setF$ is $\LCT{f}$
      %   and the variable associated with edge $e \in \setE$ is $\LCT{x}_e \in \LCTset{X}_{e}$.}
  
    \end{itemize}
  


  \end{enumerate}
  \edefinition
\end{definition}

\begin{remark}
  \label{sec:LCT:rem:1}
  The following remarks provide insights into the limitations and characteristics of the LCT in different scenarios.
  %----------------------------------------------------------------------------
  \begin{enumerate}
    \item There are S-NFGs where it is not possible to obtain $ M_{\efi} $ and $ M_{\efj} $ for $ e =(f_{i}, f_{j}) \in \setEfull $ based on the SPA fixed-point messages. 
    Consider a single-cycle S-NFG in Item~\ref{sec:SNFG:remk:1:item:2} in Remark~\ref{sec:SNFG:remk:1}. 
    % with local functions 
    % $\left(\begin{smallmatrix}
    %     1 & 1 \\ 0 & 1
    % \end{smallmatrix}\right)$ 
    % and 
    % $\left(\begin{smallmatrix}
    %     1 & 0 \\ 0 & 1
    % \end{smallmatrix}\right)$. 
    The SPA fixed-point message vector satisfies
    $ Z_e = 0 $ for all $ e \in \setEfull $ and thus the LCT does not work due to the equations~\eqref{sec:LCT:exp:3}--\eqref{sec:LCT:exp:5}. The existence of the LCT for this single-cycle S-NFG would contradict the non-diagonalizability of the matrix 
    $\left(\begin{smallmatrix}
        1 & 1 \\ 0 & 1
    \end{smallmatrix}\right)$. 
    % For more details, see also Item~\ref{sec:SNFG:remk:1:item:2} in Remark~\ref{sec:SNFG:remk:1}.

    \item\label{remk: LCT on snfg results an NFG with negative fun nodes}  The LCT $\LCT{\graphN}$ of $\graphN$ is in general \textbf{not} an S-NFG. This
    is because some of the local functions of $\LCT{\graphN}$ might take on
    negative real values. With that, also the global function of $\LCT{\graphN}$
    might take on negative real values.

    \item In the case of a binary alphabet $\set{X}_e$, the LCT we obtain is the same 
    as the one presented in~\cite{Chertkov2006}. However, for non-binary alphabets $\set{X}_e$,
    our LCT, although inspired by previous works such as~\cite{Chertkov2006, Chernyak2007, Mori2015}, is in general different. Notably, our approach does not require any assumption of non-zeroness on the SPA fixed-point messages.
  \end{enumerate}
  
 \eremark
\end{remark}

%***************************************************************************
%***************************************************************************

\begin{proposition}
  \label{sec:LCT:prop:1}
  \label{SEC:LCT:PROP:1}
  Consider an S-NFG $\graphN$ and let
  $\vmu $ be an SPA
  fixed-point message vector for $\graphN$.  
  The LCT of $ \graphN $, as specified in
  Definition~\ref{sec:LCT:def:1}, is denoted by $\LCT{\graphN}$. 
  (Recall that in Assumption~\ref{asmp: assume messages are non-negative}, 
  we assume $ Z_e(\vmu) >0 $ for all $ e \in \setEfull $, which ensures that the LCT of $ \graphN $ is well-defined.) 
  The main properties of $\LCT{\graphN}$ are listed as follows.
  \begin{enumerate}

  \item\label{sec:LCT:prop:1:item:1} The partition function remains the same:
    \begin{align*}
      Z(\graphN)
        &= Z\bigl( \LCT{\graphN} \bigr).
    \end{align*}

  \item\label{sec:LCT:prop:1:item:2} The SPA-based Bethe partition function of the original S-NFG is equal to the global function value of the all-zero configuration of
    $\LCT{\graphN}$:
    \begin{align*}
      \ZBSPA(\graphN,\vmu)
        &= \LCT{g}(\vect{0}).
    \end{align*}

  \item\label{sec:LCT:prop:1:item:3} For every $f \in \setF$ and every $\LCTvxf \in \LCTsetxf$ with
    exactly one nonzero component, \ie,
    %------------------------------------------------------------------------
    \begin{align*}
         \wh( \LCTvxf ) 
         = 1,
    \end{align*}
    %------------------------------------------------------------------------
    % where $  \wh( \LCTvxf )  \defeq \sum_{e \in \setpf} [\LCT{x}_{e} \!\neq\! 0] $,
    it holds that
    \begin{align*}
      \LCT{f}(\LCTvxf)
        &= 0,
    \end{align*}
    where $ \wh( \cdot ) $ is the Hamming weight of the argument.

  \item\label{sec:LCT:prop:1:item:4} 
    For any configuration $\LCTv{x} \in \prod_{e} \LCTset{X}_{e}$ in $ \LCT{\graphN} $, 
    we define 
    the associated subgraph $\bigl( \setF,\setE'(\LCTv{x}) \bigr)$, which consists of
    the set of vertices $ \setF $
    and the set of edges
    \begin{align*}
        \setE'(\LCTv{x})= \{ e \in \setE \ | \ \LCT{x}_{e} \neq 0 \}.
    \end{align*}
    The subgraph $\bigl( \setF,\setE'(\LCTv{x}) \bigr)$ is called a generalized loop 
    if this subgraph
    does not contain any leaves (vertices of degree one). (Note that for the all-zero
    configuration $\LCTv{x} = \vect{0}$, the subgraph $(\setF,\setE'(\LCTv{x}))$ 
    is also considered as a generalized loop.)

    It holds that if $ \LCTv{x} $ is a valid configuration for $ \LCT{\sfN} $,
    then the subgraph $ \bigl( \setF,\setE'(\LCTv{x}) \bigr) $ is a generalized
    loop, or equivalently, 
    if $ \bigl( \setF,\setE'(\LCTv{x}) \bigr) $ is not a generalized loop
    for the configuration $ \LCTv{x} $, then $\LCT{g}(\LCTv{x}) = 0$. 
    If $\graphN$ is cycle free and with that
    also $\LCT{\graphN}$ is cycle free, then 
    $\LCT{\graphN}$ has only one valid configuration, which is 
    the all-zero configuration and corresponds to a generalized loop.

  \item\label{sec:LCT:prop:1:item:5} 
  If $ \ZBSPA(\graphN,\vmu) \in \sR_{>0} $,
  it holds that
    \begin{align*}
      Z(\graphN)
        &= \ZBSPA(\graphN,\vmu)
           \cdot
           \left(
             1
             +
             \sum_{\LCTv{x}}
               \frac{\LCT{g}(\LCTv{x})}
                    {\LCT{g}(\vect{0})}
           \right), 
    \end{align*}
    where the summation is over all $ \LCTv{x} \in \prod_{e} \LCTset{X}_{e} $ such that $ \setE'(\LCTv{x}) $ corresponds to a nonzero generalized loop of
    $\LCT{\graphN}$. The term $\LCT{g}(\LCTv{x})/\LCT{g}(\vect{0})$ can
    be considered to be ``correction terms'' to the Bethe approximation. Note
    that if $\graphN$ is cycle free then there are no correction terms,
    implying the well-known result that
    $Z(\graphN) = \ZBSPA(\graphN,\vmu)$.

  \item\label{sec:LCT:prop:1:item:6} The SPA fixed-point message vector
    $\vmu $ for
    $\graphN$ induces an SPA fixed-point message vector
    $\LCTv{\mu} \defeq ( \LCTv{\mu}_{\ef} )_{f \in \setpe, e \in \setEfull}$ for
    $\LCT{\graphN}$ such that
    \begin{align*}
      \LCTv{\mu}_{\ef}
        &= \begin{pmatrix}
          1, & 0, & \cdots & 0
        \end{pmatrix}^{\!\!\!\tran} \in \sC^{|\LCTset{X}_{e}|},
        \qquad e \in \setE,\, f \in \setpe.
    \end{align*}

  \item\label{sec:LCT:prop:1:item:7} While the above properties are shared by all variants of the LCT, the
    LCT in Definition~\ref{sec:LCT:def:1} has the following additional
    properties (that are not necessarily shared by the other LCT variants):
    \begin{enumerate}
 
    \item For every $e = (f_{i},f_{j}) \in \setE$, the functions $M_{\efi}$ and
      $M_{\efj}$ are formally symmetric in the sense that swapping $f_{i}$ and
      $f_{j}$ in the definition of $M_{\efi}$ leads to the definition of
      $M_{\efj}$, and vice-versa.

    \item\label{sec:LCT:prop:1:item:7:b} Assume that $M_{\efi}$ and $M_{\efj}$ are defined based on the
      choices $\zeta_{\efi} = \zeta_{\efj} \defeq Z_e^{-1/2}$,
      $\chi_{\efi} = \chi_{\efj} \defeq 1$,
      $\delta_{\efi} = \delta_{\efj} \defeq Z_e^{1/2}$. Let
      $e = (f_{i},f_{j}) \in \setE$ be an edge such that
      $\mu_{\efi}(\xe) = \mu_{\efj}(\xe) \in \sR$ for all $x_e \in \set{X}_e$. Then
      the matrices $\matr{M}_{\efi}$
      and $\matr{M}_{\efj}$ are equal
      and orthogonal.

    \end{enumerate}

  \end{enumerate}
\end{proposition}

%***************************************************************************

\begin{proof}
  See Appendix~\ref{apx:property of SNFGs}.
\end{proof}

We conclude this section with some remarks.
%---------------------------------------------------------------------------
\begin{itemize}
  
    \item Property~\ref{sec:LCT:prop:1:item:2} in Proposition~\ref{sec:LCT:prop:1} states that the LCT is a reparamerization of the global function based on the SPA fixed point message vector $ \vmu $ such that 
    the global function evaluated at $ \LCTv{x} = \vect{0} $ equals the $\vmu$-based Bethe partition function. The LCT can be viewed as shifting the bulk of the sum over the variables of the global function to some known configuration as well as keeping the partition function unchanged.

    \item Property~\ref{sec:LCT:prop:1:item:6} in Proposition~\ref{sec:LCT:prop:1} highlights that after applying the LCT on $\graphN$ based on the SPA fixed-point message vector $\vmu$, one of the SPA fixed-point message vectors for the LCT-transformed factor graph $\LCT{\graphN}$ has a simple structure. 
    Specifically, this simple SPA fixed-point message vector, denoted by $ \LCT{\vmu} $, satisfies 
    \begin{align*}
      \ZBSPA( \graphN, \vmu ) &= \ZBSPA( \LCT{\graphN}, \LCT{\vmu} ), \nonumber\\
      \LCT{\mu}_{\efi}(\LCT{x}_e) 
      &= \LCT{\mu}_{\efj}(\LCT{x}_e) = [\LCT{x}_e \! = \! 0], \qquad
      \LCT{x}_{e} \in \LCTset{X}_{e},\, e = (f_{i}, f_{j}) \in \setEfull.
    \end{align*}
    This simple structure partially motivates the proof of the graph-cover theorem in Section~\ref{sec:CheckCon}.

\end{itemize}
%---------------------------------------------------------------------------



%***************************************************************************
%***************************************************************************

\section{LCT for DE-NFGs}
\label{sec:LCT:DENFG:1}

% \input{figures/lct_examples/penfg/main_pic.tex}

The LCT for DE-NFGs has many similarities to the LCT for S-NFGs. Therefore, we will mostly highlight the differences in this section. 
% We also give a high-level introduction of the LCT for DE-NFGs by considering a
% specific DE-NFG $\graphN$ and assume that some part of it looks as shown in Fig.~\ref{sec:LCT:fig:7}. Let $\vmu $ be some SPA
% fixed-point message vector for $\graphN$ satisfying~\eqref{sec:DENFG:eqn:15}. The LCT of this DE-NFG involves a series of operations, including opening-the-box and closing-the-box operations. 
% \begin{enumerate}

% \item The DE-NFG in Fig.~\ref{sec:LCT:fig:8} is obtained from the DE-NFG
%   in Fig.~\ref{sec:LCT:fig:7} by applying suitable opening-the-box
%   operations. Assumption~\ref{sec:DENFG:asum:2} states that the considered DE-NFG $ \graphN $ is a strict-sense DE-NFG. By~\eqref{sec:DENFG:eqn:5}--\eqref{sec:DENFG:eqn:8}, each local function $ f $ in $ \graphN $ can be decomposed in terms of the eigenvalue $ \lambda_{f} $ and the eigenvector $ u_{f} $ of the associated Choi-matrix representation $ \matr{C}_{f} $. Specifically, for function nodes $f_i$ and $f_j$ in Fig.~\ref{sec:LCT:fig:8}, we have
%   %-----------------------------------------------------------------------
%   \begin{align*}
%     f_{i}(\vx_{\pone},\vx_{\ptwo},\vx_{\pthre}) 
%     &= \sum_{\ell_{f_{i}} \in \set{L}_{f_{i}}}
%         \lambda_{f_{i}}(\ell_{f_{i}}) \cdot
%         u_{f_{i}}(x_{1},x_{2},x_{3},\ell_{f_{i}}) 
%         \cdot 
%         \overline{u_{f_{i}}(x_{\upone},x_{\uptwo},x_{\upthre},\ell_{f_{i}})}, \nonumber\\
%     f_{j}(\vx_{\pone},\vx_{\pfor},\vx_{\pfif}) 
%     &= \sum_{\ell_{f_{j}} \in \set{L}_{f_{j}}}
%         \lambda_{f_{j}}(\ell_{f_{j}}) \cdot
%         u_{f_{j}}(x_{1},x_{4},x_{5},\ell_{f_{j}}) 
%         \cdot 
%         \overline{u_{f_{j}}(x_{\upone},x_{\upfor},x_{\upfif},\ell_{f_{j}})}.
%   \end{align*}
%   %-----------------------------------------------------------------------
 

%     \item The DE-NFG in Fig.~\ref{sec:LCT:fig:9} is constructed based on the original DE-NFG in Fig.~\ref{sec:LCT:fig:8}, taking into account the SPA fixed-point message vector $\vmu$. The construction ensures that the partition function remains unchanged. 
%     %----------------------------------------------------------------------------
%     \begin{itemize}
%         \item For example, for the edge $1$ connecting function nodes $f_{i}$ and $f_{j}$, as shown in Fig.~\ref{sec:LCT:fig:8}, we introduce function nodes $h_3$ and $h_8$ with local functions $h_3: \set{X}_{1} \times \LCTset{X}_{1} \to \sC$ and $h_8: \set{X}_{1} \times \LCTset{X}_{1} \to \sC$, where $\LCTset{X}_{1} \defeq \bigl\{ 0, 1, \ldots, |\set{X}_{1}| \! - \! 1 \bigr\}$ and $ \set{X}_{1}$ is the alphabet of edge $ 1 $ as defined in Definition~\ref{sec:DENFG:def:4}.

%         \item Because of the property of the SPA in Lemma~\ref{sec:DENFG:lem:2}, we introduce local functions
%         $ \overline{ h_{3}(x_{\upone}, \LCT{x}_{\upone}) } $ 
%         and 
%         $ \overline{ h_{8}(x_{\upone}, \LCT{x}_{\upone}) } $ for edge $ \upone $.
%     \end{itemize}
%     %----------------------------------------------------------------------------
%     The partition function of the DE-NFG is unchanged because $h_3$ and $h_8$ are defined such that  $\sum_{\LCT{x}_{1}} h_3(x_{1,f_{i}}, \LCT{x}_{1}) \cdot h_8(x_{1,f_{j}}, \LCT{x}_{1}) = [x_{1,f_{i}} \! = \!  x_{1,f_{j}}]$ for all $ x_{1,f_{i}}$ and  $ x_{1,f_{j}} $ in $ \setx_{1} $. 
    

%     \item The DE-NFG in Fig.~\ref{sec:LCT:fig:10} is essentially the same as the DE-NFG in Fig.~\ref{sec:LCT:fig:9}.
  
%     \item The DE-NFG in Fig.~\ref{sec:LCT:fig:11} is obtained by applying suitable closing-the-box operations, as introduced in Section~\ref{sec:LCT:SNFG:1}, to the DE-NFG in Fig.~\ref{sec:LCT:fig:10}. For example, we define the function $u'_{f_{i}}$ in Fig.~\ref{sec:LCT:fig:11} to be  the resulting exterior function obtained by closing the upper left dashed box in Fig.~\ref{sec:LCT:fig:10}, \ie,
%       \begin{align*}
%           u'_{f_{i}}(\LCT{x}_{1}, \LCT{x}_{2}, \LCT{x}_{3},\ell_{f_{i}})
%           &\defeq \sum_{x_{1}, x_{2}, x_{3}}
%                 u_{f_{i}}(x_{1}, x_{2}, x_{3},\ell_{f_{i}})
%                 \cdot
%                 h_3(x_{1}, \LCT{x}_{1})
%                 \cdot
%                 h_2(x_{2}, \LCT{x}_{2})
%                 \cdot
%                 h_4(x_{3}, \LCT{x}_{3}), \qquad 
%           \ell_{f_{i}} \in \set{L}_{f_{i}}.
%       \end{align*}
%       Similarly, the local function $ \overline{u'_{f_{i}}} $ in Fig.~\ref{sec:LCT:fig:11}, which corresponds to the exterior function of the lower left dashed box in Fig.~\ref{sec:LCT:fig:10},
%       is introduced.
%       Because of the way that $u'_{f_{i}}$ and $ u'_{f_{j}} $ are defined, the partition function of the DE-NFG in Fig.~\ref{sec:LCT:fig:11} is unchanged.

%     \item The DE-NFG in Fig.~\ref{sec:LCT:fig:12} is obtained by applying suitable closing-the-box operations to the DE-NFG in
%     Fig.~\ref{sec:LCT:fig:11}:
%     %-----------------------------------------------------------------------
%   \begin{align*}
%     \LCT{f}_{i}(\LCTv{x}_{\pone},\LCTv{x}_{\ptwo},\LCTv{x}_{\pthre}) 
%     &= \sum_{\ell_{f_{i}} \in \set{L}_{f_{i}}}
%         \lambda_{f_{i}}(\ell_{f_{i}}) \cdot
%         u'_{f_{i}}(\LCT{x}_{1},\LCT{x}_{2},\LCT{x}_{3},\ell_{f_{i}}) 
%         \cdot 
%         \overline{
%             u'_{f_{i}}(\LCT{x}_{\upone},\LCT{x}_{\uptwo},
%             \LCT{x}_{\upthre},\ell_{f_{i}})
%         }, \nonumber\\
%     \LCT{f}_{j}(\LCTv{x}_{\pone},\LCTv{x}_{\pfor},\LCTv{x}_{\pfif}) 
%     &= \sum_{\ell_{f_{j}} \in \set{L}_{f_{j}}}
%         \lambda_{f_{j}}(\ell_{f_{j}}) \cdot
%         u'_{f_{j}}(\LCT{x}_{1},\LCT{x}_{4},\LCT{x}_{5},\ell_{f_{j}}) 
%         \cdot 
%         \overline{
%             u'_{f_{j}}(\LCT{x}_{\upone},\LCT{x}_{\upfor},\LCT{x}_{\upfif},\ell_{f_{j}})
%         }.
%   \end{align*}
%   %-----------------------------------------------------------------------
 
  
% \end{enumerate}


\begin{definition}
    \label{def:DENFG:LCT:1}
    \index{LCT!for DE-NFG}
    The LCT for DE-NFGs is a natural extension of the LCT for S-NFG in Definition~\ref{sec:LCT:def:1}. 
    Further definitions are made for DE-NFGs.
    For each edge $ e \in \setEfull $, we apply the following changes.
    \begin{itemize}

        \item The alphabet $\set{X}_e$ is replaced by the alphabet $\tset{X}_e = \set{X}_e \times \set{X}_e$.

        \item The special element $0 \in \set{X}_e$ is replaced by the special element
        $\tzero \defeq (0,0) \in \tset{X}_e$.

        \item The variable $x_e \in \set{X}_e$ is replaced by the variable
        $\tx_e = (x_e,x'_e) \in \tset{X}_e$.

        \item The alphabet
        $\LCTset{X}_e \defeq \set{X}_e$ is
        replaced by the alphabet
        $\LCTtset{X}_e \defeq \tset{X}_e$.

        \item The element $0 \in \LCTset{X}_e$ is replaced by the element
        $\tzero\in \LCTtset{X}_e$.

        \item The variable $\LCT{x}_e \in \LCTset{X}_e$ is replaced by the variable
        $\LCTt{x}_e = (\LCT{x}_e, \LCT{x}'_e) \in \LCTtset{X}_{e}$.

    \end{itemize}
    Note that in the definition for DE-NFG, we consider that the constants $\zeta_{\efj}$, $\chi_{\efj}$, $\delta_{\ef}$, and $\epsilon_{\ef}$ are real-valued.

    For any finite set $ \set{I} \subseteq \setEfull $, we define
    %--------------------------------------------------------------------
    \begin{align*}
        \LCTtset{X}_{ \set{I} }
        \defeq \prod_{e \in \set{I}} \LCTtset{X}_{ e }
        = \LCTset{X}_{ \set{I} } \times \LCTset{X}_{ \set{I} },
    \end{align*}
    %--------------------------------------------------------------------
    where
    \begin{align*}
      \LCTset{X}_{ \set{I} } \defeq 
        \prod_{e \in \set{I}} \LCTset{X}_{e}.
    \end{align*}
    The associated collection of variables is defined to be
    \begin{align*}
      \LCTtv{x}_{\set{I}} \defeq ( \LCTv{x}_{\set{I}}, \LCTv{x}_{\set{I}}' )
      \in \LCTtset{X}_{ \set{I} }
    \end{align*}
    % %------------------------------------------------------------------------
    % \begin{align*}
    %     , \qquad 
    %     \LCTv{x}_{\set{I}} \defeq (\LCT{x}_{e})_{e \in \set{I}}
    %     \in \LCTsetx_{\set{I}}, \qquad  
    %     \LCTv{x}_{\upset{I}} \defeq (\LCT{x}_{\upe})_{\upe \in \upset{I}}
    %     \in \LCTset{X}_{\upset{I}}.
    %     % \label{sec:LCT:eqn:13}
    % \end{align*}
    % %------------------------------------------------------------------------

    % For $ \set{I} \subseteq \setEfull $, we define
    %  %--------------------------------------------------------------------
    %  \begin{align*}
    %       \LCTtset{X}_{ \set{I} }
    %       \defeq \prod_{e \in \set{I}} \LCTtset{X}_{e}.
    %  \end{align*}
    %  %--------------------------------------------------------------------

     For each $ f \in \setF $, we define
      \begin{align}
        \LCT{f}(\LCTtv{x}_{\setpf})
            &\defeq \sum_{\tvx_{\setpf}}
            f(\tvx_{\setpf})
            \cdot
            \prod_{e \in \setpf}
              M_{\ef}(\tx_{e}, \LCTt{x}_e),
        \qquad \LCTtv{x}_{\setpf} \in \LCTtset{X}_{\setpf}.
        \label{sec:LCT:eqn:1}
      \end{align}

    %----------------------------------------------------------------------------
    % \begin{enumerate}
    %     \item \label{def:DENFG:LCT:1:item:3} For every edge 
    %     $ e \in \setEfull $, we define 
    %     $ \LCTtset{X}_{e} \defeq \LCTset{X}_{e} \times \LCTset{X}_{e}$
    %     where $
    %     \LCTset{X}_{e} \defeq 
    %     \bigl\{ 0, 1, \ldots, |\set{X}_{e}| \! - \! 1 \bigr\}$. 
    %     The associated variable is $ \LCTt{x}_{e} = 
    %     ( \LCT{x}_{e}, \LCT{x}_{e}' ) \in \LCTtset{X}_{e} $.

    %     \item Similar to Definition~\ref{sec:LCT:def:1}, for each $ e = (f_{i}, f_{j}) \in \setEfull $, we define the functions $ M_{\efi} $ and $ M_{\efj} $ based on the SPA fixed-point message vectors $ \vmu_{\efi} $ and $ \vmu_{\efj} $. 

        % \item For each $ \upe = (f_{i}, f_{j}) \in \upsetEfull $, motivated by $ \vmu_{\upefi} = \overline{\vmu_{\efi}} $ and $ \vmu_{\upefj} = \overline{\vmu_{\efj}} $ as proven in Lemma~\ref{sec:DENFG:lem:2}, we define
        % %-----------------------------------------------------------------------
        % \begin{align*}
        %     M_{\upefi}(x_{\upe},\LCT{x}_{\upe}) \defeq 
        %     \overline{ M_{\efi}(x_{\upe},\LCT{x}_{\upe}) }, \qquad 
        %     M_{\upefj}(x_{\upe},\LCT{x}_{\upe}) \defeq 
        %     \overline{ M_{\efj}(x_{\upe},\LCT{x}_{\upe}) }, \qquad 
        %     x_{\upe} \in \setxupe, \, 
        %     \LCT{x}_{\upe} \in \LCTset{X}_{\upe}.
        % \end{align*}
        % %-----------------------------------------------------------------------

      % \item\label{} The alphabet
      %   $\LCTset{X}_{e} \defeq \bigl\{ 0, 1, \ldots, |\set{X}_e| \! - \! 1 \bigr\}$ is
      %   replaced by the alphabet
      %   $\LCTset{X}_{e} \defeq \bigl\{ 0, 1, \ldots, |\set{X}_e| \! - \! 1 \bigr\}^2 = \LCTset{X}_{e} \times \LCTset{X}_{\upe}
      %   $ for the pair of variables $ \xpe $, where $ \LCTset{X}_{e} \defeq \bigl\{ 0, 1, \ldots, |\set{X}_e| \! - \! 1 \bigr\} $ and $ \LCTset{X}_{\upe} \defeq  \bigl\{ 0, 1, \ldots, |\set{X}_e| \! - \! 1 \bigr\} $.

    % \end{enumerate}
    % %----------------------------------------------------------------------------

    % apart from
    % the following changes in Definition~\ref{sec:LCT:def:1}. 
    % For each edge $ e \in \setEfull  $, we make the following changes.
    % \begin{enumerate}

    %     \item The variable $x_e \in \set{X}_e$ is replaced by the pair of variables
    %     $\xpe = (\xe,x_{\upe}) \in \set{X}_{e}$.

    %     
    %     \item The special element $0 \in \set{X}_e$ is replaced by the special element
    %     $(0,0) \in \set{X}_{e}$.

    %     \item The element $0 \in \LCTset{X}_{e}$ is replaced by the element
    %     $(0,0) \in \LCTset{X}_{e}$.

    %     \item The variable $\LCT{x}_e \in \LCTset{X}_{e}$ is replaced by the variable
    %     $\LCTv{x}_{e} = (\LCT{x}_e, \LCT{x}_{\upe}) \in \LCTset{X}_{e}$.

    % % \end{enumerate}
    % \begin{enumerate}
    % %   \setcounter{enumi}{1}
    %    \item\label{def:DENFG:LCT:1:item:1} 
       
    %   The associated variable is given by
    %    %------------------------------------------------------------------------
    %    \begin{align*}
    %         \LCTtv{x}_{\set{I}} = ( \LCTtv{x}_{e} )_{ e \in \set{I} }
    %         \in \LCTset{X}_{ \set{I} }.
    %         % \label{sec:LCT:eqn:13}
    %    \end{align*}
    %    %------------------------------------------------------------------------
        % For each $ f \in \setF $, the alphabet for $\LCT{f}$ is given by the alphabet
        % $\LCTsetxpf \defeq \LCTsetxf \times \LCTset{X}_{\upsetpf}$ and the associated argument is $ \LCTv{x}_{\setpf} $
      

       %  \item\label{def:DENFG:LCT:1:item:4} 
       %  We define the variable $ \vx_{\setpf,f} $ to be
       %  %-----------------------------------------------------------------------
       %  \begin{align*}
       %    \vx_{\setpf,f} \defeq ( x_{ef})_{e \in \setpf} \in \setxpf,
       %  \end{align*}
       %  %----------------------------------------------------------------------- 
       % where the set $ \setxpf $ is defined in Item~\ref{sec:DENFG:def:4:item:3} in Definition~\ref{sec:DENFG:def:4}. We also define
       % %--------------------------------------------------------------------
       % \begin{align}
       %  \LCTv{x}_{\setpf,f} \defeq (\LCT{x}_{e,f})_{e \in \setpf} 
       %  \in \LCTsetxf. \label{sec:LCT:eqn:16}
       % \end{align}
       % %--------------------------------------------------------------------
        

        % \item\label{def:DENFG:LCT:1:item:2} 

        % \item We define the global function to be 
        % $ \LCT{g}(\LCTtv{x}) \defeq \prod_{f} \LCT{f}(\LCTtv{x}_{\setpf}) $ with 
        % $ \LCTtv{x} \defeq ( \LCTtv{x}_{e} )_{ e \in \setEfull } 
        % \in \prod_{e \in \setEfull} \LCTsetx_{e} $.
    % \end{enumerate}
    % where $ \sum_{\vx_{\setpf}} $ is a shorthand of $ \sum_{\vx_{\setpf,f}\in \setxpf} $.
    \edefinition
\end{definition}


If there is no ambiguity, for any $ \set{I} \subseteq \setEfull $,
we will use $ \sum_{ \LCTtv{x}_{\set{I}} } $ instead of 
$ \sum_{ \LCTtv{x}_{ \set{I} } \in \LCTtset{X}_{\set{I}} } $ for simplicity.


%***************************************************************************

\begin{proposition}
  \label{prop:DENFG:LCT:1}
  \label{PROP:DENFG:LCT:1}

  Consider a DE-NFG $\graphN$ and an SPA
  fixed-point message vector $ \vmu $ for $\graphN$. 
  Let $\LCT{\graphN}$ denote the LCT of $\graphN$ obtained by $\vmu$, as specified in
  Definition~\ref{def:DENFG:LCT:1}. The main properties of $\LCT{\graphN}$ are listed as follows.
  \begin{enumerate}

  \item Natural extension of Property~\ref{sec:LCT:prop:1:item:1} in Proposition~\ref{sec:LCT:prop:1}:
  $
      Z(\graphN)
        = Z\bigl( \LCT{\graphN} \bigr).
  $
  % (modulo the notational changes mentioned in Definition~\ref{def:DENFG:LCT:1})
  \item\label{prop:DENFG:LCT:1:item:4} Natural extension of Property~\ref{sec:LCT:prop:1:item:2} in Proposition~\ref{sec:LCT:prop:1}:
    \begin{align*}
      \ZBSPA(\graphN,\vmu)
        = \LCT{g}(\tv{0}) = \prod_{f} \LCT{f}(\tv{0}),
    \end{align*}
    where $ \tv{0} = ( \tzero,\ldots,\tzero ) $.

  \item\label{sec:LCT:prop:1:item:8} Natural extension of Property~\ref{sec:LCT:prop:1:item:3} in Proposition~\ref{sec:LCT:prop:1}: for every $f \in \setF$ and every $\LCTv{x}_{\setpf} \in \LCTsetx_{\setpf}$ with exactly one nonzero component, 
  \ie, 
    %------------------------------------------------------------------------
    \begin{align*}
        \wh( \LCTv{x}_{\setpf} )
        = 1,
    \end{align*}
    %------------------------------------------------------------------------
    with $ \wh( \LCTv{x}_{\setpf} ) \defeq 
    \sum_{ e \in \setpf } \bigl[ \LCTt{x}_{e} \!\neq\! \tzero \bigr] $,
    it holds that
    \begin{align*}
      \LCT{f}(\LCTtv{x}_{\setpf})
        &= 0.
    \end{align*}
  % (modulo the notational changes mentioned in
    % Definition~\ref{def:DENFG:LCT:1} and the replacement of ``nonzero
    % component'' by ``component not equal to $(0,0)$'')

  \item Natural extension of Property~\ref{sec:LCT:prop:1:item:4} in Proposition~\ref{sec:LCT:prop:1}.
    % (modulo the notational changes mentioned in
    % Definition~\ref{def:DENFG:LCT:1}).

  \item Natural extension of Property~\ref{sec:LCT:prop:1:item:5} in Proposition~\ref{sec:LCT:prop:1}.
    % (modulo the notational changes mentioned in
    % Definition~\ref{def:DENFG:LCT:1}).

  \item Natural extension of Property~\ref{sec:LCT:prop:1:item:6} in Proposition~\ref{sec:LCT:prop:1}
    % (modulo the notational changes mentioned in
    % Definition~\ref{def:DENFG:LCT:1}). 
    Nevertheless, because of its importance
    for later parts of this thesis, the statement is included here. Namely, the
    SPA fixed-point message vector
    $\vmu$ for
    $\graphN$ induces an SPA fixed-point message vector $ \LCTv{\mu} 
    = ( \LCTv{\mu}_{e,f} )_{e \in \setpf, f \in \setF} $
    for
    $\LCT{\graphN}$ with
    \begin{align*}
        \LCT{\mu}_{e,f}(\LCTt{x}_{e})
        &= \left[ \LCTt{x}_{e} \! = \! \tzero \right],
        \qquad
        \LCTt{x}_{e} \in \LCTtset{X}_{e}.
        % \\
        % \LCT{\mu}_{\upefi}(\LCT{x}_{\upe}) & 
        % = \bigl[ \LCT{x}_{\upe} \! = \! 0 \bigr],
        %    \qquad e =(e,\upe) \in \setEfull, \, 
        %    f \in \setpe,\, 
        %    \LCT{x}_{\upe} \in \LCTset{X}_{\upe}. \nonumber
    \end{align*}
    %-----------------------------------------------------------------------
    % Recall $  \setppe = \setpe =  \setupe $ as defined in Definition~\ref{sec:DENFG:def:4}. 
    % where is defined in item~\ref{def:DENFG:LCT:1:item:3} in Definition~\ref{def:DENFG:LCT:1}.

  \item Natural extension of Property~\ref{sec:LCT:prop:1:item:7} in Proposition~\ref{sec:LCT:prop:1}.
    % (modulo the notational changes mentioned in
    % Definition~\ref{def:DENFG:LCT:1}). 
    Note that Property~\ref{sec:LCT:prop:1:item:7:b} is slightly different:
    Assume that $M_{\efi}$ and $M_{\efj}$ are defined based on the
    choices $\zeta_{\efi} = \zeta_{\efj} \defeq Z_e^{-1/2}$,
    $\chi_{\efi} = \chi_{\efj} \defeq 1$,
    $\delta_{\efi} = \delta_{\efj} \defeq Z_e^{1/2}$. Let
    $e = (f_{i},f_{j}) \in \setE$ be an edge such that
    $\mu_{\efi}(\txe) = \overline{\mu_{\efj}(\txe)}$ for all $x_e \in \set{X}_e$. In this case, both $ \matr{M}_{\efi} $ and $ \matr{M}_{\efj} $ are unitary matrices with row indices $ \xe $ and column indices $ \LCT{x}_{e} $, and they satisfy
    $ \matr{M}_{\efi} = \matr{M}_{\efj}^{\Herm} $.

    \item\label{prop:DENFG:LCT:1:item:1} For each $ e = (f_{i}, f_{j}) $, the Choi-matrix representations 
    $ \matr{ C }_{ M_{\efi} } $ and $ \matr{ C }_{ M_{\efi} } $
    are complex-valued Hermitian matrices.


    \item\label{prop:DENFG:LCT:1:item:2} For each $f \in \setF$, 
      the Choi-matrix representation $\matr{C}_{\LCT{f}}$ is a complex-valued Hermitian matrix,
      where $ \matr{C}_{\LCT{f}} $ is defined to be a matrix with row indices $ \LCTv{x}_{\setpf} $ and column indices $ \LCTv{x}_{\setpf}' $ such that
      %-------------------------------------------------------------------
      \begin{align}
          \matr{C}_{\LCT{f}} \defeq 
          \Bigl( \LCT{f}(\LCTv{x}_{\setpf}, \LCTv{x}_{\setpf}') 
          \Bigr)_{ (\LCTv{x}_{\setpf}, \LCTv{x}_{\setpf}') 
          \in \LCTtset{X}_{\setpf} }.
          \label{sec:LCT:eqn:6}
      \end{align}
      %-------------------------------------------------------------------

      

    % \item\label{prop:DENFG:LCT:1:item:5} For each $ f \in \setF $, 
    %     there exist a finite set $\LCTset{L}_{f} = \{ 0, 1, \ldots, \bigl|\LCTsetxf \bigr|-1 \}$, 
    %     a variable $\LCTellf \in \LCTset{L}_{f}$,  
    %     a coefficient $\LCT{\lambda}_{f}\bigl( \LCTellf \bigr) \in \sR_{\geq 0} $, and
    %     functions $\LCT{u}_{f}$ and $ \LCT{L}_{f} $ such that
    %     \begin{align}
    %         \LCT{f}(\LCTv{x}_{\setpf})
    %         &= \sum_{\LCTellf }
    %             \LCT{\lambda}_{f}\bigl( \LCTellf \bigr) \cdot
    %             \LCT{u}_{f}\bigl( \LCTv{x}_{\setpf}, \LCTellf \bigr) 
    %         \cdot 
    %         \overline{ 
    %             \LCT{u}_{f}
    %             (\LCTv{x}_{\unpair{\setpf}}, \LCTellf)
    %         } \label{sec:LCT:eqn:2}\\
    %         %----------------------------------------------------------
    %         &= \sum_{\LCTellf }
    %             \LCT{L}_{f}\bigl( \LCTv{x}_{\setpf}, \LCTellf \bigr) 
    %         \cdot 
    %         \overline{ 
    %             \LCT{L}_{f}\bigl( \LCTv{x}_{\setpf}, \LCTellf \bigr)
    %         }, \qquad \LCTv{x}_{\setpf} \in \LCTsetxpf, \label{sec:LCT:eqn:17} \\
    %         %----------------------------------------------------------
    %         \Bigl[ \LCT{\ell}_{f} \!=\! \LCT{\ell}_{f}' \Bigr]
    %         &= \sum_{ 
    %           \LCTv{x}_{\setpf} 
    %         }
    %         \LCT{u}_{f}\bigl( \LCTv{x}_{\setpf}, \LCT{\ell}_{f} \bigr) 
    %         \cdot 
    %         \overline{\LCT{u}_{f}
    %         \bigl( \LCTv{x}_{\setpf}, \LCT{\ell}_{f}' \bigr)},
    %         \qquad
    %         \LCT{\ell}_{f},\LCT{\ell}_{f}' \in \LCTset{L}_{f},
    %         \label{sec:LCT:eqn:5}\\
    %         %----------------------------------------------------------
    %         \LCT{\lambda}_{f}\bigl( \LCTellf \bigr) &\in \sR_{\geq 0}, \qquad 
    %         \LCTellf \in \LCTset{L}_{f}, \qquad
    %         \LCT{\lambda}_{f}(0) \geq \LCT{\lambda}_{f}(1) \geq \cdots 
    %         \geq \LCT{\lambda}_{f}\Bigl( \bigl|\LCTsetxf \bigr| -1 \Bigr),
    %         \label{sec:LCT:eqn:3}
    %     \end{align}
    %   where 
    %   %------------------------------------------------------------------------
    %     \begin{align}
    %         \LCT{L}_{f}\bigl( \LCTv{x}_{\setpf}, \LCTellf \bigr) 
    %         &\defeq \sqrt{ \LCT{\lambda}_{f}\bigl( \LCTellf \bigr) } \cdot
    %           \LCT{u}_{f}\bigl( \LCTv{x}_{\setpf}, \LCTellf \bigr),
    %         \qquad \LCTv{x}_{\setpf} \in \LCTsetx_{\setpf},\,
    %         \LCTellf \in \LCTset{L}_{f}. 
    %         \label{def: the cholesky decomposition of LCT of f} 
    %     \end{align}
    %     %------------------------------------------------------------------------
    %   If we define $ \LCTv{u}_{f}(\ell_f) $ to be the column vector associated with 
    %   $ \LCT{u}_{f} $:
    %   %-----------------------------------------------------------------------
    %   \begin{align}
    %     \LCTv{u}_{f}\bigl( \LCT{\ell}_f \bigr) \defeq
    %     \Bigl( 
    %       \LCT{u}_{f}\bigl( \LCTv{x}_{\setpf}, \ell_f \bigr) 
    %     \Bigr)_{ \LCTv{x}_{\setpf} \in \LCTsetxf } 
    %     \in \sC^{ | \LCTsetxf |},
    %     \label{sec:LCT:eqn:8}
    %   \end{align}
    %   %-----------------------------------------------------------------------
    %   then the conditions in~\eqref{sec:LCT:eqn:2}--\eqref{sec:LCT:eqn:3} are equivalent to
    %   %-------------------------------------------------------------------
    %   \begin{align}
    %     \matr{C}_{\LCT{f}} &= \sum_{\LCT{\ell}_f } 
    %     \LCT{\lambda}_{f}\bigl( \LCT{\ell}_{f} \bigr)
    %     \cdot \LCTv{u}_{f}\bigl( \LCT{\ell}_f \bigr)
    %     \cdot \Bigl( \LCTv{u}_{f}\bigl( \LCT{\ell}_f \bigr) \Bigr)^{\!\!\Herm},
    %     \nonumber \\
    %     [\LCT{\ell}'_f \!=\! \LCT{\ell}_f] &= 
    %     \Bigl( \LCTv{u}_{f}\bigl( \LCT{\ell}'_f \bigr) \Bigr)^{\!\!\Herm} 
    %     \cdot \LCTv{u}_{f}\bigl( \LCT{\ell}_f \bigr), \qquad 
    %     \LCT{\ell}_{f},\LCT{\ell}_{f}' \in \LCTset{L}_{f}.
    %     \nonumber
    %   \end{align}
    %   %-------------------------------------------------------------------
      
    %   The collections of vectors 
    %   $ \bigl( \LCTv{u}_{f}\bigl( \LCT{\ell}_f \bigr) \bigr)_{\LCT{\ell}_{f} \in \LCTset{L}_{f}} $ 
    %   and the coefficients 
    %   $ \bigl( \LCT{\lambda}_{f}\bigl( \LCT{\ell}_{f} \bigr) \bigr)_{\LCT{\ell}_{f} \in \LCTset{L}_{f}} $ form an eigenvalue decomposition of $ \matr{C}_{\LCT{f}} $, where for each $ \LCT{\ell}_{f} \in \LCTset{L}_{f} $, the scalar $ \LCT{\lambda}_{f}\bigl( \LCT{\ell}_{f} \bigr) $ is the eigenvalue and the vector $\LCTv{u}_{f}(\LCT{\ell}_f)$ is the associated right eigenvector. 
 
    \item The resulting DE-NFG $\LCT{\graphN}$ is again a weak-sense DE-NFG. 

  \end{enumerate}

\end{proposition}

\begin{proof}
  See Appendix~\ref{apx:LCT DENFGs}.
\end{proof}


Most of the LCT properties for S-NFG can be straightforwardly extended to the case of DE-NFG. We note that applying the LCT to a strict-sense DE-NFG or a weak-sense DE-NFG yields in another weak-sense DE-NFG, which is similar to the property of the LCT for S-NFG as discussed in Item~\ref{remk: LCT on snfg results an NFG with negative fun nodes} in Remark~\ref{sec:LCT:rem:1}.

==> preliminaries.tex <==
In this chapter, we introduce preliminaries of this thesis. We first introduce basic definitions and notations used in this thesis in Section~\ref{sec: basic definition}. Then we review basic concepts of a standard normal factor graph (S-NFG) in Section~\ref{sec:SNFG}. In Section~\ref{sec: snfg for permanent of nonnagtive square matrix}, we study a class of S-NFGs such that the partition function induced by each of these S-NFGs equals the permanent of a non-negative square matrix. In Section~\ref{sec: basic of denfg}, we move to the quantum case where we consider the double-edge normal factor graph (DE-NFG). Finally, in Section~\ref{sec: finite graph covers}, we present the finite graph covers of the factor graphs introduced in this chapter.

\section{Basic Definition and Notations}
\label{sec: basic definition}

If not mentioned otherwise, all variable alphabets are assumed to be finite.
We will use, without essential loss of generality, normal
factor graphs (NFGs), \ie, factor graphs where variables are associated with
edges~\cite{Forney2001, Loeliger2004}.

  
Let $n$ be a positive integer and let $\mtheta \in \sR_{\geq 0}^{n \times
  n}$. We define $\suppmtheta$ to be the support of $\mtheta$, \ie,
\begin{align*}
  \suppmtheta 
    &\defeq
       \bigl\{ 
         (i,j) \in [n] \times [n] 
       \bigm|
         \theta(i,j) > 0
       \bigr\}.
\end{align*}

%***************************************************************************

Consider two finite subsets $ \set{I} $ and $ \set{J} $ of $[n]$ such that
$ |\set{I}| = | \set{J} | $. The set $ \setS_{\set{I} \to \set{J}} $ is
defined to be the set of all bijections from $ \set{I} $ to $ \set{J} $. In
particular, if $ \set{I} = \set{J} $, then the set
$ \setS_{\set{I} \to \set{J}} $ represents the set of all permutations of the
elements in $ \set{I} $, and we simply write $ \setS_{\set{I}} $ instead of
$\setS_{\set{I} \to \set{J}}$. Given
$ \sigma \in \setS_{\set{I} \to \set{J}} $, we define the matrix
$ \mP_{\sigma} \in \sZp^{\set{I} \times \set{J}} $ to be
\begin{align*}
  \mP_{\sigma} 
    &\defeq 
       \bigl(
         P_{\sigma}( i, j )
       \bigr)_{\! (i,j) \in \set{I} \times \set{J}} \, , 
       \ \ \ 
  P_{\sigma}( i, j )
     \defeq 
       \begin{cases}
         1 & \sigma(i) = j \\
         0 & \text{otherwise}
     \end{cases}.
     \nonumber
       % \label{sec:1:eqn:209}
\end{align*}
Note that $\mP_{\sigma}$ is a permutation matrix, \ie, a matrix where all
entries are equal to $0$ except for exactly one $1$ per row and exactly one
$1$ per column. Moreover, given a set $ \setS_{\set{I} \to \set{J}} $, the set
$\setP_{\set{I} \to \set{J}}$ is defined to be the set of the associated
permutation matrices, \ie,
\begin{align}
  \setP_{\set{I} \to \set{J}}
    &\defeq
       \bigl\{ 
         \mP_{\sigma} 
       \bigm|
         \sigma \in \setS_{\set{I} \to \set{J}}
       \bigr\}. 
         \label{sec:1:eqn:181}
\end{align}
If $\set{I} = \set{J}$, we simply write $\setP_{\set{I}}$ instead of
$\setP_{\set{I} \to \set{J}}$. A particularly important special case for this
thesis is the choice $\set{I} = \set{J} = [n]$: the set $\setP_{[n]}$
represents the set of all permutation matrices of size $n \times n$ where the
rows and columns are indexed by $[n]$.


%***************************************************************************

We define $\Gamma_n$ be the set of all doubly stochastic
matrices of size $n \times n$, \ie,
\begin{align*}
  \Gamma_n
    &\defeq
       \left\{ 
         \vgam
         = \bigl(
             \gamma(i,j)
           \bigr)_{\! i,j \in [n]}
      \ \middle| \ 
        \begin{array}{l}
          \gamma(i,j) \in \sR_{\geq 0}, \, \forall i,j \in [n] \\
          \sum\limits_{j \in [n]} \gamma(i,j) = 1, \, \forall i \in [n] \\
          \sum\limits_{i \in [n]} \gamma(i,j) = 1, \, \forall j \in [n]
        \end{array}
      \right\}.
\end{align*}
Moreover, for $M \in \sZpp$, we define $\Gamma_{M,n}$ to be the subset of
$\Gamma_{n}$ that contains all matrices where the entries are multiples of
$1/M$, \ie,
\begin{align*}
  \Gamma_{M,n} 
    &\defeq 
       \bigl\{ 
         \vgam \in \Gamma_n
       \bigm|
         M \cdot \gamma(i,j) \in \sZp, \ \forall i,j \in [n]
       \bigr\}.
\end{align*}
Observe that $\Gamma_{1,n} = \setP_{[n]}$.

%***************************************************************************

All logarithms in this thesis are natural logarithms and the value of
$0 \cdot \log(0)$ is defined to be $ 0 $.

%***************************************************************************

In this thesis, given an arbitrary $ n \in \sZpp $, if there is no ambiguity,
we use $ \prod_{i,j} $, $ \prod_{i} $, $ \prod_{j} $, $ \sum_{i,j} $,
$ \sum_{i} $, and $ \sum_{j} $ for $ \prod_{i,j \in [n]} $, $ \prod_{i \in [n]} $,
$ \prod_{j \in [n]} $, $ \sum_{i,j \in [n]} $, $ \sum_{i \in [n]} $, and
$ \sum_{j \in [n]} $, respectively.


\section{Standard Normal Factor Graphs (S-NFGs)}
\label{sec:SNFG}

%***************************************************************************

In this section, we review some basic concepts and properties of an S-NFG along with the associated Bethe approximation of the partition function.  We
use an example to introduce the key concepts of an S-NFG.


\input{figures/snfg_example.tex}

\begin{example}\label{sec:SNFG:exp:1}

  Consider the multivariate function
  $g(x_{1},\ldots,x_{5}) \defeq f_{1}(x_{1},x_{2},x_{3}) \cdot f_{2}(x_{1},x_{4})
  \cdot f_{3}(x_{2},x_{5})\cdot f_{4}(x_{3},x_{4},x_{5})$, where $g$, the
  so-called global function, is defined to be the product of the so-called
  local functions $f_{1}$, $f_{2}$, $f_{3}$ and $f_{4}$. We can visualize the factorization of $g$ with the help of the S-NFG $\graphN$ in
  Fig.~\ref{sec:SNFG:fig:1}. Note that the S-NFG $\graphN$ shown in
  Fig.~\ref{sec:SNFG:fig:1} consists of four function nodes
  $f_1, \ldots, f_4$ and five (full) edges with associated variables
  $x_1, \ldots, x_5$.
  \eexample
\end{example}

%***************************************************************************

%***************************************************************************

An edge that connects to two function nodes is called a full edge, whereas an edge
that is connected to only one function node is called a half edge. For the
purposes of this thesis, it is sufficient to consider only S-NFGs with full
edges, because S-NFGs with half edges can be turned into S-NFGs with only full
edges by attaching a dummy $1$-valued function node to the other end of every half edge without changing any marginals or the partition function.

%***************************************************************************

\begin{definition}(S-NFG)
  \label{def: def of snfg}
  \index{S-NFG}
  An S-NFG $\graphN(\setF, \setEfull, \set{X})$ consists of the following
  objects:
  \begin{enumerate}
    
  \item The graph $(\setF,\setEfull)$ with vertex set $\setF$ and edge set
    $\setEfull$, where $\setF$ is also known as the set of function nodes. (As
    mentioned above, every edge $e \in \setEfull$ will be assumed to be a full
    edge connecting two function nodes.)

  \item The alphabet $\set{X} \defeq \prod_{e \in \setEfull} \setxe$, where
    $\setxe$ is the alphabet of the variable $\xe$ associated with the edge
    $e \in \setEfull$. In this thesis, without loss of generality, we suppose that $ 0 \in \setxe$ for all $ e \in \setEfull $.

  \end{enumerate} 
  For a given S-NFG $\graphN(\setF,\setEfull,\set{X})$, we fix the order of the function nodes by $ \set{F} = \{ f_{1},\ldots,f_{|\set{F}|} \}. $ Then we make the following definitions.
  %------------------------------------------------------------------------
  % \begin{align*}
  %   \set{F} = \{ f_{1},\ldots,f_{|\set{F}|} \}.
  %   % \qquad
  %   % \setEfull = \bigl[ |\setEfull| \bigr] = \{0,1,\ldots,|\setEfull|-1\} .
  % \end{align*}
  %------------------------------------------------------------------------
  
  \begin{enumerate}
    \setcounter{enumi}{2}

  \item For every function node $f \in \setF$, the set $\setpf$ is defined to be the set of edges incident on $f$.

  \item For every edge $e = (f_{i}, f_{j}) \in \setEfull$, the pair $(f_{i}, f_{j})$ is defined to be the pair of function nodes that are connected to edge $e$ such that $ i < j $. The set $ \partial e $ is defined to be the set of function nodes incident on $e$, \ie, $ \partial e \defeq \{f_{i}, f_{j}\} $. Note that for notational convenience, here we impose a direction on every edge $(f_{i}, f_{j})$, \ie, the inequality $ i < j $, that is irrelevant for our results.

  \item For any finite set $ \set{I} \subseteq \setEfull $, we define
   %-----------------------------------------------------------------------
   \begin{align*}
         \setx{ \set{I} } \defeq 
         \prod_{ e \in \set{I} } \setxe, \qquad 
         \vx_{\set{I}} \defeq (\xe)_{e \in \set{I}}
         \in \setx{ \set{I} }.
   \end{align*}
   %-----------------------------------------------------------------------


  \item An assignment $\vx \defeq (\xe)_{e \in \setEfull} \in \set{X}$ is called a
    configuration of the S-NFG $ \sfN $. For each $f \in \setF$, a configuration
    $\vx \in \set{X}$ induces the vector $\xf \defeq (x_{e})_{e \in \setpf} \in \setxf$.

  \item For every $f \in \setF$, the local function associated with $f$ is,
    with some slight abuse of notation, also called $f$. Here, the local
    function $f$ is an arbitrary mapping from $\setxf$ to
    $\sRp$.

  \item The global function $g$ is defined to be the mapping
    $g:\set{X}\to \sRp, \ \vx\mapsto \prod_{f \in \setF} f(\xf)$.

  \item A configuration $\vx \in \set{X}$ satisfying $g(\vx) \neq 0$ is called a
    valid configuration. The set of valid configurations is defined to be
    \begin{align*}
      \set{C} \defeq \{ \vx \in \set{X} \ | \ g(\vx) \neq 0 \}.
    \end{align*}

  \item The partition function is defined to be
    $Z(\graphN) \defeq \sum_{\vx \in \set{C}}g(\vx)$.\footnote{In this thesis, the
      partition function $Z(\graphN)$ of $\graphN$ is a scalar, \ie, it
      is not really a function. If $\graphN$ depends on some parameter
      (say, some temperature parameter), then $Z(\graphN)$ is a function of
      that parameter.} Clearly, the partition function satisfies
    $Z(\graphN) \in \sRp$.
    \label{partition function of snfg}
  \end{enumerate}
  \edefinition
\end{definition}

%***************************************************************************

In the following, we will only consider the S-NFG $\graphN$ for which
$Z(\graphN) \in \sRpp$.

%***************************************************************************

If there is no ambiguity, when we consider S-NFG, we will use the short-hands
$\sum_{\vx}$, 
$\sum_{\xe}$, 
$\sum_e$, 
$\sum_{f}$, 
$\prod_{\vx}$,  
$\prod_{\xe}$,
$\prod_e$, 
$\prod_{f}$,
$ (\cdot)_{\xe} $,
and
$ (\cdot)_{e} $ for
$\sum_{\vx \in \set{X}}$, 
$\sum_{\xe \in \setxe}$, 
$\sum_{e \in \setEfull}$, 
$\sum_{f \in \setF}$,
$\prod_{\vx \in \set{X}}$, 
$\prod_{\xe \in \setxe}$, 
$\prod_{e \in \setEfull}$, 
$\prod_{f \in \setF}$, 
$ (\cdot)_{\xe \in \setxe} $,
and 
$ (\cdot)_{e\in \setEfull} $,
respectively. 
For any set $ \set{I} \subseteq \setEfull $, we will use the short-hands 
$\sum_{\vx_{\set{I}}}$,
$\prod_{\vx_{\set{I}}}$, 
and $ (\cdot)_{\vx_{\set{I}}} $
for 
$\sum_{ \vx_{\set{I}} \in \setx{\set{I}} }$,
$\prod_{ \vx_{\set{I}} \in \setx{\set{I}} }$, 
and $ (\cdot)_{ \vx_{\set{I}} \in \setx{\set{I}} } $.
Moreover, $\setpf \setminus e$ will be short-hand notation for
$\setpf \setminus \{ e \}$.

Now we introduce the Gibbs free energy function, which provides an alternative expression of the partition function.
%----------------------------------------------------------------------------
\begin{definition}
  (The Gibbs free energy function)
  \index{Gibbs free energy function!for S-NFG}
  Consider some S-NFG $\sfN$ and $ \bm{p} \defeq \bigl( p(\vx) \bigr)_{\vx \in \set{C}} \in \Pi_{\set{C}} $.
  The Gibbs free energy function is defined to be the mapping
  (see, \eg, \cite[Definition 9]{Vontobel2013})
  \begin{align*}
    F_{\mathrm{G}}: \Pi_{\set{C}} &\to \sR \nonumber\\
    \qquad \bm{p} &\mapsto U_{\mathrm{G}}(\bm{p}) - H_{\mathrm{G}}(\bm{p}),
  \end{align*}
  where
  \begin{alignat*}{4}
    U_{\mathrm{G}}: \Pi_{\set{C}} &\to \sR, \qquad 
    &\bm{p} &\mapsto& -\sum_{ \vx \in \set{C} } 
    p(\vx) \cdot \log\bigl( g(\vx) \bigr),
    \nonumber\\
    H_{\mathrm{G}}: \Pi_{\set{C}} &\to \sR, \qquad 
    &\bm{p} &\mapsto& -\sum_{ \vx \in \set{C} } 
    p(\vx) \cdot \log\bigl( p(\vx) \bigr).
  \end{alignat*}
  \edefinition
\end{definition}
%----------------------------------------------------------------------------
%----------------------------------------------------------------------------
\begin{proposition}
  \label{prop: minimum of FG relates to Z}
  It holds that $  F_{\mathrm{G}}(\bm{p}) $ is a convex function w.r.t. 
  $ \bm{p} \in \Pi_{\set{C}} $ and
  \begin{align*}
    Z(\sfN) = \exp( - \min_{ \bm{p} \in \Pi_{\set{C}} } F_{\mathrm{G}}(\bm{p}) ).
  \end{align*}
\end{proposition}
%----------------------------------------------------------------------------
%----------------------------------------------------------------------------
\begin{proof}
  See, \eg,~\cite[Lemma 8]{Vontobel2013}.
\end{proof}
%----------------------------------------------------------------------------

In general, neither the direct evaluation of the partition function nor solving the convex optimization problem in Proposition~\ref{prop: minimum of FG relates to Z} leads to a tractable computational problem, except for small-scaled S-NFG. 
This limitation motivates the study of alternative approaches, specifically approximations of the partition function and the Gibbs free energy function. 


In the following, we introduce the SPA, whose fixed points often provide decent approximation to the partition function. Note that we only give the technical details of the SPA on an S-NFG; for a general discussion with respect to (w.r.t.) the motivations behind the SPA, see, \eg,~\cite{Kschischang2001,Loeliger2004}.
\begin{definition}\label{sec:SNFG:def:4}
  (The SPA on S-NFG)
  \index{SPA!on S-NFG}
  Consider some S-NFG $\graphN$. The SPA is an iterative algorithm that
  sends messages along edges, where messages are functions over the alphabet
  associated with an edge. (Note that for every iteration and every edge, two
  messages are sent along that edge, one in both directions.) More precisely,
  the SPA consists of the following steps:
  \begin{enumerate}

  \item (Initialization) For every $e \in \setEfull$, $f \in \setF$, the
    message $\mu_{\etof}^{(0)}: \setxe \to \sR_{\geq 0} $, is defined to be some
    arbitrary function. (Typically, $\mu_{\etof}^{(0)}(\xe) \defeq 1 / |\setxe|$
    for all $\xe \in \setxe$.)

  \item (Iteration) For $t = 1, 2, 3, \ldots$, do the following calculations
    until some termination criterion is met:\footnote{The termination
      criterion is typically a combination of numerical convergence and an
      upper bound on the number of iterations.}
    \begin{enumerate}
        \item  For every $e = (f_{i}, f_{j}) \in \setEfull$, we define the scaling factor $ \kappa_{\efj}^{(t)} $ to be
        %--------------------------------------------------------------------
        \begin{align*}
            \kappa_{\efj}^{(t)}
            &\defeq
            \sum_{\xfi}
            f_{i}(\xfi)
            \cdot
            \prod_{e' \in \setpfi \setminus e}
            \mu_{\epfi}^{(t-1)}(x_{e'}).
            % \nonumber\\
            % \kappa_{\efi}^{(t)} &\defeq
            % \sum_{\xfj}
            % f_{j}(\xfj)
            % \cdot
            % \prod_{e' \in \setpfj \setminus e}
            % \mu_{\epfj}^{(t-1)}(x_{e'}).
        \end{align*}
        %--------------------------------------------------------------------
        One can obtain the definition of $ \kappa_{\efi}^{(t)} $ by switching $ f_{i} $ with $ f_{j} $ in the above definition.
        
        \item If 
        $ 
            \prod_{e \in \setEfull} 
            \prod_{f \in \setpe}
            \kappa_{\ef}^{(t)} = 0 
        $,
        we randomly generate each element in $ \vmu^{(t)} $ following uniform distribution in $ [0,1] $.


        \item  If 
        $ 
            \prod_{e \in \setEfull} 
            \prod_{f \in \setpe}
            \kappa_{\ef}^{(t)} \neq 0 
        $, for every $e \in \setEfull$, 
        we define the messages from edge $ e = (f_{i}, f_{j}) $ to the function node 
        $ f_{j} $ to be the mapping:\footnote{If desired or necessary, other generalization procedures is allowed.}
        \begin{align}
          \mu_{\efj}^{(t)}:\, \set{X}_{e} &\to \sR_{\geq 0}, \quad
          z_{e} \mapsto 
          \bigl( \kappa_{\efj}^{(t)} \bigr)^{\! -1}
          \cdot
          \sum_{\xfi: \, x_{e} = z_{e}}
            f_{i}(\xfi)
            \cdot
            \prod_{e' \in \setpfi \setminus e}
              \mu_{\epfi}^{(t-1)}(x_{e'}). \label{sec:SNFG:eqn:8}
        % \\
        % \mu_{\efj}^{(t)}:\, \set{X}_{e} &\to \sR_{\geq 0}, \quad
        %   z_{e} &\mapsto&
        %   \bigl( \kappa_{\efi}^{(t)} \bigr)^{\! -1}
        %   \cdot
        %   \sum_{\xfj: \, x_{e} = z_{e}}
        %     f_{j}(\xfj)
        %     \cdot
        %     \prod_{e' \in \setpfj \setminus e}
        %       \mu_{\epfj}^{(t-1)}(x_{e'}). \label{sec:SNFG:eqn:7}
        \end{align}
        One can obtain the definition of $ \mu_{\efi}^{(t)} $ by switching $ f_{i} $ with $ f_{j} $ in~\eqref{sec:SNFG:eqn:8}.
        


    \item For every $f \in \setF$, we define
    %------------------------------------------------------------------------
    \begin{align*}
        \kappa_f^{(t)} \defeq 
            \sum_{ \xf }
            f(\xf) \cdot \prod_{e \in \setpf} \mu_{\etof}^{(t)}(\xe).
    \end{align*}
    %------------------------------------------------------------------------
    If $ \kappa_f^{(t)} \neq 0 $, then we define the belief function at function node $f$ to be the mapping
      \begin{align}
        \beli_f^{(t)}: \setxf \to \sR_{\geq 0}, \quad
          \xf
          &\mapsto 
            \bigl( \kappa_f^{(t)} \bigr)^{\! -1}
              \cdot
              f(\xf)
              \cdot
              \prod_{e \in \setpf}
                \mu_{\etof}^{(t)}(\xe).
                    \label{sec:SNFG:eqn:1}
      \end{align}
      The associated vector is defined to be
      $ \vbeli_{f}^{(t)} \defeq \bigl( \beli_f^{(t)}(\xf) \bigr)_{ \! \xf \in \set{X}_{\setpf} } $.
    
    \item For every $e \in \setEfull$, we define
    %------------------------------------------------------------------------
    \begin{align*}
        \kappa_e^{(t)} \defeq \sum_{\xe} 
        \prod_{f \in \setpe}
        \mu_{\ef}^{(t)}(\xe).
    \end{align*}
    %------------------------------------------------------------------------
    If $  \kappa_e^{(t)}\neq 0 $, then we define the belief function at edge $e$ to be the mapping
      \begin{align}
        \beli_e^{(t)}: \setxe \to \sR_{\geq 0}, \quad
        \xe
        &\mapsto
        \bigl( \kappa_e^{(t)} \bigr)^{-1}
        \cdot
        \mu_{\efi}^{(t)}(\xe)
        \cdot
        \mu_{\efj}^{(t)}(\xe).
        \label{sec:SNFG:eqn:2}
      \end{align}
      The vector $ \vbeli_e^{(t)} $ is defined to be $ \vbeli_e^{(t)} \defeq \bigl( \beli_e^{(t)}(\xe) \bigr)_{ \! \xe \in \setxe } $.
    \end{enumerate}
    
    \item At iteration $t \in \sZpp$, the SPA messages can be collected as the SPA message vector:
    %--------------------------------------------------------------------
    \begin{align*}
      \vmu^{(t)} \defeq 
      \bigl( \vmu_{\etof}^{(t)} \bigr)_{\! e \in \setpf,\, f \in \setF},
    \end{align*}
    %--------------------------------------------------------------------
    where $ \vmu_{\ef}^{(t)} \defeq \bigl( \mu_{\ef}^{(t)}(\xe) \bigr)_{ \! \xe } $. 
    With this, the SPA message update rules can be written as
    %--------------------------------------------------------------------
    \begin{align*}
      \vmu^{(t)} = \fSPAN\bigl( \vmu^{(t-1)} \bigr)
    \end{align*}
    %--------------------------------------------------------------------
    for some suitably defined function $\fSPAN$. 

    \item The beliefs at function nodes and edges can be collected as the following vector:
    %-----------------------------------------------------------------------
    \begin{align*}
       \vbeli^{(t)} \defeq \Bigl( 
       ( \vbeli_f^{(t)} )_{f \in \setF}, \,
      ( \vbeli_e^{(t)} )_{e \in \setE} \Bigr).
    \end{align*}
    %-----------------------------------------------------------------------

    \item \index{SPA fixed point!for S-NFG} 
    An SPA message vector
    %--------------------------------------------------------------------
    \begin{align}
      \vmu \defeq ( \vmu_{\etof} )_{e \in \setpf,\, f \in \setF}
      \label{sec:SNFG:eqn:10}
    \end{align}
    %--------------------------------------------------------------------
    with 
    $ \vmu_{\etof} \defeq \bigl( \mu_{\etof}(\xe) \bigr)_{\xe} $
    is called an SPA fixed-point message vector if 
    %--------------------------------------------------------------------
    \begin{align}
      \vmu = \fSPAN(\vmu). \label{sec:SNFG:eqn:11}
    \end{align}
    %-------------------------------------------------------------------- 
    % where $ \mu_{\etof} : \setxe \to \sR $ is an arbitrary mapping and $ \vmu_{\etof} = ( \mu_{\etof}(\xe) )_{\xe} $.

    % \item The beliefs evaluated at an SPA message vector $ \vmu $ are given by 
    % %-----------------------------------------------------------------------
    % \begin{align}
    %     \beli_{f,\vmu}(\xf)
    %     &\defeq \kappa_f
    %       \cdot
    %       f(\xf)
    %       \cdot
    %       \prod_{e \in \setpf}
    %         \mu_{\etof}(\xe),
    %           \quad \xf \in \setxf,\, \kappa_f \in \sR_{>0}, 
    %     \label{sec:DENFG:eqn:12} \\
    %     \beli_{e,\vmu}(\xe)
    %     &\defeq \kappa_e
    %     \cdot
    %     \mu_{\efi}(\xe)
    %     \cdot
    %     \mu_{\efj}(\xe),
    %     \quad \xe \in \setxe,\, \kappa_e \in \sR_{>0}, 
    %     \label{sec:DENFG:eqn:13}.
    % \end{align}
    % %-----------------------------------------------------------------------

  \end{enumerate}
  (If desired or necessary, other normalization procedures for messages and
  beliefs can be specified.)
  \edefinition
\end{definition}

%***************************************************************************

\begin{definition}
  \label{def:belief at SPA fixed point for S-NFG}
  Consider some S-NFG $\graphN$ and let
  $\vmu $ be some SPA fixed-point
  message vector for $\graphN$ as defined in~\eqref{sec:SNFG:eqn:10} and~\eqref{sec:SNFG:eqn:11}. The collection of the beliefs 
  %-----------------------------------------------------------------------
  \begin{align}
     \vbeli \defeq \Bigl( ( \vbeli_f )_{f \in \setF}, \,
    ( \vbeli_e )_{e \in \setE} \Bigr).
    \label{eqn: def of beliefs}
  \end{align}
  %-----------------------------------------------------------------------
  induced by the SPA fixed-point messages is computed as follows with 
  $ \vmu_{\etof}^{(t)} = \vmu_{\etof} $ for all $ e \in \setEfull $ and $ f \in \setF $:
  %----------------------------------------------------------------------------
  \begin{enumerate}
    \item for every $f \in \setF$, if 
    \begin{align}
        \sum_{ \xf }
        f(\xf) \cdot \prod_{e \in \setpf} \mu_{\etof}(\xe)
        >0, \label{eqn: positive of belief at f}
    \end{align}
      then the elements in the vector $\vbeli_f$ are 
      obtained by letting $ \vbeli_{f} = \vbeli_{f}^{(t)} $, where the elements in $ \vbeli_{f}^{(t)} $ are given in~\eqref{sec:SNFG:eqn:1};

    \item for every $e \in \setEfull$, if
    \begin{align}
        \sum_{\xe} 
        \prod_{f \in \setpe}
        \mu_{\ef}(\xe) > 0,
        \label{eqn: positive of belief at e}
     \end{align} 
    then the elements in the vector $\vbeli_e$ 
    are obtained by letting $ \vbeli_{e} = \vbeli_{e}^{(t)} $, where the elements in $ \vbeli_{e}^{(t)} $ are given in~\eqref{sec:SNFG:eqn:2}.
  \end{enumerate}
  %----------------------------------------------------------------------------
  \edefinition
\end{definition}

%**************************************************************************

%***************************************************************************



%***************************************************************************

\begin{assumption}
  \label{asmp: assume messages are non-negative}
  In the context of S-NFG, if not mentioned otherwise, we will only consider the following normalization procedure for the SPA 
  message vectors $\vmu^{(t)} $ and the collection of the beliefs $ \vbeli^{(t)} $:
  \begin{align*}
    \vmu_{\etof}^{(t)} &\in \Pi_{\setxe}, \qquad e \in \setpf,\, f \in \setF,
    \nonumber\\
    \vbeli^{(t)}_{e} &\in \Pi_{\setxe}, \qquad e \in \setEfull, \nonumber\\
    \vbeli^{(t)}_{f} &\in \Pi_{\setxf}, \qquad f \in \setF.
  \end{align*}
  
  Furthermore, we only consider the SPA fixed-point message vector $ \vmu $ such that
  the strict inequality in~\eqref{eqn: positive of belief at e} 
  holds for all $ e \in \setEfull $.
  % %----------------------------------------------------------------------------
  % \begin{enumerate}

  %   \item the strict inequality in~\eqref{eqn: positive of belief at f}
  %    holds for all $ f \in \setF $;

  %   \item 
  % \end{enumerate}
  % %----------------------------------------------------------------------------
  (See Item~\ref{sec:SNFG:remk:1:item:2} in Remark~\ref{sec:SNFG:remk:1} for a non-trivial S-NFG with an SPA fixed-point message vector such that the inequality in~\eqref{eqn: positive of belief at e} does not satisfy for some $ e \in \setEfull $.)
  \eassumption
\end{assumption}

%***************************************************************************

%----------------------------------------------------------------------------
\begin{proposition}\hspace{-0.1 cm}\cite[Proposition 5]{Yedidia2005}
  For the S-NFG such that $ f(\xf) \in \sR_{>0} $ for all $ \xf \in \setx{\setpf} $ and $ f \in \setF $, the inequality~\eqref{eqn: positive of belief at e} holds for all $ f \in \setF $ and the inequality~\eqref{eqn: positive of belief at e} holds for all $ e \in \setEfull $.
  \eproposition
\end{proposition}
%----------------------------------------------------------------------------

%***************************************************************************

% %----------------------------------------------------------------------------
% \begin{proposition}
%   Consider running the SPA defined in Definition~\ref{sec:SNFG:def:4} on some S-NFG $\graphN$. 
%    It holds that $\vmu_{\etof}^{(t)} \in \sRp^{|\setxe|}$ for all $e \in \setpf$,
%       $f \in \setF$, and $t \geq 1$. Moreover, it holds that 
%       $\vbeli_f^{(t)} \in \Pi_{\setxf}$ for all
%       $f \in \setF$ and $\vbeli_e^{(t)} \in \Pi_{\setxe}$ for all $e \in \setEfull$.
% \end{proposition}
% %----------------------------------------------------------------------------
% %----------------------------------------------------------------------------
% \begin{proof}
%    This is a straightforward consequence of Assumption~\ref{asmp: assume messages are non-negative}, the SPA message update rules in Definition~\ref{sec:SNFG:def:4} and the fact that the local functions of an S-NFG take on only non-negative real values.
% \end{proof}
% %----------------------------------------------------------------------------


Now we introduce the Bethe free energy function, which gives an S-FG based approximation to the Gibbs free energy function. Proposition~\ref{prop: minimum of FG relates to Z} states that the value of the partition function can be evaluated by the minimum of the Gibbs free energy function. Therefore, the minimum of the Bethe free energy function yields an approximation to the partition function. The following definitions are adapted from~\cite[Section V]{Yedidia2005} to S-NFGs.

%***************************************************************************

\begin{definition}\label{sec:SNFG:def:3}
  \!\cite[Section V]{Yedidia2005}
  \index{Local marginal polytope!for S-NFG}
  Let $\graphN$ be some S-NFG. Recall that 
  the collection of the beliefs $  \vbeli $ is defined in~\eqref{eqn: def of beliefs}.
  The local marginal polytope $\LMP(\graphN)$
  associated with $\graphN$ is defined to be the following set:
  \begin{align}
    \LMP(\graphN)
      &\defeq \left\{ 
        \vbeli
      \ \middle| \ 
        \begin{array}{c}
          \vbeli_f \in \Pi_{\setxf} \ \text{for all} \ f \in \setF \\
          \vbeli_e \in \Pi_{\setxe} \ \text{for all} \ e \in \setE \\[0.10cm]
          \sum\limits_{\xf: \, \xe = \ze}
            \beli_f(\xf)
              = \beli_e(\ze) \\
                  \ \text{for all} \ 
                  e \in \setpf, f \in \setF, \ze \in \setxe
        \end{array}
      \right\}. \label{sec:SNFG:eqn:12}
  \end{align}

  \edefinition
\end{definition}

%***************************************************************************

\begin{definition}
  \label{sec:SNFG:def:1}
  \index{Bethe free energy function!for S-NFG}
  \!\cite[Section V]{Yedidia2005}
  Let $\graphN$ be some S-NFG. The Bethe free energy function
  is defined to be the following mapping:
  \begin{align*}
    \FB(\vbeli): \LMP(\graphN) &\to \sR, \quad
      \vbeli \mapsto  U_{\mathrm{B}}(\vbeli) -  H_{\mathrm{B}}(\vbeli),
                 % \label{sec:SNFG:eqn:3}
  \end{align*}
  where
  %------------------------------------------------------------------------
  \begin{align}
    U_{\mathrm{B}}(\vbeli): \LMP(\graphN) &\to \sR,\quad
    \vbeli \mapsto 
    \sum_{f} U_{\mathrm{B},f}(\vbeli_{f}), 
    \nonumber\\
    H_{\mathrm{B}}(\vbeli): \LMP(\graphN) &\to \sR,\quad
    \vbeli \mapsto \sum_{f}
    H_{\mathrm{B},f}(\vbeli_{f})
    - \sum_{e} H_{\mathrm{B},e}(\vbeli_{e}), \label{sec:SNFG:eqn:9}
  \end{align}
  %------------------------------------------------------------------------
  with
  %------------------------------------------------------------------------
  \begin{align*}
    U_{\mathrm{B},f}(\vbeli_{f}): \Pi_{\setxf} \to \sR,\quad
    &\vbeli_{f} \mapsto
    -\sum_{\xf} 
      \beli_f(\xf)
      \cdot
        \log\bigl( f(\xf) \bigr), \nonumber\\
    H_{\mathrm{B},f}(\vbeli_{f}): \Pi_{\setxf} \to \sR,\quad
    &\vbeli_{f} \mapsto
    -\sum_{\xf} 
      \beli_f(\xf)
      \cdot
        \log\bigl( \beli_f(\xf) \bigr), \nonumber\\
    H_{\mathrm{B},e}(\vbeli_{e}): \Pi_{\setxe} \to \sR,\quad
    & \vbeli_{e} \mapsto -\sum_{\xe} 
      \beli_{e}(\xe)
      \cdot
      \log\bigl( \beli_{e}(\xe) \bigr).
  \end{align*}
  %------------------------------------------------------------------------
  Here, $ U_{\mathrm{B}} $ is the Bethe average energy function and $ H_{\mathrm{B}} $ is the Bethe entropy function.
  (Note that for NFGs with full and half edges, the sum in $ \sum_{e} H_{\mathrm{B},e}(\vbeli_{e}) $ is only over all full
  edges.)  The Bethe approximation of the partition function, henceforth
  called the Bethe partition function, is defined to be
  \begin{align}
    \ZB(\graphN)
      &\defeq 
      \exp
            \left( 
              -
              \min_{\vbeli \in \LMP(\graphN)}
                \FB(\vbeli)
            \right).
              \label{sec:SNFG:eqn:4}
  \end{align}
  \index{Bethe partition function!for S-NFG}This definition is often viewed as the primal formulation of the Bethe partition function.
  \edefinition
\end{definition}

% \subsection{Cycle-free S-NFG}
% %***************************************************************************

% \begin{proof}
%   The statement in Item~\ref{sec:SNFG:lem:1:item:1} is a straightforward consequence of Assumption~\ref{asmp: assume messages are non-negative}, the SPA message update rules in Definition~\ref{sec:SNFG:def:4} and the fact that the local functions of an S-NFG take on only non-negative real values.

%   The statement in Item~\ref{sec:SNFG:lem:1:item:2} is a consequence of the SPA message update rules in Definition~\ref{sec:SNFG:def:4} and the definition of the SPA fixed-point message vector.
% \end{proof}

%***************************************************************************
% In this section, we present properties for a cycle free S-NFG.
%----------------------------------------------------------------------------
\begin{proposition}
  \label{prop: property of the SPA and ZB for cycle free SNFG}
  Consider $\graphN$ to be cycle free.
  %----------------------------------------------------------------------------
  \begin{enumerate}
    \item\label{item: cycle free SNFG ZB equals Z}\cite[Proposition 3]{Yedidia2005} It holds that $ \ZB(\graphN) = Z(\graphN) $.

    \item (See, \eg,~\cite[Section 2.5]{JWainwright2008}.) The SPA on $ \graphN $ converges to a unique fixed point and the beliefs evaluated by the SPA fixed-point messages, as defined in Definition~\ref{def:belief at SPA fixed point for S-NFG}, is at the location of the minimum of the Bethe free energy function, \ie, the value of the Bethe partition function can be evaluated by the fixed-point messages. 
  \end{enumerate}
  %----------------------------------------------------------------------------
  By these two properties, we know that for the cycle-free S-NFG $\graphN$, 
  the value of the partition function can be evaluated by the SPA fixed-point messages.
  \eproposition
\end{proposition}
%----------------------------------------------------------------------------

\begin{remark}
  Consider some S-NFG $ \sfN $ with cycles. 
  Suppose that we get an SPA fixed-point message vector $ \vmu $ and obtain a collection of the beliefs $ \vbeli $ based on $ \vmu $, following Definition~\ref{def:belief at SPA fixed point for S-NFG}. 
  One can verify that 
  \begin{align*}
    \vbeli \in \LMP(\graphN).
  \end{align*}
  Therefore, the value of the function $ \exp \bigl( -\FB(\vbeli) \bigr) $, which is obtained by $ \vmu $, can be viewed as an approximation of the value of the Bethe partition function.
\end{remark}


For an S-NFG with cycles, the behavior of the SPA varies and the Bethe partition function provides an approximation of the partition function. One of the main results in the paper by Yedidia \etal~\cite[Section V]{Yedidia2005} is a characterization of stationary points of the Bethe free energy function in terms of SPA fixed-point message vectors. 
%---------------------------------------------------------------------------
\begin{theorem}
  \label{thm: Yedidia results on SPA and FB}
  Consider some S-NFG $ \sfN $.
  % %-----------------------------------------------------------------------
  \begin{enumerate}

    \item\hspace{-0.01cm}\cite[Theorem 2]{Yedidia2005} If the stationary point of the Bethe free energy function is in the interior of the LMP, \ie, 
    \begin{align*}
      \vbeli \in \LMP(\graphN),\quad \vbeli_{f} \in \sR_{>0}^{|\setx{\setpf}|}, \qquad 
      f \in \setF,
    \end{align*}
    then this stationary point corresponds to an SPA fixed point of $ \sfN $.

    \item\hspace{-0.01cm}\cite[Theorem 3]{Yedidia2005} If all the local functions in $ \sfN $ are positive-valued, \ie,  
    \begin{align*}
        f(\xf) \in \sR_{>0}, \qquad
        \xf \in \prod_{e \in \setpf} \setxe,\, f \in \setF ,
    \end{align*}
    then each of the local minima of the Bethe free energy function corresponds to an SPA fixed point of $ \graphN $. 
  \end{enumerate}
  %-----------------------------------------------------------------------
  \etheorem
\end{theorem}
%---------------------------------------------------------------------------


For S-NFG $ \sfN $ with cycles, 
the SPA on $ \sfN $ might converge to a fixed point, or it might fail to converge.
The Bethe partition function $\ZB(\graphN)$ can be smaller,
equal, or larger than the partition function $\ZB(\graphN)$.
%***************************************************************************

%---------------------------------------------------------------------------
\begin{enumerate}

    \item In~\cite[Corollary 4.2]{Ruozzi2012}, Ruozzi proved that the Bethe partition function lower bounds the partition function for binary, log-supermodular graphical models. Based on that, Ruozzi in~\cite{Ruozzi2013} further showed that this lower bound  holds for other graphical models that are not necessarily binary or
    log-supermodular, including the ferromagnetic Potts models with a uniform external field~\cite[Theorems 5.2 and 5.4]{Ruozzi2013} and its generalizations~\cite[Theorem 5.6]{Ruozzi2013} and a certain class of graphical models whose partition function equals the number of a weighted graph homomorphism~\cite[Theorem 6.2]{Ruozzi2013}. 

    \item In~\cite{Vontobel2013a}, Vontobel studied the S-NFG whose partition function equals the permanent of a non-negative square matrix, and he showed that for such S-NFG,  the Bethe free energy function is a convex function and the SPA finds the minimum of the Bethe free energy function exponentially fast. Huang and Vontobel in~\cite{Huang2024} extended Vontobel’s results in~\cite{Vontobel2013a} by considering a class of bipartite S-FGs where each local function is defined based on a (possibly different) multi-affine homogeneous real stable (MAHRS) polynomial. Huang and Vontobel~\cite{Huang2024} showed that a certain projection of the local marginal polytope equals the convex hull of the set of valid configurations, that the Bethe free energy function possesses some convexity properties, and, for the typical case where the S-FG has an SPA fixed point consisting of positive-valued messages only, that the SPA finds the value of the Bethe partition function exponentially fast.

    \item Gurvits in~\cite[Theorem 2.2]{Gurvits2011} proved that for the S-NFG considered in~\cite{Vontobel2013a}, the Bethe partition function lower bounds the partition function,
    \ie, the lower bound in~\eqref{eq:ratio:permanent:bethe:permanent:1}. Then Straszak and Vishnoi in~\cite[Theorem 3.2]{Straszak2019} and Anari and Gharan~\cite[Theorem 1.1]{Anari2021} proved this lower bound holds even for the
    S-NFG where each local function corresponds to a (possibly different) multi-affine real stable polynomial. (Note that they did not assume homogenity.) 
    The class of the S-NFGs considered in~\cite{Straszak2019,Anari2021} is a generalization of the class of the S-NFGs studied in~\cite{Vontobel2013a}.
    
\end{enumerate}
%---------------------------------------------------------------------------

%***************************************************************************
Besides bounding the partition function via the Bethe partition function, one can connect the partition function and the Bethe partition function via the finite graph covers.  
In contrast to the analytical definition of the Bethe partition function $\ZB(\graphN)$ in~\eqref{sec:SNFG:eqn:4}, Vontobel in~\cite{Vontobel2013} gave a combinatorial characterization of $\ZB(\graphN)$ via finite graph covers of $ \sfN $: for $ M = 1 $, the $M$-covers' average partition function is equal to the partition function; for $ M \to \infty $, the limit superior of the $M$-covers' average partition function is equal to the Bethe partition function. This characterization is based on using the method of types to characterize the valid configurations in the $M$-covers. The technical details of the $M$-covers for an S-NFG $ \sfN $ are presented in Section~\ref{sec:GraCov}. 

%***************************************************************************

Given that the Bethe partition function is closely related to the SPA, in the following, we give a pseudo-dual formulation of the Bethe partition function based on the SPA fixed-point message vectors.

%***************************************************************************

\begin{definition}(The pseudo-dual formulation of the Bethe partition function for S-NFGs)
  \label{sec:SNFG:def:2}
  \index{Pseudo-dual Bethe partition function!for S-NFG}
  Consider some S-NFG $\graphN$ and let
  $\vmu $ be some SPA
  message vector for $\graphN$ as defined in~\eqref{sec:SNFG:eqn:10}.\footnote{The SPA message vector $\vmu$ does
    not necessarily have to be an SPA fixed-point message vector.} 
  If 
  \begin{align}
    Z_e(\vmu) > 0, \qquad e \in \setEfull,
    \label{eqn:positivity of SNFG Ze}
  \end{align}
  then we define the
  $\vmu$-based Bethe partition function to be
  \begin{align}
    \ZBSPA(\graphN,\vmu)
    &\defeq 
    \frac{\prod_f Z_f(\vmu)
    }{\prod_e Z_e(\vmu)},
    \label{sec:SNFG:eqn:5}
  \end{align}
  where
  \begin{alignat}{2}
    Z_f(\vmu)
    &\defeq
      \sum_{\xf}
        f(\xf)
          \cdot
          \prod_{e \in \setpf}
            \mu_{\etof}(\xe),
            \ 
            \qquad f \in \setF,
                \nonumber \\
    Z_e(\vmu)
      &\defeq
        \sum_{\xe}
          \prod_{f \in \setpe}
          \mu_{\ef}(\xe),
          \qquad e \in \setEfull.
              \label{sec:SNFG:eqn:6}
  \end{alignat}
  (For NFGs with full and half edges, the product in the denominator on the
  right-hand side of~\eqref{sec:SNFG:eqn:5} is only over all full
  edges. Moreover, note that the expression for $\ZBSPA(\graphN,\vmu)$ is scaling
  invariant, \ie, if any of the messages $\mu_{\ef}$ is multiplied by a
  nonzero complex number then $\ZBSPA(\graphN,\vmu)$ remains unchanged.)
  The SPA-based Bethe partition function $\ZBSPA^{*}(\graphN)$ is then defined
  to be
  \begin{align*}
    \ZBSPA^{*}(\graphN)
        &\defeq \max_{\vmu}
        \ZBSPA(\graphN,\vmu)
        \nonumber\\
        &\qquad \mathrm{s.t.} \
        \text{$\vmu$ is an SPA fixed-point message vector 
        satisfy~\eqref{eqn:positivity of SNFG Ze}.}
  \end{align*}
  The above definition is viewed as the pseudo-dual formulation of the Bethe partition function.
  \edefinition
\end{definition}



 \begin{remark}\label{sec:SNFG:remk:1}
   Let us make some remarks on the pseudo-dual formulation of the Bethe partition function in Definition~\ref{sec:SNFG:def:2}.
   %---------------------------------------------------------------------------
   \begin{enumerate}
        \item Consider an arbitrary cycle-free S-NFG $\graphN$. 
        Proposition~\ref{prop: property of the SPA and ZB for cycle free SNFG} 
        states that the SPA on $\graphN$ converges to a unique fixed point
         and that $ \ZB(\graphN) = Z(\graphN) $.
        Denote the associated SPA fixed-point message vector by~$\vmu$. 
        One can verify that $\ZBSPA(\graphN,\vmu) = Z(\graphN)$. 

        \item By Assumption~\ref{asmp: assume messages are non-negative}, in this thesis, we only consider the S-NFGs where $  \ZBSPA^{*}(\graphN) $, as defined in Definition~\ref{sec:SNFG:def:2}, is well-defined, \ie, the SPA fixed-point messages $ \vmu $ such that
        %-----------------------------------------------------------------------
        \begin{align*}
            \ZBSPA(\graphN,\vmu) = \ZBSPA^{*}(\graphN), \qquad
            Z_e(\vmu) >0, \qquad e \in \setEfull.
        \end{align*}
        %-----------------------------------------------------------------------
        See Item~\ref{sec:SNFG:remk:1:item:2} for a non-trivial S-NFG where this condition is not satisfied.

        \begin{figure}[t]
            \centering
            \captionsetup{font=scriptsize}
            %----------------------------
            \begin{minipage}[t]{0.4\linewidth}
              \centering
              \begin{tikzpicture}[node distance=2cm, remember picture]
                \tikzstyle{state}=[shape=rectangle,fill=white, draw, minimum width=0.2cm, minimum height = 0.2cm,outer sep=-0.3pt]
                \tikzset{dot/.style={circle,fill=#1,inner sep=0,minimum size=3pt}}
                \node[state] (f2) at (0,0) [label=above: $f_{2}$] {};
                \node[state] (f1) at (0,1) [label=above: $f_{1}$] {};
                \node [dot=black] at (f2.west) {};
                \node [dot=black] at (f1.west) {};
                \node (x1) at (-0.8,0.5) [label=left: $x_{1}$] {};
                \node (x2) at (0.8,0.5) [label=right: $x_{2}$] {};
                %----------------------------------------------------------------------------
                \begin{pgfonlayer}{background}
                  \draw[-,draw]
                      (1,0) -- (-1,0) (1,0) -- (1,1) (-1,0) -- (-1,1) 
                      (-1,1) -- (1,1);
                \end{pgfonlayer}
                %----------------------------------------------------------------------------
              \end{tikzpicture}
            \end{minipage}%
            \caption{S-NFG $\sfN$ in Item~\ref{sec:SNFG:remk:1:item:2} in Remark~\ref{sec:SNFG:remk:1}.\label{sec:SNFG:fig:2}}
        \end{figure}

        \item\label{sec:SNFG:remk:1:item:2} Let us consider the S-NFG in Fig.~\ref{sec:SNFG:fig:2}, where the dots are used for denoting the row index of the matrices $ \matr{f}_{1} $ and $ \matr{f}_{2} $ w.r.t. the function nodes $ f_{1} $ and $ f_{2} $, respectively. In particular, these matrices are given by
        %-------------------------------------------------------------------
        \begin{align*}
            \matr{f}_{1} &\defeq 
            \bigl( f_{1}(x_{1},x_{2}) \bigr)_{x_{1} \in \setx{1},x_{2} \in \setx{2}},
            \qquad 
            \matr{f}_{2} \defeq 
            \bigl( f_{2}(x_{1},x_{2}) \bigr)_{x_{1} \in \setx{1},x_{2} \in \setx{2}}
        \end{align*}
        %-------------------------------------------------------------------
        with row indexed by $ x_{1} $ and column indexed by $ x_{2} $. Running the SPA on this S-NFG is equivalent to applying the power method to the matrix $ \matr{f}_{1} \cdot \matr{f}_{2}^{\tran} $. If we set
        %-----------------------------------------------------------------------
        \begin{align*}
            \matr{f}_{1} 
            = \begin{pmatrix}
              1 & 1 \\ 0 & 1
            \end{pmatrix},
            \qquad 
            \matr{f}_{2} 
            = \begin{pmatrix}
              1 & 0 \\ 0 & 1
            \end{pmatrix},
        \end{align*}
        %-----------------------------------------------------------------------
        then the SPA fixed-point messages are given by
        %-------------------------------------------------------------------
        \begin{align*}
            \vmu_{1,f_{1}}= \vmu_{2,f_{2}} = \begin{pmatrix}
                0, & 1
            \end{pmatrix}^{\!\!\tran}, \quad
            \vmu_{2,f_{1}}= \vmu_{1,f_{2}} = \begin{pmatrix}
                1, & 0
            \end{pmatrix}^{\!\!\tran}, \quad
        \end{align*}
        %-------------------------------------------------------------------
        which results in 
        %-----------------------------------------------------------------------
        \begin{align*}
            Z_{1}(\vmu) 
            = Z_{2}(\vmu) = 0.
        \end{align*}
        %-----------------------------------------------------------------------
        We cannot evaluate $ \ZBSPA(\graphN,\vmu) $ for this S-NFG $ \graphN $.

        \item~\cite[Section VI-C]{Yedidia2005} A sufficient condition for $ \ZBSPA^{*}(\graphN) $ being well-defined for the S-NFG $ \sfN $ is that the local functions in
        $ \sfN $ satisfy
        %-----------------------------------------------------------------------
        \begin{align*}
            f(\vxf) > 0, \qquad \vxf \in \setxf,\, f \in \setF.
        \end{align*}
        %-----------------------------------------------------------------------
        For such S-NFG $ \sfN $, both the SPA fixed-point messages and the beliefs at the locations of the local minima of the Bethe free energy function are positive-valued. 
        Thus the function $ \ZBSPA^{*}(\graphN) $ is well-defined. The statement proven by Yedidia \etal~in~\cite[Theorem 3]{Yedidia2005} further implied that 
        \begin{align*}
            \ZB(\graphN) = \ZBSPA^{*}(\graphN).
        \end{align*}

        \item 
        Consider running the SPA defined in Definition~\ref{sec:SNFG:def:4} on some S-NFG $\graphN$. 
        Then we obtain 
        the collection of the beliefs $ \vbeli \in \LMP(\sfN) $ induced by an SPA fixed-point message vector $\vmu$, following Definition~\ref{def:belief at SPA fixed point for S-NFG}.
        The Bethe free energy function can be related 
        to the $\vmu$-based Bethe partition function:
        \begin{align*}
            \exp \bigl( -\FB(\vbeli) \bigr) = \ZBSPA(\graphN,\vmu).
        \end{align*}
   \end{enumerate}
   %---------------------------------------------------------------------------
  \eremark
\end{remark}


\section[The S-NFG for the Matrix Permanent]{The S-NFG \texorpdfstring{$\sfN(\mtheta)$}{} for the Permanent of a Non-negative Square Matrix \texorpdfstring{$\mtheta$}{} }
\label{sec: snfg for permanent of nonnagtive square matrix}

% Factor graphs are powerful graphical tools to depict the factorization of
% multivariate functions. Many well-known approximation methods, \eg, the
% Bethe~\cite{Yedidia2005} and Sinkhorn\cite{Linial2000} approximations, are
% formulated based on factor graphs. In this thesis, we consider standard normal
% factor graphs (S-NFGs), \ie, factor graphs where the local functions are
% non-negative real-valued, and variables are associated with
% edges~\cite{Forney2001, Loeliger2004}.

%***************************************************************************

The main purpose of this section is to present an S-NFG whose partition
function equals the permanent of a non-negative matrix~$\mtheta$ of size
$n \times n$. There are different ways to develop such
S-NFGs~\cite{Greenhill2010, Vontobel2013a}. (For a comparison between the ways
in~\cite{Greenhill2010, Vontobel2013a}, see\cite[Section
VII-E]{Vontobel2013a}.) In this thesis, we consider the S-NFG $ \sfN(\mtheta) $
defined in~\cite{Vontobel2013a}. Throughout this section, let $\mtheta$ be a
fixed non-negative matrix of size $n \times n$.

%***************************************************************************

\begin{definition}
  \label{sec:1:def:5}
  \label{def: details of S-NFG of permanent}
  % unify the above labels
  \index{S-NFG!associated with the matrix permanent}
  We define the S-NFG
  $ \sfN(\mtheta) \defeq \sfN( \setF, \setEfull, \set{X}) $ as follows (see
  also Fig.~\ref{sec:1:fig:15} for the special case $n = 3$). Note that $ \sfN(\mtheta) $ is a special case of the S-NFG defined in Definition~\ref{def: def of snfg}.
  \begin{enumerate}

  \item The set of vertices (also called function nodes) is
    \begin{align*}
      \set{F}
        &\defeq
           \{ \fr{i} \}_{i \in [n]} 
           \ \cup \ 
           \{ \fc{j} \}_{j \in [n]}.
    \end{align*}
    Here, the letter ``$\mathrm{r}$'' in $ \fr{i} $ means that $ \fr{i} $
    corresponds to the $ i $-th row of $\mtheta$, whereas the letter
    ``$\mathrm{c}$'' in $ \fc{j} $ means that $ \fc{j} $ corresponds to the
    $ j $-th column of $\mtheta$.

  \item The set of edges is defined to be
    \begin{align*}
      \setEfull
        &\defeq
           [n] \times [n] 
          = \bigl\{ 
              (i,j) 
            \bigm|
              i , j \in [n] 
            \bigr\}.
    \end{align*}

  \item The alphabet associated with edge $ e = (i,j) \in \setEfull $ is
    $ \setx{e} = \setx{i,j} \defeq \{0,1\} $.  

  \item The set $ \set{X} $ is defined to be
    \begin{align*}
      \set{X}
        &\defeq
           \prod_{e}
             \setx{e} 
         = \prod_{i,j}
             \setx{i,j}
    \end{align*}
    and is called the configuration set of $ \sfN(\mtheta) $.

  \item A matrix like
    \begin{align*}
      \vgamzo
        &\defeq
           \bigl( 
             \gamzo(i,j)
           \bigr)_{\! (i,j) \in [n] \times [n]}
             \in \setX
    \end{align*} 
    is used to denote an element of $ \set{X} $, \ie, a configuration of
    $ \sfN(\mtheta) $. Here, $ \gamma(i,j) $ is associated with edge
    $ e = (i,j) \in \setEfull$. In the following, the $i$-th row and the
    $j$-th column of $\vgamzo$ will be denoted by $ \vgamzo(i,:) $ and
    $ \vgamzo(:,j) $, respectively.

  \item For a given configuration $\vgamzo \in \setX$, the value of the local
    functions of $\sfN(\mtheta)$ are defined as follows. Namely, for every
    $ i \in [n] $, the local function $ \fr{i} $ is defined to
    be\footnote{Note that, with a slight abuse of notation, we use the same
      label for a function node and its associated local function.}
    \begin{align*}
      \fr{i}\bigl( \vgamzo(i,:) \bigr)
        &\defeq
           \begin{cases}
             \sqrt{ \theta(i,j) } & \vgamzo(i,:) = \vuj  \\
             0                    & \text{otherwise}
          \end{cases}.
    \end{align*}
    For every $ j \in [n] $, the local function $ \fc{j} $ is defined to be
    \begin{align*}
        \fc{j}\bigl( \vgamzo(:,j) \bigr) \defeq
        \begin{cases}
            \sqrt{ \theta(i,j) } & \vgamzo(:,j) = \vui \\
            0 & \text{otherwise}
        \end{cases}.
    \end{align*}
    Here we used the following notation: the vector $\vuj$ stands for a row
    vector of length $n$ whose entries are all equal to~$0$ except for the
    $j$-th entry, which is equal to~$1$. The column vector $\vui$ is defined
    similarly.
  
  \item For a given configuration $\vgamzo \in \setX$, the value of the global
    function $g$ of $\sfN(\mtheta)$ is defined to be the product of the values
    of the local functions, \ie,
    \begin{align*}
      \gtheta(\vgamzo)
        &\defeq
           \Biggl( 
             \prod_{i} 
               \fr{i}\bigl( \vgamzo(i,:) \bigr)
           \Biggr)
          \cdot
          \Biggl(
            \prod_{j}
              \fc{j}\bigl( \vgamzo(:,j) \bigr) 
          \Biggr) .
    \end{align*}
  
  \item The set of valid configurations of $ \sfN(\mtheta) $ is
    defined to be
    \begin{align*}
      \setA(\mtheta)
        &\defeq
           \setA\bigl( \sfN(\mtheta) \bigr)
         \defeq 
           \bigl\{
             \vgamzo \in \setX
           \bigm|
             \gtheta(\vgamzo) > 0
           \bigr\}.
    \end{align*}
    
  \item The partition function of $ \sfN(\mtheta) $ is defined to be
    \begin{align*}
      Z\bigl( \sfN(\mtheta) \bigr)
        &\defeq 
           \sum_{\vgamzo \in \setX }
             \gtheta(\vgamzo)
         = \sum_{\vgamzo \in \setA(\mtheta) }
             \gtheta(\vgamzo).
    \end{align*}
    \label{partition function of N theta}

  \end{enumerate}
  \vspace{-0.25cm}
  \edefinition
\end{definition}

%***************************************************************************

\begin{figure}[t]
  \centering
  \input{figures/example_snfg_permanent_3by3.tex}
  \caption{The S-NFG $ \sfN(\mtheta) $ for the special case $ n = 3 $.}
  \label{sec:1:fig:15}
  \vspace{-0.0cm}
\end{figure}

%***************************************************************************

We make the following observations:
\begin{enumerate}

\item One can verify that $Z\bigl( \sfN(\mtheta) \bigr) = \perm(\mtheta)$.

\item If $ \gtheta(\vgamzo) > 0 $, then $ \vgamzo \in \setP_{[n]} $,
  \ie, $\vgamzo$ is a permutation matrix of size $n \times n$. (In
  fact, if all entries of $\mtheta$ are strictly positive, then
  $ \gtheta(\vgamzo) > 0 $ if and only if $ \vgamzo \in \setP_{[n]} $.)

\end{enumerate}

%***************************************************************************

For the following definition, recall that $\Gamma_{n}$ is the set of all
doubly stochastic matrices of size $n \times n$ and that $\Gamma_{M,n}$ is the
set of all doubly stochastic matrices of size $n \times n$ where all entries
are multiples of $1/M$.

For the following definition, recall that $\Gamma_{n}$ is the set of all
doubly stochastic matrices of size $n \times n$ and that $\Gamma_{M,n}$ is the
set of all doubly stochastic matrices of size $n \times n$ where all entries
are multiples of $1/M$.

%***************************************************************************

\begin{definition}
  \label{sec:1:def:10}

  Consider the S-NFG $ \sfN(\mtheta) $. Let $M \in \sZpp $.  We make the
  following definitions.
  \begin{enumerate}

  \item We define $\Gamnthe$ to be the set of matrices in $\Gamma_{n}$ whose
    support is contained in the support of $\mtheta$, \ie,
    \begin{align*}
      \Gamnthe
        &\defeq 
           \bigl\{ 
             \vgam \in \Gamma_{n}
           \bigm|
             \gamma(i,j) = 0 \text{ if } \theta(i,j) = 0
           \bigr\}.
    \end{align*}

  \item We define $\GamMnthe$ to be the set of matrices in $\Gamma_{M,n}$
    whose support is contained in the support of $\mtheta$, \ie,
     \begin{align*}
       \GamMnthe
         &\defeq 
            \bigl\{ 
              \vgam \in \Gamma_{M,n}
            \bigm|
              \gamma(i,j) = 0 \text{ if } \theta(i,j) = 0
            \bigr\}.
     \end{align*}

  \item We define $\PiA{\mtheta}$ to be the set of vectors representing
    probability mass functions over $\setP_{[n]}$ whose support is contained
    in $\setA(\mtheta)$, \ie,
    \begin{align*}
    \PiA{\mtheta} \defeq
         \left\{ 
           \vp = \bigl( p(\mP_{\sigma}) \bigr)_{\! \mP_{\sigma} \in \setP_{[n]}}
        \ \middle| \!
          \begin{array}{c}
            p(\mP_{\sigma}) \geq 0, \, 
              \forall \mP_{\sigma} \in \setP_{[n]} \\
            p(\mP_{\sigma}) = 0, \, 
              \forall \mP_{\sigma} 
                        \notin \set{A}(\mtheta) \\
            \sum\limits_{\mP_{\sigma} \in \setP_{[n]}} p(\mP_{\sigma}) = 1
          \end{array} \!
        \right\}.
    \end{align*}

  \item Let $\vgam \in \Gamma_n$. We define
    \begin{align*}
      \PiA{\mtheta}( \vgam )
        &\defeq 
          \left\{ 
              \vp 
              \in \PiA{\mtheta}
          \ \middle| \ 
              \sum_{\mP_{\sigma} \in \setP_{[n]}}
                p(\mP_{\sigma}) \cdot \mP_{\sigma} = \vgam
          \right\}.
    \end{align*}

   \item For any matrix $ \matr{B} \in \sR^{n \times n}_{\geq 0} $, we define
   \begin{align*}
       \setS_{[n]}(\matr{B})
         &\defeq 
            \bigl\{ 
              \sigma \in \setS_{[n]} 
            \bigm|
              B\bigl( i, \sigma(i) \bigr) > 0, \, \forall i \in [n]
            \bigr\} \\
         &= \left\{ 
              \sigma \in \setS_{[n]} 
            \ \middle| \ 
              \prod_i 
                B\bigl( i, \sigma(i) \bigr) > 0
            \right\}.
   \end{align*}
   
   \item We define 
     \begin{align*}
       \vsigma_{[M]}
         &\defeq
            (\sigma_{m})_{m \in [M]} \in (\setS_{[n]})^{M}\, , \\
       \mP_{\vsigma_{[M]}}
         &\defeq
            ( \mP_{\sigma_{m}} )_{ m \in [M] } \in (\setP_{[n]})^{M}.
     \end{align*}

   \item Let $ \vgam \in \Gamma_{M,n} $. We define
     \begin{align*}
       \mtheta^{ M \cdot \vgam }
         &\defeq
            \prod_{i,j}
              \bigl(
                \theta(i,j)
              \bigr)^{\! M \cdot \gamma(i,j)}.
     \end{align*}

   \item Let $\pmtheta$ be the probability mass function on $\setS_{[n]}$
     induced by~$\mtheta$, \ie,
     \begin{align*}
       \pmtheta(\sigma)
         &\defeq
            \frac{ \prod\limits_{i \in [n]} \theta\bigl( i,\sigma(i) \bigr)}
                 { \perm(\mtheta) }
          = \frac{ \mtheta^{\mP_{\sigma}}}
                 { \perm(\mtheta) }\, , 
                   \quad \sigma \in \setS_{[n]}.
     \end{align*}
     Clearly, $\pmtheta(\sigma) \geq 0$ for all $\sigma \in \setS_{[n]}$ and
     $\sum\limits_{\sigma \in \setS_{[n]}} \pmtheta(\sigma) = 1$.

   \end{enumerate}
  \edefinition
\end{definition}

%***************************************************************************
Note that if $\matr{B}$ is a doubly stochastic matrix of size $n \times n$, then
  the set $\setS_{[n]}(\matr{B})$ is non-empty. Indeed, this follows from
  considering
   \begin{align*}
      \perm( \matr{B} ) 
      = \sum_{\sigma \in \setS_{[n]}(\matr{B})} 
      \prod_{i}
      B\bigl( i, \sigma(i) \bigr) 
      \overset{(a)}{\geq} n!/n^{n} > 0\, ,
   \end{align*}
   where step $(a)$ follows from van der Waerden's inequality, which was
   proven in~\cite[Theorem 1]{Egorychev1981} and~\cite[Theorem
   1]{Falikman1981}.
% %----------------------------------------------------------------------------
% \begin{lemma}
%    \label{lem: nonemptyness of setS n B}
%    If $ \matr{B} \in \sR^{n \times n}_{\geq 0} $ is a doubly stochastic matrix, 
%    then the set $ \setS_{[n]}(\matr{B}) $ is non-empty.
% \end{lemma}
% %----------------------------------------------------------------------------
% %----------------------------------------------------------------------------
% \begin{proof}
   % The non-emptyness of $ \setS_{[n]}(\matr{B}) $ follows from
   % \begin{align*}
   %    \perm( \matr{B} ) 
   %    = \sum_{\sigma \in \setS_{[n]}(\matr{B})} 
   %    \prod_{i}
   %    B\bigl( i, \sigma(i) \bigr) 
   %    \overset{(a)}{\geq} n!/n^{n} > 0,
   % \end{align*}
   % where step $(a)$ follows from van der Waerden's inequality proven
   % in~\cite[Theorem 1]{Egorychev1981} and~\cite[Theorem 1]{Falikman1981}. 
% \end{proof}
% %----------------------------------------------------------------------------

\begin{lemma}
  \label{sec:1:lemma:8}

  The set of valid configurations $ \setA(\mtheta) $ of $\sfN(\mtheta)$
  satisfies
  \begin{align*}
    \setA(\mtheta) = 
      \left\{ 
         \left. 
         \mP_{\sigma} \in \setP_{[n]}
      \ \right| \ 
          \sigma \in \setS_{[n]}(\vtheta)
      \right\}\, , 
      % \label{sec:1:eqn:118}
  \end{align*}
  which implies a bijection between $ \setA(\mtheta) $ and
  $ \setS_{[n]}(\vtheta) $.
\end{lemma}

%***************************************************************************

\begin{proof}
  This result follows from the Observation~2 after
  Definition~\ref{sec:1:def:5}.
\end{proof}

\section{Free Energy Functions Associated with 
               \texorpdfstring{$\sfN(\mtheta)$}{}}
\label{sec:free:energy:functions:1}

We introduce various free energy functions associated with
$\sfN(\mtheta)$. First we introduce the Gibbs free energy function, whose
minimum yields $\perm(\mtheta)$. Afterwards, we introduce the Bethe free
energy function and the scaled Sinkhorn free energy function, which are
approximations of the Gibbs free energy functions. Their minima yield the
Bethe permanent $\permb(\mtheta)$ and the scaled Sinkhorn permanent
$\permscs(\mtheta)$, respectively, which are approximations of
$\perm(\mtheta)$. Finally, we introduce the degree-$M$ Bethe permanent
$\permbM{M}(\mtheta)$ and the degree-$M$ scaled Sinkhorn permanent
$\permscsM{M}(\mtheta)$.

%***************************************************************************

\begin{definition}
  \label{sec:1:def:18}
  \index{Gibbs free energy function! for S-NFG associated with the matrix permanent}
  Consider the S-NFG $ \sfN(\mtheta) $. The Gibbs free energy function
  associated with $ \sfN(\mtheta) $ (see~\cite[Section III]{Yedidia2005}) is
  defined to be
  \begin{align*}
    \FGthe: \ \PiA{\mtheta} &\to \sR \\
              \vp           &\mapsto \UGthe(\vp) - \HG(\vp)
  \end{align*}
  with
  \begin{align*}
    \UGthe(\vp)   
      &\defeq 
         - 
         \sum_{\mP_{\sigma} \in \setP_{[n]}}
           p( \mP_{\sigma} ) \cdot \log \bigl( g( \mP_{\sigma} ) \bigr)\, , \\
    \HG(\vp)   
      &\defeq 
         - 
         \sum_{\mP_{\sigma} \in \setP_{[n]}} 
         p( \mP_{\sigma} ) \cdot \log \bigl( p( \mP_{\sigma} ) \bigr)\, ,
  \end{align*}
  where $ \UGthe $ and $ \HG $ are called the Gibbs average
  energy function and the Gibbs entropy function, respectively.\footnote{Note
    that $\set{P}_{[n]} \subseteq \set{X}$, where the configuration set
    $\set{X}$ of $\sfN(\mtheta)$ was defined in Definition~\ref{def: details
      of S-NFG of permanent}. With this, $\mP_{\sigma} \in \setP_{[n]}$ is a
    configuration of $\sfN(\mtheta)$ and $g(\mP_{\sigma})$ is well defined.}
  \edefinition
\end{definition}

%***************************************************************************

One can verify that
\begin{align*}
  Z\bigl( \sfN(\mtheta) \bigr) 
    &= \exp
         \biggl( 
           - \min_{\vp \in \PiA{\mtheta}} \FGthe(\vp)
         \biggr).
\end{align*}

%***************************************************************************

Recall the Birkhoff--von Neumann theorem (see, \eg,~\cite[Theorem
4.3.49]{Horn2012}), which states that the convex hull of all permutation
matrices of size $n \times n$ equals the set of all doubly stochastic matrices
of size $ n \times n $. Because $\vp \in \PiA{\mtheta}$ is a probability mass
function over the set of all permutation matrices of size $n \times n$ with support contained in the support of $ \mtheta $, the
Gibbs free energy function can be reformulated as follows as a function over
$\Gamma_{n}(\mtheta)$ instead of over~$\PiA{\mtheta}$.

% For this reformulation, we will need the set
% $\PiA{\mtheta}( \vgam )$, which is defined to be the set of all
% $\vp \in \PiA{\mtheta}$ that are ``compatible'' with
% $\vgam \in \Gamma_{n}(\mtheta)$, \ie,
% \begin{align*}
%   \PiA{\mtheta}( \vgam )
%     &\defeq 
%       \left\{ 
%           \vp 
%           \in \PiA{\mtheta}
%       \ \middle| \ 
%           \sum_{ \mP_{\sigma} \in \setA(\mtheta) }
%             p(\mP_{\sigma}) \cdot \mP_{\sigma} = \vgam
%       \right\}.
% \end{align*}

%***************************************************************************

\begin{definition}
  \label{sec:1:def:18:part:2}
  \index{Gibbs free energy function! for S-NFG associated with the matrix permanent}
  Consider the S-NFG $ \sfN(\mtheta) $. The modified Gibbs free energy
  function associated with $ \sfN(\mtheta) $ is defined to be
  \begin{align*}
    \FGthe': \ \Gamma_{n}(\mtheta) &\to \sR \\
               \vgam               &\mapsto \UGthe'(\vgam) - \HG'(\vgam)
  \end{align*}
  with
  \begin{align*}
    \UGthe'(\vgam)
      &\defeq 
         - 
         \sum_{ i,j }  
           \gamma(i,j) \cdot \log\bigl( \theta(i,j) \bigr)\, , \\ 
    \HG'(\vgam)
      &\defeq
         \max_{ \vp \in \PiA{\vgam}( \vgam ) }
           \HG(\vp)\, ,
  \end{align*}
  where $ \UGthe' $ and $ \HG' $ are called the modified Gibbs average energy
  function, and the modified Gibbs entropy function, respectively.%
  \footnote{\label{footnote:PiA:support:condition:1}%
    Note that the definition
    $\HG'(\vgam) \defeq \max_{ \vp \in \PiA{\mtheta}( \vgam ) } \HG(\vp)$
    would have been more natural/straightforward. However, we prefer the
    definition
    $\HG'(\vgam) \defeq \max_{ \vp \in \PiA{\vgam}( \vgam ) } \HG(\vp)$, as it
    does not depend on $\mtheta$ and, most importantly is equivalent to the
    former definition for $\vgam \in \Gamma_{n}(\mtheta)$. This equivalence
    stems from the following observation. Namely, let
    $\vp \in \PiA{\mtheta}( \vgam )$. Then $p(\mP_{\sigma}) > 0$ only if
    $\supp(\mP_{\sigma}) \subseteq \supp(\vgam)$.} \\
  \mbox{} \edefinition
\end{definition}

% (Note that if $\supp(\mtheta) \subsetneq \supp(\vgam)$, then
% $\PiA{\mtheta}( \vgam )$ is empty.)

%***************************************************************************

One can verify that
\begin{align*}
  Z\bigl( \sfN(\mtheta) \bigr) 
    &= \exp
     \biggl( 
       - \min_{\vgam \in \Gamnthe} \FGthe'(\vgam)
     \biggr).
\end{align*}

%***************************************************************************

However, neither formulation of the Gibbs free energy function leads to a
tractable optimization problem in general unless~$n$ is small. This motivates
the study of approximations of the permanent based on approximating the Gibbs
free energy function, especially based on approximating the modified Gibbs
free energy function in the reformulation presented in
Definition~\ref{sec:1:def:18:part:2}. In the following, we will first discuss
an approximation known as the Bethe free energy function and then an
approximation known as the scaled Sinkhorn free energy function.

%***************************************************************************

In general, the Bethe free energy function associated with an S-NFG is a
function over the so-called local marginal polytope associated with the
S-NFG. (For a general discussion of the local marginal polytope associated
with an S-NFG, see, \eg, \cite[Section 4]{JWainwright2008}.) The thesis
\cite[Section~IV]{Vontobel2013a} shows that the local marginal polytope of the
$\sfN(\mtheta)$ can be parameterized by the set of doubly stochastic
matrices. This is a consequence of the Birkhoff--von Neumann theorem.

%***************************************************************************

\begin{lemma}\!\!\cite[Corollary 15]{Vontobel2013a}
  \label{sec:1:def:16}
  \index{Bethe free energy function!for S-NFG associated with the matrix permanent}
  Consider the S-NFG $ \sfN(\mtheta) $. The Bethe free energy function
  associated with $ \sfN(\mtheta) $, as defined in Definition~\ref{sec:SNFG:def:1}, 
  can be reformulated by the mapping $ \FBthe $, which is defined to be
  \begin{align*}
    \FBthe: \ \Gamma_{n}(\mtheta) &\to \sR \\
              \vgam              &\mapsto \UBthe( \vgam ) - \HBthe( \vgam )
  \end{align*}
  with
  \begin{align*}
    \UBthe(\vgam)
      &\defeq
        -\sum_{ i,j }
        \gamma(i,j) \cdot \log\bigl( \theta(i,j) \bigr)\, , \\
    \HBthe( \vgam )
      &\defeq 
        -
        \sum_{ i,j }
          \gamma(i,j) \cdot \log\bigl(  \gamma(i,j) \bigr) \\
      &\quad\ 
        + 
        \sum_{ i,j }
          \bigl( 1 - \gamma(i,j) \bigr) 
            \cdot 
            \log\bigl( 1 - \gamma(i,j) \bigr).
  \end{align*}
  Here, $ \UBthe $ and $ \HBthe $ are called the Bethe average energy function
  and the Bethe entropy function, respectively. With this, we have
  \begin{align*}
      \ZB\bigl( \sfN(\mtheta) \bigr) = \permb(\mtheta),
  \end{align*}
  where the Bethe permanent $ \permb(\mtheta) $ is defined to be
  \begin{align}
    \permb(\mtheta)
      &\defeq 
         \exp
           \biggl(
             - \min_{\vgam \in \Gamnthe} \FBthe( \vgam ) 
           \biggr).
        \label{sec:1:eqn:192}
  \end{align}
  \index{Bethe permanent}
  \elemma
\end{lemma}

%***************************************************************************


The degree-$M$ Bethe permanent of $\mtheta$ was defined
in~\cite{Vontobel2013a} and yields a combinatorial characterization of the
Bethe permanent. (Note that the definition of $\permb(\mtheta)$
in~\eqref{sec:1:eqn:192} is analytical in the sense that $\permb(\mtheta)$ is
given by the solution of an optimization problem.)

%***************************************************************************

\begin{definition}
  \label{def:matrix:degree:M:cover:1}
  \index{Degree-$M$ Bethe permanent}
  \index{Degree-$M$ Bethe partition function!for S-NFG associated with the matrix permanent}
  Consider the S-NFG $ \sfN(\mtheta) $. Let $M \in \sZpp$.  The degree-$M$
  Bethe permanent is defined to be
  \begin{align*}
    \permbM{M}(\mtheta)
      &\defeq
        \sqrt[M]{
          \bigl\langle
            \perm( \mtheta^{\uparrow \mP_{M}} )
          \bigr\rangle_{\mP_{M} \in \tPsi_{M} }
       } \, , 
         % \label{eq:def:degree:M:Bethe:permanent:1:part:2}
  \end{align*}
  where 
  \begin{align*}
    \tPsi_{M}
      &\defeq 
        \left\{ 
          \mP_{M} \defeq \Bigl( \mP^{(i,j)} \Bigr)_{\!\! i,j\in [n]}
        \ \middle| \ 
          \mP^{(i,j)} \in \setP_{[M]}
        \right\}\, ,
  \end{align*}
  where $ \setP_{[M]} $ is defined in~\eqref{sec:1:eqn:181} and the
  $ \mP_{M} $-lifting of $ \mtheta $ is defined to be a real-valued matrix of size $ M n $-by-$Mn$:
  \begin{align*}
    \!\!
    \mtheta^{\uparrow \mP_{M}}
      &\defeq 
        \begin{pmatrix}
            \theta(1,1) \cdot  \mP^{(1,1)} 
            & \cdots & \theta(1,n) \cdot  \mP^{(1,n)} \\
            \vdots & \ddots & \vdots \\
            \theta(n,1) \cdot  \mP^{(n,1)} 
            & \cdots & \theta(n,n) \cdot  \mP^{(n,n)} 
           \end{pmatrix} 
        .
  \end{align*}
  \edefinition
\end{definition}

%***************************************************************************

\begin{proposition}
  \label{sec:1:thm:8}
  \index{Graph-cover theorem!for S-NFG associated with the matrix permanent}
  Consider the S-NFG $ \sfN(\mtheta) $. It holds that
  \begin{align}
    \permbM{M}(\mtheta) &= \ZBM\bigl( \sfN(\mtheta) \bigr), 
    \qquad M \in \sZpp, \nonumber\\
    \limsup_{M \to \infty} \,
      \permbM{M}(\mtheta)
      &= \permb(\mtheta). 
            \label{sec:1:eqn:193}
  \end{align}
  The limit in~\eqref{sec:1:eqn:193} is visualized in
  Fig.~\ref{fig:combinatorial:characterization:1}~(left).
\end{proposition}

%***************************************************************************

\begin{proof}
  See~\cite[Section~VI]{Vontobel2013a}.
\end{proof}

As we will see in Section~\ref{sec: finite graph covers}, the degree-$M$ Bethe permanent $ \permbM{M}(\mtheta) $ is equal to the average of the degree-$M$ covers' the partition functions of the S-NFG $ \sfN(\mtheta) $, and the proof of Proposition~\ref{sec:1:thm:8} is based on using the method of types to characterize the valid configurations in the degree-$M$ covers of the S-NFG $ \sfN(\mtheta) $.

%***************************************************************************

The Sinkhorn free energy function was defined in~\cite{Vontobel2014}. Here we
consider a variant called the scaled Sinkhorn free energy function that was
introduced in~\cite{N.Anari2021}. These free energy functions are also defined
over $\Gamma_{n}(\mtheta)$.

%***************************************************************************

\begin{definition} 
  \label{sec:1:def:20}
  \index{(Scaled) Sinkhorn free energy function!for S-NFG associated with the matrix permanent}
  Consider the S-NFG $ \sfN(\mtheta) $. The scaled Sinkhorn free energy
  function associated with $ \sfN(\mtheta) $ is defined to be
  \begin{align*}
    \FscSthe: \ \Gamma_{n}(\vtheta) &\to \sR \\
                \vgam          &\mapsto \UscSthe( \vgam ) - \HscSthe( \vgam )
  \end{align*}
  with
  \begin{align*}
    \UscSthe(\vgam) 
      &\defeq
         - 
         \sum_{ i,j }
           \gamma(i,j) \cdot \log\bigl( \theta(i,j) \bigr)\, , \\
    \HscSthe(\vgam)
      &\defeq 
         - \,
         n
         -
         \sum_{ i,j }
           \gamma(i,j) \cdot 
             \log\bigl( \gamma(i,j) \bigr).
    \end{align*}
    Here, $ \UscSthe $ and $ \HscSthe $ are called the scaled Sinkhorn average
    energy function and the scaled Sinkhorn entropy function,
    respectively. With this, the scaled Sinkhorn permanent is defined to be
    \begin{align}
      \permscs(\mtheta)
        &\defeq 
           \exp
             \biggl(
               - \min_{\vgam \in \Gamnthe} \FscSthe( \vgam ) 
             \biggr).
          \label{sec:1:eqn:192:part:2}
    \end{align}
    \index{(Scaled) Sinkhorn permanent}
    \edefinition
\end{definition}

%***************************************************************************

Note that $\HscSthe(\vgam)$ can be obtained from $\HBthe( \vgam )$ by
approximating $\bigl( 1 - \gamma(i,j) \bigr) \cdot \log( 1 - \gamma(i,j) )$ by
the first-order Taylor series expansion term $- \gamma(i,j)$ and using the
fact that the sum of all entries of the matrix
$ \vgam \in \Gamma_{n}(\vtheta) $ equals $n$.

%***************************************************************************

In the following, we introduce the degree-$M$ scaled Sinkhorn permanent of
$\mtheta$, which yields a combinatorial characterization of the scaled
Sinkhorn permanent of $\mtheta$. (Note that the definition of
$\permscs(\mtheta)$ in~\eqref{sec:1:eqn:192:part:2} is analytical in the sense
that $\permscs(\mtheta)$ is given by the solution of an optimization problem.)

%***************************************************************************

\begin{definition}
  \label{def:Sinkhorn:degree:M:cover:1}
  \index{Degree-$M$ (scaled) Sinkhorn permanent}
  Consider the S-NFG $ \sfN(\mtheta) $. Let $M \in \sZpp$.  The degree-$M$
  scaled Sinkhorn permanent is defined to be
  \begin{align*}
    \permscsM{M}(\mtheta)
      &\defeq 
         \sqrt[M]{
           \perm
             \Bigl(
               \bigl\langle
                 \mtheta^{\uparrow \mP_{M}}
               \bigr\rangle_{\mP_{M} \in \tPsi_{M} }
             \Bigr)
         } \nonumber \\
      &= \sqrt[M]{
           \perm\bigl( \mtheta \otimes \mU_{M,M}\bigr)
         } \, , 
   % \label{eq:def:degree:M:scaled:Sinkhorn:permanent:1}
  \end{align*}
  where $\otimes$ denotes the Kronecker product of two matrices and where
  $ \mU_{M,M} $ is the matrix of size $M \times M$ with all entries equal to
  $1/M$.\edefinition
\end{definition}

%***************************************************************************

\begin{proposition}
  \label{sec:1:prop:14}
  \label{SEC:1:PROP:14}
    
  Consider the S-NFG $ \sfN(\mtheta) $. It holds that
  \begin{align}
    \limsup_{M \to \infty} \,
      \permscsM{M}(\mtheta)
      &= \permscs(\mtheta). 
            \label{sec:1:eqn:193:part:2}
  \end{align}
  The limit in~\eqref{sec:1:eqn:193:part:2} is visualized in
  Fig.~\ref{fig:combinatorial:characterization:1}~(right).
\end{proposition}

%***************************************************************************

\begin{proof}
  See Appendix~\ref{apx:24}. (Note that this proof needs some results from
  Lemma~\ref{lem: expression of permanents w.r.t. C} and
  Proposition~\ref{prop:coefficient:asymptotitic:characterization:1}, which
  are proven only in the upcoming sections. Of course, Lemma~\ref{lem:
    expression of permanents w.r.t. C} and
  Proposition~\ref{prop:coefficient:asymptotitic:characterization:1} are
  proven independently of the statement in Proposition~\ref{sec:1:prop:14}.)
\end{proof}

%***************************************************************************

Except for small values of $n$, computing $ \permbM{M}(\mtheta) $ and
$ \permscsM{M}(\mtheta) $ appears to be intractable in general for finite
$M$.\footnote{More formally, we leave it as an open problem to show that
  computing $ \permbM{M}(\mtheta) $ and $ \permscsM{M}(\mtheta) $ is in the
  complexity class \#P for finite $ M \in \sZpp $.} However, as $ M $ goes to
infinity, the limit superior of $ \permbM{M}(\mtheta) $ and
$ \permscsM{M}(\mtheta) $ are equal to $ \permb(\mtheta) $ and
$ \permscs(\mtheta) $, respectively, and they can be computed
efficiently~\cite{Vontobel2013a,Linial2000}.

Note that the modified Gibbs entropy function $ \HG'(\vgam) $, the Bethe entropy function  $ \HBthe( \vgam ) $, and the scaled Sinkhorn entropy function $ \HscSthe(\vgam) $, as defined in Definitions~\ref{sec:1:def:18:part:2},~\ref{sec:1:def:16}, and~\ref{sec:1:def:20}, respectively, are well defined for $ \vgam \in \Gamma_n $, not just for $ \vgam \in \Gamma_n(\vtheta) $. This observation allows us to consider $ \vgam \in \Gamma_{M,n} $ 
in Proposition~\ref{prop:coefficient:asymptotitic:characterization:1}, \ie, $\vgam$ is an element of a set that is independent of $\mtheta$.


\section{Double-Edge Normal Factor Graphs (DE-NFGs)}
\label{sec: basic of denfg}

Now we move to the quantum case. Instead of using the bra-ket notation of quantum mechanics, we will use standard linear algebra notation similar as in~\cite{Loeliger2017,Loeliger2020}.

In this section, we review DE-NFG, which is based on the works in~\cite{Loeliger2017,Loeliger2020,Cao2017}. In general, a DE-NFG can
contain four types of edges: full double edges, full single edges, half double
edges, and half single edges. For the purposes of this thesis, it is sufficient
to consider only DE-NFGs where all the edges are full double edges. The
reasoning is as follows: similar to Section~\ref{sec:SNFG}, half
(double/single) edges can be turned into full
(double/single) edges by attaching a dummy $1$-valued function node to every
half (double/single) edge without changing any marginals or the partition
function. Moreover, DE-NFGs with full single edges can be turned into DE-NFGs
with only full double edges by changing full single edges into full double
edges and suitably reformulating function nodes.

We start by presenting an example DE-NFG.
%*****************************************************************************

\begin{example}
  \label{sec:DENFG:exp:1}

  % \input{figures/penfg_example_main}

  % The NFG on the left-hand side in Fig.~\ref{sec:DENFG:fig:1} depicts the following factorization
  % \begin{align*}
  %   g(x_{1},\ldots,x_{5},x_{1}',\ldots,x_{\upfif})
  %   &\defeq
  %     f_{1}(x_{1},x_{2},x_{3},x_{1}',x_{2}',x_{\upthre}) 
  %     \cdot f_{2}(x_{1},x_{4},x_{1}',x_{\upfor})\\
  %   &\quad \cdot f_{3}(x_{2},x_{5},x_{2}',x_{\upfif})
  %     \cdot f_{4}(x_{3},x_{4},x_{5},x_{\upthre},x_{\upfor},x_{\upfif}).
  % \end{align*}
  % In an NFG, each edge corresponds to a variable, and every pair of edges, denoted as $ (e, \upe) $ represents a pair of variables $\tx_{e} = (\xe, x_{\unpair{e}})$. Here $x_e \in \tset{X}_{e}$ and $x_{\unpair{e}} \in \tset{X}_{\upe}$ with $ \tset{X}_{e} = \tset{X}_{\upe} $ are variables corresponding to edges $ e $ and $ \unpair{e} $, respectively. The term "paired" indicates that if edge $e$ is incident on a function node $f$, then $ \unpair{e} $ is also incident on $ f $, implying that the variable pair $\tx_{e}$ is an argument of 
  % the local function $f$. 

  % In Fig.~\ref{sec:DENFG:fig:1}, both the DE-NFG on the left-hand side and the DE-NFG on the right-hand side are equivalent. Specifically, for the DE-NFG on the right-hand side in Fig.~\ref{sec:DENFG:fig:1}, we establish an association between each edge $ e \in \{ 1,\ldots,5 \} $ and another edge $ \unpair{e} \in \{ \upone, \uptwo,\ldots,\upfif \} $. 

  \input{figures/denfg_example}
  The DE-NFG in Fig.~\ref{sec:DENFG:fig:4} depicts the following factorization
  \begin{align*}
      g(x_{1},\ldots,x_{5},x_{1}',\ldots,&x_{5}')
      \defeq f_{1}(x_{1},x_{2},x_{3},x_{1}',x_{2}',x_{3}') 
          \nonumber\\
          &
          \cdot f_{2}(x_{1},x_{4},x_{1}',x_{4}')
          \cdot f_{3}(x_{2},x_{5},x_{2}',x_{5}')
          \cdot f_{4}(x_{3},x_{4},x_{5},x_{3}',x_{4}',x_{5}').
  \end{align*}
  For each double edge $e \in [5]$, we associate it with the variable
  $\tx_e = (x_e, x'_e)$, where $x_e$ and $x'_e$ take values in the same
  alphabet $\set{X}_e$. Moreover, if $e$ is incident on a function node
  $f$, then $\tx_e$ is an argument of the local function $f$, \ie, both
  $x_e$ and $x'_e$ are arguments of $f$.

  \eexample
\end{example}

% In general, a DE-NFG
% contains full edges and half edges. For the same reason as mentioned in the statements below Example~\ref{sec:SNFG:exp:1}, it is sufficient for us to consider the DE-NFGs where all the edges are full edges.

%***************************************************************************

\begin{definition}\label{sec:DENFG:def:4}
  (DE-NFG)
  \index{DE-NFG}
  A DE-NFG $\graphN(\setF,\setEfull,\tset{X})$ consists of the following
  objects:
  \begin{enumerate}

    \item\label{sec:DENFG:def:4:item:5} A graph $(\setF,\setEfull)$ with vertex set $\setF$ and edge set
    $\setEfull$. The set $ \setF $ represents the set of function nodes, while $ \setEfull $ represents the set of full double edges. (As
    mentioned above, every edge $e \in \setEfull$ will be assumed to be a full
    double edge connecting two function nodes.)

    \item\label{sec:DENFG:def:4:item:1} An alphabet $\tset{X}\defeq\prod_{e \in \setEfull}\tset{X}_e$, where
    $\tset{X}_e\defeq \set{X}_e\times \set{X}_e$ is the alphabet of variable
    $\tx_e \defeq (x_e,x_e')$ associated with edge $e \in \setEfull$. 
    Without loss of generality,
    for each $ e \in \setEfull $, we suppose that $ (0,0) \in \tset{X}_e $.

  \end{enumerate}
    For a given DE-NFG $\graphN(\setF,\setEfull,\tset{X})$, we fix the order of the function nodes by $ \set{F} = \{ f_{1},\ldots,f_{|\set{F}|} \}. $ Then we make the following definitions.
    %------------------------------------------------------------------------
    % \begin{align*}
        
        % \setEfull = \{ \pone,\ldots,\pair{(|\setEfull|-1)} \}.
        % \qquad
        % \setEfull = \{ 1,\ldots,(|\setEfull|-1) \},\qquad
        % \unpair{\setEfull} = \{ \upone,\ldots,\unpair{(|\setEfull|-1)} \}.
    % \end{align*}
    %------------------------------------------------------------------------
    % where 
    % %-----------------------------------------------------------------------
    % \begin{align*}
    %     |\setEfull| = |\setEfull| = |\unpair{\setEfull}|.
    % \end{align*}
    % %-----------------------------------------------------------------------
    
  \begin{enumerate}
    \setcounter{enumi}{3}
%  \item A set of local functions $\{f\}_{f \in \setF}$. Note that each
%    $f$ corresponds to function node $f \in \setF$.

    \item\label{sec:DENFG:def:4:item:2} For every function node $f \in \setF$, the set $\setpf$ is defined to be
    the set of edges incident on $f$. 

    % The degree of function node $ f $ in DE-NFG is given by the cardinality of $ \setpf $, \ie, $ |\setpf| $.

    \item For every edge $e \in \setEfull$, the set $\setpe$ represents the set
    of function nodes that are connected to $e$. 
    % For consistency, we also define $ \setpe $ and $ \setupe $ to be the set of function nodes that are connected to edges $ e $ and $ \upe $, respectively. It is straightforward to see that $ \setppe = \setpe = \setupe. $
    % In the following, we use $ \setpe $ for convenience.

    \item\label{sec:DENFG:def:4:item:3} Consider $ \set{I} \subseteq \setEfull $. The alphabets $ \tset{X}_{\set{I}} $ and $ \set{X}_{\set{I}} $ are defined to be
    %------------------------------------------------------------------------
    \begin{align*}
      \tset{X}_{\set{I}} \defeq \prod_{e \in \set{I}} \tset{X}_{e}
      = \prod_{e \in \set{I}} ( \set{X}_e \times \set{X}_e ), \qquad 
      \set{X}_{\set{I}} \defeq \prod_{e \in \set{I}} \set{X}_{e}.
    \end{align*}
    %------------------------------------------------------------------------
    For any mapping $ h: \tset{X}_{\set{I}} \to \sC $, we define
    the following complex-valued square matrix:
    \begin{align}
        \matr{C}_{h}
        &\defeq 
        \bigl( 
          h( \vx_{\set{I}}, \vx_{\set{I}}' )
        \bigr)_{ \tvx_{\set{I}} = 
        (\vx_{\set{I}}, \vx_{\set{I}}') \in \tset{X}_{\set{I}}}
        \in \sC^{|\set{X}_{\set{I}}| \times |\set{X}_{\set{I}}|}
        \label{eqn: def of Choi matrix representation}
    \end{align}
    with row indices $\vx_{\set{I}}$ and column indices $\vx_{\set{I}}'$.

    % For a collection of finite sets $ \set{I} = (\set{I},\upset{I}) $, 
    % the set $\tset{X}_{\set{I}}$ is defined to be
    % %-----------------------------------------------------------------------
    % \begin{align*}
    %    \tset{X}_{\set{I}} \defeq 
    %    \prod_{e \in \set{I}} \tset{X}_{e}
    %    \times 
    %    \prod_{\upe \in \upset{I}} \tset{X}upe.
    %   % = \tset{X}_{\set{I}} \times \tset{X}_{\upset{I}}
    %   % = \tset{X}_{\set{I}}^{2}.
    % \end{align*}
    % %-----------------------------------------------------------------------
    % Note that $ |\set{I}| $ can be different from $ |\upset{I}| $.
    
    \item Consider $ \set{I} \subseteq \setEfull $. The sets 
    $ \setHerm{ \set{X}_{\set{I}} }$ and 
    $ \setPSD{ \set{X}_{\set{I}} } $ are defined to be 
    the set of Hermitian matrices of size 
    $ |\set{X}_{\set{I}}| \times |\set{X}_{\set{I}}|$
    and 
    % the set of Hermitian matrices of size $|\tset{X}_{\set{I}}| \times |\tset{X}_{\set{I}}|$ and trace one, 
    the set of Hermitian, positive semi-definite (PSD) matrices of size 
    $|\set{X}_{\set{I}}| \times |\set{X}_{\set{I}}|$, respectively.

    \item An assignment $\tvx \defeq ( \tvx_{e} )_{e \in \setEfull} \in \tset{X}$
    is called a configuration of the DE-NFG. For each $f \in \setF$, a
    configuration $\tvx \in \tset{X}$ induces the vector
    \begin{align*}
      \tvx_{\setpf} = (\tx_{e})_{e \in \setpf} \in \tset{X}_{\setpf}.
    \end{align*}


    % \item The alphabet for $f \in \setF$ is given by
    % $ \tset{X}_{\setpf} \defeq \tset{X}_{\setpf} \times \tset{X}_{\upsetpf} $,
    % where $ \tset{X}_{\setpf} \defeq \prod_{e \in \setpf} \tset{X}_{e} $ and 
    % $ \tset{X}_{\setpf} \defeq \prod_{e \in \upsetpf} \tset{X}upe = \tset{X}_{\setpf} $.

  \item\label{sec:DENFG:def:4:item:4} For each function node $f \in \setF$, there is a local function associated with it,  with some slight abuse of notation, also called $f$. Depending on the
    conditions imposed on $f$, we distinguish between a strict-sense and a
    weak-sense DE-NFG.
    \begin{enumerate}

    \item\label{sec:DENFG:def:4:item:4:item:1} In the case of a \textbf{strict-sense DE-NFG}, the local function
      $f$ can be an arbitrary mapping from $\tset{X}_{\setpf}$ to $\sC$ satisfying
      the following property: the square matrix 
      \begin{align}
          \matr{C}_f
          \in \setPSD{ \set{X}_{\setpf} }
          \label{sec:DENFG:eqn:6}
      \end{align}
      with row indices $\vx_{\setpf}$ and column indices $\vx_{\setpf}'$ is a complex-valued,
      Hermitian, positive semi-definite (PSD) matrix. Motivated by the use of
      DE-NFG in quantum information processing (see, \textit{e.g.},
      \cite{Wood2015}), the matrix $\matr{C}_f$ will be
      called the Choi-matrix representation of $f$ or the Choi matrix associated
      with $f$. 
  
    \item In the case of a \textbf{weak-sense DE-NFG}, we require that
      $\matr{C}_f \in \setHerm{ \set{X}_{\setpf} } $, \ie, the matrix $ \matr{C}_f $ is a complex-valued, Hermitian matrix. However, we do
      \emph{not} require $\matr{C}_f$ to be a PSD matrix.  

    \item For each $ f \in \setF $ in a strict-sense or weak-sense DE-NFG, 
        the mappings 
        \begin{align*}
          u_{f, \ell_f}: \tset{X}_{\setpf} 
          &\to \sC, \qquad \ell_f \in \set{L}_f, \nonumber\\
          \lambda_{f}: \set{L}_f  &\to \sR
        \end{align*}
        are defined to be the mappings satisfying
        \begin{align}
          f\bigl( \tvx_{\setpf} \bigr) 
            &= \sum_{\ell_f \in \set{L}_f}
                \lambda_{f}(\ell_f) \cdot
                 u_{f,\ell_f}(\vx_{\setpf}) 
                 \cdot 
                 \overline{u_{f,\ell_f}(\vx_{\setpf}')},
                 \qquad \tvx_{\setpf} \in \tset{X}_{\setpf},
                 \label{sec:DENFG:eqn:5}
            \\
            [\ell_f \!=\! \ell_f']
            &= \sum_{\tvx_{\setpf} \in \tset{X}_{\setpf}}
            u_{f,\ell_f}(\vx_{\setpf}) 
            \cdot 
            \overline{u_{f,\ell_f'}(\vx_{\setpf}')},,\qquad
            \ell_f,\ell_f' \in \set{L}_f, 
            \\
            \lambda_{f}(0) &\geq \lambda_{f}(1) \geq 
            \cdots \geq \lambda_{f}(|\set{L}_f|-1),
            \label{sec:DENFG:eqn:8}
        \end{align}
        where $\set{L}_f = \{0,\ldots,|\set{L}_f|-1\}$ 
        is a finite set with $ |\set{L}_f| = |\tset{X}_{\setpf}| $.
        If we define $ \vect{u}_{f,\ell_f} $ to be the column vector associated with $ u_{f} $:
        %-----------------------------------------------------------------------
        \begin{align}
          \vect{u}_{f,\ell_f} \defeq \bigl( 
            u_{f,\ell_f}(\vx_{\setpf}) 
          \bigr)_{\! \vx_{\setpf} \in \set{X}_{\setpf} } 
          \in \sC^{|\set{X}_{\setpf}|},
          \label{exp:uf}
        \end{align}
        %-----------------------------------------------------------------------
        then the conditions in~\eqref{sec:DENFG:eqn:5}--\eqref{sec:DENFG:eqn:8} are equivalent to
        %-------------------------------------------------------------------
        \begin{align}
          \matr{C}_f &= \sum_{\ell_f \in \set{L}_f} 
          \lambda_{f}(\ell_{f}) \cdot \vect{u}_{f,\ell_f} 
          \cdot \bigl( \vect{u}_{f,\ell_f} \bigr)^{\!\Herm},
          \label{sec:DENFG:eqn:9}\\
          \bigl( \vect{u}_{f,\ell'_f} \bigr)^{\!\Herm} 
          \cdot \vect{u}_{f,\ell_f} &= 
          \bigl[ \ell'_f \!=\! \ell_f \bigr], \qquad 
          \ell_f, \ell'_f \in \set{L}_f.
          \nonumber
        \end{align}
        %-------------------------------------------------------------------
        
        In summary, the vectors $ \bigl( \vect{u}_{f,\ell_f} \bigr)_{ \ell_{f} \in \set{L}_f } $ and the coefficients $ \bigl( \lambda_{f}(\ell_{f}) \bigr)_{ \ell_{f} \in \set{L}_f } $ form an eigenvalue decomposition of the matrix $ \matr{C}_f $, where $ \lambda_{f}(\ell_{f}) $ is the eigenvalue associated with the right-eigenvector 
        $\vect{u}_{f,\ell_f}$.
  \end{enumerate}

  \item The global function $g$ is defined to be the mapping
    \begin{align*}
      g: \tset{X} \to \sC, \qquad \tvx \mapsto \prod_{f \in \setF} 
      f\bigl( \tvx_{\setpf} \bigr).
    \end{align*}

  \item A configuration $\tvx \in \tset{X}$ satisfying $g(\tvx) \neq 0$ is
    called a valid configuration.

  \item The partition function is defined to be
   \begin{align*}
      Z(\graphN) \defeq \sum_{\tvx \in \tset{X}}g(\tvx).
   \end{align*}
    For a strict-sense
    DE-NFG, the partition function satisfies $Z(\graphN) \in \sRp$, whereas
    for a weak-sense DE-NFG, the partition function satisfies
    $Z(\graphN) \in \sR$ (see
    Appendix~\ref{apx:property of ZN}).
    \label{partition function of denfg}

  \end{enumerate}
  \edefinition
\end{definition}

%***************************************************************************
If there is no ambiguity, when we consider S-NFG, we will use the short-hands
$\sum_{\tvx}$, 
$\sum_{\txe}$, 
$\sum_e$, 
$\sum_{f}$, 
$\prod_{\tvx}$,  
$\prod_{\txe}$,
$\prod_e$, 
$\prod_{f}$,
$ (\cdot)_{\txe} $,
and
$ (\cdot)_{e} $ for
$\sum_{\tvx \in \tset{X}}$, 
$\sum_{\txe \in \tset{X}_{e}}$, 
$\sum_{e \in \setEfull}$, 
$\sum_{f \in \setF}$,
$\prod_{\tvx \in \tset{X}}$, 
$\prod_{\txe \in \tset{X}_{e}}$, 
$\prod_{e \in \setEfull}$, 
$\prod_{f \in \setF}$, 
$ (\cdot)_{\txe \in \tset{X}_{e}} $,
and 
$ (\cdot)_{e\in \setEfull} $,
respectively. 
For any $ \set{I} \subseteq \setEfull$, we will use the short-hands
$\sum_{\tvx}$, $\sum_{\tvx_{\set{I}}}$, $\prod_{\tvx}$, $\prod_{\tvx_{\set{I}}}$, 
$(\cdot)_{ \tvx_{\set{I}} }$,
and $\max_{\tvx_{\set{I}}}$ for
$\sum_{\tvx \in \tset{X}}$, 
$\sum_{\tvx_{\set{I}} \in \tset{X}_{\set{I}}}$, 
$\prod_{\tvx \in \tset{X}}$, 
$\prod_{ \tvx_{\set{I}} \in \tset{X}_{\set{I}} }$, 
$(\cdot)_{ \tvx_{\set{I}} \in \tset{X}_{\set{I}} }$,
and $\max_{\tvx_{\set{I}} \in \tset{X}_{\set{I}}}$,
respectively. 
Moreover, $\setpf \setminus e$ will be short-hand notation for
$\setpf \setminus \{ e \}$.

%***************************************************************************

\begin{assumption}\label{sec:DENFG:asum:2}
  In the following, unless stated otherwise, when referring to a DE-NFG, we mean a strict-sense DE-NFG, \ie, we consider $ \lambda_{f}(\ell_{f}) \in \sR_{\geq 0} $ for all $ \ell_{f} \in \set{L}_{f} $ and $ f \in \setF $. 

  Furthermore, we will only consider the (strict-sense) DE-NFG
  $\graphN$ for which $Z(\graphN) \in \sRpp$.\footnote{In this thesis, we only consider the NFGs whose pseudo-dual formulation of the Bethe partition function is well-defined. (See the detailed discussion for S-NFG and DE-NFGs in 
  Remark~\ref{sec:SNFG:remk:1} and Assumptions~\ref{sec:DENFG:asum:2} and~\ref{sec:DENFG:remk:1}.)}
  \eassumption
\end{assumption}

%***************************************************************************

One of the motivations for considering DE-NFGs is that many NFGs
with complex-valued local functions in quantum information processing
can be transformed into DE-NFGs. (See~\cite{Cao2017} for further examples and details on this transformation.)

%--------------------------
\input{figures/penfg_example_qip}
%------------------------------------
\begin{example}[\cite{Loeliger2012,Loeliger2017}]\label{sec:DENFG:exp:2}
  Let us consider an NFG in Fig.~\ref{sec:DENFG:fig:2}(left). Note that at the end of each edge there is a dot used for denoting the row index of the matrix w.r.t. the local function. In particular, it describes a quantum system with two consecutive unitary evolutions:
  \begin{itemize}
    \item At the first stage, a quantum mechanical system is 
    prepared in a mixed state represented by a complex-valued PSD density matrix 
    $\matr{\rho}$ with  
    \begin{align*}
        \matr{\rho} \defeq \bigl( \rho(x_{1},x_{1}') 
        \bigr)_{\! x_{1},x_{1}' \in \set{X}_{1} } \in \setPSD{ \set{X}_{1} }
    \end{align*}
    with trace one, where the row is indexed by $ x_{1} $ and the column indexed by $ x_{1}' $.

    \item Then the system experiences two consecutive unitary 
    evolutions, which are represented by the pair of function nodes 
    $U$ and $B$, respectively. The associated matrices $ \bigl( U(x_{2},x_{1}) \bigr)_{\!x_{2} \in \set{X}_{2},x_{1} \in \set{X}_{1}} $ with row indices $ x_{2} $ and column indices $ x_{1} $ and $ \bigl( B(x_{3},x_{2}) \bigr)_{\!x_{3} \in \tset{X}_{3},x_{2} \in \tset{X}_{2}} $ with row indices $ x_{3} $ and column indices $ x_{2} $ are unitary.
  \end{itemize}
  In order to transform this NFG into a DE-NFG, certain modifications are made:
  %----------------------------------------------------------------------------
  \begin{itemize}
    \item The variables $ x_{e} \in \set{X}_{e} $ 
    and $ x_{e}' \in \set{X}_{e} $ are merged into the variable 
    $ \tx_{e} = ( x_{e}, x_{e}' ) \in \tset{X}_{e} $ for $ e \in [3] $.

    \item New local functions are defined based on the rearranged variables.
  \end{itemize}
  %----------------------------------------------------------------------------
  The resulting DE-NFG is shown in Fig.~\ref{sec:DENFG:fig:2}(right). 
  As an example, the entries in the matrix $\tilde{\matr{U}}$ are 
  given by
  $\tilde{U}(\tx_{2},\tx_{1}) \defeq U(x_{2},x_{1})
  \cdot \overline{U(x_{2}',x_{1}')}$ with $ \tx_{2} \in \tset{X}_{2} $ and 
  $ \tx_{1} \in \tset{X}_{1} $. One can verify that 
  $\tilde{\matr{U}}$ is a PSD matrix with row indices 
  $(x_{2},x_{1})$ and 
  column indices 
  $(x_{2}',x_{1}')$.
  \eexample
\end{example}

%***************************************************************************

%***************************************************************************
\begin{definition}\label{sec:DENFG:def:2}
  \index{SPA!on DE-NFG}
    Consider a DE-NFG denoted by $\graphN$. The SPA for DE-NFG is a straightforward application of the SPA to the NFG under consideration, which is specified as follows.

    \begin{enumerate}

        \item (Initialization) For every $e \in \setEfull$, $f \in \setpe$, the
        messages $\mu_{\ef}^{(0)}: \tset{X}_{e} \to \sC$, are initialized as some
        arbitrary function. (A typical choice is 
        $\mu_{\ef}^{(0)}(\txe) \defeq |\tset{X}_{e}|^{-1} $ for
        all $\tx_e \in \tset{X}_{e}$.) 
     
        \item\label{details of SPA in DE-NFG} (Iteration) For $t = 1, 2, 3, \ldots$, the following calculations are performed until a termination criterion is met.\footnote{The termination
          criterion is typically a combination of numerical convergence and an
          upper bound on the number of iterations.}
        \begin{enumerate}

        \item\label{sec:DENFG:def:2:item:1} For $ e = (f_{i},f_{j}) \in \setEfull $,
        we define the scaling factors $\kappa_{\efj}^{(t)} \in \sC $ to be
        %------------------------------------------------------------------------
        \begin{align*}
            \kappa_{\efj}^{(t)} &\defeq 
            \sum_{\tvx_{\setpfi}}
            f_{i}\bigl( \tvx_{\setpfi} \bigr) 
            \cdot \prod_{e' \in \setpfi \setminus e}
            \mu_{\epfi}^{(t-1)}(\tx_{e'}).
        \end{align*}
        %------------------------------------------------------------------------
        One can obtain the definition of $ \kappa_{\efi}^{(t)} $ by switching $ f_{i}  $ with $ f_{j} $ in the above definition.

        \item If $ \prod_{e \in \setEfull} \bigl(\kappa_{\efi}^{(t)} \cdot \kappa_{\efj}^{(t)} \bigr) = 0 $, we generate random values for each element in the message vector $\vmu_{\etof}^{(t)}$ by sampling from a uniform distribution in the interval $[0, 1]$. 
        
        \item If $ \prod_{e \in \setEfull} \bigl(\kappa_{\efi}^{(t)} \cdot \kappa_{\efj}^{(t)} \bigr) \neq 0 $, valid message updates are performed. 
        For each $ e = (f_{i},f_{j}) \in \setEfull $, we define the messages
        $\mu_{\efi}^{(t)}: \tset{X}_{e} \to \sC$ to be\footnote{If desired or necessary, other generalization procedures is allowed.}
        \begin{align}
            \mu_{\efi}^{(t)}(\tze)
              &\defeq 
                 \bigl( \kappa_{\efi}^{(t)} \bigr)^{\!-1}
                 \cdot
                 \sum_{\tvx_{\setpfj}: \, \txe = \tze}
                  f_{j}\bigl( \tvx_{\setpfj} \bigr)
                   \cdot \prod_{e'\in \setpfj \setminus e}
                    \mu_{\epfj}^{(t-1)}(\tx_{e'}),
              \quad \tze \in \tset{X}_{e}.
              \label{sec:DENFG:eqn:10}
              % \mu_{\upefi}^{(t)}(\zupe)
              % &\defeq 
              %    \bigl( \kappa_{\upefi}^{(t)} \bigr)^{\!-1}
              %    \cdot
              %    \sum_{\tvx_{\setpfj}: \, \xupe = \zupe}
              %     f_{j}\bigl( \tvx_{\setpfj} \bigr)
              %      \cdot
              %      \mu_{\efj}^{(t-1)}(\xe)
              %      \cdot
              %      \prod_{e'\in \setpfj \setminus e}
              %       \mu_{\epfj}^{(t-1)}(x_{e'})
              %       \cdot \mu_{\upepfj}^{(t-1)}(x_{\upe'}),
              % \quad \zupe \in \upset{X}_{e}. \label{sec:DENFG:eqn:11}
        \end{align}
        One can obtain the definition of $ \kappa_{\efi}^{(t)} $ by switching $ f_{i}  $ with $ f_{j} $ in the above definition. 


        \item For every $f \in \setF$, we define
        %--------------------------------------------------------------------
        \begin{align*}
          \kappa_f^{(t)} \defeq
          \sum_{ \tvx_{\setpf} }
          f\bigl( \tvx_{\setpf} \bigr)
          \cdot
          \prod_{e \in \setpf}
          \mu_{\ef}^{(t)}(\txe)
        \end{align*}
        %--------------------------------------------------------------------
        If $ \kappa_f^{(t)} \neq 0 $, then we define the belief function
        $\beli_f: \tset{X}_{\setpf} \to \sC$ at the function node $f$ to be
        \begin{align}
            \beli_f^{(t)}\bigl( \tvx_{\setpf} \bigr)
            &\defeq 
              \bigl( \kappa_f^{(t)} \bigr)^{\!-1}
              \cdot
              f\bigl( \tvx_{\setpf} \bigr)
              \cdot
              \prod_{e \in \setpf}
                \mu_{\ef}^{(t)}(\txe),
                  \quad \tvx_{\setpf} \in \tset{X}_{\setpf}.
            \label{sec:DENFG:eqn:1}
        \end{align}
      % The Choi matrix associated with $ \beli_f^{(t)} $ is given by
      % %-----------------------------------------------------------------------
      % \begin{align*}
      %   \matr{C}_{\beli_f^{(t)}} \defeq 
      %   \Bigl( 
      %       \beli_f^{(t)}\bigl( \tvx_{\setpf},\tvx_{\upsetpf} \bigr) 
      %   \Bigr)_{ \tvx_{\setpf} \in \tset{X}_{\setpf}}
      % \end{align*}
      % %-----------------------------------------------------------------------
      % with row indices $ \tvx_{\setpf} $ and column indices $ \tvx_{\upsetpf} $.
      
    \item For every $e \in \setEfull$, we define
    %------------------------------------------------------------------------
    \begin{align*}
        \kappa_e^{(t)} \defeq
        \sum_{\txe}
        \prod_{f \in \setpe}
        \mu_{\ef}^{(t)}(\txe).
    \end{align*}
    %------------------------------------------------------------------------
    If $ \kappa_e^{(t)} \neq 0 $, then we define the belief function $\beli_{e}: \tset{X}_{e} \to \sC$ at edge $e$ to be
      \begin{align}
        \beli_{e}^{(t)}(\txe)
          &\defeq 
            \bigl( \kappa_e^{(t)} \bigr)^{\!-1}
            \cdot
            \prod_{f \in \setpe}
            \mu_{\ef}^{(t)}(\txe),
            \quad \tx_{e} \in \tset{X}_{e}.
            \label{sec:DENFG:eqn:2}
      \end{align}
      

    \end{enumerate}
     \item At iteration $t \in \sZpp$, the SPA messages can be collected as the SPA message vector $ \vmu^{(t)} $:
      %--------------------------------------------------------------------
      \begin{align*}
          \vmu^{(t)} \defeq 
          \Bigl( 
            \vmu_{\etof}^{(t)}
          \Bigr)_{\! e \in \setpf,\, f \in \setF}, 
      \end{align*}
      %--------------------------------------------------------------------
      where
      \begin{align*}
          \vmu_{\etof}^{(t)} \defeq 
          \Bigl( \mu_{\etof}^{(t)}(\txe) \Bigr)_{\!\txe}.
      \end{align*}
      With this, the SPA message update rules at Step~\ref{details of SPA in DE-NFG} can be written as
      %--------------------------------------------------------------------
      \begin{align*}
        \vmu^{(t)} = \fSPAN\bigl( \vmu^{(t-1)} \bigr)
      \end{align*}
      %--------------------------------------------------------------------
      for some suitably defined function $\fSPAN$.
      

      \item \index{SPA fixed point!for DE-NFG} 
      An SPA message vector 
      $ \vmu \defeq ( \vmu_{\etof} )_{e \in \setpf, f \in \setF} $ with 
      $
        \vmu_{\etof} \defeq 
        \bigl( \mu_{\etof}(\txe) \bigr)_{ \txe }
      $
      is called an SPA fixed-point message vector if 
      %--------------------------------------------------------------------
      \begin{align}
        \vmu = \fSPAN(\vmu).  \label{sec:DENFG:eqn:15}
      \end{align}
      %-------------------------------------------------------------------- 
      The definitions of the belief functions $ \beli_f $ and $ \beli_e $
      evaluated by the SPA fixed-point message vector $ \vmu $ 
      are defined similarly as the definitions in~\eqref{sec:DENFG:eqn:1} 
      and~\eqref{sec:DENFG:eqn:2}, where we need to replace 
      $ \vmu_{\etof}^{(t)} $ with $ \vmu_{\etof} $ for all
      $ e \in \setpf $ and $ f \in \setF $.
      % where $ \mu_{\etof} : \tset{X}_{e} \to \sC $ is an arbitrary mapping.

  \end{enumerate}
  (If desired or necessary, other normalization procedures for messages and
  beliefs can be specified. Note that other normalization procedures for beliefs do not change the results in this thesis.)
  \edefinition
\end{definition}

\begin{assumption}
  \label{asmp: assume messages are PSD}
  In the context of DE-NFG, if not mentioned otherwise, we will only consider SPA
  message vectors $ \vmu^{(t)} $ for
  which 
  \begin{align*}
    \vmu_{\etof}^{(t)} \in \setPSD{\setxe}, \qquad 
  \end{align*}
  for all $e \in \setpf$,
  $f \in \setF$.
  Furthermore, we consider the following normalization procedure for the SPA message vectors $ \vmu^{(t)} $ and the collection of the beliefs $ \vbeli^{(t)} $:
  \begin{align*}
      \sum_{\txe} \mu_{\etof}^{(t)}(\txe) &= 1, \qquad e \in \setpf, \, f \in \setF,
      \nonumber\\
      \sum_{ \txe } \beli^{(t)}_{e}(\txe) &= 1, \qquad e \in \setEfull, \nonumber\\
      \sum_{ \tvx_{\setpf} } \beli^{(t)}_{f}(\tvx_{\setpf}) &= 1, \qquad f \in \setF.
  \end{align*}

  Furthermore, we only consider the SPA fixed-point message vector $ \vmu $ such that
  \begin{align}
      \sum_{\txe}
      \prod_{f \in \setpe}
      \mu_{\ef}(\txe) \neq 0, \qquad e \in \setEfull.
      \label{eqn:assume that Ze is positive}
  \end{align}
  \eassumption
\end{assumption}


\begin{lemma}
  \label{sec:DENFG:lem:1}
  Consider running the SPA defined in Definition~\ref{sec:DENFG:def:2} on a DE-NFG $\graphN$. The resulting belief functions $ \beli_f^{(t)} $ and $ \beli_e^{(t)} $ for $ f \in \setF $ and $ e \in \setEfull $ have the following properties.
  %---------------------------------------------------------------------------
  \begin{enumerate}

    \item\label{sec:DENFG:lem:1:item:1} For all $t \in \sZpp $, we have 
    $ C_{\mu_{\ef}^{(t)}} \in \setPSD{\set{X}_{e}} $ for all $ e \in \setpf $ and $ f \in \setF $, which further implies
    $\matr{C}_{\beli_f^{(t)}} \in \setPSD{\tset{X}_{\setpf}}$ for all $f \in \setF$ and 
    $\matr{C}_{\beli_{e}^{(t)}} \in \setPSD{\set{X}_e}$ for all $e \in \setE$.

    \item\label{sec:DENFG:lem:1: PSD of SPA fixed point message} For any SPA fixed-point message vector $ \vmu $, it holds that $ \matr{C}_{\mu_{\ef}} \in \setPSD{\set{X}_{e}} $ for all $ e \in \setpf $ and $ f \in \setF $

    \item\label{sec:DENFG:lem:1:item:2} The beliefs induced by an SPA fixed-point message vector $\vmu$ satisfy the following consistency properties:
    %-----------------------------------------------------------------------
    \begin{align*}
         \sum_{ \tvz_{\setpf}:\, \tze = \tx_{e}} 
         \beli_f(\tvz_{\setpf}) 
         = \beli_{e}(\tx_{e}), \qquad 
         \txe \in \tset{X}_{e}, \, e \in \setEfull,\, f \in \setpe.
    \end{align*}
    %-----------------------------------------------------------------------
  \end{enumerate}
  %---------------------------------------------------------------------------
\end{lemma}

%***************************************************************************

\begin{proof}
  The proof for each statement in the lemma is listed as follows.
  %----------------------------------------------------------------------------
  \begin{enumerate}
    \item The statement in Item~\ref{sec:DENFG:lem:1:item:1} is a consequence of Assumption~\ref{asmp: assume messages are PSD} and a variant of Schur's product theorem, which states that the entry-wise
  product of two PSD matrices is again a PSD
  matrix.\footnote{Schur's product theorem states that the entry-wise product
    of two positive definite matrices is a positive definite matrix. Note that
    the entry-wise product of two matrices is also known as the Hadamard
    product.} 

    \item The statement in Item~\ref{sec:DENFG:lem:1: PSD of SPA fixed point message} is a straightforward result of Item~\ref{sec:DENFG:lem:1:item:1}.

    \item The statement in Item~\ref{sec:DENFG:lem:1:item:2} is a consequence of the SPA message update rules.
  \end{enumerate}
  %----------------------------------------------------------------------------
  
\end{proof}

%***************************************************************************

The following definition generalizes Definition~\ref{sec:SNFG:def:2}
from S-NFGs to DE-NFGs.

%***************************************************************************

\begin{definition}(The pseudo-dual formulation of the Bethe partition function for DE-NFGs)\label{sec:DENFG:def:3}
  \index{Pseudo-dual Bethe partition function!for DE-NFG} 
  Consider a DE-NFG $\graphN$ and let
  $\vmu $ be an SPA
  message vector for $\graphN$, as defined in~\eqref{sec:DENFG:eqn:15}.\footnote{The SPA message vector $\vmu$ does
    not necessarily have to be an SPA fixed-point message vector.} Define  the following quantities:
    %------------------------------------------------------------------------
    \begin{align*}
        Z_{e}(\vmu)
      &\defeq
        \sum_{\txe}
            \mu_{\efi}(\txe)
            \cdot
            \mu_{\efj}(\txe), \qquad e \in \setEfull,
    \end{align*}
    %------------------------------------------------------------------------
   If 
   \begin{align}
    Z_{e}(\vmu) \neq 0, \qquad e \in \setEfull,
    \label{eqn:positivity of Ze}
   \end{align}
   then we define the $\vmu$-based Bethe partition function to be
  \begin{align}
    \ZBSPA(\graphN,\vmu)
      &\defeq \frac{\prod\limits_f Z_f(\vmu)}
        {\prod\limits_{e} Z_{e}(\vmu)},
        \label{sec:DENFG:eqn:3}
  \end{align}
  where
  \begin{align*}
    Z_f(\vmu)
    &\defeq
      \sum_{\tvx_{\setpf}}
    f\bigl( \tvx_{\setpf} \bigr)
        \cdot
        \prod_{e \in \setpf}
        \mu_{\ef}(\txe), \qquad
        f \in \setF.
  \end{align*}
  (For DE-NFGs with full and half edges, the product in the denominator on the
  right-hand side of~\eqref{sec:DENFG:eqn:3} is only over all full
  edges. Note that the expression for $\ZBSPA(\graphN,\vmu)$ is scaling
  invariant, meaning that if any of the messages in $\vmu$ is multiplied by a
  nonzero complex number, then $\ZBSPA(\graphN,\vmu)$ remains unchanged.)
  (As we will see in the following lemma, the function $ \ZBSPA(\graphN,\vmu) $ is non-negative real-valued for any SPA messages vector $ \vmu $.)
  The SPA-based Bethe partition function $\ZBSPA^{*}(\graphN)$ is then defined
  to be
  \begin{align*}
    \ZBSPA^{*}(\graphN)
      &\defeq 
      \max_{\vmu}
      \ZBSPA(\graphN,\vmu)
      \nonumber\\
      &\qquad \mathrm{s.t.} \
      \text{$\vmu$ is an SPA fixed-point message vector 
      satisfy~\eqref{eqn:positivity of Ze}.}
  \end{align*}
  \edefinition
\end{definition}


\begin{lemma}\label{lem: non-negative of ZBSPA for DE-NFG}
  Consider a DE-NFG $\graphN$ and an SPA message vector $ \vmu $. It holds that 
  %------------------------------------------------------------------------
    \begin{align}
        Z_f(\vmu) &\in  \sR_{\geq 0}, \qquad f \in \setF, \\
        Z_{e}(\vmu)
        & \in \sRp,
        \qquad e \in \setEfull.
        \label{sec:DENFG:eqn:14}
    \end{align}
    %------------------------------------------------------------------------
\end{lemma}

%***************************************************************************

\begin{proof}
    By Lemma~\ref{sec:DENFG:lem:1}, we know that $ \vmu_{\ef} \in \setPSD{\set{X}_{e}} $ for all $ e \in \setpf $ and $ f \in \setF $. Then we
    can use Schur's product theorem to show that 
    the following matrix with row indices $ \vx_{\setpf} $ and column indices $ \vx_{\setpf}' $ is a PSD matrix:
    \begin{align*}
      \Biggl( 
        f\bigl( \tvx_{\setpf} \bigr)
        \cdot
        \prod_{e \in \setpf}
        \mu_{\ef}(\txe)
      \Biggr)_{ \!\! \vx_{\setpf}, \vx_{\setpf}' \in \set{X}_{\setpf} }.
    \end{align*}
    Therefore, we get
    \begin{align*}
      Z_f(\vmu) 
      = 
      \sum_{\tvx_{\setpf}} 
      f\bigl( \tvx_{\setpf} \bigr)
      \cdot
      \prod_{e \in \setpf}
      \mu_{\ef}(\txe) \in \sR_{\geq 0}.
    \end{align*}

    The proof of $ Z_{e}(\vmu) \in \sR_{\geq 0} $ for all $ e \in \setEfull $ is similar and thus it is omitted here.
\end{proof}

\begin{remark}\label{sec:DENFG:remk:1}
    In Assumption~\ref{asmp: assume messages are PSD}, we assume that the strict inequalities in~\eqref{eqn:assume that Ze is positive}.
    Then we know that $\ZBSPA^{*}(\graphN)$ is well-defined, \ie, there exists an SPA fixed-point message vector $ \vmu $ that satisfies 
    %-----------------------------------------------------------------------
    \begin{align*}
        \ZBSPA(\graphN,\vmu) &= \ZBSPA^{*}(\graphN), \nonumber\\
        Z_{e}(\vmu) &\in \sR_{> 0}, \qquad e \in \setEfull.
    \end{align*}
    %-----------------------------------------------------------------------
    \eremark
\end{remark}

\begin{proposition}
  \label{prop: sufficient condition for pd messages}
  \label{PROP: SUFFICIENT CONDITION FOR PD MESSAGES}

  A sufficient condition for $ \ZBSPA(\graphN,\vmu) \in \sR_{>0} $ for all SPA fixed-point message vector $ \vmu $ is that 
  for each $ f \in \setF $ in $ \graphN $, 
  the associated Choi-matrix representation $ \matr{C}_{f} $ is a positive definite matrix.
  
\end{proposition}
%----------------------------------------------------------------------------
\begin{proof}
    See Appendix~\ref{apx: sufficient condition for pd messages}.
\end{proof}
%----------------------------------------------------------------------------


%----------------------------------------------------------------------------
\begin{proposition}\label{sec:DENFG:prop:1}
    For any cycle-free DE-NFG $\graphN$,
    the SPA has a unique fixed-point message vector $ \vmu $, 
    and the SPA-based Bethe partition function 
    gives the exact value of the partition function, 
    \ie, 
    \begin{align*}
      \ZBSPA^{*}(\graphN) 
      = \ZBSPA(\graphN,\vmu) 
      = Z(\graphN).
    \end{align*}
\end{proposition}
%----------------------------------------------------------------------------
%----------------------------------------------------------------------------
\begin{proof}
    The proof is straightforward and thus is omitted here. 
\end{proof}



%***************************************************************************


Although \emph{formal}
Definitions~\ref{sec:SNFG:def:3} and~\ref{sec:SNFG:def:1} could be potentially extended from S-NFGs to DE-NFGs, there is a challenge in dealing with the multi-valued nature of the complex logarithm function. We leave this issue for
future research.

In conclusion, this section provides interesting insights and remarks regarding the DE-NFGs and their associated SPA. In the following, we summarize these points:
%----------------------------------------------------------------------------
\begin{enumerate}
  \item For each DE-NFG, the SPA fixed point messages are utilized to define the Bethe partition function, which serves as an approximation of the partition function.

  \item For any strict-sense DE-NFG $ \sfN $, both the partition function $Z(\graphN)$ and the Bethe partition function $\ZBSPA^{*}(\graphN)$ are non-negative real-valued functions. 

  \item Each S-NFG can be viewed as a special case of a DE-NFG. This observation indicates that the concepts, techniques, and theoretical results that are developed for DE-NFGs, can be applied to S-NFGs as well.

\end{enumerate}
%----------------------------------------------------------------------------




\section{Finite Graph Covers}
\label{sec: finite graph covers}
\label{sec:GraCov}

%***************************************************************************

%***************************************************************************

This section reviews the concept of finite graph covers of a factor graph in general~\cite{Stark:Terras:96:1, Koetter2007,Vontobel2013}.

%***************************************************************************

\begin{definition}
  A graph $\hat{\mathsf{G}} = (\hat{\set{V}}, \hat{\set{E}})$ with vertex set
  $\hat{\set{V}}$ and edge set $\hat{\set{E}}$ is the cover of a graph
  $\mathsf{G} = (\set{V}, \set{E})$ if there exists a graph homomorphism
  $\pi: \hat{\set{V}} \to \set{V}$ such that for each $v \in \set{V}$ and
  $\hat{v} \in \pi^{-1}(v)$, where $\pi^{-1}$ is the pre-image of $v$ under
  the mapping $\pi$, the neighborhood of $\hat{v}$, \ie, 
  the set of all vertices in $ \hat{\set{V}} $ adjacent to $ \hat{v} $, is
  mapped bijectively onto the neighborhood of $v$, \ie, the set of all vertices in $ \set{V} $ adjacent to $ v $. Given a cover
  $\hat{\mathsf{G}} = (\hat{\set{V}}, \hat{\set{E}})$, if there is a positive
  integer $M$ such that $|\pi^{-1}(v)| = M$ for all $v\in \set{V}$, then
  $\hat{\mathsf{G}}$ is called an $M$-cover.
  \edefinition
\end{definition}

%***************************************************************************


Without loss of generality, we can denote the vertex set of an $M$-cover by
$\hat{\set{V}} \defeq \set{V} \times [M]$ and define the mapping
$\pi: \hat{\set{V}} \to \set{V}$ to be such that $\pi((v,m)) = v$ for all
$(v,m) \in \hat{\set{V}}$. Consider an edge in the original graph connecting nodes $v$ and $v'$, and the corresponding edge in the $M$-cover connecting $(v,m)$ and $(v',m')$. It holds that
\begin{align*}
  \Bigl( \pi \bigl( (v,m) \bigr), \pi \bigl( (v',m') \bigr) \Bigr) = (v,v').
\end{align*}
For every edge $e =(v,v')$ in the original graph, there exists a permutation $\sigma_e \in \set{S}_{[M]}$ associated with the corresponding edges in the $M$-cover such that the set of the corresponding edges can be represented by the following set:
\begin{align*}
  \left\{ 
    \Bigl( (v,m),\bigl(v',\sigma_{e}(m)\bigr) \Bigr) 
    \ \middle| \ 
    m \in [M] 
  \right\}.
\end{align*}
This observation motivates the following definition.

%***************************************************************************

\begin{definition}(\textbf{Degree-$M$ finite graph covers of NFGs})
  \label{sec:GraCov:def:1}
  \index{Finite graph covers} 
  Given an NFG $\mathsf{G} = (\set{F}, \set{E}, \set{X})$, we define
  $\hat{\set{G}}_{M}$ to be the set of all graphs
  $\hat{\mathsf{G}} = (\hat{\set{F}}, \hat{\set{E}})$ with vertex set
  $\hat{\set{F}} \defeq \set{F} \times [M]$ and edge set $\hat{\set{E}}$,
  where 
  \begin{align*}
    \hat{\set{E}}
      &\defeq \left\{
            \bigl( (f_{i},m_{i}), (f_{j},m_{j}) \bigr)
         \ \middle|\ 
           m_{j} = \sigma_{e}(m_{i}), 
           \ e = (f_{i}, f_{j}) \in \set{E},\, m_{i}, m_{j} \in [M]
         \right\}
  \end{align*}
  for some permutation $( \sigma_{e} )_{e \in \setEfull} \in \set{S}_{[M]}^{|\setEfull|}$.
  \edefinition
\end{definition}

%***************************************************************************

For a given graph $\mathsf{G}$, we consider all graphs in $\set{G}_{M}$ to be
distinct graphs, despite the fact that some graphs in the set $\set{G}_{M}$
might be isomorphic to each other. (See also the comments on labeled graph
covers after~\cite[Definition~19]{Vontobel2013}.)

%***************************************************************************

Let $\graphN$ be some S-NFG or DE-NFG. It is straightforward to
define the set $ \setcovN{M} $ of $M$-covers $\hgraphN$ of $\graphN$. (For a
technical description, see~\cite{Vontobel2013}.) More importantly, for the finite graph covers of DE-NFGs, the double edges are permuted together\footnote{ A graph-cover definition based on splitting the two edges comprising a double edge could be considered. However, the resulting graph covers would not be immediately relevant for analyzing the SPA in the way that it is formulated. We leave it for future research.}


\begin{figure}[t]
  \begin{center}
    \input{figures/graph_cover_example.tex}
    \medskip
    \caption{Left: NFG $\graphN$. Right: samples of possible 2-covers
    $\mathsf{\hat N}$ of $\graphN$.\label{sec:GraCov:fig:9}}

    \vspace{1cm} 

    \input{figures/graph_cover_example_denfg.tex}
    \medskip
    \caption{
      Left: DE-NFG $\graphN$. Right: samples of possible 2-covers
      $\mathsf{\hat N}$ of $\graphN$.
    }\label{fig:Exam_Graph_cover_DE_NFG}
  
  \end{center}
\end{figure}


%***************************************************************************

\begin{example}
  % \begin{figure}[t]
  %   \centering
  %   \captionsetup{font=scriptsize}
  %   \subfloat{
  %     \input{figures/graph_cover_example.tex}
  %     % \input{figures/graph_cover_example_penfg.tex}

  %     \input{figures/graph_cover_example_denfg.tex}
  %   }
  % \end{figure}

  An S-NFG $\graphN$ is depicted in
  Fig.~\ref{sec:GraCov:fig:9}(left), consisting of $4$ vertices and $5$ edges. Fig.~\ref{sec:GraCov:fig:9}(right) shows possible $2$-covers of $\graphN$. It is mentioned that  for $ M \in \sZpp$, any $M$-cover of $\graphN$ has $M\cdot 4$ function nodes and
  $M\cdot 5$ edges.

  % A DE-NFG $\graphN$ is illustrated in
  % Fig.~\ref{sec:GraCov:fig:10}(left), which is a single-cycle DE-NFG consisting of $2$ vertices and $2$ edges. Fig.~\ref{sec:GraCov:fig:10}(right) shows possible $2$-covers of $\graphN$. Similar to S-NFG, it is stated that any $M$-cover of $\graphN$ has $M\cdot 2$ function nodes and $M\cdot 2$ edges for $ M \in \sZpp$.

  For comparison, a DE-NFG $\graphN$ is shown in
  Fig.~\ref{fig:Exam_Graph_cover_DE_NFG}(left), which consists of $4$ vertices and $5$ double edges. 
  The possible $2$-covers of $\graphN$ are
  shown in Fig.~\ref{fig:Exam_Graph_cover_DE_NFG}(right). Similarly, for $ M \in \sZpp$, each $M$-cover of $\graphN$ has $M\cdot 4$ function nodes and
  $M\cdot 5$ double edges.
  \eexample
\end{example}

%***************************************************************************
%***************************************************************************

% \subsection{Characterization of the Bethe Approximation}

%***************************************************************************


\begin{definition}\label{sec:GraCov:def:2}
  \index{Degree-$M$ Bethe partition function}
  Let $\graphN$ be an S-NFG or a DE-NFG. For any positive integer $M$, we
  define the degree-$M$ Bethe partition function of $\graphN$ to be
  \begin{align*}
    \ZBM(\graphN) 
      \defeq \sqrt[M]{
           \Bigl\langle
             Z\bigl( \hgraphN \bigr)
           \Bigr\rangle_{ \!\! \hgraphN \in \hat{\set{N}}_{M}}
         } \ ,
  \end{align*}
  where
  \begin{align*}
    \bigl\langle Z\bigl( \hgraphN \bigr) \bigr\rangle_{ \hgraphN \in \hat{\set{N}}_{M}}\
    \defeq
    \frac{1}{|\hat{\set{N}}_{M}|}
    \cdot \sum_{ \hgraphN \in \hat{\set{N}}_{M} }
    Z\bigl( \hgraphN \bigr)
  \end{align*}
  represents the average (more precisely, the arithmetic mean) of
  $Z\bigl( \hgraphN \bigr)$ over all $\hgraphN \in \hat{\set{N}}_{M}$, 
  where
  $\hat{\set{N}}_{M}$ is the set of all $M$-covers of $\graphN$ (see
  Definition~\ref{sec:GraCov:def:1}).
  \edefinition
\end{definition}

%***************************************************************************

% The following characterization of S-NFGs' Bethe partition functions in
% terms of finite graph covers was given in~\cite{Vontobel2013}.

%***************************************************************************

\begin{figure}[t]
  \centering
  \begin{tikzpicture}
    \pgfmathsetmacro{\Ws}{1.3};
    % Expression on the LHS and RHS
    %----------------------------------------------------------------------------
    \begin{pgfonlayer}{main}
      \node (ZB1)     at (0,0) [] 
      {$\qquad\qquad\qquad\quad\left. \ZBM(\sfN) \right|_{M = 1} = Z(\sfN)$};
      \node (ZBM)     at (0,\Ws) [] {$\hspace{0.5 cm}\ZBM(\sfN)$};
      \node (ZBinfty) at (0,2*\Ws) {$\qquad\qquad\qquad\qquad
      \left. \ZBM(\sfN) \right|_{M \to \infty} 
      = \ZB(\sfN)$};
    %----------------------------------------------------------------------------
      \draw[]
        (ZB1) -- (ZBM) -- (ZBinfty);
    \end{pgfonlayer}
    % \begin{pgfonlayer}{glass}
    %   \node (1) at (0.25, \Ws) [] {$\ZBM(\sfN)$};
    % \end{pgfonlayer}
    %\vspace{0.3cm}
  \end{tikzpicture}
  \caption{Combinatorial characterizations of the Bethe partition function.
  \label{fig: combinatorial chara for snfg}}
\end{figure}

\begin{theorem}[\!\!\cite{Vontobel2013}]
  \label{sec:GraCov:thm:1}
  \index{Graph-cover theorem!for S-NFG}
  Consider some S-NFG $\graphN$. It holds that
  \begin{align*}
    \limsup_{M\to \infty}
      \ZBM(\graphN)
      &= \ZB(\graphN).
      \nonumber
  \end{align*}
  This combinatoral characterization is visualized in Fig.~\ref{fig: combinatorial chara for snfg}.
  \etheorem
\end{theorem}

\begin{remark}
  Consider the S-NFG $ \sfN(\mtheta) $ defined in Definition~\ref{def: details of S-NFG of permanent}. 
  Vontobel in~\cite[Definition 38]{Vontobel2013a} showed that 
  \begin{align*}
    \ZBM\bigl( \sfN(\mtheta) \bigr) 
    = \permbM{M}\bigl( \mtheta \bigr)
  \end{align*}
  where the degree-$M$ Bethe permanent is defined in Definition~\ref{def:matrix:degree:M:cover:1}.
  Also Theorem~\ref{sec:GraCov:thm:1} is equivalent to Proposition~\ref{sec:1:thm:8} in this case.
\end{remark}

%***************************************************************************

Given the fact that DE-NFGs are in many ways a natural generalization of
S-NFGs, one wonders if there is a characterization of the Bethe partition
function of a DE-NFG in terms of the partition functions of its graph covers
analogous to Theorem~\ref{sec:GraCov:thm:1}, which motivates the following conjecture.
Note that the right-hand side of the expression in the following conjecture
features $\ZBSPA^{*}(\graphN)$, not $\ZB(\graphN)$, because only the
former is defined for DE-NFGs.

%***************************************************************************

\begin{conjecture}
  \label{sec:GraCov:conj:1}

  Consider some DE-NFG $\graphN$. It holds that
  \begin{align}
    \limsup_{M\to \infty}
      \ZBM(\graphN)
      &= \ZBSPA^{*}(\graphN).
      \label{sec:CheckCon:eqn:25}
  \end{align}
  \econjecture
\end{conjecture}

%***************************************************************************

As already mentioned in the introduction, the proof of
Theorem~\ref{sec:GraCov:thm:1} heavily relies on
the method of types and the primal formulation of the Bethe partition function. However, the method of types does not seem to be useful
for proving Conjecture~\ref{sec:GraCov:conj:1}, and it is unclear how to generalize the primal formulation of the Bethe partition function, \ie, Definition~\ref{sec:SNFG:def:1}, to the case of DE-NFGs, so novel techniques have to be developed. In Theorem~\ref{sec:CheckCon:thm:1} in Section~\ref{sec:CheckCon}, we prove
Conjecture~\ref{sec:GraCov:conj:1} for the DE-NFGs
satisfying an easily checkable condition. We conjecture that it holds for more general DE-NFGs.

In the following, we provide promising numerical results supporting
Conjecture~\ref{sec:GraCov:conj:1}.

%***************************************************************************



% \input{figures/Numerical_Results_cover_conjecture_2.tex}

\input{figures/graph_cov_thm/numerical_result_main}

%***************************************************************************
\begin{example}
  \label{sec:GraCov:exp:1}

  Consider the DE-NFG $\graphN$ in Fig.~\ref{sec:GraCov:fig:1}, where
  $\set{X}_e = \{ 0, 1 \}$ and $ \tset{X}_e  = \{ (0,0),(0,1),(1,0), (1,1) \} $ 
  for all $e \in \setEfull$. Here, $\graphN$ is a
  randomly generated DE-NFG, where the function nodes are independently
  generated. 

  For each instance of $\graphN$, we run the SPA until it reaches
  a fixed point and compute $\ZBSPA^{*}(\graphN)$. (We assume that
  $\ZBSPA^{*}(\graphN) = \ZBSPA(\graphN,\vmu)$, where $\vmu$ is the
  obtained SPA fixed-point message vector.) For
  each instance of $\graphN$, we compute $\ZBM(\graphN)$ for $ M \in [4]$. The following simulation results are for $3000$ randomly
  generated instances of $\graphN$. 

  Specifically, Fig.~\ref{sec:GraCov:fig:3} shows the cumulative distribution
  function (CDF) of
  $\bigl( \ZBM(\graphN) \! - \! \ZBSPA^{*}(\graphN) \bigr) /
  \ZBSPA^{*}(\graphN)$ for $ M \in \{1,2,3,4\} $. (Note that 
  $ Z_{\mathrm{B},1}(\graphN) = Z(\graphN) $.) 
  Fig.~\ref{sec:GraCov:fig:4} presents the mean $\mu$ 
  and standard deviation $\sigma$ of the empirical distribution of
  $\bigl| \ZBM(\graphN) \! - \! \ZBSPA^{*}(\graphN) \bigr| /
  \ZBSPA^{*}(\graphN)$. 

  The simulation results indicate that, as $M$ increases, the degree-$M$ Bethe
  partition function $\ZBM(\graphN)$ approaches SPA-based Bethe partition function $\ZBSPA^{*}(\graphN)$.
  \eexample
\end{example}
%***************************************************************************

\begin{example}
  \label{sec:GraCov:exp:2}

  The setup in this example is essentially the same as the setup in Example~\ref{sec:GraCov:exp:1}. However,
  instead of the DE-NFG in Fig.~\ref{sec:GraCov:fig:1}, we consider the DE-NFG in
  Fig.~\ref{sec:GraCov:fig:5}. The simulation results for $780$ randomly
  generated instances of $\graphN$ are presented in
  Figs.~\ref{sec:GraCov:fig:7} and~\ref{sec:GraCov:fig:8} 
  \eexample
\end{example} 






==> shorts.tex <==
% %!TEX root = main.tex
% \usepackage{amsmath,amssymb,amsthm}
% \usepackage{tikz,enumerate}
% \usepackage{bbm}
% \usepackage{cite,mathtools}
% \usepackage{pgffor}
% \usepackage{pgfplots}
% \usepackage{mathrsfs}
% \usepackage{cancel}
% \usepackage{CJKutf8}
% %\usepackage{etex}
% %\usepackage[normalem]{ulem}
% %\usepackage{graphicx}
% %\reserveinserts{28}
% %theorem styles
% %the following is for drawing graph
% \pgfplotsset{compat=1.16}
% \usetikzlibrary{arrows,calc}
% \usepgfplotslibrary{fillbetween}
% \usetikzlibrary{patterns}
% \tikzset{
% %Define standard arrow tip
% >=stealth',
% %Define style for different line styles
% help lines/.style={dashed, thick},
% axis/.style={<->},
% important line/.style={thick},
% connection/.style={thick, dotted},
%  }
% \tikzstyle{box}=[rectangle, draw, text centered]%, text width=1.2cm
% %\tikzstyle{Channel}=[rectangle, draw, text centered, minimum height=0.6cm]%, text width=1.9cm
% \tikzstyle{line} = [draw, -latex']
% %the above is for drawing graph




% %\usepackage[utf8]{inputenc} % set input encoding (not needed with XeLaTeX)

% %%% Examples of Article customizations
% % These packages are optional, depending whether you want the features they provide.
% % See the LaTeX Companion or other references for full information.

% %%% PAGE DIMENSIONS
% %\usepackage{geometry} % to change the page dimensions
% %\geometry{letterpaper} % or a4paper, letterpaper (US) or a5paper or....
% %\geometry{left=1in,right=1in,top=1in,bottom=1in} % for example, change the margins to 2 inches all round
% % \geometry{landscape} % set up the page for landscape
% %   read geometry.pdf for detailed page layout information

% \usepackage{graphicx} % support the \includegraphics command and options
% \usepackage{color}
% \usepackage{bbm}

% % \usepackage[parfill]{parskip} % Activate to begin paragraphs with an empty line rather than an indent

% %%% PACKAGES
% \usepackage{booktabs} % for much better looking tables
% \usepackage{array} % for better arrays (eg matrices) in maths
% \usepackage{paralist} % very flexible & customisable lists (eg. enumerate/itemize, etc.)
% \usepackage{verbatim} % adds environment for commenting out blocks of text & for better verbatim
% %\usepackage{subfigure} % make it possible to include more than one captioned figure/table in a single float
% \usepackage{amsmath}
% \usepackage{amssymb,amsthm}
% % These packages are all incorporated in the memoir class to one degree or another...
% \usepackage{ulem}
% \usepackage{dsfont}
% %% 
% %% Common definitions
% %% Only contains the definitions, not formatting information
% %%

% \usepackage{xspace}
% \usepackage{mathrsfs}
% \usepackage{amsopn}
% \usepackage{tikz}
% \usepackage{bbm}

% \usepackage{hyperref}
% \usepackage[capitalize]{cleveref}
% \usepackage{mathtools}
% %\usepackage{pgfplots}
% %\usepackage[normalem]{ulem}
% \usepackage{cite}

% %\usepackage{etex}
% %\reserveinserts{28}

% %%% HEADERS & FOOTERS
% %\usepackage{fancyhdr} % This should be set AFTER setting up the page geometry
% %\pagestyle{fancy} % options: empty , plain , fancy
% %\renewcommand{\headrulewidth}{0pt} % customise the layout...
% %\lhead{}\chead{}\rhead{}
% %\lfoot{}\cfoot{\thepage}\rfoot{}

% %%% SECTION TITLE APPEARANCE
% %\usepackage{sectsty}
% %\allsectionsfont{\sffamily\mdseries\upshape} % (See the fntguide.pdf for font help)
% % (This matches ConTeXt defaults)
% %\usepackage{hyperref}

% %%% ToC (table of contents) APPEARANCE
% %\usepackage[nottoc,notlof,notlot]{tocbibind} % Put the bibliography in the ToC
% %\usepackage[titles]{tocloft} % Alter the style of the Table of Contents
% %\renewcommand{\cftsecfont}{\rmfamily\mdseries\upshape}
% %\renewcommand{\cftsecpagefont}{\rmfamily\mdseries\upshape} % No bold!


% \definecolor{Red}{rgb}{1,0,0}
% \definecolor{Blue}{rgb}{0,0,1}
% \definecolor{Olive}{rgb}{0.41,0.55,0.13}
% \definecolor{Green}{rgb}{0,1,0}
% \definecolor{MGreen}{rgb}{0,0.8,0}
% \definecolor{DGreen}{rgb}{0,0.55,0}
% \definecolor{Yellow}{rgb}{1,1,0}
% \definecolor{Cyan}{rgb}{0,1,1}
% \definecolor{Magenta}{rgb}{1,0,1}
% \definecolor{Orange}{rgb}{1,.5,0}
% \definecolor{Violet}{rgb}{.5,0,.5}
% \definecolor{Purple}{rgb}{.75,0,.25}
% \definecolor{Brown}{rgb}{.75,.5,.25}
% \definecolor{Grey}{rgb}{.5,.5,.5}

% \def\red{\color{Red}}
% \def\blue{\color{Blue}}
% \def\olive{\color{Olive}}
% \def\green{\color{Green}}
% \def\mgreen{\color{MGreen}}
% \def\dgreen{\color{DGreen}}
% \def\yellow{\color{Yellow}}
% \def\cyan{\color{Cyan}}
% \def\magenta{\color{Magenta}}
% \def\orange{\color{Orange}}
% \def\violet{\color{Violet}}
% \def\purple{\color{Purple}}
% \def\brown{\color{Brown}}
% \def\grey{\color{Grey}}

% \def\jtc{\color{Olive}}
% \def\cn{\color{Violet}}


% %%%% definitions of math statemebt
% \newcommand{\msout}[1]{\text{\sout{\ensuremath{#1}}}}

% %\newtheorem{fact}[propo]{Fact}



% \theoremstyle{plain}

% \newtheorem{theorem}{Theorem}[chapter] 
% \newtheorem{proposition}{Proposition}[chapter] 
% \newtheorem{corollary}{Corollary}[chapter]
% \newtheorem{claim}{Claim}[chapter]
% \newtheorem{lemma}{Lemma}[chapter]
% \newtheorem{conj}{Conjecture}[chapter]
% \newtheorem{bound}{Bound}[chapter]
% \newtheorem{hypothesis}{Hypothesis}[chapter]


% \theoremstyle{remark}

% \newtheorem{remark}{Remark}[chapter]
% \newtheorem{observation}{Observation}[chapter]

% \theoremstyle{definition}
% \newtheorem{definition}{Definition}[chapter]
% %% Boldface vectors
% %%

% \newcommand{\av}{{\bf a}}
% \newcommand{\bv}{{\bf b}}
% \newcommand{\ev}{{\bf e}}
% \newcommand{\Xv}{{\bf X}}
% \newcommand{\Yv}{{\bf Y}}
% \newcommand{\Zv}{{\bf Z}}
% \newcommand{\Uv}{{\bf U}}
% \newcommand{\Vv}{{\bf V}}
% \newcommand{\Sv}{{\bf S}}
% \newcommand{\fv}{{\bf f}}
% \newcommand{\gv}{{\bf g}}
% \newcommand{\xv}{{\bf x}}
% \newcommand{\pv}{{\bf p}}
% \newcommand{\tv}{{\bf t}}
% \newcommand{\yv}{{\bf y}}
% \newcommand{\zv}{{\bf z}}
% \newcommand{\uv}{{\bf u}}
% \newcommand{\vv}{{\bf v}}
% \newcommand{\sv}{{\bf s}}
% \newcommand{\Wv}{{\bf W}}
% \newcommand{\onev}{{\bf 1}}
% \newcommand{\alphav}{\boldsymbol \alpha}
% \newcommand{\betav}{\boldsymbol \beta}
% \newcommand{\gammav}{\boldsymbol \gamma}
% \newcommand{\muv}{\boldsymbol \mu}

% %% Probability and expectation
% \DeclareMathOperator\E{E}
% \let\P\relax
% \DeclareMathOperator\P{P}
% %% \def\E{\mathrm{E}}
% %% \def\P{\mathrm{P}}

% %% Mathcal (discrete sets)
% \newcommand{\Ac}{\mathcal{A}}
% \newcommand{\Bc}{\mathcal{B}}
% \newcommand{\Cc}{\mathcal{C}}
% \newcommand{\cc}{\text{\footnotesize $\mathcal{C}$} }
% \newcommand{\Dc}{\mathcal{D}}
% \newcommand{\Ec}{\mathcal{E}}
% \newcommand{\Fc}{\mathcal{F}}
% \newcommand{\Gc}{\mathcal{G}}
% \newcommand{\Hc}{\mathcal{H}}
% \newcommand{\Ic}{\mathcal{I}}
% \newcommand{\Jc}{\mathcal{J}}
% \newcommand{\Kc}{\mathcal{K}}
% \newcommand{\Lc}{\mathcal{L}}
% %\renewcommand{\Mc}{\mathcal{M}}
% \newcommand{\Nc}{\mathcal{N}}
% \newcommand{\Oc}{\mathcal{O}}
% \newcommand{\Pc}{\mathcal{P}}
% \newcommand{\Qc}{\mathcal{Q}}
% \newcommand{\Rc}{\mathcal{R}}
% \newcommand{\Sc}{\mathcal{S}}
% \newcommand{\Tc}{\mathcal{T}}
% \newcommand{\Uc}{\mathcal{U}}
% \newcommand{\Vc}{\mathcal{V}}
% \newcommand{\Wc}{\mathcal{W}}
% \newcommand{\Xc}{\mathcal{X}}
% \newcommand{\Yc}{\mathcal{Y}}
% \newcommand{\Zc}{\mathcal{Z}}

% %% scr
% \newcommand{\As}{\mathscr{A}}
% \newcommand{\Rs}{\mathscr{R}}


% %% Hats
% \newcommand{\Kh}{{\hat{K}}}
% \newcommand{\Lh}{{\hat{L}}}
% \newcommand{\Mh}{{\hat{M}}}
% \newcommand{\Sh}{{\hat{S}}}
% \newcommand{\Th}{{\hat{T}}}
% \newcommand{\Uh}{{\hat{U}}}
% \newcommand{\Vh}{{\hat{V}}}
% \newcommand{\Wh}{{\hat{W}}}
% \newcommand{\Xh}{{\hat{X}}}
% \newcommand{\Yh}{{\hat{Y}}}
% \newcommand{\Zh}{{\hat{Z}}}
% \newcommand{\kh}{{\hat{k}}}
% \newcommand{\gh}{{\hat{g}}}
% \newcommand{\lh}{{\hat{l}}}
% \newcommand{\mh}{{\hat{m}}}
% \newcommand{\ph}{{\hat{p}}}
% \newcommand{\sh}{{\hat{s}}}
% \newcommand{\uh}{{\hat{u}}}
% \newcommand{\vh}{{\hat{v}}}
% \newcommand{\wh}{{\hat{w}}}
% \newcommand{\xh}{{\hat{x}}}
% \newcommand{\yh}{{\hat{y}}}
% \newcommand{\fh}{{\hat{f}}}


% %% Bars
% \newcommand{\kb}{{\bar{k}}}
% \newcommand{\pb}{{\bar{p}}}
% \newcommand{\qb}{{\bar{q}}}


% % %% Tildes
% % \newcommand{\Bt}{{\tilde{B}}}
% % \newcommand{\Ct}{{\tilde{C}}}
% % \newcommand{\Kt}{{\tilde{K}}}
% % \newcommand{\Lt}{{\tilde{L}}}
% % \newcommand{\Mt}{{\tilde{M}}}
% % \newcommand{\Rt}{{\tilde{R}}}
% % \newcommand{\St}{{\tilde{S}}}
% % \newcommand{\Ut}{{\tilde{U}}}
% % \newcommand{\Vt}{{\tilde{V}}}
% % \newcommand{\Wt}{{\tilde{W}}}
% % \newcommand{\Xt}{{\tilde{X}}}
% % \newcommand{\Yt}{{\tilde{Y}}}
% % \newcommand{\Zt}{{\tilde{Z}}}
% % \newcommand{\kt}{{\tilde{k}}}
% % \newcommand{\lt}{{\tilde{l}}}
% % \newcommand{\mt}{{\tilde{m}}}
% % \newcommand{\rt}{{\tilde{R}}}
% % \newcommand{\st}{{\tilde{s}}}
% % \newcommand{\ut}{{\tilde{u}}}
% % \newcommand{\vt}{{\tilde{v}}}
% % \newcommand{\wt}{{\tilde{w}}}
% % \newcommand{\xt}{{\tilde{x}}}
% % \newcommand{\yt}{{\tilde{y}}}
% % \newcommand{\zt}{{\tilde{z}}}
% % \newcommand{\pt}{{\tilde{p}}}



